Distributed Approximation Algorithms for Weighted Shortest Paths

A distributed network is modeled by a graph having $n$ nodes (processors) and diameter $D$. We study the time complexity of approximating {\em weighted} (undirected) shortest paths on distributed networks with a $O(\log n)$ {\em bandwidth restriction} on edges (the standard synchronous \congest model). The question whether approximation algorithms help speed up the shortest paths (more precisely distance computation) was raised since at least 2004 by Elkin (SIGACT News 2004). The unweighted case of this problem is well-understood while its weighted counterpart is fundamental problem in the area of distributed approximation algorithms and remains widely open. We present new algorithms for computing both single-source shortest paths (\sssp) and all-pairs shortest paths (\apsp) in the weighted case. Our main result is an algorithm for \sssp. Previous results are the classic $O(n)$-time Bellman-Ford algorithm and an $\tilde O(n^{1/2+1/2k}+D)$-time $(8k\lceil \log (k+1) \rceil -1)$-approximation algorithm, for any integer $k\geq 1$, which follows from the result of Lenzen and Patt-Shamir (STOC 2013). (Note that Lenzen and Patt-Shamir in fact solve a harder problem, and we use $\tilde O(\cdot)$ to hide the $O(\poly\log n)$ term.) We present an $\tilde O(n^{1/2}D^{1/4}+D)$-time $(1+o(1))$-approximation algorithm for \sssp. This algorithm is {\em sublinear-time} as long as $D$ is sublinear, thus yielding a sublinear-time algorithm with almost optimal solution. When $D$ is small, our running time matches the lower bound of $\tilde \Omega(n^{1/2}+D)$ by Das Sarma et al. (SICOMP 2012), which holds even when $D=\Theta(\log n)$, up to a $\poly\log n$ factor.

==> G_prime.tex <==
\section{Using {\large$\mathbf{(G'_{\lowercase{\large u}}, w')}$} (Proposition~\ref{prop:G prime})} \label{sec:G prime}

In this section, we show the key proposition that proves the correctness of our exact algorithm (Proposition~\ref{prop:G prime}): For any nodes $u$ and $v$ in clusters $C_j$ and $C_j'$, respectively,  $\dist_{G, w_i}(u, v)=\dist_{G'_u, w'}(c_j, c_{j'})$, where  $G'_u$ is as constructed in Line~\ref{line:G prime} of Algorithm~\ref{algo:apsp}.

To prove the proposition, first observe that if $j=j'$ then the proposition is clearly true since the distance between nodes in the same cluster have distance zero in $(G, w_i)$. So, we will assume that $j\neq j'$ in the rest of this section.

Let $P=\langle u=x_0, x_1, \ldots, x_\ell=v\rangle$ be any shortest $u$-$v$ path in $(G, w_i)$. We decompose $P$ into simple paths $P_1, P_2, \ldots, P_t$, for some $t$, as follows. Initially, let $j=1$. While $j\leq \ell$ and $x_j$ is in the cluster $C_{j'}$ that contains $x_0$ or $|C_{j'}|\leq \sqrt{n}$, we increase $j$. When we stop increasing $j$, we let $P_1=\langle x_0, \ldots, x_j\rangle$. We then repeat the same process to construct other subpaths on $\langle x_j, \ldots, x_\ell\rangle$.

Note the following properties of $P_1, \ldots, P_t$. Let  $P_i=\langle x_i^0, x_i^1, \ldots, x_i^{\ell_i}\rangle$, for some $\ell_i$, and let $C_i^j$ be the cluster containing $x_i^j$. Then, (1) for any $i$, $C_i^0\neq C_i^{\ell_i}$, (2) for any $i$ and $j<\ell_i$, either $C_i^j=C_i^0$ or $|C_i^j|\leq \sqrt{n}$, and (3) for any $i>1$, $|C_i^0|>\sqrt{n}$.


%with the following properties for every $i$: (1) two end nodes in $P_i$ are in different clusters and (2) every node in $P_i$ is either in the same cluster as one of the end nodes of $P_i$ or in a small cluster (of size at most $\sqrt{n}$).
%
%To be precise, denote every path $P_i$ by  $P_i=\langle x_i^0, x_i^1, \ldots, x_i^{\ell_i}$, for some $\ell_i$, and let $C_i^j$ be the cluster containing $x_i^j$. (Note that $x_i^0=x_{i-1}^{\ell_{i-1}}$.) We want that, for any $i$, (1) $C_i^0\neq C_i^{\ell_i}$, and (2) for any $j$, either $x_i^j\in C_i^0$, $x_i^j\in C_i^{\ell_i}$ or $|C_i^j|\leq \sqrt{n}$.

%We can always decompose any path $P$ into paths with the above properties, as follows. Let $P_1$ be the longest path containing $x_0$ that satisfies the second property above. We then remove edges in $P_1$ and repeat the process.
%
%Note that $P_1$ contains at least one edge since a path having one edge always satisfy the the second property. Moreover, $P_1$ must satisfy the first property; otherwise, we can include one more node to $P_1$ while satisfying the seconding property, contradicting the fact that $P_1$ is the longest path satisfying the second property.

Consider any subpath $P_i$. Let $j'$ be the maximum  number such that $x_i^{j'}\in C_i^0$. Let $P'_i=\langle x_i^{j'}, \ldots, x_i^{\ell_i}\rangle$ be the subpath of $P_i$ starting at $x_i^{j'}$. Observe that all internal nodes of $P'_i$ are in small clusters (of size at most $\sqrt{n}$), by the second property. So, $P'_i$ is also a path in $H$. In other words, $\dist_{G, w_i}(x_i^{j'}, x_i^{\ell_i})=\dist_{H, w_i}(x_i^{j'}, x_i^{\ell_i})$. Thus, by Proposition~\ref{prop:G prime}, $d'(x_i^{j'}, x_i^{\ell_i})=\dist_{G, w_i}(x_i^{j'}, x_i^{\ell_i})$. It follows that $d'(C_i^0, C_i^{\ell_i})=d'(C_i^{j'}, C_i^{\ell_i})\leq \dist_{G, w_i}(x_i^{j'}, x_i^{\ell_i})=\dist_{G, w_i}(x_i^{0}, x_i^{\ell_i}).$ So,
%
$$\sum_{i=1}^{t} d'(C_i^0, C_i^{\ell_i})\leq \sum_{i=1}^{t} d'(x_i^0, x_i^{\ell_i})=w_i(P)\,.$$
%
Since $P$ is a shortest $u$-$v$ path, we have that $\sum_{i=1}^{t} d'(C_i^0, C_i^{\ell_i})=w_i(P)$. 
%
Finally, we claim that we have edges $c_i^0c_i^{\ell_i}$ of weight $d'(C_i^0, C_i^{\ell_i})$ for all $i$; in other words, $u$ knows $d'(C_i^0, C_i^{\ell_i})$ for all $i$. This is clear for $i=1$ since $u\in C_i^0$ and so we compute $d'(C_i^0, C_i^{\ell_i})$ from Line~\ref{line:collect distance within cluster} of Algorithm~\ref{algo:apsp}. For $i>1$, the third property implies that $|C_i^0|>\sqrt{n}$. Thus, $u$ will know $d'(C_i^0, C_i^{\ell_i})$ from Line~\ref{line:broadcast big cluster} of Algorithm~\ref{algo:apsp}.



==> approx_algo.tex <==
\section{Approximation Algorithms}\label{sec:approx}

%
% ---------------- The commented text here is already moved -----------------
%
%\subsection{Pseudo-Polynomial Time Algorithm for {\large $\mathbf{K}$}-APSP (Proof of Proposition~\ref{PROP:PSEUDOPOLY TIME})}\label{sec:proof of PROP:PSEUDOPOLY TIME}
%We first argue that there exists a $O(n+K)$-time algorithm for $K$-\apsp on network $G$ with positive symmetric integral weight $w$, as claimed in Proposition~\ref{PROP:PSEUDOPOLY TIME}. This algorithm is pseudo-polynomial since $K$ could be as large as $D(G, w)$.
%
%{\renewcommand{\thetheorem}{\ref{prop:pseudopoly time}}
%\begin{proposition}[Restated]
%$K$-\apsp on network $G$ with {\em positive symmetric} integral weight $w$ can be solved in $O(n+K)$-time.
%\end{proposition}
%\addtocounter{theorem}{-1}
%}
%
%Consider Algorithm~2 in \cite{HolzerW12} which is used for the problem called {\em $\cS$-shortest paths} (computing distances from sources in $\cS$ on an unweighted network $G$). This algorithm is outlined in Algorithm~\ref{algo:HolzerW12}. This algorithm executes the breadh-first search (BFS) algorithms from $q$ different sources in $\cS$ in parallel, where the BFS algorithm starting at node $u$ forwards $u$ (representing the unique ID of node $u$) in the BFS manner until every node receives $u$. We let BFS$_i$ denote the BFS algorithm starting at $s_i$, and $T_{s_i}$ denote the BFS tree constructed by BFS$_i$.
%
%
%
%\begin{algorithm}
%\caption{$K$-\apsp $(G, \cS=\{s_1, \ldots, s_q\})$ \cite{HolzerW12}}\label{algo:HolzerW12}
%{\bf Input:} Unweighted undirected graph $G$ and set $\cS$ of $q$ source nodes $s_1, \ldots s_q$. %Assume wlog that $s_1<s_2<\ldots s_K$.
%
%{\bf Output:} Every node $u$ knows $\dist^K_G(s, u)$.
%
%%\medskip $\bullet$ Let $t$ be the time this algorithm starts. We can assume that all nodes know $t$.
%
%\medskip $\bullet$ Initially, source nodes $s_1, \ldots, s_q$ trigger the algorithm to start by sending a message $(s, 0)$ to itself.
%
%
%%\medskip\textit{\textbf{Main subroutine:}}
%
%$\bullet$ When a node $u$ receives a message $(s_i, \ell)$ for some $\ell$, it does the following.
%
%\begin{algorithmic}[1]
%
%%\algrestore{bfsone}
%
%\If{$u$ has {\em not} already received $(s_i, \ell')$ for any $\ell'$}
%
%\State $u$ now knows that $\dist_{G}(s, u)=\ell$.\label{line:HolzerW compute distance}
%
%%\State $u$ sends through all directed edges $\overrightarrow{uv}$ a message $(s, t, \ell+w(\overrightarrow{uv}))$ at time $t+\ell+w(\overrightarrow{uv})$.\label{line:bfs send message}
%
%\State $u$ sends message $(s_i, \ell+1)$ to all its neighbors that have not sent any message of the form $(s_i, \ell')$ to $u$.
%
%\State For any neighbor $v$ of $u$, if there are many messages of the form $(s', \ell'+1)$ that $u$ and $v$ want to send to each other, we allow them to send only the message with smallest $s'$ (if there are ties, send the one with smallest $\ell'$). (Thus, there are at most one message sent between $u$ and $v$ in each round.) For other messages that are not sent, $u$ and $v$ will try to send them again in the next rounds.\label{line:HolzerW main trick}
%\EndIf
%
%\end{algorithmic}
%\end{algorithm}
%
%
%
%The important trick of this algorithm is that, when there are many messages that the algorithm wants to send on the same edge at the same time (on any direction), we allow it to send only one message with the smallest ID, as described in the Line~\ref{line:HolzerW main trick} of Algorithm~\ref{algo:HolzerW12}.
%%
%We use the following two properties claimed in the proof of Theorem~3 of \cite{HolzerW12}.
%
%\noindent {\bf P1:} For any nodes $v_1$ an $v_2$, messages containing the ID of $s_i$ are sent over the edge $(v_1 , u)$ earlier than over edge $(v_2 , u)$ if and only if $\dist_{G}(s_i, v_1 ) < \dist_G(s_i, v_2 )$.
%
%\noindent {\bf P2:}  For any indices $i$ and $j$ and node $u$, during traveling on any $s_i$-$u$ path of $T_{s_i}$, the message of ID $s_i$ gets delayed {\em at most once} by the computation BFS$_j$ if ID $s_j$ is strictly smaller then ID $s_i$.
%
%Property P2 implies that any message of the form $(s_i, \ell)$ will arrive at any node $u$ in $\ell+|\cS|-1$ rounds since it will be delayed by at most $|\cS|-1$ times (by $|\cS|-1$ other messages). Property P1 guarantees that each node $u$ of distance $\ell$ from $s_i$ will receive message $(s_i, \ell)$ without receiving any message $(s_i, \ell')$ earlier, for any other value of $\ell'$. This guarantees the correctness of the algorithm (as in Line~\ref{line:HolzerW compute distance} of Algorithm~\ref{algo:HolzerW12}). We conclude these properties by the following observation.
%%
%\begin{observation}
%For any $K$ and $s_i\in \cS$, after $K+|\cS|-1$ rounds every node $u$ such that $\dist_G(s_i, u)\leq K$ knows $\dist_G(s_i, u)$.
%\end{observation}
%%
%Now, to solve $K$-\apsp on a weighted network $(G, w)$, we construct a network $G'$ where we replace each edge $uv$ of length $w(uv)$ in $(G, w)$ by a $w(uv)$-length path of $\langle u=x_0, x_1, \ldots, x_{w(uv)}=v\rangle$. Network $(G, w)$ will simulate an algorithm on $G'$  by letting one of $u$ and $v$ simulate the computation of $x_1, \ldots, x_{w(uv)-1}$. In particular, $(G, w)$ will simulate Algorithm~\ref{algo:HolzerW12} on $G'$ with $\cS=V(G)$ for $K$ step. By the above observation, when the simulation is finished, for every $u, v\in V(G)\subseteq V(G')$ such that $\dist_{G'}(u, v)\leq K$, node $v$ knows $\dist_{G'}(u, v)$ which is equal to $\dist_{G, w}(u, v)$. Node $v$ can then use this solution to answer $K$-\apsp on $(G, w)$.\danupon{To do: Solve $(\cS, K)$-\ksp instead}


\subsection{Approximating Diameter and Radius in {\large $\mathbf{O(n)}$} time (Theorem~\ref{theorem:diameter girth})}\label{sec:approx diameter}



%\paragraph{Approximating Diameter in $O(n)$ time (Theorem~XXX)}
We now prove Theorem~\ref{theorem:diameter girth}. 
%; i.e., we show that, for any constant $\epsilon>0$, there is an $O(n)$-time deterministic distributed algorithm such that, for any weighted network $(G, w)$, the algorithm outputs $\tilde D$ such that $D(G, w)\leq \tilde{D} \leq (1+\epsilon)D(G, w)$.

{\renewcommand{\thetheorem}{\ref{theorem:diameter girth}}
\begin{theorem}[Restated]
For any $\epsilon>0$, there are deterministic $(1+\epsilon)$-approximation $O((1+\frac{1}{\epsilon})n)$-time algorithms for diameter and girth computation. 
\end{theorem}
\addtocounter{theorem}{-1}
}

\begin{algorithm}\caption{{Approximate Diameter in $O(n)$ time}}\label{algo:approx diameter}
\begin{algorithmic}[1]
\State Solve single-source shortest path (\sssp) from an arbitrary node $s$ using the distributed version of Bellman-Ford's algorithm~\cite{peleg,Lynch-Book,Santoro-book}. Let $D'=2\max_{u\in V(G)} \dist_{G, w}(s, u)$. {\small // $O(n)$ time. We claim that $D(G, w)\leq D'\leq 2D(G, w)$ (Claim~\ref{claim:two approx of diameter}).}\label{line:two approx diameter}

\State For any edge $uv$ in $G$, let $w'(uv)=\lceil \frac{2n w(uv)}{\epsilon D'}\rceil$. {\small // No communication is needed}\label{line:round weight for approx diameter}

\State Network $G$ uses the algorithm in Proposition~\ref{prop:pseudopoly time} to compute $K$-\apsp on $(G, w')$ where $K=(1+2/\epsilon)n$. {\small // Takes $O(K+n)=O((1+1/\epsilon)n)$ time.}\label{line:approx diameter run pseudoply algo}

\State \label{line:approx diameter output} Output $\tilde D = \frac{\epsilon D'}{2n}D(G, w')$.
\end{algorithmic}
\end{algorithm}

\paragraph{Approximating Diameter} We first show how to approximate the diameter. Approximating the radius will be done by slightly modifying the algorithm for approximating the diameter. 
%
We use the algorithm outlined in Algorithm~\ref{algo:approx diameter}. First, in {\bf Line~\ref{line:two approx diameter}}, we compute $D'=2\max_{u\in V(G)} \dist_{G, w}(s, u)$ for an arbitrary node $s$. This can be done in $O(n)$ time by the distributed version of Bellman-Ford's algorithm \cite{peleg}. Observe that $D'$ two-approximates $D(G, w)$:
\begin{claim}\label{claim:two approx of diameter}
$D(G, w)\leq D'\leq 2D(G, w)$.
\end{claim}
\begin{proof}
By definitions of $D'$ and $D(G, w)$,
$$D'=2\max_{u\in V(G)} \dist_{G, w}(s, u)\leq 2\max_{s,u\in V(G)} \dist_{G, w}(s, u)=2D(G, w),$$
proving the second inequality. For the first inequality, observe that for any $u, v\in V(G)$, $\dist_{G, w}(u, v)\leq \dist_{G, w}(s, u)+\dist_{G, w}(s, v)\leq 2\max_{u\in V(G)} \dist_{G, w}(s, u)=D'$. Thus, $D(G, w)= \max_{u,v\in V(G)} \dist_{G, w}(u, v)\leq D'$ as claimed.
\end{proof}
%
Next, in {\bf Line~\ref{line:round weight for approx diameter}}, we compute weight $w'$. We now prove the nice property of $w'$ as in Proposition~\ref{prop:approx diameter guarantee}.

{
\renewcommand{\thetheorem}{\ref{prop:approx diameter guarantee}}
\begin{proposition}[Restated]
%$D(G, w')=(1+2/\epsilon)n$ and $D(G, w)$ $\leq$ $D'\times D(G, w')$ $\leq$ $(1+\epsilon)D(G, w).$
\begin{align}
D(G, w')& \leq(1+2/\epsilon) n, ~~~and \label{eq:approx diameter main one}\\
D(G, w) \leq\frac{\epsilon D'}{2n}\times D(G, w')&\leq(1+\epsilon)D(G, w).\label{eq:approx diameter main two}
\end{align}
\end{proposition}
\addtocounter{theorem}{-1}
}
%\begin{align}
%D(G, w')& =(1+2/\epsilon) n, ~~~and \label{eq:approx diameter main one}\\
%D(G, w) \leq\frac{\epsilon D'}{2n}\times D(G, w')&\leq(1+\epsilon)D(G, w).\label{eq:approx diameter main two}
%\end{align}
%
%\begin{proposition}\label{prop:approx diameter guarantee}
%$D(G, w')=O(n)$ and $D(G, w)$ $\leq$ $D'\cdot D(G, w')$ $\leq$ $(1+\epsilon)D(G, w).$
%\end{proposition}
%
\begin{proof}%[of Proposition~\ref{prop:approx diameter guarantee}]
For any nodes $u$ and $v$, let $P=\langle u=x_0, x_1, \ldots, x_\ell=v\rangle$ be any shortest $u$-$v$ path. Then,
\begin{align}
\dist_{G, w'}(u, v)&=\sum_{i=0}^{\ell-1} \left\lceil \frac{2n w(x_ix_{i+1})}{\epsilon D'}\right\rceil \label{eq:diameter approx one}\\
&\leq \frac{2n}{\epsilon D'}\sum_{i=0}^{\ell-1} w(x_ix_{i+1}) + (\ell-1) \label{eq:diameter approx two}\\
&\leq \frac{2n}{\epsilon D'}D(G, w) + (n-1) \label{eq:diameter approx three}\\
&\leq (1+2/\epsilon)n \label{eq:diameter approx four}
\end{align}
where the last inequality is because $D'\geq D(G, w)$, by Claim~\ref{claim:two approx of diameter}. It follows that
$$D(G, w')=\max_{u, v} \dist_{G, w'}(u, v)\leq (1+1/2\epsilon) n$$
as claimed in Eq.~\eqref{eq:approx diameter main one}

Using Eq.\eqref{eq:diameter approx three}, we also have that
\begin{align*}
\frac{\epsilon D'}{2n}\times D(G, w') & = \frac{\epsilon D'}{2n}\times \max_{u, v} \dist_{G, w'}(u, v)\\
&\leq \frac{\epsilon D'}{2n}\times \left( \frac{2n}{\epsilon D'}D(G, w) + (n-1)\right)\\
&\leq D(G, w)+\frac{\epsilon}{2} D'\\
&\leq (1+\epsilon) D(G, w)
\end{align*}
where the last inequality is because $D'\leq 2D(G, w)$ by Claim~\ref{claim:two approx of diameter}. This proves the second inequality of Eq.~\eqref{eq:approx diameter main two}.

Finally, observe that for the path $P$ defined as before, we have
\begin{align}
\dist_{G, w'}(u, v)&\geq \sum_{i=0}^{\ell-1} \frac{2n w(x_ix_{i+1})}{\epsilon D'}\nonumber\\
&\geq \frac{2n}{\epsilon D'}  \dist_{G, w}(u, v)\label{eq:diameter approx five}\,.
\end{align}
It follows that
%
\begin{align*}
\frac{\epsilon D'}{2n}\times D(G, w') & \geq \frac{\epsilon D'}{2n}\times \max_{u, v} \dist_{G, w'}(u, v)\\
& \geq \frac{\epsilon D'}{2n}\times \max_{u, v}  \frac{2n}{\epsilon D'}  \dist_{G, w}(u, v)\\
& = D(G, w)
\end{align*}
%
where the second inequality is by Eq.\eqref{eq:diameter approx five}. This proves the first inequality of Eq.\eqref{eq:approx diameter main two} and completes the proof of Proposition~\ref{prop:approx diameter guarantee}.
\end{proof}


Now, in {\bf Line~\ref{line:approx diameter run pseudoply algo}}, we execute the pseudo-polynomial time algorithm in Proposition~\ref{prop:pseudopoly time} on $(G, w')$ using $K=(1+2/\epsilon)n$. Since $D(G, w')\leq (1+2/\epsilon)n$ (cf. Proposition~\ref{prop:approx diameter guarantee}), we will end up with the solution of \apsp on $(G, w')$, thus having the value of $D(G, w')$.
%
Finally, in {\bf Line~\ref{line:approx diameter output}}, we output $\frac{\epsilon D'}{2n}\times D(G, w')$ which is guaranteed to be $(1+\epsilon)$-approximation by Proposition~\ref{prop:approx diameter guarantee}. This completes the $O((1+1/\epsilon)n)$-time $(1+\epsilon))$-approximation algorithm for computing weighted diameter $D(G, w)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Approximating Radius in {\large $\mathbf{O(n)}$} time}

\paragraph{Radius} 
The algorithm is almost the same as the case of approximating the diameter. The only change is that we define $D'$ to be $D'=\max_{u\in V(G)} \dist_{G, w}(s, u)$. See Algorithm~\ref{algo:approx radius}. 

\begin{algorithm}\caption{{Approximate Radius in $O(n)$ time}}\label{algo:approx radius}
\begin{algorithmic}[1]
\State Solve single-source shortest path (\sssp) from an arbitrary node $s$ using the distributed version of Bellman-Ford's algorithm~\cite{peleg,Lynch-Book,Santoro-book}. Let $D'=\max_{u\in V(G)} \dist_{G, w}(s, u)$. {\small // $O(n)$ time. We claim that $\rad(G, w)\leq D'\leq 2\rad(G, w)$ (Claim~\ref{claim:two approx of diameter}).}\label{line:two approx radius}

\State For any edge $uv$ in $G$, let $w'(uv)=\lceil \frac{2n w(uv)}{\epsilon D'}\rceil$. {\small // No communication is needed}\label{line:round weight for approx radius}

\State Network $G$ uses the algorithm in Proposition~\ref{prop:pseudopoly time} to compute $K$-\apsp on $(G, w')$ where $K=(1+2/\epsilon)n$. {\small // Takes $O(K+n)=O((1+1/\epsilon)n)$ time.}\label{line:approx radius run pseudoply algo}

\State Output $\tilde R= \frac{\epsilon D'}{2n}\rad(G, w')$.\label{line:approx radius output}
\end{algorithmic}
\end{algorithm}

We use the following claim which is identical to Claim~\ref{claim:two approx of diameter}. 
%
\begin{claim}\label{claim:two approx of radius}
$\rad(G, w)\leq D'\leq 2\rad(G, w)$.
\end{claim}
\begin{proof}
By definitions of $D'$ and $\rad(G, w)$,
$$D'=\max_{u\in V(G)} \dist_{G, w}(s, u)\geq \min_{s\in V(G)} \max_{u\in V(G)} \dist_{G, w}(s, u)=\rad(G, w),$$
proving the first inequality. For the second inequality, let $u^*=\arg\min_{u\in V(G)} \max_{v\in V(G)} \dist_{G, w}(u, v)$. In other words, $u^*$ is such that $\max_{v\in V(G)} \dist_{G, w}(u^*, v)=\rad(G, w)$. Observe that for any $v\in V(G)$, $\dist_{G, w}(s, v)\leq \dist_{G, w}(u^*, s)+\dist_{G, w}(u^*, v)\leq 2R(G, w)$. Thus,
$D'=\max_{s, v\in V(G)}\dist_{G, w}(s, v)\leq 2R(G, w)$
as claimed.
\end{proof}

%
%
%The rest of the analysis is identical to the case of approximating the diameter. 
%
We can then use an analysis identical to the case of approximating the diameter to obtain the following.%\selfnote{CHECK!!!}
{
%\renewcommand{\thetheorem}{\ref{prop:approx raduis guarantee}}
\begin{proposition}\label{prop:approx radius guarantee}
$\rad(G, w')\leq (1+2/\epsilon)n$ and $\rad(G, w)$ $\leq$ $\frac{\epsilon D'}{2n}\times \rad(G, w')$ $\leq$ $(1+\epsilon)\rad(G, w).$
%\begin{align}
%D(G, w')& =(1+2/\epsilon) n, ~~~and \label{eq:approx diameter main one}\\
%D(G, w) \leq\frac{\epsilon D'}{2n}\times D(G, w')&\leq(1+\epsilon)D(G, w).\label{eq:approx diameter main two}
%\end{align}
\end{proposition}
%\addtocounter{theorem}{-1}
%}
The correctness of Algorithm~\ref{algo:approx radius} follows. Its running time is clearly $O((1+1/\epsilon)n)$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Approximating All-Pairs Shortest Paths in {\large $\mathbf{O(n \log n)}$} time (Theorem~\ref{theorem:approx apsp})}\label{sec:approx apsp}

\selfnote{Note that we cannot solve $\cS$-\ksp faster since the ``diameter'' will be $n$ anyway.}

The algorithm for approximating \apsp is outlined in Algorithm~\ref{algo:approx apsp}. It is similar to the algorithm for approximating the diameter, except that we do not have $D'$, the two-approximation of the diameter. Instead, we will ``guess'' all possible values of the distance between every pair of nodes, using $D'_i=2^i$, as shown in the for-loop of Algorithm~\ref{algo:approx apsp}.

\begin{algorithm}\caption{{Approximate All-Pairs Shortest Paths in $O(n\log n)$ time}}\label{algo:approx apsp}
\begin{algorithmic}[1]

\State Let $w_{max}=\max_{uv\in E(G)} w(uv)$.

\For{$i=1, 2, 3, \ldots, \log w_{max}$}

\State Let $D'_i=2^i$.

\State For any edge $uv$ in $G$, let $w'_i(uv)=\lceil \frac{2n w(uv)}{\epsilon D'_i}\rceil$. {\small // No communication is needed.}\label{line:round weight for approx apsp}

\State Network $G$ uses the algorithm in Proposition~\ref{prop:pseudopoly time} to compute $K$-\apsp on $(G, w'_i)$ where $K=(1+2/\epsilon)n$. {\small // Takes $O(K+n)=O(n)$ time. As a result, every node $u$ knows $\dist_{G, w'_i}^{(1+2/\epsilon)n}(s, u)$, for all $s$.}\label{line:approx apsp run pseudoply algo}

\EndFor

\State For every node $u$ and $s$, node $u$ sets the approximate distance from $s$ to be $\tilde \dist_{G, w}(s, u) = \min_i \frac{\epsilon D'_i}{2n} \dist_{G, w'_i}^{(1+2/\epsilon)n}(s, u)$.\label{line:approx apsp output}
\end{algorithmic}
\end{algorithm}

%
% ------  This part is already moved to other sections -----------
%
%Correctness of the algorithm is guaranteed by Proposition~\ref{prop:approx apsp guarantee} which follows easily from the following lemma.
%
%\begin{lemma}\label{lem:approx apsp guarantee}
%Consider any node $u$ and $v$. For any $i$,
%\begin{align}
%\frac{\epsilon D'_{i}}{2n}\times \dist_{G, w'_i}(u, v)\geq \dist_{G, w}(u, v).\label{eq:apsp approx main one}
%\end{align}
%Moreover, for $i^*$  such that $D'_{i^*-1}\leq \dist_{G, w}(u, v)\leq D'_{i^*}$, we have that
%\begin{align}
%\dist_{G, w'_{i^*}}(u, v)&\leq (1+2/\epsilon)n ~~\mbox{and}\label{eq:apsp approx main two}\\
%\frac{\epsilon D_{i^*}}{2n}\times \dist_{G, w'_{i^*}}(u, v) &\leq (1+\epsilon)\dist_{G, w}(u, v).\label{eq:apsp approx main three}
%\end{align}
%\end{lemma}
%\begin{proof}
%Let $P=\langle u=x_0, x_1, \ldots, x_\ell=v\rangle$ be any shortest $u$-$v$ path (thus $2^{i^*}\leq w(P)\leq 2^{i^*+1}$). Then,
%\begin{align}
%\dist_{G, w'_{i^*}}(u, v)&=\sum_{j=0}^{\ell-1} \left\lceil \frac{2n w(x_jx_{j+1})}{\epsilon D'_{i^*}}\right\rceil\label{eq:apsp approx one} \\
%&\leq \frac{2n}{\epsilon D'_{i^*}}\sum_{j=0}^{\ell-1} w(x_jx_{j+1}) + (\ell-1)\label{eq:apsp approx two}\\
%&\leq \frac{2n}{\epsilon D'_{i^*}}\dist_{G, w}(u, v) + (n-1) \label{eq:apsp approx three}\\
%&\leq (1+2/\epsilon)n \label{eq:apsp approx four}
%\end{align}
%where the last inequality is because $D'_{i^*}\geq \dist_{G, w}(u,v)$. This proves Eq.\eqref{eq:apsp approx main two}.
%
%Using Eq.\eqref{eq:apsp approx three}, we also have that
%\begin{align*}
%\frac{\epsilon D'_{i^*}}{2n}\times \dist_{G, w'_{i^*}}  & \leq \frac{\epsilon D'_{i^*}}{2n}\times \left(\frac{2n}{\epsilon D'_{i^*}}\dist_{G, w}(u, v) + (n-1)\right)\\
%&\leq \dist_{G, w}(u, v)+\frac{\epsilon}{2}D'_{i^*}\\
%&\leq (1+\epsilon)\dist_{G, w}(u, v)
%\end{align*}
%where the last inequality is because $D'_{i^*}=2D'_{i^*-1}\leq 2\dist_{G, w}(u, v)$. This proves Eq.\eqref{eq:apsp approx main three}
%
%Finally, observe that for any $i$ and the path $P$ defined as before, we have
%\begin{align*}
%\dist_{G, w'_{i}}(u, v)&\geq \sum_{j=0}^{\ell-1} \frac{2n w(x_jx_{j+1})}{\epsilon D'_i}\nonumber\\
%&\geq \frac{2n}{\epsilon D'_i}  \dist_{G, w}(u, v)\,.%\label{eq:diameter approx five}\,.
%\end{align*}
%It follows that
%%
%\begin{align*}
%\frac{\epsilon D'_i}{2n}\times\dist_{G, w'_i}(u, v) & \geq \frac{\epsilon D'_i}{2n}\times \left(\frac{2n}{\epsilon D'_i}  \dist_{G, w}(u, v)\right)\\
%&\geq \dist_{G, w}(u, v)\,.
%\end{align*}
%%
%This proves Eq.\eqref{eq:apsp approx main one} and completes the proof of Lemma~\ref{lem:approx apsp guarantee}.
%\end{proof}
%
% ---------------------------------------------------------------

Now we prove Proposition~\ref{prop:approx apsp guarantee}.

{\renewcommand{\thetheorem}{\ref{prop:approx apsp guarantee}}
\begin{proposition}[Restated]
For any nodes $u$ and $v$, if we let $\tilde d_{G, w}(u, v)$ = $\min_i  \frac{\epsilon D'_{i}}{2n}\times \dist^{(1+2/\epsilon)n}_{G, w'_i}(u, v)$, then $\dist_{G, w}(u, v)\leq \tilde d_{G,w}(u, v)\leq (1+\epsilon)\dist_{G, w}(u, v)$.
\end{proposition}
\addtocounter{theorem}{-1}
}
\begin{proof} Note that
$$\tilde d_{G, w}(u, v)= \min_i \frac{\epsilon D'_{i}}{2n}\times\dist^{(1+2/\epsilon)n}_{G, w'_i}(u, v)= \min_i \frac{\epsilon D'_{i}}{2n}\times\dist_{G, w'_i}(u, v)$$
where the second equality is due to Eq.\eqref{eq:apsp approx main two}. Then, Eq.\eqref{eq:apsp approx main one} and \eqref{eq:apsp approx main three} imply that $\tilde \dist_{G, w}(u, v)\geq \dist_{G, w}(u, v)$ and $\tilde \dist_{G, w}(u, v)\leq (1+\epsilon)\dist_{G, w}(u, v)$, respectively.
\end{proof}


==> arXiv/G_prime.tex <==
\section{Using {\large$\mathbf{(G'_{\lowercase{\large u}}, w')}$} (Proposition~\ref{prop:G prime})} \label{sec:G prime}

In this section, we show the key proposition that proves the correctness of our exact algorithm (Proposition~\ref{prop:G prime}): For any nodes $u$ and $v$ in clusters $C_j$ and $C_j'$, respectively,  $\dist_{G, w_i}(u, v)=\dist_{G'_u, w'}(c_j, c_{j'})$, where  $G'_u$ is as constructed in Line~\ref{line:G prime} of Algorithm~\ref{algo:apsp}.

To prove the proposition, first observe that if $j=j'$ then the proposition is clearly true since the distance between nodes in the same cluster have distance zero in $(G, w_i)$. So, we will assume that $j\neq j'$ in the rest of this section.

Let $P=\langle u=x_0, x_1, \ldots, x_\ell=v\rangle$ be any shortest $u$-$v$ path in $(G, w_i)$. We decompose $P$ into simple paths $P_1, P_2, \ldots, P_t$, for some $t$, as follows. Initially, let $j=1$. While $j\leq \ell$ and $x_j$ is in the cluster $C_{j'}$ that contains $x_0$ or $|C_{j'}|\leq \sqrt{n}$, we increase $j$. When we stop increasing $j$, we let $P_1=\langle x_0, \ldots, x_j\rangle$. We then repeat the same process to construct other subpaths on $\langle x_j, \ldots, x_\ell\rangle$.

Note the following properties of $P_1, \ldots, P_t$. Let  $P_i=\langle x_i^0, x_i^1, \ldots, x_i^{\ell_i}\rangle$, for some $\ell_i$, and let $C_i^j$ be the cluster containing $x_i^j$. Then, (1) for any $i$, $C_i^0\neq C_i^{\ell_i}$, (2) for any $i$ and $j<\ell_i$, either $C_i^j=C_i^0$ or $|C_i^j|\leq \sqrt{n}$, and (3) for any $i>1$, $|C_i^0|>\sqrt{n}$.


%with the following properties for every $i$: (1) two end nodes in $P_i$ are in different clusters and (2) every node in $P_i$ is either in the same cluster as one of the end nodes of $P_i$ or in a small cluster (of size at most $\sqrt{n}$).
%
%To be precise, denote every path $P_i$ by  $P_i=\langle x_i^0, x_i^1, \ldots, x_i^{\ell_i}$, for some $\ell_i$, and let $C_i^j$ be the cluster containing $x_i^j$. (Note that $x_i^0=x_{i-1}^{\ell_{i-1}}$.) We want that, for any $i$, (1) $C_i^0\neq C_i^{\ell_i}$, and (2) for any $j$, either $x_i^j\in C_i^0$, $x_i^j\in C_i^{\ell_i}$ or $|C_i^j|\leq \sqrt{n}$.

%We can always decompose any path $P$ into paths with the above properties, as follows. Let $P_1$ be the longest path containing $x_0$ that satisfies the second property above. We then remove edges in $P_1$ and repeat the process.
%
%Note that $P_1$ contains at least one edge since a path having one edge always satisfy the the second property. Moreover, $P_1$ must satisfy the first property; otherwise, we can include one more node to $P_1$ while satisfying the seconding property, contradicting the fact that $P_1$ is the longest path satisfying the second property.

Consider any subpath $P_i$. Let $j'$ be the maximum  number such that $x_i^{j'}\in C_i^0$. Let $P'_i=\langle x_i^{j'}, \ldots, x_i^{\ell_i}\rangle$ be the subpath of $P_i$ starting at $x_i^{j'}$. Observe that all internal nodes of $P'_i$ are in small clusters (of size at most $\sqrt{n}$), by the second property. So, $P'_i$ is also a path in $H$. In other words, $\dist_{G, w_i}(x_i^{j'}, x_i^{\ell_i})=\dist_{H, w_i}(x_i^{j'}, x_i^{\ell_i})$. Thus, by Proposition~\ref{prop:G prime}, $d'(x_i^{j'}, x_i^{\ell_i})=\dist_{G, w_i}(x_i^{j'}, x_i^{\ell_i})$. It follows that $d'(C_i^0, C_i^{\ell_i})=d'(C_i^{j'}, C_i^{\ell_i})\leq \dist_{G, w_i}(x_i^{j'}, x_i^{\ell_i})=\dist_{G, w_i}(x_i^{0}, x_i^{\ell_i}).$ So,
%
$$\sum_{i=1}^{t} d'(C_i^0, C_i^{\ell_i})\leq \sum_{i=1}^{t} d'(x_i^0, x_i^{\ell_i})=w_i(P)\,.$$
%
Since $P$ is a shortest $u$-$v$ path, we have that $\sum_{i=1}^{t} d'(C_i^0, C_i^{\ell_i})=w_i(P)$. 
%
Finally, we claim that we have edges $c_i^0c_i^{\ell_i}$ of weight $d'(C_i^0, C_i^{\ell_i})$ for all $i$; in other words, $u$ knows $d'(C_i^0, C_i^{\ell_i})$ for all $i$. This is clear for $i=1$ since $u\in C_i^0$ and so we compute $d'(C_i^0, C_i^{\ell_i})$ from Line~\ref{line:collect distance within cluster} of Algorithm~\ref{algo:apsp}. For $i>1$, the third property implies that $|C_i^0|>\sqrt{n}$. Thus, $u$ will know $d'(C_i^0, C_i^{\ell_i})$ from Line~\ref{line:broadcast big cluster} of Algorithm~\ref{algo:apsp}.



==> arXiv/abstract.tex <==
\begin{abstract}

A distributed network is modeled by a graph having $n$ nodes (processors) and  diameter $\diam$. We study the time complexity of approximating {\em weighted} (undirected) shortest paths on distributed networks with a $O(\log n)$ {\em bandwidth restriction} on edges (the standard synchronous \congest model). The question whether approximation algorithms help speed up shortest paths computation was raised since at least 2004 by Elkin (SIGACT News 2004). The unweighted case of problem is well-understood while its weighted counterpart is  fundamental problem in the area of distributed approximation algorithms and remains widely open. We present new algorithms for computing both single-source shortest paths (\sssp) and all-pairs shortest paths (\apsp) in the weighted case. 

Our main result is an algorithm for \sssp. Previous results are the classic $O(n)$-time Bellman-Ford algorithm and an $\tilde O(n^{1/2+1/2k}+D)$-time $(8k\lceil \log (k+1) \rceil -1)$-approximation algorithm, for any integer $k\geq 1$, which follows from the result of Lenzen and Patt-Shamir (STOC 2013). (Note that Lenzen and Patt-Shamir in fact solve a harder problem, and we use $\tilde O(\cdot)$ to hide the $O(\poly\log n)$ term.) We present an $\tilde O(n^{1/2}D^{1/4}+D)$-time $(1+o(1))$-approximation algorithm for \sssp. This algorithm is {\em sublinear-time} as long as $D$ is sublinear, thus yielding a sublinear-time algorithm with almost optimal solution. When $D$ is small, our running time matches the lower bound of $\tilde \Omega(n^{1/2}+D)$ by Das Sarma et al. (SICOMP 2012), which holds even when $D=\Theta(\log n)$, up to a $\poly\log n$ factor. 

%In particular, in the typical case of low-diameter networks (i.e. $D=\tilde O(1)$), which is sometimes of a special interest, our running time is tight.  


As a by-product of our technique, we obtain a simple $\tilde O(n)$-time $(1+o(1))$-approximation algorithm for \apsp, improving the previous $\tilde O(n)$-time $O(1)$-approximation algorithm following from the results of Lenzen and Patt-Shamir. We also prove a matching lower bound. 
%
Our techniques also yield an $\tilde O(n^{1/2})$ time algorithm on fully-connected networks, which guarantees an exact solution for \sssp and a $(2+o(1))$-approximate solution for \apsp. 
%
All our algorithms rely on two new simple tools: {\em light-weight algorithm for bounded-hop \sssp} and {\em shortest-path diameter reduction via shortcuts}. These tools might be of an independent interest and useful in designing other distributed algorithms. 
\end{abstract}

\endinput

% ------- The version below is for STOC 2014 Submission ------

\begin{abstract}

A distributed network is modeled by a {\em weighted} undirected graphs, having $n$ nodes (processors), $m$ edges (links), and diameter $\diam$. We study the time complexity of approximating shortest paths on distributed networks with a $O(\log n)$ {\em bandwidth restriction} on edges (the standard CONGEST model). The question whether approximation algorithms help speed up shortest paths computation was raised since at least 2004 by Elkin (SIGACT News 2004). The unweighted case of problem is well-understood while its weighted counterpart is among fundamental problems in the area of distributed approximation algorithms that remain widely open. We present new algorithms for computing both single-source shortest paths (SSSP) and all-pairs shortest paths (APSP) in the weighted case. 

Our main result is an algorithm for SSSP. Previous results are the classic $\tilde O(n)$-time Bellman-Ford algorithm and a $\tilde O(n^{1/2+1/2k}+D)$-time $(8k\lceil \log (k+1) \rceil -1)$-approximation algorithm, for any integer $k\geq 1$, by Lenzen and Patt-Shamir (STOC 2013). (We use $\tilde O(\cdot)$ to hide the $O(\poly\log n)$ term.) We present a $\tilde O(n^{1/2}D^{1/4}+D)$-time $(1+o(1))$-approximation algorithm for SSSP. This algorithm is {\em sublinear-time} as long as $D$ is sublinear, thus yielding a sublinear-time algorithm with almost optimal solution. Our running time almost matches the lower bound of $\tilde \Omega(n^{1/2}+D)$ by Das Sarma et al. (STOC 2011) which holds even when $D=\Theta(\log n)$. In particular, in the typical case of low-diameter networks (i.e. $D=\tilde O(1)$), which is sometimes of a special interest, our running time is tight.  


As a by-product of our technique, we obtain a simple $\tilde O(n)$-time $(1+o(1))$-approximation algorithm for APSP, improving the previous $\tilde O(n)$-time $O(1)$-approximation algorithm of Lenzen and Patt-Shamir. We also prove a matching lower bound. Our techniques also yield a $\tilde O(n^{1/2})$ time algorithm on fully-connected networks, which guarantees an exact solution for SSSP and a $(2+o(1))$-approximate solution for APSP. All our algorithms rely on two new simple tools: {\em light-weight algorithm for bounded-hop SSSP} and {\em shortest-path diameter reduction via shortcuts}. These tools might be of an independent interest and useful in designing other distributed algorithms. 
\end{abstract}

% -- 03 Nov 2013 --
%
%\begin{abstract}
%We study the fundamental problem of computing shortest paths on bandwidth-constrained distributed networks (the standard CONGEST model). Our main results concern two open problems raised almost a decade ago by Elkin [SIGACT News 2004] in the area of {\em distributed approximation}. The first question concerns the complexity of the single-source shortest paths (SSSP) problem. It is known that no algorithm (even an approximation one) can be faster than $O(n^{1/2}+D)$ time, where $n$ is the number of nodes in the network and $D$ is the network diameter. No non-trivial algorithm is known. We almost settle this question by showing an {\em almost tight} sublinear-time approximation algorithm for this problem: in $\tilde O(n^{1/2}D^{1/4}+D)$ time, we can $(1+o(1))$-approximate SSSP where $\tilde O$ hides an $O(\poly\log n)$ factor. The second question asks for lower bounds on computing single-source and all-pairs shortest paths (APSP) on {\em fully-connected networks}. While we do not directly answer this question, we show that this model also admits non-trivial {\em sublinear-time} {\em upper} bounds: In  $\tilde O(\sqrt{n})$ time, SSSP can be solved exactly and APSP can be $(2+o(1))$-approximated. Our algorithms crucially rely on two new simple tools called {\em light-weight bounded-hop SSSP algorithm} and {\em shortest-path diameter reduction techniques via shortcuts}, which might be of an independent interest and useful in other applications. 
%\end{abstract}


% -- 03/07/2013 --
%
%\begin{abstract}
%We study the fundamental problem of computing All-Pairs Shortest Paths (\apsp) on bandwidth-constrained distributed networks. We focus on the {\em weighted} case which remains open despite so much recent progress on the unweighted one.
%
%We present a randomized $O(n\sqrt{n}\log^2 n)$-time {\em exact} algorithm for this problem, where $n$ is the number of nodes in the network. This is the {\em first} non-trivial exact algorithm, improving the previous trivial $O(m)$-time algorithm, where $m$ is the number of edges in the network, on dense graphs.
%
%Moreover, we present a deterministic $O(n\log n)$-time $(1+\epsilon)$-approximation algorithm, for any constant $\epsilon>0$. This improves many previous algorithms based on low-distortion sparse embeddings, in both time and approximation guarantees. We also observe that this algorithm is {\em tight} in the sense that no algorithm can be significantly faster, unless the approximation guarantee is prohibitively large.
%
%Our algorithms can be easily extended to computing or approximating other problems on weighted networks, such as diameter, girth, radius, center and peripheral vertices. For approximating diameter and radius, we show that the running time could be slightly improved to $O(n)$.
%\end{abstract}



%\begin{abstract}
%We study the fundamental issue of time complexity of computing all-pairs shortest paths (\apsp) on an $n$-node $m$-edge bandwidth-constrained distributed network. We focus on the {\em weighted} case which remains fairly open compared to its unweighted counterpart.
%
%We present a randomized $O(n\sqrt{n}\log^2 n)$-time {\em exact} algorithm for this problem. This is the {\em first} non-trivial exact algorithm and improves the previous trivial $O(m)$-time algorithm for the case of dense graph.
%
%Moreover, we present a deterministic $O(n\log n)$-time $(1+\epsilon)$-approximation algorithm, for any $\epsilon>0$. This improves previous $(2k-1)$-approximation $O(kn^{1+1/k})$-time algorithms, for any $k$, based on low-distortion embedding techniques. We also show that our algorithm is {\em tight} in the sense that no algorithm can run faster than $\Omega(n/\poly\log n)$, even on low-diameter unweighted networks, unless the approximation ratio is fairly large ($\Omega(\poly\log n)$).
%
%Our algorithms can be easily extended to computing or approximating other problems on weighted networks, such as diameter, girth, radius, center and peripheral vertices. For approximating diameter and radius, we show that the running time could be slightly improved to $O(n)$.\danupon{Write something for radius. Key: Eccentricity $\geq radius$ and $\leq 2radius$; so, $rad\geq ecc/2 \geq rad/2$.}
%%
%%We also present a deterministic $O(n)$-time $(1+\epsilon)$-approximation algorithm for computing the network's weighted diameter. Due to the known lower bound, this algorithm is {\em tight} in the sense that the running time cannot be improved further, even in the unweighted case, unless the approximation ratio is relaxed to at least $3/2$.\danupon{Can also use this idea to compute girth, etc.?}
%%
%\end{abstract}

%\begin{abstract}
%We study time complexity of the fundamental problem of computing all-pairs shortest paths (\apsp) on {\em weighted} $n$-node $m$-edge distributed networks. While this problem is well-understood in the unweighted case, not much is previously known in the weighted case: no exact algorithm is known except the trivial $O(m)$-time algorithm (aggregating the whole network at one node), and the only known non-trivial algorithm is the $(2k-1)$-approximation $O(kn^{1+1/k})$-time algorithm, for any $k$, via spanners. In this paper, we show the followings.
%%
%\begin{itemize}[noitemsep]
%\item Randomized (Las Vegas) $O(n\sqrt{n}\log^2 n)$-time {\em exact} algorithm for \apsp.
%\item Deterministic $(1+\epsilon)$-approximation $O(n\log n)$-time algorithm for \apsp.
%\end{itemize}
%%
%Additionally, we show a deterministic $(1+\epsilon)$-approximation $O(n)$-time algorithm for computing the network's (weighted) diameter, matching the algorithms for the unweighted case.
%%
%We also show that our approximation algorithm for \apsp is tight up to a $\poly \log n$ factor in the sense that the running time {\em cannot} be improved further, even when we allow a {\em large approximation factor}.
%\end{abstract}



%\begin{abstract}
%We show a randomized distributed algorithm for computing all-pair shortest path (APSP) of $n$-node {\em weighted} networks that finishes in  $\tilde O(n)$ time with high probability, where $\tilde O$ hides a $\poly\log n$ factor. Our running time significantly improves the previous pseudo-polynomial time and $O(n^2)$-time algorithms, and matches the optimal $O(n)$-time distributed algorithm for the {\em unweighted} case by Holzer and Wattenhofer [PODC'12] and Peleg, Roditty and Tal [ICALP'12], up to a logarithmic factor. Our algorithm is {\em optimal} due to the $\tilde \Omega(n)$ lower bound by Frischknecht, Holzer and Wattenhofer [SODA'12]. We also show a simple proof that our algorithm is optimal even when we allow {\em approximation algorithm}: Any approximation distributed algorithm (for any degree of approximation) requires $\tilde \Omega(n)$ time.\danupon{This is actually $\Omega(n/B)$.}
%\end{abstract}


==> arXiv/approx_algo.tex <==
\section{Approximation Algorithms}\label{sec:approx}

%
% ---------------- The commented text here is already moved -----------------
%
%\subsection{Pseudo-Polynomial Time Algorithm for {\large $\mathbf{K}$}-APSP (Proof of Proposition~\ref{PROP:PSEUDOPOLY TIME})}\label{sec:proof of PROP:PSEUDOPOLY TIME}
%We first argue that there exists a $O(n+K)$-time algorithm for $K$-\apsp on network $G$ with positive symmetric integral weight $w$, as claimed in Proposition~\ref{PROP:PSEUDOPOLY TIME}. This algorithm is pseudo-polynomial since $K$ could be as large as $D(G, w)$.
%
%{\renewcommand{\thetheorem}{\ref{prop:pseudopoly time}}
%\begin{proposition}[Restated]
%$K$-\apsp on network $G$ with {\em positive symmetric} integral weight $w$ can be solved in $O(n+K)$-time.
%\end{proposition}
%\addtocounter{theorem}{-1}
%}
%
%Consider Algorithm~2 in \cite{HolzerW12} which is used for the problem called {\em $\cS$-shortest paths} (computing distances from sources in $\cS$ on an unweighted network $G$). This algorithm is outlined in Algorithm~\ref{algo:HolzerW12}. This algorithm executes the breadh-first search (BFS) algorithms from $q$ different sources in $\cS$ in parallel, where the BFS algorithm starting at node $u$ forwards $u$ (representing the unique ID of node $u$) in the BFS manner until every node receives $u$. We let BFS$_i$ denote the BFS algorithm starting at $s_i$, and $T_{s_i}$ denote the BFS tree constructed by BFS$_i$.
%
%
%
%\begin{algorithm}
%\caption{$K$-\apsp $(G, \cS=\{s_1, \ldots, s_q\})$ \cite{HolzerW12}}\label{algo:HolzerW12}
%{\bf Input:} Unweighted undirected graph $G$ and set $\cS$ of $q$ source nodes $s_1, \ldots s_q$. %Assume wlog that $s_1<s_2<\ldots s_K$.
%
%{\bf Output:} Every node $u$ knows $\dist^K_G(s, u)$.
%
%%\medskip $\bullet$ Let $t$ be the time this algorithm starts. We can assume that all nodes know $t$.
%
%\medskip $\bullet$ Initially, source nodes $s_1, \ldots, s_q$ trigger the algorithm to start by sending a message $(s, 0)$ to itself.
%
%
%%\medskip\textit{\textbf{Main subroutine:}}
%
%$\bullet$ When a node $u$ receives a message $(s_i, \ell)$ for some $\ell$, it does the following.
%
%\begin{algorithmic}[1]
%
%%\algrestore{bfsone}
%
%\If{$u$ has {\em not} already received $(s_i, \ell')$ for any $\ell'$}
%
%\State $u$ now knows that $\dist_{G}(s, u)=\ell$.\label{line:HolzerW compute distance}
%
%%\State $u$ sends through all directed edges $\overrightarrow{uv}$ a message $(s, t, \ell+w(\overrightarrow{uv}))$ at time $t+\ell+w(\overrightarrow{uv})$.\label{line:bfs send message}
%
%\State $u$ sends message $(s_i, \ell+1)$ to all its neighbors that have not sent any message of the form $(s_i, \ell')$ to $u$.
%
%\State For any neighbor $v$ of $u$, if there are many messages of the form $(s', \ell'+1)$ that $u$ and $v$ want to send to each other, we allow them to send only the message with smallest $s'$ (if there are ties, send the one with smallest $\ell'$). (Thus, there are at most one message sent between $u$ and $v$ in each round.) For other messages that are not sent, $u$ and $v$ will try to send them again in the next rounds.\label{line:HolzerW main trick}
%\EndIf
%
%\end{algorithmic}
%\end{algorithm}
%
%
%
%The important trick of this algorithm is that, when there are many messages that the algorithm wants to send on the same edge at the same time (on any direction), we allow it to send only one message with the smallest ID, as described in the Line~\ref{line:HolzerW main trick} of Algorithm~\ref{algo:HolzerW12}.
%%
%We use the following two properties claimed in the proof of Theorem~3 of \cite{HolzerW12}.
%
%\noindent {\bf P1:} For any nodes $v_1$ an $v_2$, messages containing the ID of $s_i$ are sent over the edge $(v_1 , u)$ earlier than over edge $(v_2 , u)$ if and only if $\dist_{G}(s_i, v_1 ) < \dist_G(s_i, v_2 )$.
%
%\noindent {\bf P2:}  For any indices $i$ and $j$ and node $u$, during traveling on any $s_i$-$u$ path of $T_{s_i}$, the message of ID $s_i$ gets delayed {\em at most once} by the computation BFS$_j$ if ID $s_j$ is strictly smaller then ID $s_i$.
%
%Property P2 implies that any message of the form $(s_i, \ell)$ will arrive at any node $u$ in $\ell+|\cS|-1$ rounds since it will be delayed by at most $|\cS|-1$ times (by $|\cS|-1$ other messages). Property P1 guarantees that each node $u$ of distance $\ell$ from $s_i$ will receive message $(s_i, \ell)$ without receiving any message $(s_i, \ell')$ earlier, for any other value of $\ell'$. This guarantees the correctness of the algorithm (as in Line~\ref{line:HolzerW compute distance} of Algorithm~\ref{algo:HolzerW12}). We conclude these properties by the following observation.
%%
%\begin{observation}
%For any $K$ and $s_i\in \cS$, after $K+|\cS|-1$ rounds every node $u$ such that $\dist_G(s_i, u)\leq K$ knows $\dist_G(s_i, u)$.
%\end{observation}
%%
%Now, to solve $K$-\apsp on a weighted network $(G, w)$, we construct a network $G'$ where we replace each edge $uv$ of length $w(uv)$ in $(G, w)$ by a $w(uv)$-length path of $\langle u=x_0, x_1, \ldots, x_{w(uv)}=v\rangle$. Network $(G, w)$ will simulate an algorithm on $G'$  by letting one of $u$ and $v$ simulate the computation of $x_1, \ldots, x_{w(uv)-1}$. In particular, $(G, w)$ will simulate Algorithm~\ref{algo:HolzerW12} on $G'$ with $\cS=V(G)$ for $K$ step. By the above observation, when the simulation is finished, for every $u, v\in V(G)\subseteq V(G')$ such that $\dist_{G'}(u, v)\leq K$, node $v$ knows $\dist_{G'}(u, v)$ which is equal to $\dist_{G, w}(u, v)$. Node $v$ can then use this solution to answer $K$-\apsp on $(G, w)$.\danupon{To do: Solve $(\cS, K)$-\ksp instead}


\subsection{Approximating Diameter and Radius in {\large $\mathbf{O(n)}$} time (Theorem~\ref{theorem:diameter girth})}\label{sec:approx diameter}



%\paragraph{Approximating Diameter in $O(n)$ time (Theorem~XXX)}
We now prove Theorem~\ref{theorem:diameter girth}. 
%; i.e., we show that, for any constant $\epsilon>0$, there is an $O(n)$-time deterministic distributed algorithm such that, for any weighted network $(G, w)$, the algorithm outputs $\tilde D$ such that $D(G, w)\leq \tilde{D} \leq (1+\epsilon)D(G, w)$.

{\renewcommand{\thetheorem}{\ref{theorem:diameter girth}}
\begin{theorem}[Restated]
For any $\epsilon>0$, there are deterministic $(1+\epsilon)$-approximation $O((1+\frac{1}{\epsilon})n)$-time algorithms for diameter and girth computation. 
\end{theorem}
\addtocounter{theorem}{-1}
}

\begin{algorithm}\caption{{Approximate Diameter in $O(n)$ time}}\label{algo:approx diameter}
\begin{algorithmic}[1]
\State Solve single-source shortest path (\sssp) from an arbitrary node $s$ using the distributed version of Bellman-Ford's algorithm~\cite{peleg,Lynch-Book,Santoro-book}. Let $D'=2\max_{u\in V(G)} \dist_{G, w}(s, u)$. {\small // $O(n)$ time. We claim that $D(G, w)\leq D'\leq 2D(G, w)$ (Claim~\ref{claim:two approx of diameter}).}\label{line:two approx diameter}

\State For any edge $uv$ in $G$, let $w'(uv)=\lceil \frac{2n w(uv)}{\epsilon D'}\rceil$. {\small // No communication is needed}\label{line:round weight for approx diameter}

\State Network $G$ uses the algorithm in Proposition~\ref{prop:pseudopoly time} to compute $K$-\apsp on $(G, w')$ where $K=(1+2/\epsilon)n$. {\small // Takes $O(K+n)=O((1+1/\epsilon)n)$ time.}\label{line:approx diameter run pseudoply algo}

\State \label{line:approx diameter output} Output $\tilde D = \frac{\epsilon D'}{2n}D(G, w')$.
\end{algorithmic}
\end{algorithm}

\paragraph{Approximating Diameter} We first show how to approximate the diameter. Approximating the radius will be done by slightly modifying the algorithm for approximating the diameter. 
%
We use the algorithm outlined in Algorithm~\ref{algo:approx diameter}. First, in {\bf Line~\ref{line:two approx diameter}}, we compute $D'=2\max_{u\in V(G)} \dist_{G, w}(s, u)$ for an arbitrary node $s$. This can be done in $O(n)$ time by the distributed version of Bellman-Ford's algorithm \cite{peleg}. Observe that $D'$ two-approximates $D(G, w)$:
\begin{claim}\label{claim:two approx of diameter}
$D(G, w)\leq D'\leq 2D(G, w)$.
\end{claim}
\begin{proof}
By definitions of $D'$ and $D(G, w)$,
$$D'=2\max_{u\in V(G)} \dist_{G, w}(s, u)\leq 2\max_{s,u\in V(G)} \dist_{G, w}(s, u)=2D(G, w),$$
proving the second inequality. For the first inequality, observe that for any $u, v\in V(G)$, $\dist_{G, w}(u, v)\leq \dist_{G, w}(s, u)+\dist_{G, w}(s, v)\leq 2\max_{u\in V(G)} \dist_{G, w}(s, u)=D'$. Thus, $D(G, w)= \max_{u,v\in V(G)} \dist_{G, w}(u, v)\leq D'$ as claimed.
\end{proof}
%
Next, in {\bf Line~\ref{line:round weight for approx diameter}}, we compute weight $w'$. We now prove the nice property of $w'$ as in Proposition~\ref{prop:approx diameter guarantee}.

{
\renewcommand{\thetheorem}{\ref{prop:approx diameter guarantee}}
\begin{proposition}[Restated]
%$D(G, w')=(1+2/\epsilon)n$ and $D(G, w)$ $\leq$ $D'\times D(G, w')$ $\leq$ $(1+\epsilon)D(G, w).$
\begin{align}
D(G, w')& \leq(1+2/\epsilon) n, ~~~and \label{eq:approx diameter main one}\\
D(G, w) \leq\frac{\epsilon D'}{2n}\times D(G, w')&\leq(1+\epsilon)D(G, w).\label{eq:approx diameter main two}
\end{align}
\end{proposition}
\addtocounter{theorem}{-1}
}
%\begin{align}
%D(G, w')& =(1+2/\epsilon) n, ~~~and \label{eq:approx diameter main one}\\
%D(G, w) \leq\frac{\epsilon D'}{2n}\times D(G, w')&\leq(1+\epsilon)D(G, w).\label{eq:approx diameter main two}
%\end{align}
%
%\begin{proposition}\label{prop:approx diameter guarantee}
%$D(G, w')=O(n)$ and $D(G, w)$ $\leq$ $D'\cdot D(G, w')$ $\leq$ $(1+\epsilon)D(G, w).$
%\end{proposition}
%
\begin{proof}%[of Proposition~\ref{prop:approx diameter guarantee}]
For any nodes $u$ and $v$, let $P=\langle u=x_0, x_1, \ldots, x_\ell=v\rangle$ be any shortest $u$-$v$ path. Then,
\begin{align}
\dist_{G, w'}(u, v)&=\sum_{i=0}^{\ell-1} \left\lceil \frac{2n w(x_ix_{i+1})}{\epsilon D'}\right\rceil \label{eq:diameter approx one}\\
&\leq \frac{2n}{\epsilon D'}\sum_{i=0}^{\ell-1} w(x_ix_{i+1}) + (\ell-1) \label{eq:diameter approx two}\\
&\leq \frac{2n}{\epsilon D'}D(G, w) + (n-1) \label{eq:diameter approx three}\\
&\leq (1+2/\epsilon)n \label{eq:diameter approx four}
\end{align}
where the last inequality is because $D'\geq D(G, w)$, by Claim~\ref{claim:two approx of diameter}. It follows that
$$D(G, w')=\max_{u, v} \dist_{G, w'}(u, v)\leq (1+1/2\epsilon) n$$
as claimed in Eq.~\eqref{eq:approx diameter main one}

Using Eq.\eqref{eq:diameter approx three}, we also have that
\begin{align*}
\frac{\epsilon D'}{2n}\times D(G, w') & = \frac{\epsilon D'}{2n}\times \max_{u, v} \dist_{G, w'}(u, v)\\
&\leq \frac{\epsilon D'}{2n}\times \left( \frac{2n}{\epsilon D'}D(G, w) + (n-1)\right)\\
&\leq D(G, w)+\frac{\epsilon}{2} D'\\
&\leq (1+\epsilon) D(G, w)
\end{align*}
where the last inequality is because $D'\leq 2D(G, w)$ by Claim~\ref{claim:two approx of diameter}. This proves the second inequality of Eq.~\eqref{eq:approx diameter main two}.

Finally, observe that for the path $P$ defined as before, we have
\begin{align}
\dist_{G, w'}(u, v)&\geq \sum_{i=0}^{\ell-1} \frac{2n w(x_ix_{i+1})}{\epsilon D'}\nonumber\\
&\geq \frac{2n}{\epsilon D'}  \dist_{G, w}(u, v)\label{eq:diameter approx five}\,.
\end{align}
It follows that
%
\begin{align*}
\frac{\epsilon D'}{2n}\times D(G, w') & \geq \frac{\epsilon D'}{2n}\times \max_{u, v} \dist_{G, w'}(u, v)\\
& \geq \frac{\epsilon D'}{2n}\times \max_{u, v}  \frac{2n}{\epsilon D'}  \dist_{G, w}(u, v)\\
& = D(G, w)
\end{align*}
%
where the second inequality is by Eq.\eqref{eq:diameter approx five}. This proves the first inequality of Eq.\eqref{eq:approx diameter main two} and completes the proof of Proposition~\ref{prop:approx diameter guarantee}.
\end{proof}


Now, in {\bf Line~\ref{line:approx diameter run pseudoply algo}}, we execute the pseudo-polynomial time algorithm in Proposition~\ref{prop:pseudopoly time} on $(G, w')$ using $K=(1+2/\epsilon)n$. Since $D(G, w')\leq (1+2/\epsilon)n$ (cf. Proposition~\ref{prop:approx diameter guarantee}), we will end up with the solution of \apsp on $(G, w')$, thus having the value of $D(G, w')$.
%
Finally, in {\bf Line~\ref{line:approx diameter output}}, we output $\frac{\epsilon D'}{2n}\times D(G, w')$ which is guaranteed to be $(1+\epsilon)$-approximation by Proposition~\ref{prop:approx diameter guarantee}. This completes the $O((1+1/\epsilon)n)$-time $(1+\epsilon))$-approximation algorithm for computing weighted diameter $D(G, w)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Approximating Radius in {\large $\mathbf{O(n)}$} time}

\paragraph{Radius} 
The algorithm is almost the same as the case of approximating the diameter. The only change is that we define $D'$ to be $D'=\max_{u\in V(G)} \dist_{G, w}(s, u)$. See Algorithm~\ref{algo:approx radius}. 

\begin{algorithm}\caption{{Approximate Radius in $O(n)$ time}}\label{algo:approx radius}
\begin{algorithmic}[1]
\State Solve single-source shortest path (\sssp) from an arbitrary node $s$ using the distributed version of Bellman-Ford's algorithm~\cite{peleg,Lynch-Book,Santoro-book}. Let $D'=\max_{u\in V(G)} \dist_{G, w}(s, u)$. {\small // $O(n)$ time. We claim that $\rad(G, w)\leq D'\leq 2\rad(G, w)$ (Claim~\ref{claim:two approx of diameter}).}\label{line:two approx radius}

\State For any edge $uv$ in $G$, let $w'(uv)=\lceil \frac{2n w(uv)}{\epsilon D'}\rceil$. {\small // No communication is needed}\label{line:round weight for approx radius}

\State Network $G$ uses the algorithm in Proposition~\ref{prop:pseudopoly time} to compute $K$-\apsp on $(G, w')$ where $K=(1+2/\epsilon)n$. {\small // Takes $O(K+n)=O((1+1/\epsilon)n)$ time.}\label{line:approx radius run pseudoply algo}

\State Output $\tilde R= \frac{\epsilon D'}{2n}\rad(G, w')$.\label{line:approx radius output}
\end{algorithmic}
\end{algorithm}

We use the following claim which is identical to Claim~\ref{claim:two approx of diameter}. 
%
\begin{claim}\label{claim:two approx of radius}
$\rad(G, w)\leq D'\leq 2\rad(G, w)$.
\end{claim}
\begin{proof}
By definitions of $D'$ and $\rad(G, w)$,
$$D'=\max_{u\in V(G)} \dist_{G, w}(s, u)\geq \min_{s\in V(G)} \max_{u\in V(G)} \dist_{G, w}(s, u)=\rad(G, w),$$
proving the first inequality. For the second inequality, let $u^*=\arg\min_{u\in V(G)} \max_{v\in V(G)} \dist_{G, w}(u, v)$. In other words, $u^*$ is such that $\max_{v\in V(G)} \dist_{G, w}(u^*, v)=\rad(G, w)$. Observe that for any $v\in V(G)$, $\dist_{G, w}(s, v)\leq \dist_{G, w}(u^*, s)+\dist_{G, w}(u^*, v)\leq 2R(G, w)$. Thus,
$D'=\max_{s, v\in V(G)}\dist_{G, w}(s, v)\leq 2R(G, w)$
as claimed.
\end{proof}

%
%
%The rest of the analysis is identical to the case of approximating the diameter. 
%
We can then use an analysis identical to the case of approximating the diameter to obtain the following.%\selfnote{CHECK!!!}
{
%\renewcommand{\thetheorem}{\ref{prop:approx raduis guarantee}}
\begin{proposition}\label{prop:approx radius guarantee}
$\rad(G, w')\leq (1+2/\epsilon)n$ and $\rad(G, w)$ $\leq$ $\frac{\epsilon D'}{2n}\times \rad(G, w')$ $\leq$ $(1+\epsilon)\rad(G, w).$
%\begin{align}
%D(G, w')& =(1+2/\epsilon) n, ~~~and \label{eq:approx diameter main one}\\
%D(G, w) \leq\frac{\epsilon D'}{2n}\times D(G, w')&\leq(1+\epsilon)D(G, w).\label{eq:approx diameter main two}
%\end{align}
\end{proposition}
%\addtocounter{theorem}{-1}
%}
The correctness of Algorithm~\ref{algo:approx radius} follows. Its running time is clearly $O((1+1/\epsilon)n)$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Approximating All-Pairs Shortest Paths in {\large $\mathbf{O(n \log n)}$} time (Theorem~\ref{theorem:approx apsp})}\label{sec:approx apsp}

\selfnote{Note that we cannot solve $\cS$-\ksp faster since the ``diameter'' will be $n$ anyway.}

The algorithm for approximating \apsp is outlined in Algorithm~\ref{algo:approx apsp}. It is similar to the algorithm for approximating the diameter, except that we do not have $D'$, the two-approximation of the diameter. Instead, we will ``guess'' all possible values of the distance between every pair of nodes, using $D'_i=2^i$, as shown in the for-loop of Algorithm~\ref{algo:approx apsp}.

\begin{algorithm}\caption{{Approximate All-Pairs Shortest Paths in $O(n\log n)$ time}}\label{algo:approx apsp}
\begin{algorithmic}[1]

\State Let $w_{max}=\max_{uv\in E(G)} w(uv)$.

\For{$i=1, 2, 3, \ldots, \log w_{max}$}

\State Let $D'_i=2^i$.

\State For any edge $uv$ in $G$, let $w'_i(uv)=\lceil \frac{2n w(uv)}{\epsilon D'_i}\rceil$. {\small // No communication is needed.}\label{line:round weight for approx apsp}

\State Network $G$ uses the algorithm in Proposition~\ref{prop:pseudopoly time} to compute $K$-\apsp on $(G, w'_i)$ where $K=(1+2/\epsilon)n$. {\small // Takes $O(K+n)=O(n)$ time. As a result, every node $u$ knows $\dist_{G, w'_i}^{(1+2/\epsilon)n}(s, u)$, for all $s$.}\label{line:approx apsp run pseudoply algo}

\EndFor

\State For every node $u$ and $s$, node $u$ sets the approximate distance from $s$ to be $\tilde \dist_{G, w}(s, u) = \min_i \frac{\epsilon D'_i}{2n} \dist_{G, w'_i}^{(1+2/\epsilon)n}(s, u)$.\label{line:approx apsp output}
\end{algorithmic}
\end{algorithm}

%
% ------  This part is already moved to other sections -----------
%
%Correctness of the algorithm is guaranteed by Proposition~\ref{prop:approx apsp guarantee} which follows easily from the following lemma.
%
%\begin{lemma}\label{lem:approx apsp guarantee}
%Consider any node $u$ and $v$. For any $i$,
%\begin{align}
%\frac{\epsilon D'_{i}}{2n}\times \dist_{G, w'_i}(u, v)\geq \dist_{G, w}(u, v).\label{eq:apsp approx main one}
%\end{align}
%Moreover, for $i^*$  such that $D'_{i^*-1}\leq \dist_{G, w}(u, v)\leq D'_{i^*}$, we have that
%\begin{align}
%\dist_{G, w'_{i^*}}(u, v)&\leq (1+2/\epsilon)n ~~\mbox{and}\label{eq:apsp approx main two}\\
%\frac{\epsilon D_{i^*}}{2n}\times \dist_{G, w'_{i^*}}(u, v) &\leq (1+\epsilon)\dist_{G, w}(u, v).\label{eq:apsp approx main three}
%\end{align}
%\end{lemma}
%\begin{proof}
%Let $P=\langle u=x_0, x_1, \ldots, x_\ell=v\rangle$ be any shortest $u$-$v$ path (thus $2^{i^*}\leq w(P)\leq 2^{i^*+1}$). Then,
%\begin{align}
%\dist_{G, w'_{i^*}}(u, v)&=\sum_{j=0}^{\ell-1} \left\lceil \frac{2n w(x_jx_{j+1})}{\epsilon D'_{i^*}}\right\rceil\label{eq:apsp approx one} \\
%&\leq \frac{2n}{\epsilon D'_{i^*}}\sum_{j=0}^{\ell-1} w(x_jx_{j+1}) + (\ell-1)\label{eq:apsp approx two}\\
%&\leq \frac{2n}{\epsilon D'_{i^*}}\dist_{G, w}(u, v) + (n-1) \label{eq:apsp approx three}\\
%&\leq (1+2/\epsilon)n \label{eq:apsp approx four}
%\end{align}
%where the last inequality is because $D'_{i^*}\geq \dist_{G, w}(u,v)$. This proves Eq.\eqref{eq:apsp approx main two}.
%
%Using Eq.\eqref{eq:apsp approx three}, we also have that
%\begin{align*}
%\frac{\epsilon D'_{i^*}}{2n}\times \dist_{G, w'_{i^*}}  & \leq \frac{\epsilon D'_{i^*}}{2n}\times \left(\frac{2n}{\epsilon D'_{i^*}}\dist_{G, w}(u, v) + (n-1)\right)\\
%&\leq \dist_{G, w}(u, v)+\frac{\epsilon}{2}D'_{i^*}\\
%&\leq (1+\epsilon)\dist_{G, w}(u, v)
%\end{align*}
%where the last inequality is because $D'_{i^*}=2D'_{i^*-1}\leq 2\dist_{G, w}(u, v)$. This proves Eq.\eqref{eq:apsp approx main three}
%
%Finally, observe that for any $i$ and the path $P$ defined as before, we have
%\begin{align*}
%\dist_{G, w'_{i}}(u, v)&\geq \sum_{j=0}^{\ell-1} \frac{2n w(x_jx_{j+1})}{\epsilon D'_i}\nonumber\\
%&\geq \frac{2n}{\epsilon D'_i}  \dist_{G, w}(u, v)\,.%\label{eq:diameter approx five}\,.
%\end{align*}
%It follows that
%%
%\begin{align*}
%\frac{\epsilon D'_i}{2n}\times\dist_{G, w'_i}(u, v) & \geq \frac{\epsilon D'_i}{2n}\times \left(\frac{2n}{\epsilon D'_i}  \dist_{G, w}(u, v)\right)\\
%&\geq \dist_{G, w}(u, v)\,.
%\end{align*}
%%
%This proves Eq.\eqref{eq:apsp approx main one} and completes the proof of Lemma~\ref{lem:approx apsp guarantee}.
%\end{proof}
%
% ---------------------------------------------------------------

Now we prove Proposition~\ref{prop:approx apsp guarantee}.

{\renewcommand{\thetheorem}{\ref{prop:approx apsp guarantee}}
\begin{proposition}[Restated]
For any nodes $u$ and $v$, if we let $\tilde d_{G, w}(u, v)$ = $\min_i  \frac{\epsilon D'_{i}}{2n}\times \dist^{(1+2/\epsilon)n}_{G, w'_i}(u, v)$, then $\dist_{G, w}(u, v)\leq \tilde d_{G,w}(u, v)\leq (1+\epsilon)\dist_{G, w}(u, v)$.
\end{proposition}
\addtocounter{theorem}{-1}
}
\begin{proof} Note that
$$\tilde d_{G, w}(u, v)= \min_i \frac{\epsilon D'_{i}}{2n}\times\dist^{(1+2/\epsilon)n}_{G, w'_i}(u, v)= \min_i \frac{\epsilon D'_{i}}{2n}\times\dist_{G, w'_i}(u, v)$$
where the second equality is due to Eq.\eqref{eq:apsp approx main two}. Then, Eq.\eqref{eq:apsp approx main one} and \eqref{eq:apsp approx main three} imply that $\tilde \dist_{G, w}(u, v)\geq \dist_{G, w}(u, v)$ and $\tilde \dist_{G, w}(u, v)\leq (1+\epsilon)\dist_{G, w}(u, v)$, respectively.
\end{proof}


==> arXiv/clique.tex <==
\section{Algorithms on Fully-Connected Networks}\label{sec:clique}





\subsection{$\tilde O(\sqrt{n})$-time Exact Algorithm for \sssp}\label{sec:sssp clique}



In this section, we present an algorithm that solves \sssp exactly in $\tilde O(\sqrt{n})$ time on fully-connected networks. The algorithm has two simple phases, as shown in \Cref{algo:clique SSSP}. In the first phase, it reduces the shortest-path diameter using the techniques developed in \Cref{sec:spd reduction}. In particular, every node $u$ broadcasts $k=\sqrt{n}$ edges of smallest weight. Then, every node uses the information it receives to compute a $k$-shortcut graph $(G, w')$, which can be done due to \Cref{thm:shortcuts from smallest edges}. By \Cref{thm:spd reduction}, we have 
$$\spdiam(G, w')<4\sqrt{n}~~~\mbox{and}~~~\forall u, v:~\dist_{G, w}(u, v)=\dist_{G, w'}(u, v).$$ 



\begin{algorithm}
\caption{$\tilde O(\sqrt{n})$-time Exact Algorithm for \sssp}\label{algo:clique SSSP}
{\bf Input:} A fully connected network $(G, w)$ and source node $s$. Weight $w(uv)$ of each edge $uv$ is known to $u$ and $v$. 

{\bf Output:} Every node $u$ knows $d(s, u)$ which is the equal to $\dist_{G, w}(s, u)$. 

\medskip{\bf Phase 1:} Shortest path diameter reduction. This phase gives a new weight $w'$ such that $\spdiam(G, w')<4\sqrt{n}$. The weight $w'(uv)$ of an edge $uv$ is known to its end-nodes $u$ and $v$.

\medskip\begin{algorithmic}[1]
\State Let $k=\sqrt{n}$. 
\State Each node $u$ sends $k$ edges of smallest weight, i.e. edges in $E^k(u)$ as in \Cref{def:E^k(u) set of k smallest weight }, to all other nodes. 
\State Every node $v$ uses $\bigcup_{v\in V(G)} E^k(v)$ construct  $(G^k, w)$ and compute $k$-shortcut edges, i.e. compute  $S^k_{G, w}(u)$ and $\{\dist_{G, w}(u, v)\}_{v\in S^k_{G, w}(u)}$. {\footnotesize\em // This step can be done internally (without communication) due to \Cref{thm:shortcuts from smallest edges}}. 
\State Augment $(G, w)$ with $k$-shortcut edges: for any edge $uv$, let $w'(uv)=\dist_{G, w}(u, v)$ if $u\in S^k_{G, w}(v)$ or $v\in S^k_{G, w}(u)$; otherwise, $w'(uv)=w(uv)$. {\footnotesize\em // This step can be done internally since both $u$ and $v$ know all information needed, i.e. $S^k_{G, w}(u)$,  $S^k_{G, w}(v)$,  $\{\dist_{G, w}(u, v)\}_{v\in S^k_{G, w}(u)}$, and $\{\dist_{G, w}(u, v)\}_{u\in S^k_{G, w}(v)}$.}
\algstore{cliqueSSSP}
\end{algorithmic}

\medskip{\bf Phrase 2:} Simulate Bellman-Ford algorithm on $(G, w')$. This phase makes every node $u$ knows  $d(s, u)$ where we claim that $d(s, u)=\dist_{G, w}(s, u)$. 
\medskip\begin{algorithmic}[1]
\algrestore{cliqueSSSP}
\State Let $d(s, s)=0$ and $d(s, u)=\infty$ for every node $u$.
\For{$i=1\ldots 4\sqrt{n}$}
\State Every node $u$ sends $d(s, u)$ to all other nodes. 
\State Every node $v$ updates $d(s, v)$ to $\min_{u} (d(s, u)+w'(uv))$. 
\EndFor
\end{algorithmic}
\end{algorithm}

In the second phase, the algorithm simulates Bellman-Ford's algorithm on $(G, w')$. In particular, every node iteratively uses the distance from $s$ to other nodes to update its distance; i.e., every node $v$ sets $d(s, v)$ to $\min_{u} (d(s, u)+w'(uv))$. It can be easily shown that by repeating this process for $\spdiam(G, w')$ iteration,  $d(s, u)=\dist_{G, w'}(s, u)$ for every node $u$. We provide the sketch of this claim for completeness, as follows.\danupon{To do: Use $d(u)$ instead of $d(s, u)$.}
%
\begin{claim}[Correctness of Phase 2 of \Cref{algo:clique SSSP}]\label{thm:BellmanFord}
Phase~2 of \Cref{algo:clique SSSP} returns a function $d$ such that, for every node $u$, $d(s, u)=\dist_{G, w'}(s, u)$. 
\end{claim}
\begin{proof}
We will show by induction that after the $i^{th}$ iteration, the value of $d(s, u)$ will be at most the value of the $i$-hop distance between $s$ and $u$, i.e. $d(s, u)\leq \dist_{G, w'}^i(s, u)$ (recall that $\dist_{G, w'}^i(s, u)$ is defined in \Cref{def:bounded hop sssp}). This trivially holds before we start the first iteration since $\dist_{G, w'}^0(s, s)=0$ and $\dist_{G, w'}^0(s, u)=\infty$. Assume for an induction that it holds for some $i\geq 0$. For any node $u$, let $P$ be a shortest $(i+1)$-hop $s$-$u$ path, and $v$ be the node preceding $u$ in such path. By the induction hypothesis, after the $i^{th}$ iteration, $d(s, v)\leq \dist^i_{G, w'}(s, v)$. So, after the $(i+1)^{th}$ iteration, $d(s, u)\leq d(s, v)+w'(vu)\leq \dist_{G, w'}(s, u)$. The claim thus holds for the $(i+1)^{th}$ iteration.

Let $h=\spdiam(G, w')$. Since $\dist^h_{G, w'}(s, u)=\dist_{G, w'}(s, u)$ for every node $u$, we have that $d(s, u)\leq \dist_{G, w'}(s, u)$ after $h$ iterations. Since it is clear that $d(s, u)\geq \dist_{G, w'}$, \Cref{thm:BellmanFord} follows.
\end{proof}
%
%Since $\dist_{G, w'}(s, u)=\dist_{G, w}(s, u)$ for every node $u$, we have that every node can use $d(s, u)$ as an answer to the \sssp problem. 


%
% ------------------------------------
% This is the version where we use Dijkstra's algorithm
% ------------------------------------
%
%\begin{algorithm}
%\caption{$\tilde O(\sqrt{n})$-time Exact Algorithm for \sssp}\label{algo:clique APSP}
%{\bf Input:} A fully connected network $(G, w)$. Weight $w(uv)$ of each edge $uv$ is known to $u$ and $v$. 
%
%{\bf Output:} Every node $u$ knows the value of $\dist_{G, w}(u, v)$ for every node $v$. 
%
%\medskip\begin{algorithmic}[1]
%\State Each node $u$ sets $x_0=u$ and $S_u=\{u\}$. Let $d(uu)=0$ and $d(uv)=w(uv)$ for every node $v$. 
%
%\For{$i=0 \ldots \sqrt{n}-1$} 
%
%\State Each node $u$ sends message $(x_i, d(ux_i))$ to every node $v$ through edge $uv$.
%
%\State Node $v\notin S_u$ updates $d(uv)$ to $d(uv)=\min(d(uv), d(ux_i)+w(x_iv))$, and sends the new value of $d(uv)$ to $u$. 
%
%\State Node $u$ sets $x_{i+1}$ to be the node $v\notin S_u$ with smallest $d(uv)$, i.e. $x_{i+1}=\arg\min_{v\notin S_u} d(uv)$. It adds $x_{i+1}$ to $S_u$. 
%
%\EndFor
%
%\State Every node $u$ sends all $v\in S_u$ and $d(uv)$ to all nodes in the network. Thus, every node knows $S_u$ and $d(uv)$ for all $v\in S_u$. 
%
%\State Let $(G, w')$ be the $\sqrt{n}$-shortcut graph as defined in \Cref{def:shortcut graph}. That is, we define $w'(uv)$, for any edge $uv\in E(G)$ as 
%\[w'(uv)=
%\begin{cases}
%d(uv) & \mbox{if $v\in S_u$, and}\\
%w(uv) & \mbox{otherwise}
%\end{cases}
%\]
%%
%%let $w'$ be the weight assignment defined as follows. For any nodes $u$ and $v$, if $v\in S_u$ then $w'(uv)=d(uv)$; otherwise, $w'(uv)=w(uv)$. 
%%
%{\footnotesize \em// Note that, by \Cref{thm:shortcuts}, $\spdiam(G, w')<4\sqrt{n}$.}
%\end{algorithmic}
%\end{algorithm}
%

%----------------------------------------------------------------------------------
% Below is the first version of the algorithm where we use Dijkstra's algorithm. 
%----------------------------------------------------------------------------------
%
%In this section, we present an algorithm that solves \sssp exactly in $\tilde O(\sqrt{n})$ time on fully-connected networks. In the first step of our algorithm, every node $u$ finds $\sqrt{n}$ nodes nearest to it. This as be done by simulating the Dijkstra's algorithm as follows. Initially, we let $S_u=\{u\}$ and we set the {\em candidate distance} of nodes $v\neq u$ to $w(uv)$. In each round, every node sends its candidate distance to $u$. Then $u$ picks a node not in $S_u$ that has the smallest candidate distance, say $v$. Node $u$ adds $v$ to $S_u$ and announces the ID and distance of $v$ to all other nodes. Every node then updates its candidate distance using the distance of $v$ (as in Dijkstra's algorithm). Observe that after $\sqrt{n}$ steps, $S_u$ will contain $\sqrt{n}$ nodes nearest to $u$. Observe further that this simulation of Disjkstra's algorithm only need a communication between $u$ and other nodes; in other words, only edges between $u$ and other nodes are used for communication. Thus, we can run this algorithm from all nodes in parallel, and every node $u$ will know the distance to $\sqrt{n}$ nearest nodes in $\tilde O(\sqrt{n})$ time. 
%
%
%In the second step, we use the distances from $u$ to $\sqrt{n}$ nearest nodes as shortcuts to reduce the shortest-path diameter as in \Cref{thm:spd reduction}. In particular, for any $v\in S_u$, we modify the weight of edge $uv$ to $\dist_{G, w}(u, v)$ whose value is known from the simulation of Dijkstra's algorithm. We let $w'$ be the new weight assignment. By \Cref{thm:spd reduction}, we have that $\spdiam(G, w')\leq \sqrt{n}$. 
%%
%Now that the shortest-path diameter is reduced to $\sqrt{n}$, we can solve \sssp simply by running the distributed version of Bellman-Ford's algorithm. This algorithm takes $\tilde O(\spdiam(G, w'))$ time, giving a total running time of $\tilde O(\sqrt{n})$. 

\subsection{$\tilde O(\sqrt{n})$-time $(2+o(1))$-Approximation Algorithm for \apsp}\label{sec:apsp clique}

We now present a $(2+o(1))$-approximation algorithm for \apsp, which also has $\tilde O(\sqrt{n})$ time. Our algorithm is outlined in \Cref{algo:clique APSP}. In the first phase of this algorithm is almost the same as the first phase of \Cref{algo:clique SSSP} presented in the previous section: by having every node $u$ sending out $E^{\sqrt{n}}(u)$ to all other nodes, we get a network $(G, w')$ such that 
$$\spdiam(G, w')<4\sqrt{n}~~~\mbox{and}~~~\forall u, v:~\dist_{G, w}(u, v)=\dist_{G, w'}(u, v).$$ 
%
%
%
The only difference is that, in addition to performing Phase~1 of \Cref{algo:clique SSSP} to get the properties above, we also make sure that 
\begin{align}
w'(uv)\leq \min_{z\in S^k(u)}\dist_{G, w}(u, z)+w(zv)\,.\label{eq:cliqueAPSP one}
\end{align}
%
This is done by having every node $u$ broadcasts $S^k(u)$ and $\{\dist_{G, w}(u, z)\}_{z\in S^k_{G, w}(u)}$ (which are also computed in Phase~1 of \Cref{algo:clique SSSP}) to all other nodes, where $k=\sqrt{n}$. Then every node $v$ can internally update $w'(uv)$, for every node $u$, to $w'(uv)= \min\{w'(uv), \min_{z\in S^k(u)}\dist_{G, w}(u, z)+w(zv)\}$. 
%
Phase~1 takes $\tilde O(\sqrt{n})$ time since performing Phase~1 of \Cref{algo:clique SSSP} takes $\tilde O(\sqrt{n})$ time and broadcasting $S^k(u)$ and $\{\dist_{G, w}(u, z)\}_{z\in S^k_{G, w}(u)}$, which are sets of size  $\tilde O(\sqrt{n})$, also takes  $\tilde O(\sqrt{n})$ time.



\begin{algorithm}
\caption{$\tilde O(\sqrt{n})$-time $(2+o(1))$-Approximation Algorithm for \apsp}\label{algo:clique APSP}
{\bf Input:} A fully connected network $(G, w)$. Weight $w(uv)$ of each edge $uv$ is known to $u$ and $v$. 

{\bf Output:} Every node $u$ knows $(2+o(1))$-approximate value of $\dist_{G, w}(u, v)$ for every node $v$. 


%\medskip{\bf Phase 1:} For $k=\sqrt{n}$, compute $S^k(u)$ and $\{\dist_{G, w}(u, z)\}_{z\in S^k_{G, w}(u)}$ and reduce the shortest-path diameter to $O(\sqrt{n})$. At the end of this phase, every node $v$ knows $S^k(u)$ and $\{\dist_{G, w}(u, z)\}_{z\in S^k_{G, w}(u)}$ for all $u$, and we get a network $(G, w')$ such that $\spdiam(G, w')<4\sqrt{n}$. 
%
%%Shortest path diameter reduction (see Phase~1 of \Cref{algo:clique SSSP} for details). This phase gives a new weight $w'$ such that $\spdiam(G, w')<4\sqrt{n}$. The weight $w'(uv)$ of an edge $uv$ is known to its end-nodes $u$ and $v$.
%\medskip\begin{algorithmic}[1]
%\State Let $k=\sqrt{n}$. 
%\State Each node $u$ sends $k$ edges of smallest weight, i.e. edges in $E^k(u)$ as in \Cref{def:E^k(u) set of k smallest weight }, to all other nodes. 
%\State Every node $v$ uses $\bigcup_{v\in V(G)} E^k(v)$ construct  $(G^k, w)$ and compute $k$-shortcut edges, i.e. compute  $S^k_{G, w}(u)$ and $\{\dist_{G, w}(u, v)\}_{v\in S^k_{G, w}(u)}$. {\footnotesize\em // This step can be done internally (without communication) due to \Cref{thm:shortcuts from smallest edges}}. 
%\State Augment $(G, w)$ with $k$-shortcut edges: for any edge $uv$, let $w'(uv)=\dist_{G, w}(u, v)$ if $u\in S^k_{G, w}(v)$ or $v\in S^k_{G, w}(u)$; otherwise, $w'(uv)=w(uv)$. {\footnotesize\em // This step can be done internally since both $u$ and $v$ know all information needed, i.e. $S^k_{G, w}(u)$,  $S^k_{G, w}(v)$,  $\{\dist_{G, w}(u, v)\}_{v\in S^k_{G, w}(u)}$, and $\{\dist_{G, w}(u, v)\}_{u\in S^k_{G, w}(v)}$.}
%\algstore{cliqueAPSP}
%\end{algorithmic}

\medskip{\bf Phase 1:} Let $k=\sqrt{n}$. Compute $S^{k}(u)$, for every node $u$, and weight assignment $w'$ such that  $\spdiam(G, w')<4\sqrt{n}$ and $w'(uv)\leq \min_{z\in S^k(u)}\dist_{G, w}(u, z)+w(zv)$. 


\medskip\begin{algorithmic}[1]
\State Perform Phase~1 of \Cref{algo:clique SSSP}. This step makes every node $u$ knows $S^k(u)$ and $\{\dist_{G, w}(u, z)\}_{z\in S^k_{G, w}(u)}$. 

\State Every node $u$ sends $S^k(u)$ and $\{\dist_{G, w}(u, z)\}_{z\in S^k_{G, w}(u)}$ to all other nodes. 

\State Every node $v$ updates $w'(uv)$, for every node $u$, to $w'(uv)= \min\{w'(uv), \min_{z\in S^k(u)}\dist_{G, w}(u, z)+w(zv)\}$. 
%
{\footnotesize\em // This step can be done without communication since every node $v$ knows  $S^k(u)$ and $\{\dist_{G, w}(u, z)\}_{z\in S^k_{G, w}(u)}$  for all nodes $u$}
\algstore{cliqueAPSP}
\end{algorithmic}

\medskip{\bf Phase 2:} Compute $(4\sqrt{n})$-hop $(\sqrt{n}\log n)$-source shortest paths for $\sqrt{n}\log n$ random sources.

\medskip\begin{algorithmic}[1]
\algrestore{cliqueAPSP}

\State Let $R$ be a set of randomly selected $\sqrt{n}\log n$ nodes. 

\State Run the multi-souce bounded-hop shortest paths algorithm from \Cref{thm:k-source h-hop sp} (\Cref{algo:bounded-hop multi-source}) on $(G, w')$ for $h=4\sqrt{n}$ hops using nodes in $R$ as sources. 
%
{\footnotesize // \em At the end of this process, every node $v$ knows a $(1+o(1))$-approximate value of $\dist^h_{G, w'}(r, v)$, which equals to $\dist_{G, w'}(r, v)$ since  $\spdiam(G, w')<4\sqrt{n}$, for all $r\in R$. We denote this approximate value by $d'(u, v)$; thus, $\dist_{G, w'}(r, v)\leq d'(u, v)\leq (1+o(1))\dist_{G, w'}(r, v)$.}

\State Every node $v$ sends $d'(r, v)$, for all $r\in R$, to all nodes. 
\end{algorithmic}

\medskip{\bf Final Phase:} Every node $v$ uses the information it knows so far (see \Cref{def:G_u}) to compute $d''(u, v)$ for all nodes $u$, which is claimed to be a $(2+o(1))$ approximation of $\dist_{G, w}(u, v)$ (see \Cref{thm:cliqueAPSP}). 

\end{algorithm}

In the second phase, we pick $\Theta(\sqrt{n}\log n)$ nodes uniformly at random. Let $R$ be the set of these random nodes. We run the light-weight $h$-hop $t$-source \sssp algorithm (\Cref{algo:bounded-hop multi-source}) from these random nodes using $h=\sqrt{n}$ and $t=|R|$. By \Cref{thm:k-source h-hop sp}, we will finish in $\tilde O(|R|+h) = \tilde O(\sqrt{n})$ rounds with high probability. Moreover, since the shortest-path distance is reduced to $\sqrt{n}$, every node will know an $(1+o(1))$-approximate distance to {\em all} random nodes in $R$. Every node broadcasts these distances to nodes in $R$ to all other nodes. This takes $O(|R|)$ time since the network is fully connected.
%
In the final phase, every node $u$ uses these broadcasted distances and the distances it computes in the previous step (by simulating Dijkstra's algorithm) to compute the approximate distance between itself and other nodes. 
%
In particular, for any node $u$, consider the following graph $(G_u, w_u)$.  

\begin{definition}[Graph $(G_u, w_u)$]\label{def:G_u} Graph $(G_u, w_u)$ consists of the following edges. 
\begin{enumerate}
\item edges from $u$ to all other nodes $v$ of weight $w'(u, v)$, 
\item edges from $x\neq u$ to nodes $y\in S^k(x)$ of weight $w'(x, y)=\dist_{G, w}(x, y)$, and 
\item edges from every random node $r\in R$ to all other nodes $v$ of weight $d''(r, v)$. (Recall that $\dist_{G, w}(r, v)\leq d''(r, v)\leq (1+o(1))\dist_{G, w}(r, v)$.) 
\end{enumerate}
\end{definition}
%
Node $u$ will use $\dist_{G_u, w_u}(u, v)$ as an approximate distance of $\dist_{G_u, w}(u, v)$. We now show that this gives a $(2+o(1))$-approximate distance. 

\begin{lemma}[Approximation guarantee of \Cref{algo:clique APSP}]\label{thm:cliqueAPSP}
For every pair of nodes $u$ and $v$, $\dist_{G, w}(u, v)\leq \dist_{G_u, w_u}(u, v)\leq (2+o(1))\dist_{G, w}(u, v).$
\end{lemma}
\begin{proof}
It is clear that $\dist_{G, w}(u, v)\leq \dist_{G_u, w_u}(u, v)$ since $w_u(xy)\geq \dist_{G, w}(x, y)$ for every pair of nodes $x$ and $y$. It is left to prove that $\dist_{G_u, w_u}(u, v)\leq (2+o(1))\dist_{G, w}(u, v).$
%
Let 
$$P=\langle u=x_1, x_2, \ldots, x_k=v\rangle$$  
be a shortest $u$-$v$ path. Note that we can assume that $k\leq \sqrt{n}$ since the shortest-path diameter is $\sqrt{n}$. 
%
Let $x_i$ be the furthest node from $u$ that is in $S^k(u)\cap P$ and, similarly,  let $x_j$ be the furthest node from $v$ that is in $S^k(v)\cap P$; i.e. 
$$i=\arg\max_{i'} (x_{i'}\in S^k(u)\cap P) ~~~\mbox{and}~~~ j=\arg\min_{j'} (x_{j'}\in S^k(v)\cap P) \,.$$
%
%
Note that $x_1, \ldots, x_i$ are all in $S^k(u)$ since all nodes $x_1, \ldots, x_{i-1}$ are nearer to $u$ than $x_i$. Similarly, $x_j, \ldots, x_k$ are all in $S^k(v)$. Note further that $w'(u, x_{i+1})=\dist_{G, w}(u, x_{i+1})$ since Phase~1 guarantees \Cref{eq:cliqueAPSP one} which implies that
%
\begin{align*}
w'(u, x_{i+1}) &\leq \min_{z\in S^k(u)} \dist_{G, w}(u,z)+w(zx_{i+1})\\
&\leq \dist_{G, w}(u, x_i)+w(x_ix_{i+1})  &\mbox{(since $x_i\in S^k(u)$)}\\
&= \dist_{G, w}(u, x_{i+1})\,.
\end{align*}
%
\begin{figure}
\centering
\begin{subfigure}[b]{0.45\textwidth}
\centering
\includegraphics[page=1, clip=true, trim=0.95cm 10.5cm 12.3cm 2.2cm, width=\textwidth]{pictures.pdf}
\caption{Case 1: $j\leq i+1$}
\label{fig:case1}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
\centering
\includegraphics[page=1, clip=true, trim=0.95cm 4cm 12.25cm 8cm, width=\textwidth]{pictures.pdf}
\caption{Case 2: $j> i+1$.}
\label{fig:case2}
\end{subfigure}
\caption{Outline of the proof of \Cref{thm:cliqueAPSP}}\label{fig:cliqueAPSP}
\end{figure}
%
We now consider two cases (see \Cref{fig:cliqueAPSP} for an outline). First, if $j\leq i+1$, then we have $x_{i+1}\in S^k(u)\cap S^k(v)$. This means that $w_u(x_{i+1}, v)=w'(x_{i+1}, v)=\dist_{G, w}(x_{i+1}, v)$. 
\begin{align*}
\dist_{G_u, w_u}(u, v) & \leq w_u(u, x_{i+1})+w_u(x_{i+1}, v)\\ 
& = w'(u, x_{i+1}) + w'(x_{i+1}, v)\\
& = \dist_{G, w}(u, x_{i+1}) + \dist_{G, w}(x_{i+1}, v)\\
& = \dist_{G, w}(u, v).
\end{align*}
%where the third inequality is because $x_i\in S^k(u)$ (which makes $w'(u, x_{i+1})= \dist_{G, w}(u, x_{i+1})$ as noted earlier ) and $x_{i+1}\in S^k(v)$. 
%
Now we consider the second case where $j>i+1$. %We will consider two subcases: when  $\dist_{G, w}(u, x_{i+1})\leq \dist_{G, w}(x_{i+1}, v)$ and  $\dist_{G, w}(u, x_{i+1})< \dist_{G, w}(x_{i+1}, v)$. The analyses of both cases are essentially the same, so we will only show the analysis for the first subcase. In this case, we have
%
%We will assume without loss of generality that $\dist_{G, w}(u, x_{i+1})\leq \dist_{G, w}(x_{i+1}, v)$; thus, 
%
In this case, we have that either
$$\dist_{G, w}(u, x_{i+1})\leq \dist_{G, w}(u, v)/2 ~~~\mbox{or}~~~ \dist_{G, w}(v, x_{j-1})\leq \dist_{G, w}(u, v)/2\,.$$  
%
Since the analyses for both cases are essentially the same, we will only show the analysis when $\dist_{G, w}(u, x_{i+1})\leq \dist_{G, w}(u, v)/2$.
%
Observe that, with high probability, there is a random node $r\in R$ that is in $S^k(u)$ since $|S^k(u)|\geq \sqrt{n}$ and $R$ consists of $\tilde \Theta(\sqrt{n})$ random nodes (see \Cref{thm:UllmanY}). Recall that, for every node $z$, 
$$w_u(r, z)\leq d''(r, z) \leq (1+o(1))\dist_{G, w}(r, z).$$ 
It follows that
\begin{align}
\dist_{G_u, w_u}(u, v) & \leq w_u(u, r)+w_u(r, v)\label{eq:cliqueAPSP1}\\ 
& \leq (1+o(1))(\dist_{G, w}(u, r) + \dist_{G, w}(r, v))\label{eq:cliqueAPSP2}\\
& \leq (1+o(1))(\dist_{G, w}(u, r) + (\dist_{G, w}(u, r)+\dist_{G, w}(u, v)))\label{eq:cliqueAPSP3}\\
& \leq (1+o(1))(2\dist_{G, w}(u, x_{i+1}) + \dist_{G, w}(u, v))\label{eq:cliqueAPSP4}\\
& \leq (2+o(1)) \dist_{G, w}(u, v).\label{eq:cliqueAPSP5}
\end{align}
\Cref{eq:cliqueAPSP3} is by triangle inequality. \Cref{eq:cliqueAPSP4} is because $r\in S_u$ and $x_{i+1}\notin S_u$. \Cref{eq:cliqueAPSP5} is because of the assumption that $\dist_{G, w}(u, x_{i+1})\leq \dist_{G, w}(u, v)/2$. 
\end{proof}

%Since $\dist_{G, w'}(u, v)$ is an $o(1)$-approximate value of $\dist_{G, w}(u, v)$, we have that $\dist_{G_u, w'_u}(u, v)$ $(2+o(1))$-approximates $\dist_{G, w}(u, v)$ as desired. 

%In this case, we know that $\dist_{G, w}(u, v)\geq \dist_{G, w}(u, x_i)+\dist_{G, w}(x_j, v)$. 
%
%We will assume without loss of generality that $\dist_{G, w}(u, x_i)\leq \dist_{G, w}(x_j, v)$. Observe that, with high probability, there is a random node $r\in R$ that is in $S_u$ since $|S_u|\geq \sqrt{n}$ and $R$ consists of $\tilde \Theta(\sqrt{n})$ random nodes (see \Cref{thm:UllmanY}). Recall that $w''(r, v)$ is a  $(1+o(1))$ approximation of $\dist_{G, w}(r, v)$. Moreover, $w''(u, r)=\dist_{G, w}(u, r)$. Note that $\dist_{G, w}(r, v)\leq 2\dist_{G, w}(u, x_i)+\dist_{G, w}(x_j, v)$ and $\dist_{G, w}(u, r)\leq \dist_{G, w}(u, x_i)$. 

==> arXiv/clustering.tex <==
\section{Node Clustering (Proposition~\ref{prop:clustering})}\label{sec:clustering}

In this Section, we prove Proposition~\ref{prop:clustering}: Nodes in $G$ can be partitioned into {\em clusters} $C_1, C_2, \ldots, C_k$, for some $k$, such that for any $\vec w\in \cW_i\cup \{w_i\}$, $\dist_{G, \vec w}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster. Moreover, such partition can be found in $O(n)$ time. 

%Nodes in $G$ can be partitioned into {\em clusters} $C_1, C_2, \ldots, C_k$, for some $k$, such that,for any $\vec w\in \cW_i\cup \{w_i\}$, $\dist_{G, \vec w}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster. Moreover, such partition and their sizes can be found in $O(n)$ time. In the end, every node $u$ knows which cluster every node $v$ is in; i.e., it knows the set $\{(v, \rep(C_j) \mid v\in C_j\}$ where we define $\rep(C_j)$ to be $\rep(C_j)=\min_{v\in C_j} v$.

%In this section, we prove Lemma~\ref{lem:clustering}.
%
To prove this, consider the node partition $\cC=\{C_1, \ldots, C_{k}\}$ where, for any node $u$ and $v$, $u$ and $v$ are in the same partition if and only if $\dist_{G, w_i}(u,v)=0$.
%
Note the following important property of $(G, \cW_i)$.
%
\begin{claim}\label{claim:scaling preserves zero}
For any node $s$, $u$ and $v$, $\vec w_i^s(uv)\geq 0$. Moreover, $\vec w_i^s(uv)=0$ if and only if $w_i(uv)=0$.
\end{claim}
%
\begin{proof}
Recall that $b_i(uv)$ is the $i^{th}$ bit of $w(uv)$ (cf. Definition~\ref{def:w_i}), and note that $w_{i}(uv)=2w_{i+1}(uv)+b_i(uv).$ It follows from the definition of $\vec w_i^s$ (Line~\ref{line:w_i} of Algorithm~\ref{algo:apsp}) that
\begin{align*}
\vec w_i^s(uv) &= 2\dist_{G, w_{i+1}}(s, u)-2\dist_{G,w_{i+1}}(s, v)+w_i(uv)\\
&=2\dist_{G,w_{i+1}}(s, u)-2\dist_{G,w_{i+1}}(s, v)+2w_{i+1}(uv)+b_i(uv)\\
&\geq b_i(uv)\,.
\end{align*}
Note that last inequality follows from the triangle inequality property of the distance function; i.e. for any $w'$, $\dist_{G,w'}(s, u)+w'(uv)\geq \dist_{G,w'}(s, v)$. It follows immediately that $\vec w_i^s(uv)\geq 0$.

Moreover, if $w_i(uv)>0$, then  $b_i(uv)>0$ (since $b_i(uv)$ is a bit in the {\em positive} binary representation of $w_i(uv)$); thus, $w_i(uv)>0$ implies that $\vec w_i^s(uv)>0$. 

Finally, if $w_i(uv)=0$, then clearly $w_{i+1}(uv)=0$, and thus $\dist_{G,w_{i+1}}(s, u)=\dist_{G,w_{i+1}}(s, v)$. It follows that, $\vec w_i^s(uv)= 2\dist_{G, w_{i+1}}(s, u)-2\dist_{G,w_{i+1}}(s, v)+w_i(uv)=w_i(uv)=0$.
\end{proof}
%
The above claim implies that, for any nodes $s$, $u$ and $v$, $\dist_{G, \vec w_i^s}(u, v)=0$ if and only if $\dist_{G, w_i}(u, v)=0$. It follows from the definition of $\cC$ that $\dist_{G, \vec w_i^s}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster. This shows that $\cC$ satisfies the property claimed in Proposition~\ref{prop:clustering}.

Computing $\cC$ in $O(n)$ time is very easy. First, every node broadcasts the minimum ID it has seen so far {\em through edges of weight zero only}. After repeating this for $n-1$ rounds, it is easy to see that the minimum ID that node $u$ has seen so far is exactly $\rep(C_j)$, where $j$ is such that $u\in C_j$.
%
Next, every node $u$ broadcasts to all other nodes a message $(u, \rep(C_j))$ where $C_j$ is the cluster that contains $u$. Since there are exactly $n$ messages broadcasted, we only need $O(n+D(G))=O(n)$ time for broadcasting them.
%
%(In fact, repeating this for $\max_j |C_j|$
%
%Every node $u$ then broadcasts the pair $(u, \rep(S_{w_i}(u)))$ so that other nodes knows $\rep(S_{w_i}(u))$ (this can be done by, e.g., aggregating and broadcasting on a BFS tree).
%
%Secondly, for each cluster $C_j$, $\rep(C_j)$ computes a BFS tree rooted at $u$ using only edges of weight zero. It can then use this BFS tree to compute $|C_j|$ and broadcast this value to all nodes in $S_{w_i}(u)$. The BFS trees from these nodes can be computed in parallel, taking $\max_j |C_j|=O(n)$ rounds in total.


==> arXiv/conclusion.tex <==
\danupon{To do: Mention that proving lower bound on clique is quite impossible (by Oshman's talk)}

\section{Open Problems}

%\subsection{Single-Source Shortest Paths}

The main question left by our \sssp algorithm is the following. 
%
\begin{problem}
Close the gap between the upper bound of $\tilde O(n^{1/2}\diam^{1/4})$ presented in this paper and the lower bound of $\tilde \Omega(n^{1/2})$ presented in \cite{DasSarmaHKKNPPW11} for $(1+\epsilon)$-approximating the single-source shortest paths problem on general networks. 
\end{problem}

Improving the current upper bound is important since there are many problems that can be potentially solved by using the same technique. Moreover, giving a lower bound in the form  $\tilde \Omega(n^{1/2}\diam^{\delta})$ for some $\delta>0$ will be quite surprising since such lower bound has not been observed before. 
%
%We believe that answering to the following questions will help improve our understanding on \sssp: (1) 
%
It should also be fairly interesting to refine our upper bound to achieve a $\tilde O(n^{1/2}\diam^{\epsilon})$-time $O(1/\epsilon)$-approximation algorithm for any $\delta>0$. 
%
Another question that should be very interesting is understanding the exact case: 
%
\begin{problem}
Can we solve \sssp {\em exactly} in sublinear-time? 
\end{problem}
%
It is also interesting to solve \apsp {\em exactly} in linear-time (recall that sublinear-time is not possible). In some settings, an exact algorithm for computing shortest paths is crucial; e.g. some Internet protocols such as OSPF and IS-IS use edge weights to control the traffic and using an approximate shortest paths with this protocol is unacceptable\footnote{We thank Mikkel Thorup for pointing out this fact}. 
%
%are widely used Internet protocols where the traffic follows shortest pahts, typically with even splitting in connection with ties. The weights are parameters controlled by the network operator. In connection with ties, it is not uncommon for the network operator to increase a weight by, say, 1, just to off-load a heavily used link. Approximate shortest paths would be totally unacceptable.
%
The next question is a generalization of our \sssp: 
%
\begin{problem}[Asymmetric \sssp]
How fast can we solve \sssp on networks whose edge weights could be {\em asymmetric}, i.e. if we think of each edge $uv$ as two directed edges $\overrightarrow{uv}$ and $\overrightarrow{vu}$, it is possible that $w(\overrightarrow{uv})\neq w(\overrightarrow{vu})$. 
\end{problem}
Note that we are particularly interested in the case where weights do not affect communication; in other words, if $u$ can send a message to $v$, then $v$ can also send a message to $u$. Also note that our light-weight \sssp algorithm can be used to solve this problem (but not the shortest-path diameter reduction technique). By adjusting parameters appropriately, we can $(1+\epsilon)$-approximate this problem in $\tilde O(\min(n^{2/3}, n^{1/2}D^{1/2}))$ time. 
%
In fact, improving this running time for the following very special case seems challenging already:
%\begin{quote}
\begin{problem}[$s$-$t$ Reachability Problem]
%Assuming that $w(\overrightarrow{uv})\in \{0, 1\}$ for every directed edge $w(\overrightarrow{uv})$, we want to know whether $\dist_G(s, t)$ is zero or not, for some nodes $s$ and $t$. Can we solve this faster than $\tilde O(\min(n^{2/3}, n^{1/2}D^{1/2}))$ time? 
Given a directed graph $G$ and two special nodes $s$ and $t$, we want to know whether there is a directed path from $s$ to $t$. The communication network is the underlying undirected graph; i.e. the communication can be done independent of edge directions and the diameter $\diam$ is defined to be the diameter of the underlying undirected graph. Can we answer this question in $\tilde O(\sqrt{n}+\diam)$ time?
\end{problem}
%\end{quote} 
%
This problem shows limitations of the techniques presented in this paper, and we believe that solving it will give a new insight into solving all above open problems. Our last set of questions: %is breaking the $\tilde O(n^{1/2})$-time 
%
\begin{problem}
Can we improve the $\tilde O(n^{1/2})$-time upper bound for \sssp on fully-connected networks while keeping the approximation ratio small (say, at most two)? Is it possible to prove a nontrivial $\omega(1)$ lower bound?
\end{problem}
Note that the last question was asked earlier by Elkin \cite{Elkin04}. 

%\subsection{Other Problems}



\section{Acknowledgement}
The sublinear-time \sssp algorithm was  inspired by the discussions with Jittat Fakcharoenphol and Jakarin Chawachat, who refused to co-author this paper. Several techniques borrowed from dynamic graph algorithms benefit from many intensive discussions with Sebastian Krinninger and Monika Henzinger.
%
I also would like to thank  Radhika Arava and Peter Robinson for explaining the algorithm of Baswana and Sen \cite{BaswanaS07}\danupon{Correct?} to him and Gopal Pandurangan, Chunming Li, Anisur Rahaman, David Peleg, Atish Das Sarma, Parinya Chalermsook, Bundit Laekhanukit, Boaz Patt-Shamir, Shay Kutten, Christoph Lenzen, Stephan Holzer, Mohsen Ghaffari, Nancy Lynch, and Mikkel Thorup, for discussions, comments, and pointers to related results. I also thank all reviewers of STOC 2014 for many thoughtful comments. 


\endinput

%******************************************************************************
%******************************************************************************
%******************************************************************************

\section{Conclusions and Open problems}

Conjecture: 2-approx Diameter on clique needs $\Omega(\sqrt{n})$ time. This conjecture will prove both our SSSP and APSP algorithms on clique tight. 

$\Omega(n)$ lower bound of {\em any} approximation algorithm for {\em unweighted} \apsp?

Weighted \apsp on complete graphs and low-diameter graphs.

TO DO: Change ``supernodes'' to clusters (or should I keep supernodes?). Define the SimBFS as finding distances in graphs $G_L$ obtained by deleted edges of weight zero in big clusters. Remove page number in final version.

Thanks Monika and Sebastian.

Discuss why we can't use deterministic scheduling. Basically this is because we are running BFS algorithms on many directed graphs.

Single source shortest path: Can solve in $O(\sqrt{n})$? Will imply the same running time with our algorithm.

Open: Dealing with asymmetric weights.

To get linear time, have to either avoid zero edges or deal with it quicker. In the second direction, we propose the problem on 0/1 graph as a milestone. % Maybe we can solve this problem using MST-style algorithm

Open: $k$-SP.

Algorithm on complete graph

Sub-linear time approximation algorithm

A clever way to shortcut the graph to reduce the shortest path diameter. Might be related: \url{http://www.cs.ucla.edu/~awm/papers/APPROX09-NoC.pdf} and \url{dspace.mit.edu/openaccess-disseminate/1721.1/62215}


\sssp on overlay network of $\sqrt{n}$ nodes with stretch and stress $\sqrt{n}$. 




==> arXiv/diameter_bound.tex <==
\section{Multi-Weight Diameter (Proposition~\ref{prop:multi-weight diameter})}\label{sec:multi weight diameter bound}
In this section, we prove Proposition~\ref{prop:multi-weight diameter}: $\ecc(G, \cW_i)\leq 2n.$ In particular, fix any nodes $s$ and $u$, we show that $\dist_{G, \vec w_i^s}(s, u)\leq 2n.$

To prove this, recall that $b_i(xy)$ is the $i^{th}$ bit of $w(xy)$ (cf. Definition~\ref{def:w_i}), and observe that
\begin{align}
w_{i}(xy)&=2w_{i+1}(xy)+b_i(xy). \label{eq:w_i equal w_i+1 plus b_i}
\end{align}
%Also recall from Line~\ref{line:w_i} of Algorithm~\ref{algo:apsp} that 
%$$\vec w_i^s(uv)=2\dist_{w_{i+1}}(s, u)-2\dist_{w_{i+1}}(s, v)+w_i({uv}).$$ 
%
Let $P=\langle s=x_0, x_1, \ldots, x_\ell=u\rangle$ be any shortest $s$-$u$ path in weighted network $(G, w_{i+1})$. The length of this path in $(G, \vec w_i^s)$ is

\noindent{\fontsize{8}{0}\selectfont
%\small
\noindent\hspace{-.05in}\parbox{1.06\linewidth}{
\begin{align}
\vec w_i^s(P)  &= \sum_{j=0}^{\ell-1} \vec w_i^s(x_jx_{j+1})\nonumber\\
&=\left(2\dist_{G, w_{i+1}}(s, x_0)-2\dist_{G, w_{i+1}}(s, x_{1})+w_i(x_0x_{1})\right)\nonumber\\
&\ +\left(2\dist_{G, w_{i+1}}(s, x_1)-2\dist_{G, w_{i+1}}(s, x_{2})+w_i(x_1x_{2})\right)\nonumber\\
&\ +\ldots \nonumber\\
&\ +\left(2\dist_{G, w_{i+1}}(s, x_{\ell-1})-2\dist_{G, w_{i+1}}(s, x_{\ell})+w_i(x_{\ell-1}x_{\ell})\right)\label{eq:multi diam one}\\
%&=\sum_{j=0}^{\ell-1}\left(2\dist_{G, w_{i+1}}(s, x_j)-2\dist_{G, w_{i+1}}(s, x_{j+1})+w_i(x_jx_{j+1})\right)\label{eq:multi diam one}\\
&= \sum_{j=0}^{\ell-1} w_i(x_jx_{j+1})-2\dist_{G,w_{i+1}}(s, x_k)+2\dist_{G,w_{i+1}}(s, x_0)\label{eq:multi diam two}\\
&= \sum_{j=0}^{\ell-1} w_i(x_jx_{j+1})-2\sum_{j=0}^{\ell-1} w_{i+1}(x_jx_{j+1})\label{eq:multi diam three}\\
&= \sum_{j=0}^{\ell-1} b_i(x_jx_{j+1}))\label{eq:multi diam four}
\end{align}
}
}
where Eq.\eqref{eq:multi diam one} is by the definition of $\vec w_i^s$ (cf. Line~\ref{line:w_i} of Algorithm~\ref{algo:apsp}), Eq.\eqref{eq:multi diam two} is by telescoping sum,  Eq.\eqref{eq:multi diam three} uses the fact that $s=x_0$ and $P$ is a shortest $s$-$u$ path in $(G, w_{i+1})$, and Eq.\eqref{eq:multi diam four} follows from Eq.\eqref{eq:w_i equal w_i+1 plus b_i}.

It follows that $\dist_{G, \vec w_i^s}(s, u)\leq \vec w_i^s(P)=\sum_{j=0}^{\ell-1} b_i(x_jx_{j+1})$ which is at most $2\ell$ since $b_i(xy)\leq 2$ for any edge $xy$. Thus,  $\dist_{G, \vec w_i^s}(s, u)\leq 2\ell\leq 2n$ as claimed. 


==> arXiv/dprime.tex <==
\section{Property of {\lowercase{\large$\mathbf{d'}$}} (Proposition~\ref{prop:d prime})}\label{sec:d prime}

In this section, we prove Proposition~\ref{prop:d prime}: for any $K\geq \ecc(G, \cW_i)$, we show that $d'(s, u)=2\dist_{G, w_{i+1}}(s, u)+\dist^{K}_{H, \vec w_i^s}(s, u)$ has the property that (1) $d'(u, v)\geq \dist_{G, w_i}(u, v)$, and (2) if $\dist_{H, w_i}(u, v)=\dist_{G, w_i}(u, v)$, then $d'(u, v)=\dist_{G, w_i}(u, v)$.

First, we note the following important claim.

%\begin{claim}\label{claim:dist w_i from dist w_i^u}
%For any nodes $s$ and $u$,
%$$\dist_{H, w_i}(s, u)=2\dist_{H, w_{i+1}}(s, u)+\dist_{H, \vec w_i^s}(s, u).$$
%\end{claim}
%\begin{proof}
%Let $P=\langle s=x_0, x_1, \ldots, x_\ell=u\rangle$ be any $s$-$u$ path in $G$. By definition, the length of this path in $(H, \vec w_i^s)$ is
%%
%{\small
%\begin{align*}
%\vec{w}_i^s(P)  &= \sum_{j=0}^{\ell-1}2\dist_{H, w_{i+1}}(s, x_j)-2\dist_{H, w_{i+1}}(s, x_{j+1})+w_i(x_jx_{j+1})\\
%&= 2\dist_{H, w_{i+1}}(s, x_0)-2\dist_{H, w_{i+1}}(s, x_k)+\sum_{j=0}^{k-1} w_i(x_jx_{j+1}).
%\end{align*}
%}
%%
%Using $\dist_{H, w_{i+1}}(s, x_0)=0$ (since $s=x_0$), $x_k=u$, and $\sum_{j=0}^{k-1} w_i(x_jx_{j+1})=w_i(P)$, we can rewrite this to $w_i(P)=2\dist_{H, w_{i+1}}(s, u)+\vec w_i^s(P).$ Thus,
%\begin{align*}
%\dist_{H, w_i}(s, u)&=\min_{\mbox{$P$: $s$-$u$ path}} w_i(P)\\
%&=2\dist_{H, w_{i+1}}(s, u) + \min_{\mbox{$P$: $s$-$u$ path}} w_i^s(P)\\
%&=2\dist_{H, w_{i+1}}(s, u)+\dist_{H, \vec w_i^s}(s, u)
%\end{align*}
%as claimed. \danupon{Define $w_i(P)$!!}
%\end{proof}
\begin{claim}\label{claim:dist w_i from dist w_i^u}
For any $K\geq \ecc(G, \cW_i)$ and nodes $s$ and $u$,
$$\dist_{G, w_i}(s, u)=2\dist_{G, w_{i+1}}(s, u)+\dist^{K}_{G, \vec w_i^s}(s, u).$$
\end{claim}
\begin{proof}
Note that, since $K\geq \ecc(G, \cW_i)$, $K\geq \dist_{G, \vec w_i^s}(s, u)$ for all nodes $s$ and $u$. Thus, by the definition of $\dist^K_{G, \vec w_i^s}$ (cf. Definition~\ref{def:bounded dist apsp}), $\dist^K_{G, \vec w_i^s}(s, u)=\dist_{G, \vec w_i^s}(s, u)$. So, we will drop the superscript and use $\dist_{G, \vec w_i^s}$ instead of $\dist^K_{G, \vec w_i^s}$.


Let $P=\langle s=x_0, x_1, \ldots, x_\ell=u\rangle$ be any $s$-$u$ path in $G$. By definition, the length of this path in $(G, \vec w_i^s)$ is
%
{\small
\begin{align*}
\vec{w}_i^s(P)  &= \sum_{j=0}^{\ell-1} \left(2\dist_{G, w_{i+1}}(s, x_j)-2\dist_{G, w_{i+1}}(s, x_{j+1})+w_i(x_jx_{j+1})\right)\\
&= 2\dist_{G, w_{i+1}}(s, x_0)-2\dist_{G, w_{i+1}}(s, x_k)+\sum_{j=0}^{k-1} w_i(x_jx_{j+1}).
\end{align*}
}
%
Using $\dist_{G, w_{i+1}}(s, x_0)=0$ (since $s=x_0$), $x_k=u$, and $\sum_{j=0}^{k-1} w_i(x_jx_{j+1})=w_i(P)$, we can rewrite this to 
$$w_i(P)=2\dist_{G, w_{i+1}}(s, u)+\vec w_i^s(P).$$ 
Thus (recall that $\cP_G(s, u)$ is the set of all simple paths from $s$ to $u$ in $G$),
\begin{align*}
\dist_{G, w_i}(s, u)&=\min_{P\in \cP_G(s, u)} w_i(P)\\
&=2\dist_{G, w_{i+1}}(s, u) + \min_{P\in \cP_G(s, u)} \vec w_i^s(P)\\
&=2\dist_{G, w_{i+1}}(s, u)+\dist_{G, \vec w_i^s}(s, u)
\end{align*}
as claimed.
\end{proof}
%
Now, note that $\dist^{K}_{H, \vec w_i^s}(s, u)\geq \dist^{K}_{G, \vec w_i^s}(s, u)$ since $H$ is a subgraph of $G$. Thus,
\begin{align}
d'(s, u) &= 2\dist_{G, w_{i+1}}(s, u)+\dist^{K}_{H, \vec w_i^s}(s, u)\\
&\geq 2\dist_{G, w_{i+1}}(s, u)+\dist^{K}_{G, \vec w_i^s}(s, u)\label{eq:d prime one}\\
&=\dist_{G, w_i}(s, u),
\end{align}
where the last equality is by Claim~\ref{claim:dist w_i from dist w_i^u}. This proves the first claim of Proposition~\ref{prop:d prime}.
%
For the second claim, we note that if  $\dist_{H, \vec w_i^s}(s, u)= \dist_{G, \vec w_i^s}(s, u)$ then  $\dist^{K}_{H, \vec w_i^s}(s, u)=\dist^{K}_{G, \vec w_i^s}(s, u)$ since $K\geq \ecc(G, \cW_i)\geq \dist_{G, \vec w_i^s}(s, u)$. Thus, ``$\geq$'' in Eq.~\eqref{eq:d prime one} can be replaced by ``$=$''.
%\end{proof}


==> arXiv/intro.tex <==
\section{Introduction}
%\danupon{This sentence from Roditty-Zwick might be useful in the sense that the shortest path problem also has a connection to dynamic graph problems. ``Elkin [14], extending results of Elkin and Peleg [15], shows that for any $\epsilon, \delta>0$, there exists $\beta=\beta(\epsilon, \delta)$ such that estimated distances from a set of sources S to all vertices of an unweighted undirected graph can be computed in ...''}


%Distributed computing is a very broad area that encompasses a plethora of disciplines. The particular subarea of distributed computing that is relevant to this survey focuses on the so-called message-passing model of computation


%
%While the all-pairs shortest paths problem has been recently resolved \cite{HolzerW12,PelegRT12,FrischknechtHW12} for the unweighted case, there is no non-trivial algorithm for the weighted case. For single-source shortest paths, the first sublinear-time algorithm follows from the recent breakthrough in constructing routing table \cite{LenzenP13}: one can $O(\epsilon^{-1}\log \epsilon^{-1})$-approximate single-source shortest path in $\tilde O(n^{1/2+\epsilon}+D)$ time\danupon{This is because they need $O(\log \epsilon^{-1}\log n)$-size label. I should check this one more time.}; this algorithm has a rather large approximation ratio, and a natural question is whether one can do better when we focus on the shortest path problem. 
%
%Our paper aims at resolving the remaining open problems for computing shortest paths on weighted graphs, with a focus on small approximation guarantees (mostly $(1+\epsilon)$). 

%that has been repeated asked (e.g. \cite{Elkin05,Elkin04,DasSarmaHKKNPPW11}) but 

%This problems is undoubtedly one of the most fundamental problems in computer science, and has been extensively studied in distributed computing since its early days. For example, as early as 1969, shortest path algorithms were repeatedly executed in the ARPANET and in other networks \cite{Lynch-Book,AfekR93,MRR80,Santoro-book}. %the distributed version of Bellman-Ford's algorithm were already used as early as 1969 in the ARPANET \cite[p.506]{Lynch-Book}
%Computing shortest paths, especially on large networks, has been an important primitive in network applications such as routing and load balancing and has motivated the studies of many subareas of theoretical computer science, in both sequential and distributed settings, including metric embeddings, distance labelings, spanners, and distance oracles.
%%
%%Several subareas of theoretical research have emerged centered around \apsp, in both sequential and distributed settings, such as metric embeddings, distance labelings, spanners, and distance oracles.
%%
%% Note: ARPANET is from HolzerW's PODC'12. Routing+Load Balancing is from DasSarma et al. SPAA'12.
%%
%Despite its importance and practical relevance, the basic issue of time complexity of this problem on distributed networks remains essentially unknown, especially on {\em weighted} graphs. 
%%
%%We focus on exactly this problem.
%%
%%
%%not much is known about the basic issue of {\em time-complexity} of this problem on distributed networks, especially in the general {\em weighted} case. This paper studies exactly this problem.
%%
%%
%In this paper, we focus on exactly this problem. In particular, we focus on two open problems raised by Elkin in his 2004 survey. 


\begin{comment}



 Many of such results were o with the help of {\em approximation techniques}.
 
 
%that encompasses a plethora of disciplines. 


... Introduce ``Distributed Approximation''. Say that the status up to 2004 can be seen in Elkin's survey, which motivates many later works. 

From ``Facility Location: Distributed Approximation'': During the last few years, the study of distributed approximation has attracted a lot of attention and has resulted in several fundamental results that shed new light into the possibilities and limitations of distributed computing [Elkin Survey]). The interest in distributed approximation appears natural considering that it lies on the boundary between two well established and important areas in computer science: distributed computing and approximability. In the same way as the theory of approximation has lead to an understanding of principles in complexity theory, the study of distributed approximation has the potential of providing a deeper understanding of the underlying distributed models [19, 5, 16].

Open problems from Elkin's survey. 

\begin{quote}
{\footnotesize\em
The author also wishes to draw attention to two problems in the message-passing model. Though these problems do not belong to the realm of distributed approximation, but rather have to do with the classical distributed computing, the author believes that their resolution would be instrumental for distributed approximation as well.

1. Consider a complete network of N processors in the message-passing model. Each edge of this clique is assigned a weight, but the weights do not affect the communication (i.e., delivering a short message through an edge requires one round independently of the weight of the edge). The bandwidth parameter B is log N. Prove a non-trivial ($\omega(1)$) lower bound on the complexity of the single-source distance computation in this model. A lower bound on the all-pairs-shortest-paths problem in this model will be most interesting as well.

2. (This problem was suggested by Vitaly Rubinovich in a private conversation with the author few years ago.)
%
What is the complexity of the shortest-path-tree problem in the message-passing model with small bandwidth parameter $B$ (i.e., $B = \log N$)? A lower bound of $\Omega(\sqrt{\frac{N}{B}})$ [29, 9] is known. No non-trivial upper bound is currently known. (The trivial one is $O(N)$.)
}
\end{quote}

Elkin made a progress for almost-shortest path problem (unweighted case) in PODC 2001. He also proved time-approximation tradeoff for shortest-path tree problem (weighted case) in STOC 2004. This was improved in our STOC 2011 paper. 

From STOC'11 paper: A few specific open questions include proving better lower or upper bounds for the problems of shortest s-t path, single-source distance computation, shortest path tree, s-t cut, minimum cut.

\end{comment}


%\subsection{Distributed Computing}\label{subsec:model}

%\medskip\noindent 

It is a fundamental issue to understand the possibilities and limitations of distributed/decentralized computation, i.e., to what degree local information is sufficient to solve global tasks. Many tasks can be solved entirely via local communication, for instance, how many friends of friends one has. Research in the last 30 years has shown that  some classic combinatorial optimization problems such as matching, coloring, dominating set, or approximations thereof can be solved   using small (i.e., polylogarithmic)  local communication. 
%
%For example, a maximal independent set can be computed in time $O(\log n)$ \cite{Luby86}, but not in time $\Omega(\sqrt{\log n / \log\log n})$ \cite{KuhnMW-jacm} ($n$ is the  network size). This lower bound even holds if message sizes are unbounded.
%
However, many important optimization problems  are ``global'' problems from the distributed computation point of view. To count the total number of nodes, to determining the diameter of the system, or to compute a spanning tree, information necessarily must travel to the farthest nodes in a system. If exchanging a  message over a single edge costs one time unit, one needs $\Omega(\diam)$ time units to compute the result, where $\diam$ is the network's diameter. In a model where message size could be unbounded (often known as the \local model), one can simply collect all the information in $O(\diam)$ time (ignoring time for the local computation), and then compute the result. A more realistic model, however, has to take into account the congestion issue and limits the size of a message allowed to be sent in a single communication round to some $B$ bits, where $B$ is typically set to $\log n$. This model is often called synchronous \congest (or $\congest(B)$ if $B\neq \log n$). 
%
%In this model, often called the \congest model, the above algorithmic approach will clearly require time much higher than $\diam$. It is therefore interesting to ask whether the network's diameter can still be computed in time O(D) in the CONGEST model.
%
%Hence, in order to arrive at a realistic problem, we need to introduce {\em communication limits}, i.e., each node can exchange messages with each of its neighbors in each step of a synchronous system, but each message can have at most $B$ bits; typically $B$ is small, say $O(\log n)$. 
%
Time complexity in this model is one of the major studies in distributed computing \cite{peleg}. 


Many previous works in this model, including several previous FOCS/STOC papers (e.g. \cite{GarayKP98,PelegR00,Elkin06,DasSarmaHKKNPPW11,LenzenP13}), concern {\em graph problems}. Here, we want to learn some topological properties of a network, such as minimum spanning tree (\mst), minimum cut (\mincut), and distances. 
%
These problems can be trivially solved in $O(m)$ rounds, where $m$ is the number of edges, by aggregating the whole network into one node. Of course, this is neither interesting nor satisfactory. The holy grail in the area of distributed graph algorithms is to beat this bound and, in many case, obtain a {\em sublinear-time} algorithm whose running time is in the form $\tilde O(n^{1-\epsilon}+\diam)$ for some constant $\epsilon>0$, where $n$ is the number of nodes and $\diam$ is the network's diameter.
%
%
For example, through decades of extensive research, we now have an algorithm that can find an \mst in  $\tilde O(n^{1/2}+\diam)$ time \cite{GarayKP98,KuttenP98}, and we know that this running time is tight \cite{PelegR00}. This algorithm serves as a building block for several other sublinear-time algorithms (e.g. \cite{Thurimella97,PritchardT11,GhaffariK13}). 

It is also natural to ask whether we can further improve the running time of existing graph algorithms by mean of {\em approximation}, e.g., if we allow an algorithm to output a spanning tree that is almost, but not, minimum. This question has generated a research in the direction of {\em distributed approximation algorithms} which has become fruitful in the recent years.
% (see Elkin's survey \cite{Elkin04} and recent papers such as \cite{DasSarmaHKKNPPW11,HolzerW12,PelegRT12,GhaffariK13}). 
%
On the negative side, Das Sarma et al. \cite{DasSarmaHKKNPPW11} (building on \cite{PelegR00,Elkin06,KorKP13}) show that \mst and a dozen other problems, including \mincut and computing the distance between two nodes, cannot be computed faster than $\tilde O(n^{1/2}+\diam)$ in the synchronous \congest model even when we allow a large approximation ratio. On the positive side, we start to be able to solve some problems in sublinear time by sacrifying a small approximation factor; e.g., we can $(2+\epsilon)$-approximate \mincut in $\tilde O(n^{1/2}+\diam)$ time \cite{GhaffariK13} and $(3/2)$-approximate the network's diameter in $O(n^{3/4}+\diam)$ time \cite{HolzerW12,PelegRT12}. 
%time $O(\min n^{1/2}\diam, n/\diam+\diam) = O(n^{3/4}+\diam)$ \cite{HolzerW12,PelegRT12}. 
%
The question whether distributed approximation algorithms can help improving the time complexity of computing shortest paths was raised a decade ago by Elkin \cite{Elkin04}. 
%
It is surprising that, despite so much progress on other problems in the last decade, the problem of computing shortest paths is still widely open, especially when we want a small approximation guarantee. Prior to our work, sublinear-time algorithms for computing single-source shortest path (\sssp) and linear-time algorithms for computing all-pairs shortest paths (\apsp) have to pay a high approximation factor \cite{LenzenP13}. This paper fills this gap with algorithms having small approximation guarantees. 



%However, to compute a spanning tree, even single-bit messages are enough, as one can simply  breadth-first-search the graph in time $O(D)$ and this is optimal \cite{peleg}.


\subsection{The Model}  \label{sec:model}


Consider a network of processors  modeled by an undirected unweighted  $n$-node $m$-edge 
graph $G$, where nodes model the processors and  edges model the {\em bounded-bandwidth} links between the processors. Let $V(G)$ and $E(G)$ denote the set of nodes and edges of $G$, respectively. 
%
%The processors  (henceforth, nodes) communicate  by exchanging messages via the links (henceforth, edges).  The nodes  have limited global knowledge, in particular, each of them has its own local perspective of the network (a.k.a graph), which is confined to its immediate neighborhood.  The nodes may have to compute (cooperatively) some global function of the graph, such as a minimum spanning tree (\mst) or a minimum cut (\mincut), via communicating with each other and running a distributed algorithm designed for the task at hand.
%
%There are several measures to analyze the performance of such algorithms,
%a fundamental one being the running time, defined as the worst-case number of {\em rounds} of distributed communication. This measure naturally gives rise to a  complexity measure of problems, called the {\em time complexity}.
%On each round at most $B$ bits can be sent through each edge in each direction, where $B$ is the bandwidth parameter of the network. The design of efficient algorithms for this model (henceforth, the $B$ model), as well as establishing lower bounds on the time complexity of various fundamental graph problems, has been the subject of an active area of research called (locality-sensitive)  {\em distributed computing} (see \cite{peleg} and references therein.)
%
The processors  (henceforth, nodes) are assumed to have unique IDs in the range of $\{1, \ldots, \poly(n)\}$ and infinite computational power. Each node has limited topological knowledge; in particular, it only knows the IDs of its neighbors and knows {\em no} other topological information (e.g., whether its neighbors are linked by an edge or not). Nodes may also accept some additional inputs as specified by the problem at hand.

For the case of graph problems, the additional input is {\em edge weights}.  Let $w:E(G)\rightarrow \{1, 2, \ldots, \poly(n)\}$ be the edge weight assignment. We refer to network $G$ with weight assignment $w$ as the {\em weighted network}, denoted by $(G, w)$. The weight $w(uv)$ of each edge $uv$ is known only to $u$ and $v$. As commonly done in the literature (e.g., \cite{KhanP08,LotkerPR09,KuttenP98,GarayKP98,GhaffariK13}), we will assume that the maximum weight is $\poly(n)$; so, each edge weight can be sent through an edge (link) in one round.\footnote{We note that, besides needing this assumption to ensure that weights can be encoded by $O(\log n)$ bits, we also need it in the analysis of the running time of our algorithms: most running times of our algorithms are logarithmic of the largest edge weight. This is in the same spirit as, e.g., \cite{LotkerPR09,GhaffariK13,KhanP08}.} 


%The processors  (henceforth, nodes) communicate  by exchanging messages via the links (henceforth, edges).  The nodes  have limited global knowledge, in particular, each of them has its own local perspective of the network (a.k.a graph), which is confined to its immediate neighborhood.  The nodes may have to compute (cooperatively) some global function of the graph, such as a minimum spanning tree (\mst) or a minimum cut (\mincut), via communicating with each other and running a distributed algorithm designed for the task at hand. 
%
%There are several measures to analyze the performance of such algorithms, a fundamental one being the running time, defined as the worst-case number of {\em rounds} of distributed communication. This measure naturally gives rise to a  complexity measure of problems, called the {\em time complexity}. On each round at most $B=\log n$ bits can be sent through each edge in each direction. The design of efficient algorithms for this model (henceforth, the $B$ model), as well as establishing lower bounds on the time complexity of various fundamental graph problems, has been the subject of an active area of research called (locality-sensitive)  {\em distributed computing} (see \cite{peleg} and references therein.)

%Despite having only local knowledge, nodes may have to compute (cooperatively) some {\em global} function of the network, such as a minimum spanning tree, minimum cut, and shortest paths, via communicating with each other and running a distributed algorithm designed for the task at hand. 
%%

There are several measures to analyze the performance of such algorithms, a fundamental one being the running time, defined as the worst-case number of {\em rounds} of distributed communication. 
%
%The communication is synchronous, and occurs in discrete pulses, called {\em rounds}. 
%
At the beginning of each round, all nodes wake up simultaneously. Each node $u$ then sends an arbitrary message of $B=\log n$ bits through each edge $uv$, and the message will arrive at node $v$ at the end of the round. 

%(Note that the assumption that the network is synchronous can be easily removed using the standard {\em synchronizer} \cite{peleg}.)



%
%There are several measures to analyze the performance of such algorithms, a fundamental one being the {\em running time}, defined as the worst-case number of rounds of distributed communication. 
%%
%We analyze the running time in terms of $n$ and $m$. Additionally, since global problems that we consider typically require $\Omega(\diam)$ rounds, where $\diam$ is network's diameter, we will consider $\diam$ as another parameter when we analyze the running time. Throughout, we use $\tilde O(\cdot)$ to hide the $O(\poly\log n)$ term. 

We assume that nodes always know the number of the current round. To simplify notations, we will name nodes using their IDs, i.e. we let $V(G)\subseteq \{1, \ldots, \poly(n)\}$. Thus, we use $u\in V(G)$ to represent a node, as well as its ID. The running time is analyzed in terms of number of nodes $n$, number of edge $m$, and $\diam$, the diameter of the network $G$. Since we can compute $n$ and $2$-approximate $\diam$ in $O(\diam)$ time, we will assume that every node knows $n$ and the $2$-approximate value of $\diam$. We say that an event holds {\em with high probability} (w.h.p.) if it holds with probability at least $1-1/n^c$, where $c$ is an arbitrarily large constant. 




 

%The most well-known result in this area is perhaps the sublinear-time algorithm for \mst: By the seminal papers of Garay, Kutten, and Peleg \cite{GarayKP98} and Kutten and Peleg \cite{KuttenP98}, we can find an \mst in  $\tilde O(n^{1/2}+\diam)$ time. This running time is shown to be tight by Peleg and Rubinovich \cite{PelegR00}. This algorithm serves as a building block for several other sublinear-time algorithms (e.g. \cite{Thurimella97,PritchardT11}). 
%
%%\paragraph{Distributed Approximation Algorithms}
%
%It is natural to ask whether we can further improve existing running times by mean of {\em approximation}, e.g., if we allow the algorithm to output a spanning tree that is almost, but not, minimum. This question has generated a research in the direction of {\em distributed approximation algorithms} which has become fruitful in the recent years. On the negative side, Das Sarma et al. \cite{DasSarmaHKKNPPW11} (building on \cite{PelegR00,Elkin06,KorKP13}) show that \mst and a dozen other problems, including \mincut and computing shortest paths, cannot be solved faster than $\tilde O(n^{1/2}+\diam)$ even when we allow a large approximation ratio. On the positive side, we start to be able to solve some problems in sublinear time by sacrifying a small approximation factor; notable examples are $(2+\epsilon)$-approximating the minimum cut in $\tilde O(n^{1/2}+\diam)$ time \cite{GhaffariK13} and $(3/2)$-approximating the network's diameter in time $O(\min n^{1/2}\diam, n/\diam+\diam) = O(n^{3/4}+\diam)$ \cite{HolzerW12,PelegRT12}. 
%%
%It is surprising that, despite so much progress and extensive research on this topic for decades, the problem of computing shortest paths is still widely open, especially when we want a small approximation guarantee. This paper aims at resolving this problem. 

%In the last few decades, extensive studies of graph problems on distributed networks have resulted in many surprising results, showing that many problems can be solved in a non-trivial way, e.g. a maximal independent set in $O(\log n)$ time~\cite{Luby86,KuhnMW-jacm} and a minimum spanning tree in sub-linear time~\cite{KuttenP98,GarayKP98}. 
%
%Despite so much progress on this topic, it is surprising that not much is known about a fundamental problem like \apsp.


%
%
%The study of {\em time complexity} is at the core of computer science and, not surprisingly, remains one of the central problems in the area of {\em distributed computing}. 
%%
%%in distributed systems and networking research, an equally fundamental issue of time complexity of {\em distributed algorithms} remains one of the central problems. 
%%
%%In particular, this issue is usually studied in the so-called message-passing model of computation \cite{Dijkstra74,Gallager1976shortest,Lann77,peleg}. 
%%
%%of {\em time complexity} on (message-passing) distributed networks, one of the central subareas of distributed computation. 
%%
%One important question in this area is whether there are {\em sublinear-time} algorithms in the so-called message-passing model~\cite{Dijkstra74,Gallager1976shortest,Lann77,peleg} for solving fundamental graph problems such as minimum-weight spanning tree (MST), minimum cut, and shortest paths; here, sublinear time refers to the running time of $\tilde O(n^{1-\epsilon}+D)$ for some constant $\epsilon>0$, where $n$ is the number of nodes (processors) in the distributed network, $D$ is its diameter, and $\tilde O$ hides an $O(\poly\log n)$ factor. This question has been studied for decades and has led to several new techniques and surprising results for many problems. A notable example is the MST problem which can be computed exactly in $\tilde O(n^{1/2}+D)$ time \cite{KuttenP98}. This result serves as a building block for many algorithms, including the recent progress on the minimum cut problem where one can $(2+\epsilon)$-approximate the minimum cut in $\tilde O(n^{1/2}+D)$ time \cite{GhaffariK13}\danupon{Should mention that it won best paper award}. It is also known that improving the $\tilde O(n^{1/2}+D)$ time bound further is impossible even when we allow a large approximation \cite{DasSarmaHKKNPPW11}. 
%%
%%
%% such as maximal independent set~\cite{Luby86,KuhnMW-jacm}, minimum dominating set \cite{JiaRS02,KuhnM10}, and minimum-weight spanning tree \cite{KuttenP98,GarayKP98}. 
%%
%For other problems, see the nice survey by Elkin \cite{Elkin04} and references therein. 
%%
%Despite so much progress in obtaining sublinear-time algorithms for graph problems, one fundamental problem remains embarrassingly open: computing shortest paths on weighted distributed networks. 
%%
%Our paper aims at resolving this problem. 

\subsection{Problems \& Definitions}


%\paragraph{Distance and Diameter}\footnote{For other related terms, such as  girth, center, and peripheral vertices, see \cite{HolzerW12}.}


For any nodes $u$ and $v$, a {\em $u$-$v$ path} $P$ is a path $\langle u=x_0, x_1, \ldots, x_\ell=v\rangle$ where $x_ix_{i+1}\in E(G)$ for all $i$. For any weight assignment $w$, we define the weight or distance of $P$ as $w(P)=\sum_{i=0}^{\ell-1} w(x_ix_{i+1})$. 
%
Let $\cP_G(u,v)$ denote the set of all $u$-$v$ paths in $G$. We use $\dist_{G, w}(u, v)$ to denote the distance from $u$ to $v$ in $(G,  w)$; i.e., $\dist_{G,  w}(u, v)=\min_{P\in \cP_G(u, v)}  w(P)$. We say that a path $P$ is a {\em shortest $u$-$v$ path} in $(G,  w)$ if $ w(P)=\dist_{G,  w}(u, v)$.
%
The {\em diameter} of $(G,  w)$ is $D(G,  w)=\max_{u, v} \dist_{G,  w}(u, v)$. 
%The {\em radius} of $(G,  w)$ is $\rad(G,  w)$ $=\min_u$ $\max_v$ $\dist_{G,  w}(u, v)$. 
%
When we want to talk about the properties of the underlying undirected unweighted network $G$, we will drop $ w$ from the notations. Thus, $\dist_G(u, v)$ is the distance between $u$ and $v$ in $G$ and,  $\diam(G)$ is the diameter of $G$. We refer to $\diam(G)$ by ``hop diameter'', or sometimes simply ``diameter'', and $\diam(G, w)$ by ``weighted diameter''. When it is clear from the context, we use $\diam$ to denote $\diam(G)$. We emphasize that, like other papers in the literature, the term $\diam$ which appears in the running time of our algorithms is the diameter of the underlying {\em unweighted} network $G$.  



%To avoid confusion, we note the notations we use here. 
%%We use an undirected unweighted graph $G$ to denote the input distributed network. 

%Let us first define the notion of {\em distance}, {\em diameter} and {\em radius} on networks whose weight function could be {\em symmetric} or {\em asymmetric}.
%
\begin{definition}[Single-Source and All-Pairs Shortest Paths (\sssp, \apsp)]\label{def:sssp}\label{def:apsp} 
In the {\em single-source shortest paths problem (\/\sssp)}, we are given a weighted network $(G, w)$ as above and a {\em source} node $s$ (the ID of $s$ is known to every node). We want to find the distance between $s$ and every node $v$ in $(G, w)$, denoted by $\dist_{G, w}(s, v)$. In particular, we want $v$ to know the value of $\dist_{G, w}(s, v)$.
%
In the all-pairs shortest paths problem (\apsp), we want to find $\dist_{G, w}(u, v)$ for every pair $(u, v)$ of nodes. In particular, we want both $u$ and $v$ to know the value of $\dist_{G, w}(u, v)$.
%%
\end{definition}
%
%\begin{definition}[All-Pairs Shortest Paths (\apsp)]\label{def:apsp} 
%In the all-pairs shortest paths problem (\apsp), we are given a weighted network $(G, w)$ as above and want to, for every pair $(u, v)$ of nodes, find the distance between $u$ and $v$ in $(G, w)$, denoted by $\dist_{G, w}(u, v)$. In particular, we want both $u$ and $v$ to know $\dist_{G, w}(u, v)$.\footnote{We emphasize that we do {\em not} require every node to know the distances between {\em all} pairs of nodes.} 
%%
%\danupon{This was a footnote before: Also note that, while our paper focuses on computing distances between all pairs of nodes, it can be used to compute a routing table in $O(n)$ time as well: Nodes can exchange all distance information with their neighbors in $O(n)$ time. Then, when a node $u$ wants to send a message to node $s$, it simply sends such message to the neighbor $v$ with smallest $\dist_{G, w}(u, v)$.}
%\end{definition}
%%
For any $\alpha$, we say an algorithm $\cA$ is an {\em $\alpha$-approximation} algorithm for \sssp if  it outputs $\widetilde{\dist}_{G, w}$ such that $\dist_{G, w}(s, v) \leq \widetilde{\dist}_{G, w}(s, v)\leq \alpha\dist_{G, w}(s, v)$ for all $v$. 
%
Similarly, we say that $\cA$ is an $\alpha$-approximation algorithm for \apsp if it outputs $\widetilde{\dist}_{G, w}$ such that $\dist_{G, w}(u, v) \leq \widetilde{\dist}_{G, w}(u, v)\leq \alpha\dist_{G, w}(u, v)$ for all $u$ and $v$. 
%
%We now formally define the terms that we need (including $\dist_{G, w}$). 
%In particular, we define {\em distance}, {\em diameter} and {\em radius} on networks whose weight assignment could be {\em symmetric} or {\em asymmetric}.

%\paragraph{Asymmetric Weight Assignment}
%We note that our input weighted network $(G, w)$ is always {\em symmetric} in the sense that the cost of going from $u$ to $v$ through edge $uv$ is the same as the cost of going from $v$ to $u$ through the same edge; i.e. $w(uv)=w(vu)$.
%%
%%In this case, we say that $w$ is {\em symmetric} (since its adjacency matrix is symmetric).
%%
%While our input weight assignment is always symmetric, during the course of our algorithm we will have to deal with a more general weight assignment $\vec w'$ that is {\em asymmetric}; i.e. it is possible that $\vec w'(uv)\neq \vec w'(vu)$ for some edge $uv$. We will put an arrow above $\vec w'$ to emphasize that it is asymmetric. Note that the class of asymmetric assignments also includes symmetric assignments.\danupon{Is it weird to use asymmetric like this?} Also note that the underlying network $G$ is always undirected.

%Note that the underlying network is always undirected.

%solve a problem on some network $(G', \vec w')$ where $\vec w'$ is {\em asymmetric}; i.e. it is possible that $\vec w'(uv)\neq \vec w'(vu)$ for some edge $uv$. We put an arrow above $\vec w'$ to emphasize that it is asymmetric. Note that the underlying network $G'$ is always undirected, and 

%Besides \apsp, this paper considers the following problems.
%
%\vspace{-.05in}\begin{definition}[Computing Diameter and Radius]\label{def:diameter radius}
%In the diameter and radius computation problem on weighted network $(G, w)$, we want every node to know $\diam(G, w)$ and $\rad(G, w)$, respectively. An $\alpha$-approximation algorithm is an algorithm that outputs $\tilde \diam(G, w)$ and $\tilde \rad(G, w)$ such that  $\diam(G, w)\leq \tilde \diam(G, w)\leq \alpha \diam(G, w)$ and  $ \rad(G, w)\leq \tilde \rad(G, w)\leq \alpha \rad(G, w)$. 
%\end{definition}
%
%


\paragraph{Remark} We emphasize that we do {\em not} require every node to know {\em all} distances. Also note that, while our paper focuses on computing distances between nodes, it can be used to find a routing path or compute a routing table as well. For example, after solving \apsp, nodes can exchange all distance information with their neighbors in $O(n)$ time. Then, when a node $u$ wants to send a message to node $v$, it simply sends such message to the neighbor $x$ with smallest $\dist_{G, w}(v, x)$. 
%
The name shortest paths is inherited from \cite{DasSarmaHKKNPPW11} (see the definition of shortest $s$-$t$ path problem in \cite[Section 2.5]{DasSarmaHKKNPPW11}) and in particular the lower bound in \cite{DasSarmaHKKNPPW11} holds for our problem). 


%For any path $P=\langle x_0, x_1, \ldots, x_\ell\rangle$ from node $x_0$ to node $x_\ell$, we let $w(P)$ be the length of this path; i.e., $w(P)=\sum_{i=0}^{\ell-1} w(x_$.



\begin{comment}
\begin{figure}
\small
\begin{tabular}{|c|c|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  $G$ & Distributed network\\
  \small $V(G)$, $n$ & \small Set of nodes in $G$ and $n=|V(G)|$\\
  \small $(G, w)$ & \small Weighted distributed network (Sec~XXX)\\
  \small $\dist_{G, w}(u, v)$ & \small  Distance between $u$ and $v$ in $G$ (Sec~XXX) \\
  \small $D(G, w)$ & \small  Weighted diameter of $(G, w)$ (Sec~XXX)\\
  \small $\spd(G, w)$ & \small Shortest path diameter of $(G, w)$ (Sec~XXX) \\
  \small $\ecc(G, \cW)$ & \small Multi-Weight diameter of $(G, \cW)$ (Sec~XXX)\\
  \hline
  \apsp & \small All-Pairs Shortest Path Problem (Sec~XXX)\\
  \small $K$-\apsp & \small  Bounded-Distance All-Pairs \\
  & \small Shortest Path Problem (Sec~XXX)\\
%  $\cS$-\ksp & $\cS$-Source Shortest Path Problem (Sec~XXX)\\
%  $\cS$-\asp & $\cS$-Source Almost Shortest Path Problem (Sec~XXX)\\
  \small $(\cS, K)$-\ksp & \small Bounded-Distance $\cS$-Source \\
  & \small  Shortest Path Problem (Sec~XXX)\\
  \small $(\cS, K)$-\asp & \small Bounded-Distance $\cS$-Source\\
  & \small Almost Shortest Path Problem (Sec~XXX)\\
  \hline
\end{tabular}
\caption{Notations}\label{fig:notation}
\end{figure}
\end{comment}


\begin{table*}
\centering
\begin{tabular}{ |l|l|l|l|l| }
%\hline
%\multicolumn{3}{ |c| }{Team sheet} \\
\hline
Problems & Topology & References & Time & Approximation \\ 
\hline
\multirow{5}{*}{\sssp} & \multirow{3}{*}{General} & Bellman\&Ford \cite{Bellman58,Ford56} & $\tilde O(n)$ & exact \\
& & Lenzen\&Patt-Shamir \cite{LenzenP13} & $\tilde O(n^{1/2+1/2k}+\diam)$ & $8k\lceil \log (k+1) \rceil -1$ \\
 & & {\bf this paper} & $\tilde O(n^{1/2}\diam^{1/4}+\diam)$ & $1+o(1)$ \\
 & & & ($= \tilde O(n^{3/4}+\diam)$) & \\
% & & this paper & $\tilde O(n^{1/2+1/k}+D)$ & $2k-1+o(1)$ \\
 \cline{2-5}
& \multirow{2}{*}{Fully-Connected} & Baswana\&Sen \cite{BaswanaS07} & $\tilde O(n^{1/k})$ & $2k-1$ \\
%& & Lenzen\&Patt-Shamir \cite{LenzenP13} & $\tilde O(n^{1/2+1/k})$ & $8k\lceil \log (k+1) \rceil -1$ \\
& & {\bf this paper} & $\tilde O(n^{1/2})$ & exact \\
%
\hline
%
\multirow{5}{*}{\apsp} & \multirow{3}{*}{General} & Trivial & $O(m)$ & exact \\
%& & Baswana\&Sen \cite{BaswanaS07} & $\tilde O(n^{1+\epsilon})$ & $O(\epsilon^{-1})$ \\
& & Lenzen\&Patt-Shamir \cite{LenzenP13} & $\tilde O(n)$ & $O(1)$ \\
 & & {\bf this paper} & $\tilde O(n)$ & $1+o(1)$ \\
 \cline{2-5}
& \multirow{2}{*}{Fully-Connected} & Baswana\&Sen \cite{BaswanaS07} & $\tilde O(n^{1/k})$ & $2k-1$ \\
%& & Lenzen\&Patt-Shamir \cite{LenzenP13} & $\tilde O(n^{1/2+\epsilon})$ & $O(\epsilon^{-1}\log \epsilon^{-1})$ \\
& & {\bf this paper} & $\tilde O(n^{1/2})$ & $2+o(1)$ \\
\hline
\end{tabular}
\caption{Summary of previous and our results (presented in \Cref{sec:related,sec:results}). Parameter $k\geq 1$ is an integer (note that the time complexities above are sublinear only when $k\geq 2$). Note that this table omits previous running times based on other parameters (such as shortest-path diameter).}\label{table:results summary}
\end{table*}


% ****************************************
% Tabel below use epsilon instead of k
% ****************************************

%\begin{table}
%\centering
%\begin{tabular}{ |l|l|l|l|l| }
%%\hline
%%\multicolumn{3}{ |c| }{Team sheet} \\
%\hline
%Problems & Topology & References & Time & Approximation \\ 
%\hline
%\multirow{6}{*}{\sssp} & \multirow{3}{*}{General graphs} & Bellman\&Ford \cite{Bellman58,Ford56} & $\tilde O(n)$ & exact \\
%& & Lenzen\&Patt-Shamir \cite{LenzenP13} & $\tilde O(n^{1/2+\epsilon}+D)$ & $O(\epsilon^{-1}\log \epsilon^{-1})$ \\
% & & this paper & $\tilde O(n^{1/2}D^{1/4}+D)$ & $1+o(1)$ \\
% \cline{2-5}
%& \multirow{3}{*}{Complete graphs} & Baswana\&Sen \cite{BaswanaS07} & $\tilde O(n^{1+\epsilon})$ & $O(\epsilon^{-1})$ \\
%& & Lenzen\&Patt-Shamir \cite{LenzenP13} & $\tilde O(n^{1/2+\epsilon})$ & $O(\epsilon^{-1}\log \epsilon^{-1})$ \\
%& & this paper & $\tilde O(n^{1/2})$ & exact \\
%%
%\hline
%%
%\multirow{5}{*}{\apsp} & \multirow{4}{*}{General graphs} & Trivial & $O(m)$ & exact \\
%%& & Baswana\&Sen \cite{BaswanaS07} & $\tilde O(n^{1+\epsilon})$ & $O(\epsilon^{-1})$ \\
%& & Lenzen\&Patt-Shamir \cite{LenzenP13} & $\tilde O(n)$ & $O(1)$ \\
% & & this paper & $\tilde O(n)$ & $1+o(1)$ \\
% \cline{2-5}
%& \multirow{2}{*}{Complete graphs} & Baswana\&Sen \cite{BaswanaS07} & $\tilde O(n^{\epsilon})$ & $O(\epsilon^{-1})$ \\
%%& & Lenzen\&Patt-Shamir \cite{LenzenP13} & $\tilde O(n^{1/2+\epsilon})$ & $O(\epsilon^{-1}\log \epsilon^{-1})$ \\
%& & this paper & $\tilde O(n^{1/2})$ & $2+o(1)$ \\
%\hline
%\end{tabular}
%\caption{Summary of previous and our results. Note that this table omit previous running time based on other parameters (such as shortest-path diameter).}\label{table:results summary}
%\end{table}


\subsection{Our Results}\label{sec:results}
Our and previous results are summarized in \Cref{table:results summary} (see \Cref{sec:related} for the details of previous results). As shown in the table, previous algorithms either have large approximation guarantee or large running time. In this paper, we aim at algorithms with both small approximation guarantees and small running time. We consider both \sssp and \apsp and study algorithms on both general networks and fully-connected networks.
%
Our main result is a sublinear-time $(1+o(1))$-approximation algorithm for \sssp on general graphs:
%
\begin{theorem}[\sssp on general graph]\label{thm:main sssp}
There is a distributed $(1+o(1))$-approximation algorithm that solves \sssp on any weighted $n$-node network $(G, w)$. It finishes in  $\tilde O(n^{1/2}\diam^{1/4}+\diam)$ time w.h.p.
%, where $\tilde O$ hides the $\poly\log n$ term.
\end{theorem}

%Recall that $\diam$ is the diameter of the underlying unweighted network $G$. 


For typical real-world networks (e.g., ad hoc networks and peer-to-peer networks) $\diam$ is {\em small} (usually $\tilde O(1)$). (In some networks, an even stronger property also holds; e.g., a peer-to-peer network is usually assumed to be an expander \cite{AugustinePRU12}.) It is thus of a special interest to develop an algorithm in this setting. For example, \cite{LotkerPP06} studied \mst on constant-diameter networks. Das Sarma et al. \cite{DasSarmaNPT13} developed a $\tilde O((\ell \diam)^{1/2})$-time algorithm for computing a random walk of length $\ell$, which is faster than the trivial $O(\ell)$-time algorithm when $\diam$ is small.\danupon{We may also mention $\tilde O(n^{1/2}D)$-time algorithm for approximating the diameter \cite{PelegRT12}} In the same spirit, our algorithm is faster than previous algorithms. Moreover, in this case our running time matches the lower bound of $\tilde \Omega(n^{1/2}+\diam)$ \cite{DasSarmaHKKNPPW11,ElkinKNP12}, which holds even for any algorithm with $\poly(n)$ approximation ratio; thus, our result settles the status of \sssp for this case. 
%, which also answers an open problem raised by Elkin \cite{Elkin04} a decade ago and by Das Sarma et al. \cite{DasSarmaHKKNPPW11} for low-diameter networks. 
%
Additionally, since the same lower bound also holds in the quantum setting \cite{ElkinKNP12}, our result makes \sssp among a few problems (others are \mst and \mincut) that quantum communication cannot help speeding up distributed algorithms significantly.

Observe that our running time is {\em sublinear} as long as $\diam$ is sublinear in $n$ (since $\tilde O(n^{1/2}\diam^{1/4}+\diam)$ can be written as $\tilde O(n^{3/4}+\diam)$). As shown in \Cref{table:results summary}, previously we can either solve \sssp exactly in $\tilde O(n)$ time using Bellman-Ford algorithm \cite{Bellman58,Ford56} or $(8k\lceil \log (k+1) \rceil -1)$-approximately, for any $k>1$, in  $\tilde O(n^{1/2+1/2k}+\diam)$ time by applying the algorithm of Lenzen and Patt-Shamir \cite{LenzenP13}\footnote{Note that by applying the technique of Lenzen and Patt-Shamir with carefully selected parameters, the approximation ratio can be reduced to $4k-1$. We thank Christoph Lenzen (personal communication) for this information.}. Our algorithm is the first that gives an output very close to the optimal solution in sublinear time.
%
%Our result also answers one central question in the area of distributed approximation algorithms raised by Elkin \cite{Elkin04}  (attributed to Vitaly Rubinovich) and Das Sarma et al. \cite{DasSarmaHKKNPPW11}. 
%
%
Our result also points to an interesting direction in proving a stronger lower bound for \sssp: in contrast to previous lower bound techniques which usually work on low-diameter networks, proving a stronger lower bound for \sssp needs a new technique that must exploit the fact that the network's diameter is fairly large.\danupon{Should we also mention that we can also get $(2k-1)$-approximation?}
% 
%our algorithm implies that quantum communication cannot help speeding up distributed algorithms for \sssp by more than $\diam^{1/4}$. This makes 
%
As a by-product of our techniques, we also obtain a linear-time algorithm for \apsp. 
%
\begin{theorem}[\apsp on general graphs]\label{thm:linear apsp}
There is a distributed $(1+o(1))$-approximation algorithm that solves \apsp on any weighted $n$-node network $(G, w)$ which finishes in $\tilde O(n)$ time w.h.p.
\end{theorem}
%
We also observe that this algorithm is essentially {\em tight}:
% in the sense that {\em no} algorithm can solve \apsp in sublinear time, even in the unweighted case and even when we allow a large approximation ratio.  
%
%\begin{observation}[Lower bound for \apsp]\label{observe:lower bound}
%Any $\poly(n)$-approximation algorithm for \apsp on an $n$-node weighted network $G$ requires $\Omega(\frac{n}{\log n})$ time. This lower bound holds even when the underlying network $G$ has diameter $\diam(G)=2$.
%%
%Moreover, for any $\alpha(n)=O(n)$, any $\alpha(n)$-approximation algorithm on an {\em unweighted} network requires $\Omega(\frac{n}{\alpha(n)\log n})$ time. 
%%
%\end{observation}
%
\begin{restatable}[Lower bound for \apsp]{observation}{lowerbound}\label{observe:lower bound}
Any $\poly(n)$-approximation algorithm for \apsp on an $n$-node weighted network $G$ requires $\Omega(\frac{n}{\log n})$ time. This lower bound holds even when the underlying network $G$ has diameter $\diam(G)=2$.
%
Moreover, for any $\alpha(n)=O(n)$, any $\alpha(n)$-approximation algorithm on an {\em unweighted} network requires $\Omega(\frac{n}{\alpha(n)\log n})$ time. 
\end{restatable}
%
\Cref{observe:lower bound} implies that the running time of our algorithm in \Cref{thm:linear apsp} is {\em tight} up to a $\poly\log n$ factor, unless we allow a prohibitively large approximation factor of $\poly n$. Moreover, even when we restrict ourselves to unweighted networks, we still cannot significantly improve the running time, unless the approximation ratio is fairly large; e.g., any $n^{1-\delta}$-time algorithm must allow an approximation ratio of $\Omega(n^\delta/\log n)$.
%
We note that a similar result to \Cref{observe:lower bound} has been independently proved by Lenzen and Patt-Shamir \cite{LenzenP13} in the context of name-independent routing scheme.

Other by-products of our techniques are efficient algorithms on fully-connected distributed networks, i.e., when $G$ is a complete graph. As mentioned earlier, it is of an interest to study algorithms on low-diameter networks. The case of fully-connected networks is an extreme case where $\diam=1$. This special setting captures, e.g., overlay and peer-to-peer networks, and has received a considerable attention recently (e.g. \cite{LotkerPPP03,LenzenW11,PattShamirT11,Lenzen13,DolevLP12tri,BernsHP12}). Obviously, this model gives more power to algorithms since every node can directly communicate with all other nodes; for example, MST can be constructed in $O(\log\log n)$ time \cite{LotkerPPP03}, as opposed to the $\tilde \Omega(n^{1/2}+\diam)$ lower bound on general networks. No sublinear-time algorithm for \sssp and \apsp is known even on this model if we want an optimal or near-optimal solution. 
%
%For this special case, Elkin \cite{Elkin04} asked for a non-trivial ($\omega(1)$) lower bound on the complexity of \sssp and \apsp on this model. While we do not directly answer this question (and doing will be a breakthrough \cite{Oshman13}), we show that this model also admits non-trivial {\em upper} bounds. 
%
In this paper, we show such an algorithm. First, note that our $\tilde O(n^{1/2}\diam^{1/4}+\diam)$-time algorithm in \Cref{thm:main sssp} already implies that \sssp can be $(1+o(1))$-approximated in  $\tilde O(n^{1/2})$ time. We show that, as an application of our techniques for proving \Cref{thm:main sssp}, we can get an {\em exact} algorithm within the same running time. More importantly, we show that these techniques, combined with some new ideas, lead to a $(2+o(1))$-approximation $\tilde O(\sqrt{n})$-time algorithm for \apsp. The latter result is in contrast with the general setting where we show that a sublinear running time is impossible even when we allow large approximation ratios (\Cref{observe:lower bound}). 
%
\begin{theorem}[Sublinear time algorithm on fully-connected networks]
On any fully-connected weighted network, in $\tilde O(n^{1/2})$ time, \sssp can be solved exactly and \apsp can be $(2+o(1))$-approximated w.h.p. 
\end{theorem}
 




%\subsection{OLD}

%Our main results concern two open problems raised by Elkin \cite{Elkin04}. In 2004, Elkin wrote a nice survey which has become one of the landmarks in the development of the area of {\em distributed approximation}. He presented several sublinear-time algorithms obtained by approximation techniques and proposed several directions for future research. Among the proposed directions, two questions related to computing shortest paths were highlighted. 

%\paragraph{Algorithm for SSSP}
%One question (attributed to Vitaly Rubinovich) asked for the complexity of the shortest-path-tree problem (i.e. \sssp) in the message-passing model with small bandwidth parameter $B$, i.e., $B = \log n$ (i.e. the \congest model). At the time, a lower bound of $\Omega(\sqrt{\frac{n}{B}}+\diam(G))$ \cite{PelegR00,Elkin06} was known and no non-trivial upper bound was known. (The trivial algorithm is the distributed version of Bellman-Ford's algorithm, which takes $O(n)$ time.) The lower bound of $\Omega(\sqrt{\frac{n}{B}}+\diam(G))$ has been recently shown to hold even when we allow a large approximation ratio \cite{DasSarmaHKKNPPW11} and quantum communication \cite{ElkinKNP12}. Thus, we cannot hope to have a running time significantly better than $\Omega(\sqrt{n})$. 
%%


%
%
%Their result gives the first sublinear-time algorithm for \sssp, with a rather large approximation guarantee. In this paper, we present the first sublinear-time algorithm with a very small approximation guarantee; its running time almost matches the known lower bound. 
%







\subsection{Related Work}\label{sec:related}

\paragraph{Unweighted Case} \sssp and \apsp are essentially well-understood in the unweighted case. \sssp can be trivially solved in $O(\diam)$ time using a breadth-first search tree \cite{peleg,Lynch-Book}. 
%
%\apsp has been recently resolved \cite{HolzerW12,PelegRT12}: one can solve \apsp exactly in $O(n)$ time and improving this running time is impossible, even when we want to solve the special case of computing the network's diameter \cite{FrischknechtHW12}. 
%
%Very recent sequence of results \cite{FrischknechtHW12,HolzerW12,PelegRT12} have made much progress in understanding distributed algorithms for \apsp in the unweigthed case. 
%For \apsp, 
Frischknecht, Holzer, and Wattenhofer \cite{FrischknechtHW12,HolzerW12} show a (surprising) lower bound of $\Omega(n/\log n)$ for computing the diameter of unweighted networks, which implies a lower bound for solving unweighted \apsp. This lower bound holds even for $(3/2-\epsilon)$-approximation algorithms. This lower bound is matched (up to a $\poly\log n$ factor) by  $O(n)$-time deterministic {\em exact} algorithms for unweighted \apsp found independently by \cite{HolzerW12} and \cite{PelegRT12}.
%
Another case that has been considered is when nodes can talk to any other node in one time unit. This can be thought of as a special case of \apsp on fully-connected networks where edge weights are either $1$ or $\infty$. In this case, Holzer \cite{Holzer13thesis} shows that \sssp can be solved in $\tilde O(n^{1/2})$ time\footnote{We thank Stephan Holzer for pointing this out.}. 

\paragraph{Name-Dependent Routing Scheme} 
%
%\paragraph{Weighted Case}
For the weighted \sssp and \apsp on general networks, the best known results follow from the recent algorithm for computing tables for {\em name-dependent routing} and {\em distance approximation} by Lenzen and Patt-Shamir \cite{LenzenP13}.
%
In particular, consider any integer $k>1$. Lenzen and Patt-Shamir \cite[Theorem 4.12]{LenzenP13} showed that in time $\tau=\tilde O(n^{1/2+1/2k}+\diam)$ every node $u$ can compute a {\em label} $\lambda(u)$ of size $\sigma=O(\log (k+1)\log n)$ and a function $dist_u$ that maps label $\lambda(v)$ of any  node $v$ to a distance approximation $dist_u(v)$ such that $\dist_{G, w}(u, v) \leq dist_u(v) \leq \rho\dist_{G, w}(u, v)$ where $\rho=8k\lceil \log (k+1)\rceil -1$.\footnote{We note that Lenzen and Patt-Shamir \cite[Theorem 4.12]{LenzenP13} actually allow $k=1$. However, their algorithm relies on the result of Baswana and Sen (see Theorem 4.7 in their paper) which does not allow $k=1$.}
%
\danupon{Theorem 4.19 in the arXiv version and 4.12 in the STOC version of \cite{LenzenP13}: Consider any $\alpha=1/2+\epsilon$ for some $1/2\leq \epsilon\geq 1/\log n$ (see the paper for the case where $\epsilon$ is very close to $0$ which will not be considered here). Define $k=\lceil 1/2\epsilon\rceil$. We get stretch $\rho(\alpha)=8k\lceil \log (k+1)\rceil -1\rceil$, label size $O(\log (k+1)\log n)$, time $\tilde O(n^{\alpha}+\diam)$}
%
%\danupon{*** LP \cite{LenzenP13} seems to allow $k\geq 1$. But their algorithm (especially Theorem 4.7 in the STOC version) relies on Baswana and Sen's algorithm which only works when $k>1$ (see Section 1.2 of \cite{BaswanaS07}). ***}
%
We can solve \sssp by running the above algorithm of Lenzen and Patt-Shamir and broadcasting the label $\lambda(s)$ of the source $s$ to all nodes. This takes time $\tau+\sigma = \tilde O(n^{1/2+1/2k}+\diam)$ and has an approximation guarantee of $\rho$. We can solve \apsp by broadcasting $\lambda(v)$ for all $v$, taking time $\tau+n\sigma = \tilde O(n)$.
% on general graph and $\tau+\sigma = \tilde O(n^{1/2+1/2k})$ on complete graphs. 


\paragraph{Sparsification} 
%
The shortest path problem is one of the main motivations to study distributed algorithms for graph sparsification.  
%
%More recent and more time-efficient algorithms are based on the idea of {\em approximation} via {\em low-distortion sparse embeddings}.
%
These algorithms\footnote{We note that some of these algorithms (e.g., \cite{Elkin05,KhanKMPT12}) can actually solve a more general problem called the {\em $\cS$-shortest path} problem. To avoid confusions, we will focus only on \sssp and \apsp.} have either super-linear time or large approximation guarantees.
%
For example, 
% --- Elkin is improved by Elkin-Zhang below ----
%Elkin \cite{Elkin05} presents an algorithm for the unweighted case based on a sparse spanner that takes (very roughly) $O(n^{1+\xi})$ time and gives $(1+\epsilon)$-approximate solution, 
Elkin and Zhang \cite{ElkinZ06} present an algorithm for the unweighted case based on a sparse spanner that takes (very roughly) $O(n^{\xi})$ time and gives $(1+\epsilon)$-approximate solution, for small constants $\xi$ and $\epsilon$. The algorithm is also extended to the weighted case but both running time and approximation guarantee are large (linear in terms of the largest edge weight).
%
The running time could be traded-off with the approximation guarantee using, e.g., a $(2k-1)$-spanner of size $O(kn^{1+1/k})$ \cite{BaswanaS07} where $k$ can vary; e.g., by setting $k=\log n/\log\log n$, we have an $O(n\log n)$-time $O(\log n/\log \log n)$-approximation algorithm (we need $O(k^2)$ to construct a spanner and $O(kn^{1+1/k})=O(n\log n)$ to aggregate it). The spanner of \cite{Pettie10} can also be used to get a linear-time $(2^{O(\log^*{n})}\log n)$-approximation algorithm in the unweighted case.

\danupon{According to STOC'14 committee, \cite{DerbelGPV08} (which I used to cite) needs large messages so it's quite irrelevant.}

In general, it is not clear how to use graph sparsification for computing shortest paths since we still need at least linear time to collect the sparse graph. However, it plays a crucial role in some previous algorithms, including the algorithm of Lenzen and Patt-Shamir \cite{LenzenP13}. Moreover, by running the graph sparsification algorithm of Baswana and Sen \cite{BaswanaS07} and collecting the network to one node, we can $(2k-1)$-approximate \apsp in $O(kn^{1+1/k})$ time on general networks and $O(kn^{1/k})$ time on fully-connected networks, for any integer $k\geq 2$. This gives the fastest algorithm (with high approximation guarantees) on fully-connected networks.

%In other words, for any $1/\log n\leq \epsilon \leq 1/2$, we can $O(\epsilon^{-1})$-approximate \apsp in $\tilde O(n^{1+\epsilon})$ time on general graphs and $\tilde O(n^{\epsilon})$ time on complete graphs. 


\paragraph{Other Parameters} There are also some approximation algorithms whose running time is based on other parameters. These algorithms do not give any improvement for the worst values of their parameters. We do not consider these parameters in this paper since they are less standard. 
%
One important parameter is the {\em shortest-path diameter}, denoted by $\spdiam(G, w)$. This parameter captures the number of edges in a shortest path between any pair of nodes (see \Cref{def:spdiam} for details). It naturally arises in the analysis of several algorithms. For example, Bellman-Ford algorithm \cite{Bellman58,Ford56} can be analyzed to have $O(\spdiam(G, w))$ time for \sssp. 
%
Khan et al. \cite{KhanKMPT12} gives a $\tilde O(n\cdot \spdiam(G, w))$-time $O(\log n)$-approximation algorithm via {\em metric tree embeddings}~\cite{FakcharoenpholRT04}. We can also construct {\em Thorup-Zwick distance sketches}~\cite{ThorupZ05} of size $O(kn^{1/k})$ and stretch $2k-1$ in $\tilde O(kn^{1/k}\cdot \spdiam(G, w))$ time~\cite{DasSarmaDP12}. Since $\spdiam(G, w)$ can be as large as $n$, these algorithms do not give any improvement to previous algorithms when analyzed in terms of $n$ and $\diam$. One crucial component of our algorithms involves reducing the shortest-path diameter to be much less than $n$ (more in \Cref{sec:techniques}).
%
Another shortest path algorithm with running time based on the network's {\em local path diameter} is developed as a subroutine of the approximation algorithm for \mst \cite{KhanP08}. This algorithm solves a slightly different problem (in particular, nodes only have to know the distance to some nearby nodes) and cannot be used to solve \sssp and \apsp.



\paragraph{Lower Bounds} The lower bound of Das Sarma et al. \cite{DasSarmaHKKNPPW11} (building on \cite{Elkin06,PelegR00,KorKP13}) shows that solving \sssp requires $\tilde \Omega(\sqrt{n}+\diam)$ time, even when we allow $\poly(n)$ approximation ratio and the network has $O(\log n)$ diameter. This implies the same lower bound for \apsp. Recently, \cite{ElkinKNP12} shows that the same $\tilde \Omega(\sqrt{n}+\diam)$ lower bound holds even in the quantum setting. These lower bounds are subsumed by Observation~\ref{observe:lower bound} for the case of \apsp. 
%
Das Sarma et al. (building on \cite{LotkerPP06}) also shows a polynomial lower bound on networks of diameter 3 and 4. It is still open whether there is a non-trivial lower bound on networks of diameter one and two \cite{Elkin04}. 

%However, proving such a lower bound on complete graphs will be very difficult since it will imply a breakthrough in circuit complexity \cite{Oshman13}. 

%Our simple observation in Section~\ref{sec:results} subsumes all previous lower bounds completely for the case of weighted \apsp (but not for unweighted \apsp or diameter and girth computation).

%\danupon{Say this in "our results" section: Our simple lower bound presented in Appendix~\ref{sec:lower bound} subsumes all previous lower bounds completely for the case of weighted \apsp (but not for unweighted \apsp or diameter and girth computation).}



\paragraph{Other Works} While computing shortest paths is among the earliest studied problems in distributed computing, many classic works on this problem concern other objectives, such as the message complexity and convergence. When faced with the bandwidth constraint, the time complexities of these algorithms become higher than the trivial $O(m)$-time algorithm; e.g., Bellman-Ford algorithm and algorithms in \cite{AbramR82,Haldar97,AfekR93} require $\Omega(n^2)$ time.



%***\danupon{I think the algorithm in this paper can be used to $(1+\epsilon)$ approximate their problem. Would this give any better MST approximation? Answer: No.}\danupon{Also, should we say that if S and L are known then our running time could be reduced?}

%A better algorithm is to use the randomized algorithm of \cite{BaswanaS07} to compute a $(2k-1)$-spanner of size $O(kn^{1+1/k})$ in $O(k^2)$ time, for any $k$, and then aggregate the spanner in one node. For example, for $k=\log n/\log\log n$, we get an $O(\log n/\log\log n)$-approximation $O(n\log n)$-time algorithm for \apsp.

%There are also algorithms whose running time based on other parameters. Using the distributed version of {\em metric tree embeddings}~\cite{FakcharoenpholRT04}, an $O(nS\log n)$-time $O(\log n)$-approximation algorithm is shown in \cite{KhanKMPT12}, where $S$ is the network parameter called {\em shortest path diameter}. Since $S$ can be as large as $n$, this algorithm has $O(n^2\log n)$ time in the worst case.
%
%The authors of \cite{DasSarmaDP12} show a distributed algorithm that constructs {\em Thorup-Zwick distance sketches}~\cite{ThorupZ05} of size $O(kn^{1/k})$ and stretch $2k-1$ in $O(kn^{1/k}S\log n)$ time. For the worst value of $S$, this algorithm has the same performance as when we use the spanner of \cite{BaswanaS07}.

%Another shortest path algorithm with running time based on a network's {\em local path diameter} is developed as a subroutine of the approximate MST algorithm in \cite{KhanP08}. This algorithm solves a slightly different problem (in particular, nodes only have to know the distance to some nearby nodes) and cannot be used to solve \apsp.\danupon{I think the algorithm in this paper can be used to $(1+\epsilon)$ approximate their problem. Would this give any better MST approximation? Answer: No.}\danupon{Also, should we say that if S and L are known then our running time could be reduced?}


To the best of our knowledge, there is still no exact distributed algorithm for \apsp that is faster than the trivial $O(m)$-time algorithm\footnote{The problem can also be solved by running the distributed version of Bellman-Ford algorithm \cite{peleg,Lynch-Book,Santoro-book} from every node, but this takes $O(n^2)$ time in the worst case. So this is always worse than the trivial algorithm.}, except for the special case of {\em BHC network}, whose topology is structured as a balanced hierarchy of clusters. In this special case, the problem can be solved in $O(n \log n)$-time \cite{AntonioHT92}. 
%
For the related problem of computing network's diameter and girth, many results are known in the unweighted case but none is previously known for the weighted case. Peleg, Roditty, and Tal \cite{PelegRT12} shows that we can $\frac{3}{2}$-approximate the network's diameter in $O(n^{1/2}\diam)$ time, in the unweighted case, and Holzer and Wattenhofer \cite{HolzerW12} presents an $O(\frac{n}{\diam}+\diam)$-time $(1+\epsilon)$-approximation algorithm. By combining both algorithms, we get a $\frac{3}{2}$-approximation  $O(n^{3/4}+\diam)$-time algorithm. In contrast, any $(\frac{3}{2}-\epsilon)$-approximation and $(2-\epsilon)$-approximation algorithm for computing the network's diameter and girth requires  $\Omega(n/\log n)$ time~\cite{HolzerW12}
%\danupon{Lemma 11 Section 7.1.} 
and $\Omega(\sqrt{n}/\log n)$ time~\cite{FrischknechtHW12}, respectively. These bounds imply the same lower bound for approximation algorithms for \apsp on unweighted networks. In particular, they imply that our approximation algorithms are tight, even on unweighted networks.
%
%the same approximation factor of any algorithm for approximating \apsp on unweighted networks.\danupon{Say this in "our results": These lower bounds imply that our approximation algorithms are tight, even on unweighted networks.}
%\selfnote{So far I don't see any lower bound of $(2-\epsilon)$-approx algo. In \cite{FrischknechtHW12}, the lower bound of $\sqrt{n}$ is shown for GIRTH approximation.}

 




%\begin{quote}
%{\footnotesize\em
%The author also wishes to draw attention to two problems in the message-passing model. Though these problems do not belong to the realm of distributed approximation, but rather have to do with the classical distributed computing, the author believes that their resolution would be instrumental for distributed approximation as well.
%
%1. Consider a complete network of N processors in the message-passing model. Each edge of this clique is assigned a weight, but the weights do not affect the communication (i.e., delivering a short message through an edge requires one round independently of the weight of the edge). The bandwidth parameter B is log N. Prove a non-trivial ($\omega(1)$) lower bound on the complexity of the single-source distance computation in this model. A lower bound on the all-pairs-shortest-paths problem in this model will be most interesting as well.
%
%2. (This problem was suggested by Vitaly Rubinovich in a private conversation with the author few years ago.)
%%
%What is the complexity of the shortest-path-tree problem in the message-passing model with small bandwidth parameter $B$ (i.e., $B = \log N$)? A lower bound of $\Omega(\sqrt{\frac{N}{B}})$ [29, 9] is known. No non-trivial upper bound is currently known. (The trivial one is $O(N)$.)
%}
%\end{quote}









% 
%%
%\begin{theorem}[Informal statement of \Cref{thm:light-weight sssp}]\label{thm:light-weight sssp informal} 
%There is an algorithm that can $(1+o(1))$-approximate $h$-hop \sssp in $\tilde O(h)$ time and is {\em light-weight} in the sense that every node sends a message (of size $O(\poly\log n)$) to its neighbors only $O(\log n)$ times.
%\end{theorem}
%%
%Proving the above theorem is conceptually very simple: We show that by approximating weight assignment $w$ appropriately to a new weight assignment $w'$, we can show that $\dist_{G, w'}(u, v)=\tilde O(h)$ for any nodes $u$ and $v$. Moreover, we can use $\dist_{G, w'}(u, v)=\tilde O(h)$ to compute a $(1+o(1))$-approximate value of $\dist_{G, w}(u, v)$. Thus, it is sufficient for us to compute  $\dist_{G, w'}(u, v)$ in a light-weight manner, which can be done by slightly modify the basic breadth-first search algorithm.  
%%
%The fact that this algorithm is light-weight enables us to be able to runs it in {\em in parallel} from many sources. In particular, by using the random delay technique from \cite{LeightonMR94}, we show that we can run it from $k$ sources in $\tilde O(k+h+\diam)$ time (see \Cref{thm:k-source h-hop sp} for a formal statement).
%
%
%
%
%
%Our algorithms borrow several ideas from existing sequential (non-distributed) shortest path algorithms. Specifically, we use the following fact well-known in distance oracle constructions and dynamic graph algorithms (e.g. \cite{DemetrescuFI05}): Let $S$ be a set of $\sqrt{n}$ nodes selected uniformly at random. Then, for any pair of nodes $u$ and $v$, a shortest $u$-$v$ path, say $P$, can be partitioned into subpaths $P_1, P_2, \ldots, P_k$ where each subpath $P_i$ contains $\tilde O(\sqrt{n})$ edges and has nodes in $S$ as end nodes, except $P_1$ and $P_k$ that has $u$ and $v$ as end nodes, respectively. In other words, to approximate the distance between $u$ and $v$, it is enough to know the approximate distance between 
%
%
%
%to compute the $(1+o(1))$-approximate distance between a source node $s$ and all other nodes, it is enough to know
%\begin{enumerate}[label=(\arabic{*})]
%\item the $(1+o(1))$-approximate distance between $s$ and all random nodes in $S$, and
%\item 
%\end{enumerate}
%
%
%
%%
%
%
% Using this well-known fact, we can easily conclude the following (see the formal statement and full proof in \Cref{sec:skeleton}).  
%%%
%%\begin{lemma}
%%Let $S$ be a set of $\sqrt{n}$ nodes selected uniformly at random such that the source node $s$ is also in $S$. We can solve \sssp if the followings hold. 
%%\begin{enumerate}[label=(\arabic{*})]
%%\item Every node $v$ knows the $(1+o(1))$-approximate value of $\dist_{G, w}(u, v)$ for all 
%%\end{enumerate}
%%\end{lemma}
%
% 
%
%we use the fact that if we randomly select $\sqrt{n}$ nodes, called {\em centers},then for every pair of nodes $u$ and $v$, 
%
%We note a well-known fact that a random selected of nodes $|V(G')|$ of size $\alpha$ will ``hit'' a simple path of length at least $cn\log n/|V(G')$, for some constant $c$, with high probability. To the best of our knowledge, this fact was first shown in \cite{GreenKnuth81book} and has been used many times in dynamic graph algorithms (e.g. \cite{DemetrescuFI05} and references there in). The following theorem appears as Theorem 36.5 in \cite{DemetrescuFI05} (attributed to \cite{UllmanY91}). 






\section{Overview}\label{sec:techniques}

\subsection{Tool 1: Light-Weight Bounded-Hop \sssp (Details in \Cref{sec:light-weight bounded-hop sssp})} At the core of our algorithms is the {\em light-weight} $(1+o(1))$-approximation algorithm for computing {\em bounded-hop} distances. Informally, an {\em $h$-hop path} is a path containing at most $h$ edges.  The $h$-hop distance between two nodes $u$ and $v$, denoted by $\dist_{G, w}^h(u, v)$, is the minimum weight among all $h$-hop paths between $u$ and $v$. The {\em $h$-hop \sssp problem} is to find the $h$-hop distance between a given source node $s$ and all other nodes. This problem can be solved exactly in $O(h)$ time using the distributed version of Bellman-Ford algorithm. This algorithm is, however, {\em not} suitable for parallelization, i.e. when we want to solve $h$-hop \sssp from $k$ different sources. The reason is that Bellman-Ford algorithm is {\em heavy-weight} in the sense that they require so much communication between each neighboring nodes; in particular, this algorithm may require as many as $O(h)$ messages on each edge. Thus, running $k$ copies of this algorithm in parallel may require as many as $O(hk)$ messages on each edge, which will require $O(hk)$ time. 

We show a simple algorithm that is not as accurate as Bellman-Ford algorithm but more suitable for parallelization: it can $(1+o(1))$-approximate $h$-hop \sssp in $\tilde O(h)$ time and is {\em light-weight} in the sense that every node sends a message (of size $O(\log n)$) to its neighbors only $\tilde O(1)$ times. Thus, when we run $k$ copies of this algorithm in parallel, we will require to send only $\tilde O(k)$ messages through each edge, which gives us a hope that we will require only additional $\tilde O(k)$ time. By a careful paralellization (based on the random delay technique of \cite{LeightonMR94}\footnote{Note that the random delay technique makes the algorithm randomized. Techniques in \cite{HolzerW12,PelegRT12} might enable us to get a deterministic algorithm. We do not discuss these techniques here since other parts of our algorithms will also heavily rely on randomness.}), we can solve $h$-hop \sssp from $k$ sources in $\tilde O(h+k)$ time. This is the first tool that we will use later.
%
\begin{claim}[See \Cref{thm:k-source h-hop sp} for a formal statement]\label{claim:k-source h-hop sp}
We can $(1+o(1))$-approximate $h$-hop \sssp from any $k$ nodes in $\tilde O(h+k)$ time. 
\end{claim}
%
The idea behind \Cref{claim:k-source h-hop sp} is actually very simple. Consider any path $P$ having at most $h$ hops. Let $\epsilon=1/\log n$ and $W'=(1+\epsilon)^i$ where $i$ is such that $W'\leq w(P) \leq (1+\epsilon)W'$ (recall that $w(P)$ is the sum of weights of edges in $P$). Consider changing weight $w$ slightly to $w'$ where $w'(uv)=\lceil \frac{h w(uv)}{\epsilon W'}\rceil$. Because $w'(uv)-\frac{hw(uv)}{\epsilon W'}\leq 1$, we have that  
%
$$w(uv)\leq w'(uv)\times \frac{\epsilon W'}{h} \leq w(uv)+O(\epsilon)\frac{W'}{h}.$$ 
%
It follows that  
$$w(P)\leq w'(P)\times \frac{\epsilon W'}{h} \leq w(P)+ O(\epsilon) W' = (1+o(1))w(P).$$
%
%
%$w'(uv)\times \frac{\epsilon W'}{2h} \in [w(uv), (1+O(\epsilon/h)) w(uv)]$ and thus $w'(P)\times \frac{\epsilon W'}{2h} \in [w(P), (1+O(\epsilon)) w(P)]$. 
%
In other words, it is sufficient for us to find $w'(P)$. To this end, we observe that $w'(P)=O(h/\epsilon)$. Thus, we can simply use the breadth-first search (BFS) algorithm \cite{peleg,Lynch-Book} on $(G, w')$ for $O(h/\epsilon)$ rounds. The BFS algorithm is {\em light-weight}: it sends at most one message through each edge. 
%
Now to use this algorithm to solve $h$-hop \sssp, we have to try different values of $W'$ in the form $(1+\epsilon)^i$. This makes our algorithm send $\tilde O(1)$ messages through each edge.

To the best of our knowledge, this simple technique has not been used before in the literature of distributed algorithms. In the dynamic data structure context, Bernstein has independently used a similar weight rounding technique to construct a {\em bounded-hop data structure}, which plays an important role in his recent breakthrough \cite{Bernstein13}.
%
Also, it was recently pointed out to us by a STOC 2014 reviewer that this technique is similar to the one used in the PRAM algorithm of Klein-Sairam \cite{KleinS92} which was originally proposed for VLSI routing by Raghavan and Thomson \cite{RaghavanT85}.  The main difference between this and our techniques is that we always round edge weights up while the previous technique has to round the weights up and down randomly (with some appropriate probability). So, if we adopt the previous technique, then the approximation guarantee of our light-weight \sssp algorithm will hold only with high probability (in contrast, it always holds in this paper). More importantly, randomly rounding the weight could cause some weight to have a zero weight after rounding. This problem can be handled in the PRAM setting by contracting edges of weight zero. However, this will be a serious problem for us since we do not know how to handle zero edge weight.
%(In fact, we believe that being able to handle zero edge weights is the first step to obtain an exact sublinear-time algorithm, one of the open problems we leave in this paper.)


\subsection{Tool 2: Shortest-Path Diameter Reduction Using Shortcuts (Details in \Cref{sec:spd reduction})} The other crucial idea that we need is the {\em shortest-path diameter reduction technique}. Recall that the shortest-path diameter of a weighted graph $(G, w)$, denoted by $\spdiam(G, w)$, is the minimum number $h$ such that for any nodes $u$ and $v$, there is a shortest $u$-$v$ path in $(G, w)$ having at most $h$ edges; in other words, $\dist_{G, w}^h(u, v)=\dist_{G, w}(u, v)$ for all $u$ and $v$.  
%
As discussed in \Cref{sec:related} there are algorithms that need $\tilde O(\spdiam(G, w))$ time to solve \sssp and \apsp, e.g. Bellman-Ford algorithm. 
%
%For example, if we know that $\spdiam(G, w)\leq \sqrt{n}$, then we can solve \sssp by simply solving $\sqrt{n}$-hop \sssp using either Bellman-Ford or our light-weight \sssp algorithm above. 
%
Thus, it is intuitively important to try to make the shortest-path diameter small. The second crucial tool of our algorithm is the following claim. 
\begin{claim}[See \Cref{thm:spd reduction} for a formal statement]\label{claim:spd reduction}
If we add $k$ edges called {\em shortcuts} from every node $u$ to its $k$ nearest nodes (breaking tie arbitrarily), where for each such node $v$ the shortcut edge $uv$ has weight $\dist_{G, w}(u, v)$, then we can bound the shortest-path diameter to $O(n/k)$.
\end{claim}
%
We note that the above claim would be trivially true if we add a shortcut from every node to all nodes within $h$ hops from it. The non-trivial part is showing that it is sufficient to add shortcuts to only $k$ nearest nodes. Note that this claim holds only for undirected graphs and the proof has to carefully exploit the fact that the network is undirected. 

%We also note that it is {\em not} possible to add edges to distributed networks so we cannot use this claim to directly reduce the shortest-path diameter of the original network; instead, we will use it to add {\em virtual edges} to reduce the shortest-path diameter of a {\em virtual (overlay) network} (which we will discuss next). 


To the best of our knowledge, there is no previous work that proves and uses this fact. In the {\em short-range scheme}, which is part of the algorithm of Lenzen and Patt-Shamir \cite{LenzenP13}, one also has to find the distance to $n^{1/2}$ nearest nodes. However, the purpose of this scheme is not to create shortcuts but to have information to a large number of neighbors to make sure that one of them will be in a set of $n^{1/2}$ random nodes (``skeleton nodes''). 
%
\danupon{Can we improve LZ? No. We don't know how to deal with the case where two nodes are less than $\sqrt{n}$ hops from each other.}  


\subsection{Sketches of Algorithms}

\paragraph{\apsp on General Networks (details in \Cref{sec:sssp})} Algorithm for \apsp follows almost immediately from the the first tool above. By applying \Cref{claim:k-source h-hop sp} with $h=k=n$, we can $(1+o(1))$-approximate \sssp with every node as a source in $\tilde O(n)$ time; in other words, we can $(1+o(1))$-approximate \apsp in $\tilde O(n)$ time on general networks.

\paragraph{\sssp on Fully-Connected Networks (details in \Cref{sec:sssp clique})} This result follows easily from the the second tool above. To compute \sssp exactly on fully-connected networks, we will compute $k$ shortcuts from every node, where $k=n^{1/2}$. To do this, we show that it is enough for every node to send $k$ lightest-weight edges incident to it to all other nodes (since running $k$ rounds of Dijkstra's algorithm will only need these edges). This takes $O(n^{1/2})$ time. 
%(Alternatively, every node can run Dijkstra's algorithm to find $n^{1/2}$ nearest nodes in parallel.) 
%
Using this information to modify the weight assignment from $w$ to $w'$, we can reduce the shortest-path diameter of the network to $\spdiam(G, w')\leq \sqrt{n}$ without changing the distance between nodes; this fact is due to \Cref{claim:spd reduction}. We then run Bellman-Ford algorithm on this $(G, w')$ to solve \sssp; this takes  $\spdiam(G, w')=O(n^{1/2})$ time.

\paragraph{\apsp on Fully-Connected Networks (details in \Cref{sec:apsp clique})} We will need both tools for this result. {\bf Step 1:} Like the previous algorithm for \sssp on fully-connected network, we compute $n^{1/2}$ shortcuts from every node in $O(n^{1/2})$ time. Again, by \Cref{claim:spd reduction}, this gives us a graph $(G, w')$ such that $\spdiam(G, w')=O(n^{1/2})$. Additionally, every node sends these shortcuts to all other nodes (taking $O(n^{1/2})$ time).  
%
{\bf Step 2:} We then randomly pick  $n^{1/2}\poly\log n$ nodes and run the light-weight $h$-hop \sssp algorithm from these nodes, where $h=\spdiam(G, w')=O(n^{1/2})$. By \Cref{claim:k-source h-hop sp}, this takes $\tilde O(n^{1/2})$ time w.h.p. and gives us $(1+o(1))$-approximate values of the distances $\dist_{G, w}(x, v)$ between each random node $x$ and all other nodes $v$ (known by $v$). Each node $v$ broadcasts distances to these $n^{1/2}\poly\log n$ random nodes to all other nodes, taking $\tilde O(n^{1/2})$ time.

After this, we show that every node can use the information they have received so far to compute $(2+o(1))$-approximate values of its distances to all other nodes. (In particular, every node uses the distances it receives to build a graph and uses the distances in such graph as approximate distances between itself and other nodes.)\danupon{Does this also give a $2$-spanner or emulator? That would be weird!!!}
%
To explain the main idea, we show how to prove a $(3+o(1))$ approximation factor instead of $2+o(1)$: Consider any two nodes $u$ and $v$, and let $P$ be a shortest path between them. If $v$ is one of the $n^{1/2}$ nodes nearest to $u$, then $u$ already knows $\dist_{G, w}(u, v)$ from the first step (when we compute shortcuts). Otherwise, by a standard hitting set argument, one of these $n^{1/2}$ nearest nodes must be picked as one of  $n^{1/2}\poly\log n$ random nodes; let $x$ be such a node. Observe that $\dist_{G, w}(u, x)\leq \dist_{G, w}(u, v)$. By triangle inequality 
%
$$\dist_{G, w}(x, v)\leq \dist_{G, w}(x, u)+\dist_{G, w}(u, v) \leq 2\dist_{G, w}(u, v).$$ 
%
Again, by triangle inequality, 
$$\dist_{G, w}(u, v)\leq \dist_{G, w}(u, x)+\dist_{G, w}(x, v) \leq 3\dist_{G, w}(u, v);$$ 
in other words, $\dist_{G, w}(u, x)+\dist_{G, w}(x, v)$ is a $3$-approximate value of $\dist_{G, w}(u, v)$. Note that $u$ knows the exact value of $\dist_{G, w}(u, x)$ (from the first step) and the $(1+o(1))$-approximate value of $\dist_{G, w}(x, v)$ (from the second step). So, it can compute a $(1+o(1))$-approximate value of $\dist_{G, w}(u, x)+\dist_{G, w}(x, v)$  which is a $(3+o(1))$-approximate value of $\dist_{G, w}(u, v)$. Using the same argument, $v$ can also compute a $(3+o(1))$-approximate value of $\dist_{G, w}(u, v)$. To extend this idea to a $(2+o(1))$-approximation algorithm, we use exactly the same algorithm but has to consider a few more cases.


\paragraph{\sssp on General Networks (details in \Cref{sec:sssp})} Approximating \sssp in sublinear time needs both tools above and a few other ideas. First, we let $S$ be a set of $\frac{n^{1/2}}{\diam^{1/4}}\poly\log n$ random nodes and the source $s$. We need the following.
%
\begin{claim}[details in \Cref{sec:overlay}]\label{claim:overlay network is enough}
Let $h=n^{1/2}\diam^{1/4}$. Every node $v$ can compute an approximate distance to $s$ if it knows (i) approximate $h$-hop distances between itself and all nodes in $S$, and (ii) distances between the source $s$ and all nodes in $S$ in the following weighted graph $(G', w')$: nodes in $G'$ are those in $S$, and every edge $uv$ in $G'$ has weight equal to the $h$-hop distance between $u$ and $v$ in $G$.
\end{claim}
We call graph $(G', w')$ an overlay network since it can be viewed as a network sitting on the original network $(G, w)$. The idea of using the overlay network to compute distances is not new. It is a crucial tool in the context of dynamic data structures and distance oracle (e.g. \cite{DemetrescuFI05}). In distributed computing literature, it has appeared (in a slightly different form) in, e.g., \cite{LenzenP13}. 

Our main task is now to achieve (i) and (ii) in \Cref{claim:overlay network is enough}. Achieving (i) is in fact very easy: We simply run our light-weight $h$-hop \sssp from all nodes in $S$. By \Cref{claim:k-source h-hop sp}, this takes time $\tilde O(|S|+h)=\tilde O(n^{1/2}\diam^{1/4})$.\footnote{Note that nodes actually only know $(1+o(1))$ distances. To keep our discussion simple, we will pretend that they know the real distance.} In fact, by doing this we already partly achieve (ii): every node in $S$ already know the $h$-hop distance to all other nodes in $S$, thus it already has a ``local'' perspective in the overlay network $(G', w')$. To finish (ii), it is left to solve \sssp on $(G', w')$. 

To do this, we will first reduce the shortest-path diameter of the overlay network $(G', w')$ by creating $k$ shortcuts, where $k=\diam^{1/2}$. As noted in the \sssp algorithm on fully-connected network, it is enough for every node in $(G', w')$ to send $k$ lightest-weight edges incident to it to all other nodes (since running $k$ rounds of Dijkstra's algorithm will only need these edges). Broadcasting each such edge can be done in $O(\diam)$ time via the breadth-first search tree, and broadcasting all $k|S|=\tilde O(n^{1/2}\diam^{1/4})$ edges takes $\tilde O(n^{1/2}\diam^{1/4}+\diam)$ time by pipelining. (See details in \Cref{sec:reduce spd overlay}.) Let $(G'', w'')$ be an overlay network obtained from adding $k$ shortcuts to $(G', w')$. (As usual, nodes $u$ in $(G'', w'')$ only know weights $w''(uv)$ of edges $uv$ incident to it.) By \Cref{claim:spd reduction}, $\spdiam(G'', w'') = O(|S|/k) = \tilde O(n^{1/2}/\diam^{3/4})$.
%
Finally, we simulate our light-weight $h'$-hop \sssp algorithm to solve \sssp from source $s$ on overlay $(G'', w'')$, where $h'=\spdiam(G'', w'') = \tilde O(n^{1/2}/\diam^{3/4})$. To do this efficiently, we need a slightly stronger property of our light-weight $h'$-hop \sssp algorithm: recall that we have claimed that in our light-weight \sssp algorithm, each node sends a message through each edge only $\tilde O(1)$ times. In fact, we can show the following stronger claim.
%
\begin{claim}[details in \Cref{thm:light-weight sssp}]\label{claim:light-weight sssp broadcast}
In the light-weight \sssp algorithm, each node communicates in each round by {\em broadcasting} the same message to its neighbors. Moreover, each node broadcasts messages only for $\tilde O(1)$ times.
\end{claim}
%
The intuition behind the above claim is simple: at the heart of our light-weight \sssp algorithm, we solve $\tilde O(1)$ breadth-first search algorithms where, for each of these algorithms, each node broadcasts only once; it broadcasts its distance to the root, say $d$, at time $d$.
%
Now we simulate our light-weight \sssp algorithm on $(G'', w'')$ as follows. When each node $v$ wants to broadcast a message to all its neighbors in $G''$, we broadcast this message to all nodes in $G$, using the breadth-first search tree of $G$ (see details in \Cref{sec:sssp overlay}). 
%
This takes $O(\diam)$ time. If we want to broadcast $M_i$ messages in a round $i$ of our light-weight \sssp algorithm, we can do so in $O(\diam+M_i)$ time by pipelining. It can then be shown that the time we need to simulate all $r=\tilde O(h')=\tilde O(n^{1/2}/\diam^{3/4})$ rounds of our light-weight $h'$-hop \sssp algorithm takes $\tilde O(\diam h' +\sum_{i=1}^{r} M_i) = \tilde O(n^{1/2}\diam^{1/4} + \diam)$ (note that $\sum_{i=1}^{r} M_i = \tilde O(|S|)$ by \Cref{claim:light-weight sssp broadcast}). (See details in \Cref{sec:sssp time analysis}.) This completes (ii) in \Cref{claim:overlay network is enough}, and thus we can solve \sssp on $(G, w)$ in $\tilde O(n^{1/2}\diam^{1/4}+\diam)$ time. 


\endinput


\section{Introduction (STOC version)}

%************************************************************************************
%************************************************************************************
% Previous introduction from STOC
%************************************************************************************
%************************************************************************************

%From Lynch's book: As for breadth-first search, the motivation for constructing such a tree comes  from the desire to have a convenient structure to use for broadcast communication. The weights represent costs that may be associated with the traversal  of edges, for instance, communication delay or a monetary charge. A shortest paths tree minimizes the maximum worst-case cost of communicating with any process in the network. 

% From Santoro:  Protocol IteratedConstruction is the distributed version of Bellman’s sequential algorithm designed by Lestor Ford and D. Fulkerson [13]; from the start it has been the main routing algorithm in the Internet

The all-pairs shortest paths problem (\apsp) is one of the most fundamental problems in computer science. It has appeared in an uncountable number of applications.
%
%: finding driving directions, routing information on the internet, etc. 
%
{\em Distributed networks} is among many places that this problem has been extensively studied since its early days. For example, as early as 1969, \apsp algorithms were repeatedly executed in the ARPANET and in other networks \cite{Lynch-Book,AfekR93,MRR80,Santoro-book}. %the distributed version of Bellman-Ford algorithm were already used as early as 1969 in the ARPANET \cite[p.506]{Lynch-Book}
Computing \apsp, especially on large networks, has been an important primitive in network applications such as routing and load balancing and has motivated the studies of many subareas of theoretical computer science, in both sequential and distributed settings, including metric embeddings, distance labelings, spanners, and distance oracles.
%
%Several subareas of theoretical research have emerged centered around \apsp, in both sequential and distributed settings, such as metric embeddings, distance labelings, spanners, and distance oracles.
%
% Note: ARPANET is from HolzerW's PODC'12. Routing+Load Balancing is from DasSarma et al. SPAA'12.
%
Despite its importance and practical relevance, the basic issue of {\em time complexity} of this problem on distributed networks remains essentially unknown. We focus on exactly this problem.
%
%
%not much is known about the basic issue of {\em time-complexity} of this problem on distributed networks, especially in the general {\em weighted} case. This paper studies exactly this problem.


%The problem has been studied extensively in this setting (e.g. \cite{AfekR93,AntonioHT92,CiceroneDSFM10,Elkin05,FrischknechtHW12,Haldar97,HolzerW12,KavithaLMMRUZ09,Segall83}).
%
%However, despite its importance and practical relevance, not much is known about the basic issue of {\em time-complexity} of this problem on distributed networks, especially in the general {\em weighted} case. This paper studies exactly this problem.


%\paragraph{Distributed Networks}

%\paragraph{Model \& Problem} 

\subsection{Distributed Computing Model}\label{subsec:model}

%\medskip\noindent 

We study the time complexity of solving weighted \apsp on the standard synchronous
%bandwidth-constrained point-to-point communication system called 
\congest model. It is one of the major models in the study of (locality-sensitive) distributed computation \cite{peleg}.%, especially in studying time complexity of (locality-sensitive) distributed computing \cite{peleg}.

Consider a synchronous  network of processors  modeled by an undirected $n$-node $m$-edge graph $G$, where nodes model the processors and  edges model the {\em bounded-bandwidth} links between the processors. The processors  (henceforth, nodes) are assumed to have unique IDs in the range of $\{1, \ldots, \poly(n)\}$ and infinite computational power. Each node has limited topological knowledge; in particular, it only knows the IDs of its neighbors and knows {\em no} other topological information (e.g., whether its neighbors are linked by an edge or not). Nodes may also accept some additional inputs as specified by the problem at hand.

Despite having only local knowledge, nodes may have to compute (cooperatively) some global function of the network, such as a minimum spanning tree or all-pairs shortest paths, via communicating with each other and running a distributed algorithm designed for the task at hand. 
%
The communication is synchronous, and occurs in discrete pulses, called {\em rounds}. All the nodes wake up simultaneously at the beginning of each round. In each round each node $u$ is allowed to send an arbitrary message of  $O(\log n)$ bits through each edge $e = uv$ that is adjacent to $u$, and the message will arrive to $v$ at the end of the current round. For convenience, our algorithms assume that nodes always know the number of the current round. 
%
There are several measures to analyze the performance of such algorithms, a fundamental one being the {\em running time}, defined as the worst-case number of rounds of distributed communication


\smallskip For example, consider {\em graph problems} where nodes are given {\em edge weights} as an additional input: each edge $e$ is assigned a weight $w(e)$ which is {\em known only to nodes incident to it}. As commonly done in the literature (e.g., \cite{KhanP08,LotkerPR09,KuttenP98,GarayKP98}), we will assume that the maximum weight is $\poly(n)$; so, each edge weight can be sent through an edge (link) in one round.
%
%his assumption we will exploited to obtain efficient algorithms.

Trivially, {\em all} graph problems can be solved in $O(m+n)$ rounds: Aggregate all $m$ edges and their weights into one node (this can be done in $O(m+n)$ communication rounds). Then, such node can solve any graph problem for {\em free} (since nodes have unlimited computation power).
%
%by aggregating all edge weights into one node, which can then perform a local computation for free.
%, since nodes are assumed to have an unlimited computational power.
Of course, this is neither interesting nor satisfiable. 

Fortunately, in the last few decades many graph problems on distributed networks have been found to be solvable in a more exciting and non-trivial way, e.g. a maximal independent set in $O(\log n)$ time~\cite{Luby86,KuhnMW-jacm} and a minimum spanning tree in sub-linear time~\cite{KuttenP98,GarayKP98}.
%
It is surprising that, despite so much progress and extensive research on this topic for decades, not much is known about a fundamental problem like \apsp.

%In the last few decades, extensive studies of graph problems on distributed networks have resulted in many surprising results, showing that many problems can be solved in a non-trivial way, e.g. a maximal independent set in $O(\log n)$ time~\cite{Luby86,KuhnMW-jacm} and a minimum spanning tree in sub-linear time~\cite{KuttenP98,GarayKP98}. 
%
%Despite so much progress on this topic, it is surprising that not much is known about a fundamental problem like \apsp.


\subsection{Problems \& Definitions}
%To avoid confusion, we note the notations we use here. 
%%We use an undirected unweighted graph $G$ to denote the input distributed network. 

%Let us first define the notion of {\em distance}, {\em diameter} and {\em radius} on networks whose weight function could be {\em symmetric} or {\em asymmetric}.

We use an undirected unweighted graph $G$ to represent the underlying network. Let $V(G)$ and $E(G)$ denote the set of nodes and edges of $G$, respectively. As mentioned in Section~\ref{subsec:model}, nodes have unique IDs in the range of $\{1, \ldots, \poly(n)\}$. To simplify notations, we will name nodes using their IDs, i.e. we let $V(G)\subseteq \{1, \ldots, \poly(n)\}$. Thus, we use $u\in V(G)$ to represent a node, as well as its ID. 

Let $w:E(G)\rightarrow \{1, 2, \ldots, \poly(n)\}$ be the edge weight assignment. We refer to network $G$ with weight assignment $w$ as the {\em weighted network}, denoted by $(G, w)$.  Our main problem is as follows.
%
\begin{definition}\label{def:apsp} {\sc (Apsp)}
In the all-pairs shortest paths problem (\apsp), we are given a weighted network $(G, w)$ as above and want to, for every pair $(u, v)$ of nodes, find the distance between $u$ and $v$ in $(G, w)$, denoted by $\dist_{G, w}(u, v)$. In particular, we want both $u$ and $v$ to know $\dist_{G, w}(u, v)$.\footnote{We emphasize that we do {\em not} require every node to know the distances between {\em all} pairs of nodes. 
%This is because it is not necessary in most applications and will make the problem uninteresting. 
Also note that, while our paper focuses on computing distances between all pairs of nodes, it can be used to compute a routing table in $O(n)$ time as well: Nodes can exchange all distance information with their neighbors in $O(n)$ time. Then, when a node $u$ wants to send a message to node $s$, it simply sends such message to the neighbor $v$ with smallest $\dist_{G, w}(u, v)$.}
\end{definition}
%
For any $\alpha$, we say an algorithm $\cA$ {\em $\alpha$-approximates} \apsp if it outputs $\tilde \dist_{G, w}$ such that $\dist_{G, w}(u, v) \leq \tilde \dist_{G, w}(u, v)\leq \alpha\dist_{G, w}(u, v)$ for all $u$ and $v$. 

We now formally define terms we need (including $\dist_{G, w}$). In particular, we define {\em distance}, {\em diameter} and {\em radius} on networks whose weight assignment could be {\em symmetric} or {\em asymmetric}.

\paragraph{Asymmetric Weight Assignment}
We note that our input weighted network $(G, w)$ is always {\em symmetric} in the sense that the cost of going from $u$ to $v$ through edge $uv$ is the same as the cost of going from $v$ to $u$ through the same edge; i.e. $w(uv)=w(vu)$.
%
%In this case, we say that $w$ is {\em symmetric} (since its adjacency matrix is symmetric).
%
While our input weight assignment is always symmetric, during the course of our algorithm we will have to deal with a more general weight assignment $\vec w'$ that is {\em asymmetric}; i.e. it is possible that $\vec w'(uv)\neq \vec w'(vu)$ for some edge $uv$. We will put an arrow above $\vec w'$ to emphasize that it is asymmetric. Note that the class of asymmetric assignments also includes symmetric assignments.\danupon{Is it weird to use asymmetric like this?} Also note that the underlying network $G$ is always undirected.

%Note that the underlying network is always undirected.

%solve a problem on some network $(G', \vec w')$ where $\vec w'$ is {\em asymmetric}; i.e. it is possible that $\vec w'(uv)\neq \vec w'(vu)$ for some edge $uv$. We put an arrow above $\vec w'$ to emphasize that it is asymmetric. Note that the underlying network $G'$ is always undirected, and 

\paragraph{Distance, Diameter, and Radius}\footnote{For other related terms, such as  girth, center, and peripheral vertices, see \cite{HolzerW12}.}
For any node $u$ and $v$, a {\em $u$-$v$ path} $P$ is a path $\langle u=x_0, x_1, \ldots, x_\ell=v\rangle$ where $x_ix_{i+1}\in E(G)$ for all $i$. For any (possibly asymmetric) weight function $\vec w$, we define the weight or distnace of $P$ as $\vec w(P)=\sum_{i=0}^{\ell-1} \vec w(x_ix_{i+1})$. Let $\cP_G(u,v)$ denote the set of all $u$-$v$ paths in $G$. We use $\dist_{G, \vec w}(u, v)$ to denote the distance from $u$ to $v$ in $(G, \vec w)$; i.e., $\dist_{G, \vec w}(u, v)=\min_{P\in \cP_G(u, v)} \vec w(P)$. We say that a path $P$ is a {\em shortest $u$-$v$ path} in $(G, \vec w)$ if $\vec w(P)=\dist_{G, \vec w}(u, v)$.
%
The {\em diameter} of $(G, \vec w)$ is $D(G, \vec w)=\max_{u, v} \dist_{G, \vec w}(u, v)$. The {\em radius} of $(G, \vec w)$ is $\rad(G, \vec w)$ $=\min_u$ $\max_v$ $\dist_{G, \vec w}(u, v)$. 
%We will note need the definitions of girth, center, and peripheral vertices in this paper.
%We defer the definitions of {\em girth}, {\em center} and {\em peripheral vertices} to Appendix.\selfnote{Do this!!!}

When we want to talk about the properties of the underlying undirected unweighted network $G$, we will drop $\vec w$ from the notations. Thus, $\dist_G(u, v)$ is the distance between $u$ and $v$ in $G$ and,  $\diam(G)$ and $\rad(G)$ are the diameter and radius of $G$, respectively. Besides \apsp, this paper considers the following problems.

\vspace{-.05in}\begin{definition}[Computing Diameter and Radius]\label{def:diameter radius}
In the diameter and radius computation problem on weighted network $(G, w)$, we want every node to know $\diam(G, w)$ and $\rad(G, w)$, respectively. An $\alpha$-approximation algorithm is an algorithm that outputs $\tilde \diam(G, w)$ and $\tilde \rad(G, w)$ such that  $\diam(G, w)\leq \tilde \diam(G, w)\leq \alpha \diam(G, w)$ and  $ \rad(G, w)\leq \tilde \rad(G, w)\leq \alpha \rad(G, w)$. 
\end{definition}





%For any path $P=\langle x_0, x_1, \ldots, x_\ell\rangle$ from node $x_0$ to node $x_\ell$, we let $w(P)$ be the length of this path; i.e., $w(P)=\sum_{i=0}^{\ell-1} w(x_$.



\begin{comment}
\begin{figure}
\small
\begin{tabular}{|c|c|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  $G$ & Distributed network\\
  \small $V(G)$, $n$ & \small Set of nodes in $G$ and $n=|V(G)|$\\
  \small $(G, w)$ & \small Weighted distributed network (Sec~XXX)\\
  \small $\dist_{G, w}(u, v)$ & \small  Distance between $u$ and $v$ in $G$ (Sec~XXX) \\
  \small $D(G, w)$ & \small  Weighted diameter of $(G, w)$ (Sec~XXX)\\
  \small $\spd(G, w)$ & \small Shortest path diameter of $(G, w)$ (Sec~XXX) \\
  \small $\ecc(G, \cW)$ & \small Multi-Weight diameter of $(G, \cW)$ (Sec~XXX)\\
  \hline
  \apsp & \small All-Pairs Shortest Path Problem (Sec~XXX)\\
  \small $K$-\apsp & \small  Bounded-Distance All-Pairs \\
  & \small Shortest Path Problem (Sec~XXX)\\
%  $\cS$-\ksp & $\cS$-Source Shortest Path Problem (Sec~XXX)\\
%  $\cS$-\asp & $\cS$-Source Almost Shortest Path Problem (Sec~XXX)\\
  \small $(\cS, K)$-\ksp & \small Bounded-Distance $\cS$-Source \\
  & \small  Shortest Path Problem (Sec~XXX)\\
  \small $(\cS, K)$-\asp & \small Bounded-Distance $\cS$-Source\\
  & \small Almost Shortest Path Problem (Sec~XXX)\\
  \hline
\end{tabular}
\caption{Notations}\label{fig:notation}
\end{figure}
\end{comment}

\subsection{Our Results}

We show fast algorithms for computing \apsp and related problems. 
%
Our first result is a randomized (Las Vegas) distributed algorithm that solves \apsp {\em exactly} in $O(n\sqrt{n}\log^2 n)$ time.
%
\begin{theorem}\label{theorem:exact}
There is a distributed algorithm that solves \apsp on any weighted $n$-node network $(G, w)$ which finishes in  $O(n\sqrt{n}\log^2 n)$ time with high probability.
\end{theorem}
%
To the best of our knowledge, this is the {\em first} non-trivial algorithm for solving \apsp exactly. (Previously, the best way is to aggregating the whole network topology at one node in $O(m)$ time.)%(Running multiple single-source shortest path algorithms in parallel takes more ($O(n^2)$) time.)

Next, we show that if approximation is allowed, then we can solve \apsp using a deterministic linear-time {\em approximation scheme}; i.e., the approximation ratio can be arbitrarily close to $1$:
%
\begin{theorem}\label{theorem:approx apsp}
For any $\epsilon>0$, there is a distributed algorithm that $(1+\epsilon)$-approximates \apsp on any weighted $n$-node network $(G, w)$ in  $O((1+\frac{1}{\epsilon})n\log n)$ time.
\end{theorem}
%
The above algorithm improves previous algorithms based on {\em low-distortion sparse embeddings} (e.g. \cite{Elkin05,DasSarmaHKKNPPW11,BaswanaS07,DerbelGPV08,Pettie10,KhanKMPT12}) in both approximation guarantee and running time\footnote{We note that the improved running time comes with the cost of higher message complexity} (see Section~\ref{sec:related} for more detail). To the best of our knowledge, the above algorithm is the first one that solves weighted \apsp without finding an embedding.
%
Moreover, it is only $O(\log n)$ times slower than the best algorithms for the unweighted case \cite{HolzerW12,PelegRT12}.
%
We also observe the following lower bounds.
%
%\begin{observation}\label{observe:lower bound}
%For any $n$ and $\alpha(n)= \poly(n)$, any $\alpha(n)$-approximation algorithm for \apsp on an $n$-node weighted network $G$ requires $\Omega(\frac{n}{\log n})$ time. This lower bound holds even when the underlying network $G$ has diameter $\diam(G)=2$.
%
%Moreover, for any $\alpha(n)=O(n)$, any $\alpha(n)$-approximation algorithm on an {\em unweighted} network requires $\Omega(\frac{n}{\alpha(n)\log n})$ time. 
%%
%\end{observation}
%
\begin{observation}\label{observe:lower bound}
Any $\poly(n)$-approximation algorithm for \apsp on an $n$-node weighted network $G$ requires $\Omega(\frac{n}{\log n})$ time. This lower bound holds even when the underlying network $G$ has diameter $\diam(G)=2$.
%
Moreover, for any $\alpha(n)=O(n)$, any $\alpha(n)$-approximation algorithm on an {\em unweighted} network requires $\Omega(\frac{n}{\alpha(n)\log n})$ time. 
%
\end{observation}
%
Observation~\ref{observe:lower bound} implies that the running time of our algorithm in Theorem~\ref{theorem:approx apsp} is {\em tight} up to a $\poly\log n$ factor, unless we allow a prohibitively large approximation factor of $\poly n$. Moreover, even when we restrict ourselves to unweighted networks, we still cannot significantly improve the running time, unless the approximation ratio is fairly large; e.g., any $n^{1-\delta}$-time algorithm must allow an approximation ratio of $\Omega(n^\delta/\log n)$.


%Thus, even when we want to solve \apsp on an unweighted network and allow a $\poly\log n$ approximation factor, we still need $\tilde \Omega(n)$ time to solve \apsp. In other words, the running time of our approximation in \ref{theorem:approx apsp} is {\em tight} unless we are willing to 

Note that, by using simple reductions from \cite[Section 4.2]{HolzerW12}, our \apsp algorithms can be turned into algorithms with the same running time for computing or approximating other related quantities, such as diameter, girth, radius, center and peripheral vertices (see \cite{HolzerW12} for details). However, for the case of approximating diameter and girth, we observe that one can do slightly better than Theorem~\ref{theorem:approx apsp}.
%
\begin{theorem}\label{theorem:diameter girth}
For any $\epsilon>0$, there are deterministic $(1+\epsilon)$-approximation $O((1+\frac{1}{\epsilon})n)$-time algorithms for diameter and girth computation. 
\end{theorem}
Algorithms in the above theorem have exactly the same running time with the best algorithms in the unweighted case \cite{HolzerW12,PelegRT12}. Moreover, their running time is {\em tight} among algorithms that guarantee a small approximation ratio: due to \cite{HolzerW12}, for any $\delta>0$, any $(1.5-\delta)$-approximation algorithm for diameter and girth computation requires $\Omega(n/\log n)$ time, even in the {\em unweighted} case.

\subsection{Related Work}\label{sec:related}

%While distributed \apsp has been extensively studied for several decades, early 

While \apsp is among the earliest studied problems in distributed computing, many classic works on this problem concern other objectives, such as the message complexity and convergence. When faced with the bandwidth constraint, the time complexities of these algorithms become higher than the trivial $O(m)$-time algorithm; e.g., algorithms in \cite{AbramR82,Haldar97,AfekR93} require $\Omega(n^2)$ time.
%\selfnote{Don't know where to put this: Other than this, the problem can be solved in $O(n)$ time on a weighted asynchronous network \cite{KanchiV04}. This algorithm cannot be used in the \congest model since it involves using large messages.}


%Algorithms from these works are not time-efficient when face with the bandwidth constraint since they either takes too much time or involve sending a large messages.  For example, algorithms in \cite{AbramR82,Haldar97,AfekR93} require $\Omega(n^2)$ time, which is worse than the trivial algorithm, and ...

%The time complexity of algorithms in these works are usually higher than the trivial $O(m)$-time algorithm. For example, algorithms in \cite{AbramR82,Haldar97,AfekR93} require $\Omega(n^2)$ time.

%, and \cite{AbramR78,Chen82}
%
%The problem is also considered in many other models, such as the sequential and PRAM models. These algorithms are not suitable for the distributed setting.


%\paragraph{Other Work} There are many distributed algorithms that focus on the message complexity of computing \apsp. The time complexity of these algorithms are usually higher than the trivial $O(m)$-time algorithm; for example, algorithms in \cite{Haldar97} and \cite{AfekR93} have $\Omega(n^2)$ time. The problem is also considered in many other models, such as the sequential and PRAM models. These results are generally irrelevant to this paper and will not be discussed here.

%Time-efficient algorithms studied extensively recently are based on the idea of {\em approximation} via {\em low-distortion sparse embeddings}.
%
%More recent works that are more time-efficient are {\em approximation algorithms} based on {\em low-distortion sparse embeddings}\footnote{We note that some of these algorithms (e.g., \cite{Elkin05,KhanKMPT12}) can actually solve the {\em $\cS$-shortest path} problem, which generalizes \apsp. To avoid confusion, we will focus only on \apsp.}.

More recent and more time-efficient algorithms are based on the idea of {\em approximation} via {\em low-distortion sparse embeddings}.
%
These algorithms\footnote{We note that some of these algorithms (e.g., \cite{Elkin05,KhanKMPT12}) can actually solve a more general problem called the {\em $\cS$-shortest path} problem. To avoid confusions, we will focus only on \apsp.} have either super-linear time or large approximation guarantees.
%(but sometimes with a better message complexity than our algorithms). 
%
%\selfnote{Say this in "our resutls": To the best of our knowledge, our approximation algorithms are the first ones that solve weighted \apsp without finding an embedding. ...And the first linear-time approximation algorithm.}
%
For example, \cite{Elkin05} presents an algorithm for the unweighted case based on a sparse spanner that takes (very roughly) $O(n^{1+\xi})$ time and gives $(1+\epsilon)$-approximate solution, for small constants $\xi$ and $\epsilon$. The algorithm is also extended to the weighted case but both running time and approximation guarantee are large (linear in terms of the largest edge weight).
%
%COMPARE For example, \cite{Elkin05} presents an algorithm based on a sparse spanner. In the unweighted case, this algorithm has a running time of $O(nD(G) + n^{1+\xi/2})$ and guarantees a $(1+\epsilon)$ multiplicative approximation and $\beta(\xi, \rho, \epsilon)$ is constant when $\xi$, $\rho$ and $\epsilon$ are. This algorithm is also extended to an $O(w_{max}\cdot n^{1+\zeta/2}+n\cdot D(G))$-time algorithm for the weighted case, for an arbitrarily small $\zeta$ and where $w_{max}$ is the maximum edge weight. This algorithm is quite inefficient as it has a pseudo-polynomial running time and also has $w_{max}$ in its additive error.
%
%
%which can be used to solve \apsp in $O(XXX)$ and   in the unweighted and weighted case, respectively.
%
%There are many approximation algorithms for \apsp based on 
%
The running time could be traded-off with the approximation guarantee using, e.g., a $(2k-1)$-spanner of size $O(kn^{1+1/k})$ \cite{BaswanaS07} where $k$ can vary; e.g., by setting $k=\log n/\log\log n$, we have an $O(n\log n)$-time $O(\log n/\log \log n)$-approximation algorithm. The spanner of \cite{Pettie10} can also be used to get a linear-time $(2^{O(\log^*{n})}\log n)$-approximation algorithm in the unweighted case.
%\danupon{Note: \cite{DerbelGPV08} is deterministic but work only on unweighted graphs while \cite{BaswanaS07} is randomized but works on weighted graphs}
%
%or low-stretch distance sketches~\cite{ThorupZ05,DasSarmaDP12}

There are also some approximation algorithms whose running time is based on other parameters. These algorithms do not give any improvement for the worst values of their parameters. For example, \cite{KhanKMPT12} gives an  $O(nS\log n)$-time $O(\log n)$-approximation algorithm via {\em metric tree embeddings}~\cite{FakcharoenpholRT04}, where $S$ is the  {\em shortest path diameter}. Since $S$ can be as large as $n$, this algorithm has $O(n^2\log n)$ time in the worst case. We can also construct {\em Thorup-Zwick distance sketches}~\cite{ThorupZ05} of size $O(kn^{1/k})$ and stretch $2k-1$ in $O(kn^{1/k}S\log n)$ time~\cite{DasSarmaDP12}. For the worst value of $S$, this algorithm has the same performance as when we use the spanner of \cite{BaswanaS07}.
%
Another shortest path algorithm with running time based on the network's {\em local path diameter} is developed as a subroutine of the approximation algorithm for MST \cite{KhanP08}. This algorithm solves a slightly different problem (in particular, nodes only have to know the distance to some nearby nodes) and cannot be used to solve \apsp.

%***\danupon{I think the algorithm in this paper can be used to $(1+\epsilon)$ approximate their problem. Would this give any better MST approximation? Answer: No.}\danupon{Also, should we say that if S and L are known then our running time could be reduced?}

%A better algorithm is to use the randomized algorithm of \cite{BaswanaS07} to compute a $(2k-1)$-spanner of size $O(kn^{1+1/k})$ in $O(k^2)$ time, for any $k$, and then aggregate the spanner in one node. For example, for $k=\log n/\log\log n$, we get an $O(\log n/\log\log n)$-approximation $O(n\log n)$-time algorithm for \apsp.

%There are also algorithms whose running time based on other parameters. Using the distributed version of {\em metric tree embeddings}~\cite{FakcharoenpholRT04}, an $O(nS\log n)$-time $O(\log n)$-approximation algorithm is shown in \cite{KhanKMPT12}, where $S$ is the network parameter called {\em shortest path diameter}. Since $S$ can be as large as $n$, this algorithm has $O(n^2\log n)$ time in the worst case.
%
%The authors of \cite{DasSarmaDP12} show a distributed algorithm that constructs {\em Thorup-Zwick distance sketches}~\cite{ThorupZ05} of size $O(kn^{1/k})$ and stretch $2k-1$ in $O(kn^{1/k}S\log n)$ time. For the worst value of $S$, this algorithm has the same performance as when we use the spanner of \cite{BaswanaS07}.

%Another shortest path algorithm with running time based on a network's {\em local path diameter} is developed as a subroutine of the approximate MST algorithm in \cite{KhanP08}. This algorithm solves a slightly different problem (in particular, nodes only have to know the distance to some nearby nodes) and cannot be used to solve \apsp.\danupon{I think the algorithm in this paper can be used to $(1+\epsilon)$ approximate their problem. Would this give any better MST approximation? Answer: No.}\danupon{Also, should we say that if S and L are known then our running time could be reduced?}

\medskip Very recent work \cite{FrischknechtHW12,HolzerW12,PelegRT12} has made much progress in understanding distributed algorithms for \apsp in the {\em unweigthed} case. \cite{FrischknechtHW12} shows a (surprising) lower bound of $\Omega(n/\log n)$ for \apsp and computing the diameter on unweighted networks. This holds even for $(3/2-\epsilon)$-approximation algorithms~\cite{HolzerW12}. This lower bound is matched (up to a $\poly\log n$ factor) by  $O(n)$-time deterministic {\em exact} algorithms for unweighted \apsp found independently by \cite{HolzerW12} and \cite{PelegRT12}.
%\selfnote{Will mention $\cS$-Shortest Path in overview only.}

To the best of our knowledge, there is still no exact distributed algorithm for \apsp that is faster than the trivial $O(m)$-time algorithm\footnote{The problem can also be solved by running the distributed version of Bellman-Ford algorithm \cite{peleg,Lynch-Book,Santoro-book} from every node, but this takes $O(n^2)$ time in the worst case. So this is always worse than the trivial algorithm.}, except for the special case of {\em BHC network}, whose topology is structured as a balanced hierarchy of clusters. In this special case, the problem can be solved in $O(n \log n)$-time \cite{AntonioHT92}. The lower bound of \cite{DasSarmaHKKNPPW11} (building on \cite{Elkin06,PelegR00}) shows that solving \sssp requires $\tilde \Omega(\sqrt{n}+D(G))$ time, even when we allow $\poly(n)$ approximation ratio. This implies the same lower bound for \apsp. Recently, \cite{ElkinKNP12} extends the results of \cite{DasSarmaDP12} to the quantum setting. Thus, the same $\tilde \Omega(\sqrt{n})$ lower bound holds even in the quantum setting. These lower bounds are subsumed by Observation~\ref{observe:lower bound}.

%Our simple observation in Section~\ref{sec:results} subsumes all previous lower bounds completely for the case of weighted \apsp (but not for unweighted \apsp or diameter and girth computation).

%\danupon{Say this in "our results" section: Our simple lower bound presented in Appendix~\ref{sec:lower bound} subsumes all previous lower bounds completely for the case of weighted \apsp (but not for unweighted \apsp or diameter and girth computation).}

For the related problem of computing network's diameter and girth, many results are known in the unweighted case but none is previously known for the weighted case. \cite{PelegRT12} shows that we can $\frac{3}{2}$-approximate the network's diameter in $O(D(G)\sqrt{n})$ time, in the unweighted case, and \cite{HolzerW12} presents an $O(\frac{n}{D(G)}+D(G))$-time $(1+\epsilon)$-approximation algorithm. By combining both algorithms, we get a $\frac{3}{2}$-approximation  $O(n^{3/4}+D(G))$-time algorithm.
%$O(\min\{D(G)\sqrt{n}, n/D(G)+D(G)\})=O(n^{3/4}+D(G))$. 
In contrast, any $(\frac{3}{2}-\epsilon)$-approximation and $(2-\epsilon)$-approximation algorithm for computing the network's diameter and girth, respectively, requires  $\Omega(n/\log n)$ time~\cite{HolzerW12}
%\danupon{Lemma 11 Section 7.1.} 
and $\Omega(\sqrt{n}/\log n)$ time~\cite{FrischknechtHW12}, respectively. These bounds imply the same lower bound for approximation algorithms for \apsp on unweighted networks. In particular, they imply that our approximation algorithms are tight, even on unweighted networks.
%
%the same approximation factor of any algorithm for approximating \apsp on unweighted networks.\danupon{Say this in "our results": These lower bounds imply that our approximation algorithms are tight, even on unweighted networks.}
%\selfnote{So far I don't see any lower bound of $(2-\epsilon)$-approx algo. In \cite{FrischknechtHW12}, the lower bound of $\sqrt{n}$ is shown for GIRTH approximation.}



%A trivial algorithm to solve \apsp is by aggregating the whole network topology into one node and solve \apsp internally (for free) in such node. This takes $O(m)$ time, where $m$ is the number of edges. To the best of our knowledge, this is still the best exact algorithm for \apsp in the general case\footnote{The problem can also be solved by running the distributed version of Bellman-Ford algorithm \cite{peleg} from every node but this takes $O(n^2)$ time in the worst case, thus always worse than the trivial algorithm.}
%%
%%Yet another algorithm is to convert a weighted network to a $nw_{max}$-node unweighted one, where $w_{max}$ is the largest edge weight, by replacing an edge of weight $w$ to a path of $w$ nodes. We can then run the algorithms for the unweighted case.
%%
%For the special case of {\em BHC network}, whose topology is structured as a balanced hierarchy of clusters, the problem can be solved in $O(n \log n)$-time \cite{AntonioHT92}. Other than this, the problem can be solved in $O(n)$ time on a weighted asynchronous network \cite{KanchiV04}. This algorithm cannot be used in the \congest model since it involves using large messages.

%Tight $O(n)$-time deterministic {\em exact} algorithms for unweighted \apsp are later presented independently by 


%\paragraph{Unweighted APSP} The problem is well understood in the unweighted case. The (rather surprising) lower bound of $\Omega(n/\log n)$ has been recently found \cite{FrischknechtHW12}. More recently, a tight $O(n)$-time deterministic algorithm for \apsp is found independently by \cite{HolzerW12} and \cite{PelegRT12}. In \cite{HolzerW12}, a more general problem called $\cS$-Shortest Path (also known as $k$-source shortest path \cite{Elkin05,KhanKMPT12}) is also solved in $O(n)$-time algorithm. Our $O(n)$-time deterministic approximation algorithms for weighted \apsp are based on the ideas of these algorithm.

%An earlier work for unweighted \apsp includes an approximation algorithm by Elkin \cite{Elkin05} using spanners\footnote{In fact, the problem of $\cS$-source shortest path is solved in \cite{Elkin05}}. It has a super-linear running time and gives only an approximated solution, but has better message complexity than \cite{HolzerW12} and \cite{FrischknechtHW12}. The spanner of \cite{Pettie10} can also be used to give a $2^{O(\log^*{n})}\log n$-approximation in linear time.

%The spanners of \cite{BaswanaS07} and \cite{DerbelGPV08} can also be used to give a $(2k-1)$-approximate solution within $O(n^{1+1/k})$ time, for any $k$.\danupon{Removed this since Derbel et al. uses unbounded-length message (mentioned in Pettie DiscComp08.}
%
%If we allow approximation, we can do faster. \cite{PelegRT12} shows how to $3/2$-approximate the network's diameter in $(D(G)\sqrt{n})$ time. \cite{HolzerW12} presents an $O(n/D(G)+D(G))$-time $(1+\epsilon)$-approximation algorithm. By combining both algorithms, we get a $3/2$-approximation algorithm that runs in time $O(\min\{D(G)\sqrt{n}, n/D(G)+D(G)\})=O(n^{3/4}+D(G))$.

% The best approximation algorithm seems to be the combination of the $(D(G)\sqrt{n})$-time $3/2$-approximate algorithm of \cite{PelegRT12} and the $O(n/D+D)$-time $(1+\epsilon)$-approximation algorithm of \cite{HolzerW12},

%\cite{PelegRT12} shows how to $3/2$-approximate the network's diameter in $(D(G)\sqrt{n})$ time.


%\paragraph{Weighted APSP} A trivial algorithm to solve \apsp is by aggregating the whole network topology into one node and solve \apsp internally (for free) in such node. This takes $O(m)$ time, where $m$ is the number of edges. To the best of our knowledge, this is still the best exact algorithm for \apsp in the general case\footnote{The problem can also be solved by running the distributed version of Bellman-Ford's algorithm \cite{peleg} from every node but this takes $O(n^2)$ time in the worst case, thus always worse than the trivial algorithm.}
%%
%%Yet another algorithm is to convert a weighted network to a $nw_{max}$-node unweighted one, where $w_{max}$ is the largest edge weight, by replacing an edge of weight $w$ to a path of $w$ nodes. We can then run the algorithms for the unweighted case.
%%
%For the special case of {\em BHC network}, whose topology is structured as a balanced hierarchy of clusters, the problem can be solved in $O(n \log n)$-time \cite{AntonioHT92}. Other than this, the problem can be solved in $O(n)$ time on a weighted asynchronous network \cite{KanchiV04}. This algorithm cannot be used in the \congest model since it involves using large messages.


%
%\paragraph{Lower Bounds} In the unweighted case, any $(\frac{3}{2}-\epsilon)$-approximation and $(2-\epsilon)$-approximation algorithm for computing the network's diameter and girth, respectively, requires  $\Omega(n/\log n)$ time~\cite{HolzerW12}\danupon{Lemma 11 Section 7.1.} and $\Omega(\sqrt{n}/\log n)$ time~\cite{FrischknechtHW12}, respectively. These bounds imply the same lower bound for the same approximation factor of any algorithm for approximating \apsp on unweighted networks. These lower bounds imply that our approximation algorithms are tight, even on unweighted networks.

%In the weighted case, \cite{DasSarmaHKKNPPW11} (building on \cite{Elkin06,PelegR00}) shows that solving \sssp requires $\tilde \Omega(\sqrt{n}+D(G))$ time, even when we allow $\poly(n)$ approximation ratio. This implies the same lower bound for \apsp. Recently, \cite{ElkinKNP12} extends the results of \cite{DasSarmaDP12} to the quantum setting. Thus, the same $\tilde \Omega(\sqrt{n})$ lower bound holds even in the quantum setting.
%%
%Our simple lower bound presented in Appendix~\ref{sec:lower bound} subsumes all previous lower bounds completely for the case of weighted \apsp (but not for unweighted \apsp or diameter and girth computation).
%%
%%The same argument can also be used to obtain the same result for computing weighted diameter\footnote{In particular, \cite{DasSarmaHKKNPPW11} shows that any algorithm needs $\tilde \Omega(\sqrt{n}+D(G)$ to distinguish between the case when MST has cost $n-1$ and when it contains an edge of weight at least $W$, for any $W=\poly(n)$. Observe that the former case implies that the distance between any pair of nodes is at most $n-1$ and the latter case implies that there is a pair of nodes whose distance is at least $W$ (i.e., the pair of nodes in the different connected component of the tree when we delete an edge of weight $W$ from the tree.)}.
%%
%%To the best of our knowledge, there is no lower bound specifically for algorithms on weighted network.
%%We also note that our lower bound subsumes these lower bounds for the case of \apsp (but not for diameter and girth computation).


%%%% Q: MST help???


%shows that  requires $\Omega(n/\log n)$ time\danupon{Lemma 11 Section 7.1.}. Moreover,  shows that any $(2-\epsilon)$-approximation algorithm for approximating the network girth requires $\Omega(\sqrt{n}/\log n)$ time.

%These two bounds imply a lower bound $\Imegan(n)$


%it is shown in \cite{FrischknechtHW12} that any approximation algorithm with approximation ratio less than $2$ requires $\tilde \Omega(\sqrt{n})$ time, and to get below a $3/2$ factor we need $\tilde \Omega(n)$ time~\cite{HolzerW12}\danupon{Lemma 11 Section 7.1.}.


%\subsection{REST}





%$n$ is obvious lower bound when diameter is large ...

%*** Exact algo can deal with zero edge weight

% The weights of the edges are at most polynomial in the number of vertices n, and there- fore, the weight of a single edge can be communicated in one time step. T


%\paragraph{Model} Assume synchronous \congest model. Nodes have unique IDs. Weight function $w:V\rightarrow \{1, \ldots, W\}$. As other papers in the literature (e.g., ...), we will assume that $W=\tilde O(1)$. The bandwidth is usually assumed to be $O(\log n)$ so that it is large enough to send IDs and edge weights in one round. To ease our presentation, we will relax the bandwidth restriction to $\tilde O(1)$. This can be assumed without loss of generality since we will ignore $\poly\log n$ term anyway.

%Our analysis holds for the case of $O(\log n)$ bandwidth, with additional $\tilde O(1)$ increase in the running time.


%\paragraph{Model} Assume synchronous \congest model. Nodes have unique IDs. Weight function $w:V\rightarrow \{1, \ldots, W\}$. We assume a bandwidth of $O(\log W\poly\log n)$ (see our comment on this bandwidth assumption below). In each round, ...

%
%{\bf Remarks:} First, it is usually assumed in the literature that $W=O(\poly(n))$ (WHY?). Our algorithm does {\em not} need this assumption.
%%
%It is also usually assumed in the literature that the bandwidth large is enough to send IDs and weights in one round, i.e. it is $\Theta(\log n+\log W)$. We assume a slightly larger bandwidth of $\Theta(\log W \poly\log n)$ only to simplify the analysis. We emphasize that our algorithm can also deal with the {\em general} bandwidth model, i.e. the \congestb model where the bandwidth is $B$.


%{\bf Other assumptions} We will assume that all nodes know $n$ and $W$. This can be assumed since we only need $O(n)$ to broadcast this information.


%\paragraph{Some definitions:} Let $(G, w)$ be any weighted directed graph. For any directed path $P=v_1v_2\ldots v_k$ in $G$, we let $w^i(P)=\sum_{j=1}^{k-1} (w(v_jv_{j+1}))^i$. In particular, $w^0(P)$ is the number of edges in $P$ and $w^1(P)$ is the sum of the weight of edges in $P$. Let $d^i(u, v)=\min_{P:\mbox{$u$-$v$ path}} w^i(P)$ where the minimum is over all possible paths $P$ from $u$ to $v$.

%Let $d^1_G(u, v)$ be the (weighted) distance from $u$ to $v$ and $d^0_G(u, v)$ be the distance from $u$ and $v$ in the underlying directed {\em unweighted} graph. We

%Explain why requiring one nodes to know everything doesn't make sense (i.e., clique with cut).
%Leave as open problem in Elkin's sigact.

%We note that any approximation algorithm (for any degree of approximation) has a lower bound of $\Omega(\sqrt{n/\log n})$  for SSSP \cite{DasSarmaHKKNPPW11} (CHECK) and $\Omega(n)$ for APSP (cf. Section~\ref{sec:APSP lower bound}).
%
%In the case of approximating diameter of weighted networks, things are much less known: We can trivially 2-approximate the diameter in linear-time using by computing a shortest path tree using node as a source. We are not aware of any faster or better approximation algorithm for this problem.

%Note: Lower bound of $\tilde\Omega(\sqrt{n})$ for \sssp by Elkin and the same lower bound for any approximation algorithm by Das Sarma et al. Then the surprising result of FHolzerWattenhofer follows.

% gives a fast algorithm on a weighted asynchronous network model which is not suitable for the \congest model studied in this paper since it involves using large messages.


%\cite{AntonioHT92} uses short ($O(\log n)$) messages and requires $O(n\log n)$ time for solving \apsp on a weighted {\em BHC} network whose topology is structured as a balanced hierarchy of clusters.




%\cite{HolzerW12,PelegRT12} to solve APSP in $O(nW)$ time. The analysis can be tightened to $O(n+D^1)$ where $D^1$ is the weighted diameter, which could be as large as $D^1$. \danupon{Better to avoid discuss $D^*$ since we can't get a running time based on that since finding distance in $(G, w_i)$ has nothing to do with $D^*$.}

%Single-Source Shortest Path (SSSP) can be solved in $O(D^*)$ time where $D^*$ is the {\em shortest-path diameter} (an upper bound of the depth of the shortest path tree rooted at any node $s$) by simulating Bellman-Ford's algorithm. Thus, we can solve APSP in $O(nD^*)$ time by solving SSSP from $n$ sources. This could be $O(n^2)$ for the worst value of $D^*$. The other algorithm is to aggregate all edges at one node, which takes $O(m)$ time in the worst case, where $m$ is the number of edges in the network.
%


%Single-Source Shortest Path (SSSP) can be solved in $O(D^*)$ time where $D^*$ is the {\em shortest-path diameter} (an upper bound of the depth of the shortest path tree rooted at any node $s$) by simulating Bellman-Ford's algorithm. Thus, we can solve APSP in $O(nD^*)$ time by solving SSSP from $n$ sources. This could be $O(n^2)$ for the worst value of $D^*$. The other algorithm is to aggregate all edges at one node, which takes $O(m)$ time in the worst case, where $m$ is the number of edges in the network.
%
%Yet another algorithm is to view a weighted network as an $nW$-node unweighted one by replacing an edge of weight $w$ to a path of $w$ nodes. We can then run the linear-time algorithm for the unweighted case \cite{HolzerW12,PelegRT12} to solve APSP in $O(nW)$ time. The analysis can be tightened to $O(n+D^1)$ where $D^1$ is the weighted diameter, which could be as large as $D^1$. \danupon{Better to avoid discuss $D^*$ since we can't get a running time based on that since finding distance in $(G, w_i)$ has nothing to do with $D^*$.}






%From Santoro's book The construction of routing table is a prerequisite for the functioning of many networks. One of the earliest protocols is due to William Tajibnapis [31]. ... see the protocol ``iterated routing''

%Can also use spanner algorithm of Baswana and Sen. The approximation ratio will be worse than our algorithm but the message complexity could be better.

%Elkin leaves \apsp on complete graph as an open problem.

%We can also solve \apsp on complete graph in $O(n)$ time. Is that interesting? Or can we combine with sub-linear SSSP somehow?


%**** Gopal + Kunal also have $S$-source shortest path (on weighted graph). Time depends on number of sources and ``shortest path diameter'' ($S$). Not sure if better than $n^2$. $O(\log n)$ approximation for $S$-SSP and also for metric embedding.

%**** Gopal + Khan consider the problem that every one wants to find nearest node of higher rank (rank is given arbitrarily).

%Note that can construct routing table in $O(n)$ time.

%Should we say that the problem is not interesting when $W$ is so large since we can show $\Omega(n\log W/B)$ easily (as in appendix)?


%\subsection{Preliminaries}

%Following Khan and Pandurangan \cite{KhanP08}, we let $\ell_{G, w}(u, v)$ denote the length of the minimum-length shortest path between $u$ and $v$ in $(G, w)$; i.e., if we let $\cP$ be the set of all shortest paths between $u$ and $v$ in $(G, w)$, then $\ell_{G, w}(u, v)=\max_{P\in \cP} |P|$ where $|P|$ is the length (number of edges) of $P$.


%$d_{G, w}(u, v)$ is the distance from $u$ to $v$ in weighted graph $(G, w)$. $D_{G, w}=\max_{u, v} d_{G, w}(u, v)$ is the {\em weighted} diameter of weighted graph $(G, w)$ and $D_{G, w}(s)=\max_{s, v} d_{G, w}(s, v)$. When we drop $w$ (i.e. $d_G(u, v)$, $D_G(s)$ and $D_G$), we treat all edge weight as one.



==> arXiv/lowerbound.tex <==

\section{Lower Bound for Approximating APSP (Proof of \Cref{observe:lower bound})}\label{sec:lower bound}

%\begin{theorem}
%Any approximation APSP algorithm requires $\Omega(n)$ time.
%\end{theorem}
%\begin{proof}(SKETCH)
%If we want to solve set disjointness then we can set edges on each star to be $0/1$ in such a way that if both $x[i]$ and $y[i]$ are one then $\dist(u_i, v_i)$ will be $0$. This means that {\em any} approximation algorithm will still get $\dist(u_i, v_i)=0$. Thus, we can check disjointness by checking if there is a pair of distance $0$.
%\end{proof}


\lowerbound*

%{\renewcommand{\thetheorem}{\ref{observe:lower bound}}
%\begin{observation}[Restated]
%Any $\poly(n)$-approximation algorithm for \apsp on an $n$-node weighted network $G$ requires $\Omega(\frac{n}{\log n})$ time. This lower bound holds even when the underlying network $G$ has diameter $\diam(G)=2$.
%%
%Moreover, for any $\alpha(n)=O(n)$, any $\alpha(n)$-approximation algorithm on an {\em unweighted} network requires $\Omega(\frac{n}{\alpha(n)\log n})$ time. 
%\end{observation}
%\addtocounter{theorem}{-1} % So that the \begin{theorem} above doesn't increase the counter
%} % \thetheorem is returned to its rightful definition outside of this group
\begin{proof}
Our proof simply formalizes the fact that a node needs to receive at least $n$ bits of information in order to know its distance to all other nodes. We start from the following {\em messag sending problem}: Alice receive a $\beta$-bit binary vector, denoted by $\langle x_1, \ldots, x_\beta\rangle$, where we set $\beta=n-2$. She wants to send this vector to Bob. Intuitively, to be sure that Bob gets the value of the vector correctly with a good probability, i.e. with probability at least $1-\epsilon$ for some small $\epsilon>0$, Alice has to send $\Omega(\beta)$ bits to Bob, regardless of what Bob sends to her. This fact can be formally proved in many ways (e.g., by using communication complexity lower bounds)
%; for example, if Alice can do this using $o(\beta)$ bits, then Alice and Bob can solve communication complexity problems like {\em set disjointness} using $o(\beta)$
%
and is true even in the quantum setting (see, e.g., Holevo's theorem \cite{Holevo73}). 

Now, let $\cA$ be an $\alpha(n)$-approximation $T$-time algorithm for weighted \apsp. We show that Alice can use $\cA$ to send her message to Bob using $O(T\log n)$ bits, as follows. Construct a graph $G$ consisting of $n=\beta+2$ nodes, denoted by $a_1, \ldots, a_\beta$, $a^*$ and $b$. There are edges between all nodes to $a^*$.  The weight of edge $a^*b$ is always $w(a^*b)=1$. Weight of every edge $a_ia^*$ is set by Alice: if $x_i=1$ then she sets weight of $a_ia^*$ to $w(a_ia^*)=1$; otherwise she sets it to $w(a_ia^*)=2\alpha(n)$. Then, Alice simulates $\cA$ on $a_1, \ldots, a_\beta$ and $a^*$, and Bob simulates $\cA$ on $b$. If $\cA$ wants to send any message from $a^*$ to $b$, Alice will send this message to Bob so that Bob can continue simulating $b$. Similarly, if  $\cA$ wants to send any message from $b$ to $a^*$, Bob will send this message to Alice so that Alice can continue simulating $a^*$.
%
If $\cA$ finishes in $T$ rounds, then Alice will send at most $O(T\log n)$ bits to Bob in total. 

Observe that, for any $i$, if $x_i=1$ then $\dist_{G, w}(a_i, b)=2$; otherwise, $\dist_{G, w}(a_i, b)=2\alpha(n)+1$. Since $\cA$ is $\alpha(n)$ approximation, $\cA$ must answer $\tilde \dist_{G, w}(a_i, b)\leq 2\alpha(n)$ if $x_i=1$; otherwise, $\cA$ must answer $\tilde \dist_{G, w}(a_i, b)\geq 2\alpha(n)+1$. Since $\tilde \dist_{G, w}(a_i, b)$ is known to $b$, Bob can get the value of $\tilde \dist_{G, w}(a_i, b)$ by reading it from $b$ (which he is simulating). Then he can reconstructs $x_i$. Thus, Bob can reconstruct all bits $x_1, \ldots, x_\beta$ after getting $O(T\log n)$ bits from Alice.
%
The lower bound of the message sending problem thus implies that $T=\Omega(\beta/\log n)=\Omega(n/\log n)$. 

Note that since the highest weight we can put on an edge is $\poly(n)$, we require that $\alpha(n)\leq \poly(n)$. 
%
We use the same argument for the unweighted case, but this time we use $\beta=n/\alpha(n)$ and replace an edge of weight $2\alpha(n)$ by a path of length $2\alpha(n)$. 
\end{proof}

\begin{comment}
\begin{proof}
We reduce from the two-party communication complexity called {\em set disjointness} (\disj). In this problem, each of the two parties (called Alice and Bob) receive $\beta$-bit binary vectors, denoted by $x$ and $y$, respectively. They want to cooperatively compute the inner product $\langle x, y\rangle$ and output $\disj(x, y)=1$ if $\langle x, y\rangle=0$ and $\disj(x, y)=0$ otherwise. The goal is to come up the an algorithm that allows Alice and Bob to compute $\langle x, y\rangle$ by communicating least number of bits possible. It is well known that Alice and Bob must communicate $\Omega(\beta)$ bits, even when they can make errors with a small probability.
%
\begin{theorem}[\cite{BabaiFS86,KalyanasundaramS92,Bar-YossefJKS04,Razborov92}]\label{theorem:disj}
For small enough constant $\epsilon>0$, any protocol that allows Alice and Bob to compute $\disj(x, y)$ correctly with probability at least $1-\epsilon$, for any input $x$ and $y$, requires $\Omega(\beta)$ bits of communication.
\end{theorem}
%
Theorem~\ref{theorem:lower bound} follows immediately from the following lemmas.
\begin{lemma}
For any $T(n)$ and $\alpha(n)\leq (n-2)/6$, if there exists a $T(n)$-time $\alpha(n)$-approximation distributed algorithm for \apsp on any $n$-node unweighted graph, then Alice and Bob has a protocol that can compute $\langle x, y\rangle$ on any $\beta$-bit input $(x, y)$, where $\beta\leq (n-2)(6\alpha(n))$, using $O(T(n)\log n)$ bits of communication. The same statement holds for the weighted case except that $\alpha(n)$ could be as large as $2^{O(\log n)}$. 
\end{lemma}
\begin{proof}
Let $\cA$ be the above distributed algorithm. When Alice and Bob receive $x$ and $y$, respectively, they will simulate $\cA$ on an unweighted network $G$. Alice will simulate $\cA$ on some nodes in the network and Bob will simulate the rest. They will construct the network without communicating to each other. 

Let $x[1], \ldots, x[\beta]$ and $y[1],\ldots, y[\beta]$ denote $\beta$ bits of $x$ and $y$, respectively. First, Alice and Bob add edge $a^*b^*$ to $G$. Both of them are aware of this edge. Next, for each bit $x[i]$ of Alice, she construct a path $A_i$, having $a_i$ as one end node and $a^*$ as the other. The length of $A_i$ is determined by $x[i]$: if $x[i]=1$ then $A_i$ has length one; otherwise, it has length $3\alpha(n)$. Bob does the same thing: he constructs a path $B_i$ between $b_i$ and $b^*$ whose length is one if $y[i]=1$ and $3\alpha(n)$ otherwise.

This network can be constructed without communication. The number of nodes in this network is at most $6\alpha(n)b+2\leq n$. 

Now, Alice simulates $\cA$ on nodes $a_1, \ldots, a_\beta$ and $a^*$, and Bob simulates $\cA$ on nodes $b_1, \ldots, b_\beta$ and $b^*$. They do this for $T$ rounds, and in each round Alice (respectively Bob) sends the message that $a^*$ (respectively $b^*$) sends to $b^*$ (respectively $a^*$) in $\cA$ so that both parties can keep executing $\cA$. They simulate $\cA$ until it finishes, which takes at most $T(n)$ rounds. Since, in each round, $a^*$ and $b^*$ send $O(\log n)$ bits to each other, Alice and Bob have to communicate $O(T(n)\log n)$ bits in total.

Now, observe the followings. (1) If $\disj(x, y)=0$, then there exists $i$ such that $x[i]=y[i]=1$; in this case, $\dist_G(a_i, b_i)=3$. (2) If $\disj(x, y)=1$, then, for all $i$, $x[i]=0$ or $y[i]=0$; in this case, $\dist_G(a_i, b_i)>3\alpha(n)$. Thus, if $\cA$ is an $\alpha(n)$-approximation algorithm then it will output an approximate distance $\tilde{\dist}_G(a_i, b_i)\leq 3\alpha(n)$ for some $i$ in the first case and $\tilde{\dist}_G(a_i, b_i)>3\alpha(n)$, for all $i$, in the second case. These distances are known to Alice and Bob, so they can use them to answer whether $\disj(x, y)$ is zero or one. 

For the weighted case, we will use an edge of weight $3\alpha(n)$ instead of a path of length $3\alpha(n)$. The restriction of the maximum weight we can assign allow us to use $\alpha(n)$ as large as $2^{O(\log n)}$. 
\end{proof}
The above lemma and Theorem~\ref{theorem:disj} implies that any $T(n)$-time $\alpha(n)$-approximation distributed algorithm for \apsp must have $T(n)=\Omega(\beta/\log n)$. Using $\beta=(n-2)/(6\alpha(n))$, we have $T(n)=\Omega(n/\alpha(n)\log n)$ as desired.
\end{proof}

As a corollary, no algorithm can improve the running time of our linear-time approximation algorithm for weighted \apsp significantly, even on an unweighted network, unless its approximation ratio is $\omega(\poly\log n)$. 

\begin{corollary}
Any $\poly\log n$-approximation algorithm for \apsp on unweighted networks requires $\tilde \Omega(n)$ time. 
\end{corollary}


\iffalse
\begin{theorem}
Any approximation APSP algorithm requires $\tilde \Omega(n\log W/B)$ time in the \congestb model.
\end{theorem}
\begin{proof}(SKETCH)
Consider the graph consisting of edges $u, v, v_1, \ldots, v_n$. Weights are $w(uv)=1$ and $w(vv_i)\in \{1, \ldots, W\}$. To get the $\alpha$ approximation of its distance to all other nodes, $u$ will have to terminate in $(W/\alpha)^n$ states. This means that it has to receive $\Omega(n\log (W/\alpha))$ bits.
\end{proof}
\fi
\end{comment}



Note that in the proof above we show a lower bound for computing distances between all pairs of nodes. Since the lower bound graph is a star, the routing problem is trivial (since there is always one option to send a message). We can easily modify the above graph to give the same lower bound for the routing problem on weighted graphs: First, instead of using weight $2\alpha(n)$ in the graph above, use weight $2\alpha^2(n)+\alpha(n)$ instead. Second, add a new node $c$ and edges of weight $2\alpha(n)$ between $c$ and all nodes $a_1$ and an edge of weight $1$ between $c$ and $b$. Observe that if $x_i=1$, then we have to route a message through $a^*$, giving a distance of $2$ (while routing through $c$ gives a distance of $2\alpha(n)+1$. If $x_i=0$, we should route through $c$ which gives a distance of $2\alpha(n)+1$ since routing through $a^*$ will cost $2\alpha^2(n)+\alpha(n)+1$. 



==> arXiv/main_algo5.tex <==
\section{Exact Algorithm (Main)}\label{sec:main algo}\label{sec:scaling}

\begin{algorithm*}[t]
\caption{{\sc Main}($G, w$) (detail in Section~\ref{sec:main algo})}\label{algo:apsp}
{\bf Input:} Undirected weighted network $(G, w)$ (note that $w$ is symmetric).

{\bf Output:} For every node $u$ and $v$, both $u$ and $v$ know $\dist_{G, w}(u, v)$.

\begin{algorithmic}[1]


\State Compute $w_i$ and $\beta$ as in Definition~\ref{def:w_i}. {\small \it // As a result, every node $u$ knows $\beta$ and $w_i(uv)$ for every edge $uv$ in $G$. This takes $O(n)$ time.}
%{\small \it // As a quick reminder, we write $w$ as $\beta$-bit positive binary number (cf. Def.~\ref{def:positive binary representation}), and $w_i$ consists of the $\beta^{th}$ to $i^{th}$ bits.}\label{line:beta}

\For{$i=\beta, \beta-1, \ldots, 0$} %\Comment{This is Iteration $i$.}

\State {\small\it // This is Iteration $i$. We will solve \apsp on $(G, w_i)$.} %Let $t_i$ be the round at the beginning of this iteration.


\vspace{.1em}
\State \label{line:w_i} Every node $u$ in $G$ computes $\vec w_i^s(uv)$ defined as $\vec w_i^s(uv)=2\dist_{w_{i+1}}(s, u)-2\dist_{w_{i+1}}(s, v)+w_i({uv})$, for every edge $uv\in E(G)$ and every node $s$ in the network. Let $\cW_i=\{\vec w_i^s\}_{s\in V(G)}$.  {\small \it // Can be done in $O(n)$ time (cf. Claim~\ref{claim:w_i time}).}


\vspace{.1em}
\State Partition nodes into clusters $C_1, \ldots, C_k$, for some $k$, with properties as in Proposition~\ref{prop:clustering}. As a result, every node $u$ knows which cluster every node $v$ is in; i.e., it knows the set $\{(v, \rep(C_j) \mid v\in C_j)\}$ where we define $\rep(C_j)$ to be $\rep(C_j)=\min_{v\in C_j} v$. {\small\it // $O(n)$ time by Proposition~\ref{prop:clustering}.} \label{line:clustering}

%; i.e., for every node $s$, $\dist_{G, \vec w_i^s}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster. {\small\it // As a result, every node $u$ in cluster $C_j$ knows $\rep(C_j)=\min_{v\in C_j} v$ and $|C_j|$. This step takes $O(n)$ time by Lemma~\ref{lem:clustering}.} \label{line:clustering}

%
%\hspace{.5em}
%{\small \it As a result, every node $u$ in cluster $C_j^i$ knows $\rep(C_j^i)$ the smallest ID node in $C_j^i$}


%\hspace{.5em} {\small // The above can be done in $O(n)$ time.}

\vspace{.2em}
\State For all $j$, let $E_j=\{uv\in E(G)\mid u, v\in C_j\}$.  Compute $H$ defined as the subgraph of $G$ with edge set $E(H)=E(G)\setminus (\bigcup_{j: |C_j|>\sqrt{n}} E_j)$.  {\small\it // As a result, every node in network $G$ knows which edges in $E(G)$ incident to it are in the subgraph $H$. This step needs no communication.}\label{line:compute H}
%In other words, we obtain $H$ by deleting all edges between two nodes in $C_i$ for all $C_i$ such that $|C_i|>\sqrt{n}$.



\vspace{.2em}
\State Solve multi-weight $(2n)$-\apsp (cf. Definition~\ref{def:multi weight apsp}) on $(H, \cW_i)$ using Proposition~\ref{prop:pseudopoly multi-weight} with $\zero(H, \cW_i)=\sqrt{n}$. {\small\it // Finishes in $O(n\sqrt{n}\log n)$ time with high probability. As a result, every node $u$ knows $\dist^{2n}_{H, \vec w_i^s}(s, u)$ for all $s$.} \label{line:multi-weight apsp}


\State Every node $u$ computes the candidate distance function $d'(s, u)=2\dist_{G, w_{i+1}}(s, u)+\dist^{K}_{H, \vec w_i^s}(s, u)$ for all nodes $s$, as in Proposition~\ref{prop:d prime}. {\small\it // Need no communication.}\label{line:d prime}
%See Lemma~\ref{lem:d prime} for the meaning of $d'$.}

%\State Every node $u$ computes, for all nodes $s$, $\dist^{2n}_{H, w_i}(s, u)$ using the following formula: $\dist^{2n}_{H, w_i}(s, u)=2\dist^{2n}_{G, w_{i+1}}(s, u)+\dist^{2n}_{H, \vec w_i^s}(s, u)$. {\small\it // No communication. Lemma~\ref{lem:dist w_i from dist w_i^u} guarantees correctness.}\label{line:solve apsp on H w_i}



\vspace{.2em}
\State For all $j\neq j'$, every node $u$ in cluster $C_j$ computes $d'(C_j, C_{j'})$ defined as $d'(C_j, C_{j'})=\min_{u\in C_j, v\in C_{j'}}d'(u, v)$. {\small\it // Can be done in $O(n)$ time (cf. Claim~\ref{claim: running time of line:collect distance within cluster}).}\label{line:collect distance within cluster}



\vspace{.2em}
\State For every cluster $C_j$ such that $|C_j|>\sqrt{n}$, $\rep(C_j)$ broadcasts $d'(C_j, C_{j'})$, for all $j'\neq j$, to all nodes in the network. {\small\it // Can be done in $O(n\sqrt{n})$ time since there are at most $O(n\sqrt{n})$ messages broadcasted (cf. Claim~\ref{claim: running time of line:broadcast big cluster}).}\label{line:broadcast big cluster}

%\hspace{.5em} {\small // The above can be done in $O(n\sqrt{n})$ time since there are at most $O(n\sqrt{n})$ messages broadcasted (cf. Lemma~XXX).}



\vspace{.2em}
\State For every cluster $C_j$ and node $u\in C_j$, node $u$ internally constructs graph $G'_u$ consisting of node set $V(G'_u)=\{c_1, \ldots, c_k\}$ and edge sets $E(G'_u)=E_1'\cup E'_2$ where $E_1'=\{c_jc_{j'} \mid j'\neq j\}$ and $E_2'=\{c_{j'}c_{j''} \mid j'\neq j''\ \wedge\ |C_{j'}|>\sqrt{n}\ \wedge\ |C_{j''}|>\sqrt{n}\}$. Define edge weight $w'$ as $w(c_{j'}c_{j''})=d'(C_{j'}, C_{j''})$ for any edge $c_{j'}c_{j''}$. {\small \it // Need no communication since all required information is already computed in Line~\ref{line:collect distance within cluster} and \ref{line:broadcast big cluster} (cf. Claim~\ref{claim:running time of line:G prime}).}\label{line:G prime}


\vspace{.2em}
\State Node $u$ computes, for every node $v\neq u$, $\dist_{G, w_i}(u, v)$ using Proposition~\ref{prop:G prime}: $\dist_{G, w_i}(u, v)=\dist_{G'_u, w'}(c_j, c_{j'})$ where $j$ and $j'$ are such that $u\in C_j$ and $v\in C_{j'}$. {\small // Need no communication.} \label{line:final computation}


\EndFor

\end{algorithmic}
\end{algorithm*}



%\begin{algorithm*}
%\caption{Computing $\dist_{w_i^x}(x, u)$. (Detail in Section~\ref{sec:supernode}-\ref{sec:heavy}.)}\label{algo:compute dist_i^u}
%{\bf Input:} Every node $u$ knows $w_i^x(\overrightarrow{uv})$ and $G, w_i^x(\overrightarrow{vu})$ for all neighbors $v$ and any node $x$.
%
%{\bf Output:} Every node $u$ knows $\dist_{w_i^x}(x, u)$ for all nodes $x$.
%
%\begin{algorithmic}[1]
%
%
%
%
%
%\State Now every node $u$ knows $\dist_{w_i^x}(x, u)$ for all nodes $x$, regardless of whether $(x, u)$ is $(G, w_i)$-light or $(G, w_i)$-heavy.
%\end{algorithmic}
%\end{algorithm*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this section, we explain the main algorithm for solving \apsp exactly, as outlined in Algorithm~\ref{algo:apsp}. Our algorithm uses the weight scaling technique, which is based on the {\em positive binary representation} of weights. This is similar to the standard binary representation except that every bit is either one or two:
%
\begin{definition}\label{def:positive binary representation}
For any positive integer $x$, we say that a sequence of integers $b_0, b_1, \ldots, b_k\in \{1, 2\}$ is a {\em positive binary representation} of $x$ if $x=\sum_{i=0}^k b_i2^i$.
\end{definition}
%
We note again that we cannot use the standard binary representation since Proposition~\ref{prop:clustering} will not hold in this case. Also note that, for any positive integer $x$, a positive binary representation always exists and can be easily computed by the following algorithm: Let $x_0=x$, and define $x_1, x_2, \ldots$ and $b_0, b_1, \ldots$ as follows. For any $i\geq 0$ such that $x_i>0$, if $x_i$ is odd, then we let $b_i=1$ and $x_{i+1}=(x_i-1)/2$; otherwise, let $b_i=2$ and $x_{i+1}=(x_i-2)/2$. Also note that it can be proved that any $x$ has a unique positive binary representation, but we will not need this fact here.\danupon{To do: Write this as claim.}

%Let $\beta=\lceil\log W\rceil$. Our algorithm solves \apsp on graphs $(G, w_0)$, $(G, w_1)$, $\ldots$, $(G, w_\beta)$, where  $w_i$ consists of bits of $w$ from the $i^{th}$ bit to the last bit. Formally:

Algorithm~\ref{algo:apsp} runs in {\em iterations}. In Iteration $i$, we solve \apsp on graph $G$ with weight function $w_i$, where $w_i$ is defined as the number consisting of bits of $w$ from the $i^{th}$ bit to the $k^{th}$ bit, as follows.
%
\begin{definition}[$w_i$ and $\beta$]\label{def:w_i} For any edge $uv$, let $k_{uv}$ and $b_0(uv)$, $\ldots$, $b_{k_{uv}}(uv)$ be the binary representation of $w(uv)$. Also let $b_i(uv)=0$ for all $i>k_{uv}$.
%
Let
$$\beta=\max_{uv\in E(G)} k_{uv} ~~\mbox{ and }~~ w_i(uv)=\sum_{j=i}^{\infty} b_j(uv)2^j$$
for any $i\geq 0$.
\end{definition}
%
%%
%In order to solve \apsp at Iteration $i$ quickly, we use the solution from Iteration $i+1$ (i.e. $\dist_{w_{i+1}}(uv)$ for all edges $uv$) to compute several {\em directed} weighted graphs and solve \sssp on these graphs instead. In particular, we define a weight function $w_i^x$ on directed edges as follows.
%%
%\begin{definition}\label{def:w_i^u}
%For any node $x$ and directed edge $\overrightarrow{uv}$ in $\overrightarrow{}$, define $w_i^x$ as $w_i^x(\overrightarrow{uv})=2\dist_{w_{i+1}}(x, u)-2\dist_{w_{i+1}}(x, v)+w_i(uv)$.
%\end{definition}
%
Note that $\beta=O(\log n)$ since the largest weight is $O(\poly(n))$, and we can make every node know $\beta$ in $O(D(G))=O(n)$ rounds.
%
Our algorithm starts from Iteration $\beta$ down to Iteration $0$ (see the for-loop in Algorithm~\ref{algo:apsp}). In each Iteration $i$, the algorithm does the following.

First, it transforms weight function $w_i$ to a collection $\cW_i=\{\vec w_i^s\}_{s\in V(G)}$ of $n$ weight functions, as in {\bf Line~\ref{line:w_i}} of Algorithm~\ref{algo:apsp}. At the end of this step, every node $u$ knows $\vec w_i^s(uv)$ for all neighbors $v$ and nodes $s$. We note that this step can be completed in $O(n)$ time, simply by exchanging $n$ messages between neighbors, as in the following claim.
%
\begin{claim}[Proof in Appendix~\ref{sec:omitted proofs}]\label{claim:w_i time}\label{CLAIM:W_I TIME}
Line~\ref{line:w_i} of Algorithm~\ref{algo:apsp} can be done in $O(n)$ time.
\end{claim}
%
Next, in {\bf Line~\ref{line:clustering}}, the algorithm partitions nodes into {\em clusters} using Proposition~\ref{prop:clustering} introduced in Section~\ref{sec:overview}. At the end of this step, every node $u$ knows the following information about all other nodes $v$.

For any cluster $C_j$, we define the {\em representative node of $C_j$}, denoted by $\rep(C_j)$, as the minimum node ID in $C_j$, i.e. $\rep(C_j)=\min_{v\in C_j} v$. At the end of Line~\ref{line:clustering}, we want every node $u$ to know, for all $v$, $\rep(C_j)$ where $C_j$ is the cluster that contains $v$. As claimed in Proposition~\ref{prop:clustering}, this step takes $O(n)$ time.

In {\bf Line~\ref{line:compute H}}, we compute the subgraph $H$ obtained from $G$ by deleting all edges in clusters of size more than $\sqrt{n}$ (we call these clusters {\em big clusters}); i.e., we delete all edges in $\{uv\in E(G) \mid \exists j:\ u, v\in C_j\ \&\ |C_j|>\sqrt{n}\}$. To compute $H$, every node $u$ simply check whether it is in a big cluster. If it is in a big cluster, then it marks all edges $uv$, for all neighbors $v$ that are in the same cluster, as ``deleted''. Note that this step can be done without any communication since every node knows the clusters other nodes are in from  Line~\ref{line:clustering}; so it can use  use this information to check which clusters it and its neighbors are in, as well as the sizes.

Now that we have the subgraph $H$, we will, in {\bf Line~\ref{line:multi-weight apsp}}, solve the multi-weight $K$-\apsp problem (cf. Definition~\ref{def:multi weight apsp}) on $(H, \cW_i)$, using $K=2n$. This is guaranteed to be doable in $O(n\sqrt{n}\log n)$ time, by Proposition~\ref{prop:pseudopoly multi-weight} and the following claim. (Recall that $\zero(G, \cW)$ is the longest zero path length of $(G, \cW)$ defined before we state Proposition~\ref{prop:pseudopoly multi-weight}.)
\begin{claim}
$\zero(H, \cW_i)\leq \sqrt{n}.$
\end{claim}
\begin{proof}
For any node $s$ and $\ell>0$, let $P=\langle x_0, x_1, \ldots, x_\ell\rangle$ be any simple path of distance zero in $\vec w_i^s$; i.e., $\vec w_i^s(x_ix_{i+1})=0$ for all $0\leq i\leq \ell-1$. By Proposition~\ref{prop:clustering},
$w_i(x_ix_{i+1})=0$ for all $0\leq i\leq \ell-1$. It follows that all nodes in $P$ must be in the same cluster. Since we delete all edges within big clusters (in Line~\ref{line:compute H}) and $P$ has at least one edge, nodes in $P$ must be in $C_j$ such that $|C_j|\leq \sqrt{n}$. In other words, $\ell\leq \sqrt{n}$. This implies that any simple path of distance zero (for any edge weight $\vec w_i^s$) has length at most $\sqrt{n}$, i.e., $\zero(H, \cW_i)\leq \sqrt{n}.$
\end{proof}
%
In {\bf Line~\ref{line:d prime}}, the algorithm {\em tries} to use the solution of multi-weight $(2n)$-\apsp on $(H, \cW_i)$ to solve $(2n)$-\apsp on $(G, w_i)$. This results in the {\em candidate distance function} $d'$. While it is not true that $d'(u, v)=\dist_{G, w_i}(u, v)$ for all nodes $u$ and $v$ (we would have got this if we can use Eq.\eqref{eq:ideal w_i recovery}), this is the case for the pairs of nodes whose distances are preserved by $(H, w_i)$, as shown by Proposition~\ref{prop:d prime}.
%
Note that this step needs no communication since $u$ already knows $\dist_{G, w_{i+1}}(s, v)$, for all nodes $s$, from Iteration $i+1$, and $\dist_{H, \vec w_i^s}(s, u)$ is computed in Line~\ref{line:multi-weight apsp}.
%
%The correctness of this step is guaranteed by the following lemma.
%


Next, in {\bf Line~\ref{line:collect distance within cluster}}, every node $u$ computes $d'(C_j, C_{j'})=\min_{u\in C_j, v\in C_{j'}}d'(u, v)$ for all nodes $v$, where $C_j$ and $C_{j'}$ are clusters containing $u$ and $v$, respectively. We note that the running time of this step is $O(n)$:
%
\begin{claim}\label{claim: running time of line:collect distance within cluster}
Line~\ref{line:collect distance within cluster} of Algorithm~\ref{algo:apsp} finishes in $O(n)$ time.
\end{claim}
\begin{proof}
The algorithm simply performs an ``internal communication'' within each cluster. In particular, for each cluster $C_j$, the representative node $\rep(C_j)$ collects $d'(C_j, C_{j'})$, for all $j'$. This is done by constructing a BFS tree $T$ spanning the (connected) subgraph of $G$ induced by $C_j$. Then, every node $u\in C_j$ sends to its parent
$d'(T_u, C_{j'})$ $=\min_{u'\in T_u, v\in C_{j'}}$ $d'(u', v)$
where $T_u$ is the subtree of $T$ rooted at $u$. This can be easily done in $O(\delta_T+k)$ time, where $\delta_T$ is the depth of $T$ and $k$ is the number of clusters: every node $u$ at level $\ell$ in $T$ (the root node has level $0$) sends $d'(T_u, C_{j'})$ to its parent, for any $j'$, exactly once at time $\delta_T-\ell+j'$.

After collecting the distance information, $\rep(C_j)$ can broadcast this information to all nodes in $C_j$ in $O(\delta_T+k)$ time. The total time is thus $O(\delta_T+k)=O(n)$.% This leads to the following running time claim.
\end{proof}
%
In the next step, {\bf Line~\ref{line:broadcast big cluster}}, we make sure that every node knows the value of $d'(C_j, C_{j'})$ between any big cluster $C_j$ (i.e. $|C_j|>\sqrt{n}$) and any other cluster $C_{j'}$. This is easily done by having the representative node of each big cluster $C_j$, i.e. $\rep(C_j)$, broadcasting $d'(C_j, C_{j'})$, for every $j'$, which is computed in the previous step. Since there are less than $\sqrt{n}$ big clusters and the representative node of each cluster broadcasts $k\leq n$ message (where $k$ is the number of clusters), this step can be easily done in $(n\sqrt{n})$ time (e.g., by collecting all information at one node before broadcasting).
%
\begin{claim}\label{claim: running time of line:broadcast big cluster}
Line~\ref{line:broadcast big cluster} of Algorithm~\ref{algo:apsp} finishes in $O(n\sqrt{n})$ time.
\end{claim}
%
In the last two steps, each node $u$ uses the values of $d'$ it gets from Lines~\ref{line:collect distance within cluster} and \ref{line:broadcast big cluster} to determine $\dist_{G, w_i}(u, v)$, for all nodes $v$, without communicating with other nodes. First, in {\bf Line~\ref{line:G prime}}, it constructs a weighted graph $(G'_u, w')$ which consists of nodes $c_1, \ldots, c_k$ where each node $c_j$ represents cluster $C_j$. Edges in $G'_u$ are between the pairs of clusters that $u$ knows their candidate distances $d'$. In particular, we have two types of edges: Edges of the first type (i.e. $E_1'$ in Line~\ref{line:G prime}) are in the form $c_jc_{j'}$ for any $j'$, where $C_j$ is the cluster containing $u$. Weights of these edges are candidate distances $d'(C_j, C_{j'})$ computed in Line~\ref{line:collect distance within cluster}. Edges of the second type (i.e. $E_2'$ in Line~\ref{line:G prime}) are in the form $d'(C_{j'}, C_{j''})$ for any $j'$ and $j''$ such that $|C_{j'}|>\sqrt{n}$. Weights of these edges are candidate distances $d'(C_{j'}, C_{j''})$, which are broadcasted to every node in Line~\ref{line:broadcast big cluster}. This completes the description of $G'_u$.
%
Since $u$ has all information needed to construct $G'_u$ before we start Line~\ref{line:G prime}, we have the following claim.
\begin{claim}\label{claim:running time of line:G prime}
Line~\ref{line:G prime} needs no communication.
\end{claim}
%
Finally, in {\bf Line~\ref{line:final computation}}, node $u$ uses $G'_u$ to compute distance $\dist_{G, w_i}(u, v)$  to all nodes $v$. This is done simply by using Proposition~\ref{prop:G prime}. This completes one iteration of Algorithm~\ref{algo:apsp} where we compute $\dist_{G, w_i}$.

We conclude this section with the running time of our main algorithm. Since every step takes $O(n\sqrt{n}\log n)$ time and we have $\beta=O(\log n)$ iterations, we have that Algorithm~\ref{algo:apsp} finishes in $O(n\sqrt{n}\log^2 n)$ with high probability. Theorem~\ref{theorem:exact} follows.
%
%, the following lemma easily follows.
%%
%\begin{lemma}[Time Complexity]\label{lem:time}
%Algorithm~\ref{algo:apsp} finishes in $O(n\sqrt{n}\log^2 n)$ with high probability.
%\end{lemma}
%%





==> arXiv/multi_weight_k_apsp.tex <==
\section{Multi-Weight {\large $\mathbf{K}$}-APSP (Proposition \ref{prop:pseudopoly multi-weight})}\label{sec:multi-weight k-apsp}

In this section, we prove Proposition~\ref{prop:pseudopoly multi-weight}: multi-weight $K$-\apsp on $(G, \cW)$ can be solved by an algorithm that takes $\zero(G, \cW)$ as an input and, with high probability, finishes in $O(K\zero(G, \cW)\log n+n)$ time.

The main idea of our algorithm is based on growing several BFS trees in parallel and using the random delay technique \cite{LeightonMR94} to avoid conflicts. The algorithm is outlined in Algorithm~\ref{algo:multi weight k apsp}. We will show that Algorithm~\ref{algo:multi weight k apsp} causes a congestion of at most $\log n$ with high probability; i.e., at any point in time, there will be at most $\log n$ messages sent through any edge. Moreover, we will show that Algorithm~\ref{algo:multi weight k apsp} finishes in $O(K\zero(G, \cW)+n)$ time if there is no congestion. By allowing an extra $\log n$ time between each step of Algorithm~\ref{algo:multi weight k apsp}, there will be no congestion with high probability. Additionally, if the algorithm fails to send any message due to congestion (which we can detect), we can run the trivial algorithm where we collect all information to one node. This makes the algorithm never fail and have a running time of $O((K\zero(G, \cW)+n)\log n)$ with high probability.
%
We also note that the random delay technique can also be used to remove the assumption that $\zero(G, \cW)$ is known to every node, with an extra $O(n)$ running time. However, this is not necessary for us so we do not include it here to avoid making the algorithm more complicated.




\begin{algorithm}[t]
\caption{{\sc Multi-Weight $K$-Apsp}({\small $G$, $\cW$, $K$, $\zero(G, \cW)$})}
\label{algo:multi weight k apsp}
{\bf Input:} Every node $u$ knows (1) $\vec w^s(uv)$ for all neighbors $v$ and nodes $s$, (2) $K$, and (3) $\zero(G, \cW)$.

{\bf Output:} Every node $u$ knows $\dist_{G, \vec w^s}^K(s, u)$ for all nodes $s$.

\begin{algorithmic}[1]
%\State Make every node knows $\zero(G, \cW)$. {\small\it // Can be done in $O(n)$ time. See description in text}\label{line:BFS compute zero}

\State Every node $s$ selects an integer $r_s$ uniformly at random from $[0, n-1]$ and broadcast $r_s$ to all other nodes.
{\small\it // Takes $O(n)$ time since $n$ messages are broadcasted.}\label{line:generate random delay start}


\State Let $\tau_s=t_0+r_s$ where $t_0$ is the time that the previous step finishes.\label{line:t_0}


\State Every node $s$ sends a message $(s, 0)$ to itself at time $\tau_s$ to initiate the BFS-style subroutine below.\label{line:start BFS}

\algstore{multiapsp}
\end{algorithmic}

\smallskip\textit{\textbf{BFS-Style Subroutine:}} When a node $u$ receives a message $(s, \ell)$ for some $s$ and $\ell$, it does the following.

\smallskip
\begin{algorithmic}[1]

\algrestore{multiapsp}

\If{$u$ has {\em not} already received $(s, \ell')$ for some $\ell'$}\label{line:BFS style start}

\State $u$ now knows that $\dist_{G, \vec w^s}(s, u)=\ell$. {\small \it // See Lemma~\ref{lem:correctness of light apsp} for correctness.)}\label{line:BFS style compute distance}


%\If{($\ell=0$) or ($u\in C_j\ s.t.\ |C_j|\leq \zero(G, \cW)$)}\label{line:check light}


\State $u$ sends $(s, \ell)$ through any edge $uv$ such that $\vec w^s(uv)=0$.\label{line:forward message}

\State For any neighboring nodes $v$ such that $\vec w^s(uv)>0$ and $\ell+\vec w^s(uv)\leq K$, node $u$ sends to $v$  a message $(s, \ell+\vec w^s(uv))$ at time $\tau_s+(\ell+\vec w^s(uv))\zero(G, \cW)$.\label{line:bfs style send message}

%\State If $u$ cannot send any message at the desired time (due to congestion), then the algorithm {\em fails} and solves the problem using a trivial algorithm (aggregate all information to one node) instead. \label{line:fail}

%\EndIf

\EndIf\label{line:BFS style end} %\linebreak
%
\end{algorithmic}
\end{algorithm}

%In {\bf Line~\ref{line:BFS compute zero}}, the algorithm makes sure that all nodes know $\zero(G, \cW)$. This can be easily done as follows. Initially, every node $u$, for every node $s$, sends message $(s, u)$ to all neighbors $v$ such that $\vec w^s(vu)=0$. When node $u$ receives a new message $(s, u')$, it forward this message to




Algorithm~\ref{algo:multi weight k apsp} starts, in {\bf Line~\ref{line:generate random delay start}}, by generating a random delay for each node $s$, denoted by $r_s$. Then it makes sure that every node knows $r_s$ by broadcasting these numbers. Since there are $n$ numbers broadcasted in this step, this step takes $O(n)$ time (e.g. by collecting all numbers at one node before broadcasting them out).

The algorithm waits until Line~\ref{line:generate random delay start} finishes. Then, in {\bf Line~\ref{line:t_0}-\ref{line:start BFS}}, every node $s$ starts growing a BFS tree rooted at $s$ by sending to itself a message $(s, 0)$.  This step will tricker the {\em BFS-style subroutine} to start. Instead of doing this immediately, however, node $s$ waits until time $\tau_s=t_0+r_s$,  where $t_0$ is the time the algorithm step finishes. This is the key step that will give us the claimed running time.


\paragraph{BFS-Style Subroutine} We now explain the BFS-style subroutine (Line~\ref{line:BFS style start} -- \ref{line:BFS style end} of Algorithm~\ref{algo:multi weight k apsp}). For an intuition, note that this subroutine can be viewed as a generalization the BFS tree algorithm in the sense that if we let $\vec w^s(uv)=1$ for all nodes $s$ and edge $uv$ (in this case, $\zero(G, \cW)=1$, then this algorithm will behave exactly like the BFS tree algorithm. However, for the more general case, we will insert a {\em waiting time} of $\zero(G, \cW)$ between each step.


In particular, when a node $u$ receives a message $(s, \ell)$, it does the followings.
%
First, in {\bf Line~\ref{line:BFS style start}}, it checks whether this is the first time it receives any message of the form $(s, \ell')$.
%
If this is the first time, then it knows that $\dist_{G, \vec w^s}(s, u)=\ell$, as in {\bf Line~\ref{line:BFS style compute distance}} (we show that this is correct in Lemma~\ref{lem:correctness of light apsp} below).


%Next, in {\bf Line~\ref{line:check light}}, node $u$ will proceed only if one of the following conditions hold: (1) $\ell=0$ or (2) $u$ is $w_i$-light, i.e. $|S_{w_i}(u)|\leq \sqrt{n}$. The purpose of the first condition is to allow $u$ to proceed, regardless of whether it is $w_i$-light or $w_i$-heavy when it receives a message to itself, which is sent to activate Algorithm~\ref{algo:sim bfs} (as in Line~\ref{line:delay start} of Algorithm~\ref{algo:light apsp}).
%
%The second condition is used because we want to find distances only between $w_i$-light pairs of nodes. We will show that it suffices to let a node to proceed only when it is light.


Next, in {\bf Line~\ref{line:forward message}}, node $u$ forwards the same message $(s, \ell)$ it receives to all neighbors along edges of weight zero in $\vec w^s$. This is to make sure that all nodes $v$ such that $\dist_{G, \vec w^s}(u,v)=0$ knows the current distance $\dist_{G, \vec w^s}(s, u)$. If such $v$ has not received any $(s, \ell')$ earlier, then it also sets $\dist_{G, \vec w^s}(s, v)=\ell$, by Line~\ref{line:BFS style compute distance} (Lemma~\ref{lem:correctness of light apsp} guarantees the correctness).

Finally, in {\bf Line~\ref{line:bfs style send message}}, node $u$ waits until time $\tau_s+(\ell+\vec w^s(uv))\zero(G, \cW)$ before sending the message $(s, \ell+\vec w^s(uv))$ to node $v$. The reason $u$ has to wait until this time is that it wants to make sure that no message of the form $(s, \ell')$, for any $\ell'<\ell+\vec w^s(uv)$, will be sent to $v$ {\em after} it sends $(s, \ell+\vec w^s(uv))$ to $v$. This is to guarantee that $v$ will correctly set $\dist_{G, \vec w^s}(s, v)$ to $(s, \ell+\vec w^s(uv))$ if it has not received any message $(s, \ell')$, for any $\ell'<\ell+\vec w^s(uv))$, {\em earlier}. In addition to waiting, $u$ also sends the message to $v$ only when $\ell+\vec w^s(uv)\leq K$. This is because we are only interested the distance up to $K$.


%This is similar to Line~\ref{line:bfs send message} of Algorithm~\ref{algo:bfs} where $u$ waits until time  $\tau_\vartheta+\ell+w_i^\vartheta(uv)$ before sending the message, except that there is an extra $\sqrt{n}$ term. This term is used to ensure that all nodes in $S_{ w_i}(u)$ already receive the message $(\vartheta, \tau_\vartheta, \ell)$ (by the process in Line~\ref{line:forward message}). In fact, this term will ensure that all nodes {\em in all light supernodes of distance $\ell$ from $\vartheta$} will receive such message (we will prove this shortly, in Lemma~\ref{lem:correctness of light apsp}). Thus, the message $(\vartheta, \tau_\vartheta, \ell+i)$, for any $i$, will be synchronously sent out at the same time $\tau_\vartheta+(\ell+i)\sqrt{n}$.
%
%Additionally, node $u$ will send a message to node $v$ {\em only if} $\ell+w_i^\vartheta(\vartheta, v)\leq 2n$. This is to make sure that Algorithm~\ref{algo:sim bfs} stops sending a message at time $\tau_\vartheta+n\sqrt{n}$. Sending a message after this time is unnecessary and could interrupt the communication of other algorithms (recall that we run Algorithm~\ref{algo:sim bfs} from many nodes $\vartheta$ simultaneously).

%As stated in Line~\ref{line:fail}, we say that Algorithm~\ref{algo:sim bfs} {\em fails} if some node $u$ cannot send a message at the desired time. This can happens in two cases: (1) In Line~\ref{line:forward message}, $u$ cannot send a message immediately. (2) In Line~\ref{line:bfs style send message}, $u$ cannot send a message $(\vartheta, \tau_\vartheta, \ell+w_i^\vartheta(uv))$ at time $\tau_\vartheta+(\ell+w_i^\vartheta(uv))\sqrt{n}$. The only possibility that any of these cases happens is when many copies of Algorithm~\ref{algo:sim bfs} (started at different nodes) want to send a message through the same node at the same time. We will shortly show that this is unlikely (due to the random delay). Before we doing so, let us first analyze Algorithm~\ref{algo:sim bfs} by assuming that it does not fail.

%The following lemma (proof in Appendix) guarantees the correctness of Algorithm~\ref{algo:multi weight k apsp}, assuming that there is no congestion.

%\paragraph{Analysis when there is no congestion}

\medskip Assuming that there is no congestion (i.e., all messages are sent successfully), the correctness of Algorithm~\ref{algo:multi weight k apsp} can be guaranteed as in the following lemma.
%
\begin{lemma}[Proof in Appendix~\ref{sec:omitted proofs}]\label{lem:correctness of light apsp}\label{LEM:CORRECTNESS OF LIGHT APSP}
Assume that there is no congestion. For any nodes $s$ and $v$, the followings hold.
\begin{enumerate}[noitemsep]
\item $u$ does not receive message $(s, \ell)$ for any $\dist_{G, \vec w^s}(s, u)$.
\item $u$ receives message $(s, \dist_{G, \vec w^s}(s, u))$ before round $\tau_s+(\dist_{G, \vec w^s}(s, u)+1)\zero(G, \cW)$
\end{enumerate}
\end{lemma}
%
%\begin{observation}\label{observe:runtime of algo:multi weight k apsp}
%Assume that there is no congestion. Algorithm~\ref{algo:multi weight k apsp} finishes sending messages at time $t_0+n+K\zero(G, \cW)$.
%\end{observation}
%\begin{proof}
%By the condition on Line~\ref{line:bfs style send message}, all nodes stop sending a message at time $\max_{s\in V(G)} \tau_s+K\zero(G, \cW)$. By Line~\ref{line:generate random delay start} and \ref{line:t_0}, $\tau_s\leq t_0+r_s\leq t_0+n$ for any $s$.
%\end{proof}
%

%\begin{corollary}\label{lem:runtime of light apsp}
%Algorithm~\ref{algo:light apsp} finishes Line~\ref{line:BFS style start} in $\tilde O(n\sqrt{n})$ time.
%\end{corollary}

\paragraph{Congestion Analysis}  We show that it is unlikely that Algorithm~\ref{algo:multi weight k apsp} sends many messages on one edge at the same time. In particular, we show that, with high probability, there will be at most $\log n$ messages of the form $(s, \ell)$ sent through each edge in each round.  Our analysis follows an idea in \cite{LeightonMR94}, using the special property of Algorithm~\ref{algo:multi weight k apsp} that each node $u$ sends message $(s, \ell)$ at most {\em once}.
%
\begin{lemma}[Congestion]\label{lem:no congestion}
The probability that there exists an edge $uv$ and a set $\mset=\{(s_j, \ell_j)\}_{1\leq j\leq k}$ of $k>\log n$ messages such that all messages in $\mset$ are sent on $uv$ at the same time is $O(1/n^2)$.
\end{lemma}
\begin{proof}[Sketch](Full Proof in Appendix~\ref{sec:omitted proofs}) First, observe that, in Algorithm~\ref{algo:multi weight k apsp}, for any neighboring nodes $u$ and $v$, $u$ sends message of the form $(s, \ell)$ to $v$ {\em at most once} for each $s$. In fact, this message is exactly $(s, \dist_{w^s}(s, u)+w^s(uv))$. %
Observe further that the time that $u$ sends to $v$ message $(s, \dist_{w^s}(s, u)+w^s(uv))$ is determined by $\tau_s$. Using these facts, it can be shown that the probability that there exists nodes $u$ and $v$, time $t$, and set $\mset=\{(s_j, \ell_j)\}_{1\leq j\leq k}$  of $k>\log n$ messages, such that $u$ wants to send all messages in $\mset$ at time $t$, is at most
{
\begin{align}
\sum_{k=1+\log n}^{n} 3Kn^3 \binom{n}{k}\left(\frac{1}{n}\right)^k\,.\label{eq:prob congestion happens short}
\end{align}
}
%
%We end the proof by upper bounding Eq.\eqref{eq:prob congestion happens}.
%
Note that for any $0<b<a$, $\binom{a}{b}\leq (ae/b)^b$. Thus, Eq.\eqref{eq:prob congestion happens short} is at most
%
\begin{align}
\sum_{k=1+\log n}^{n} 3Kn^3\left(\frac{ne}{k}\right)^k\left(\frac{1}{n}\right)^k \leq 3Kn^4 \left(\frac{e}{\log n}\right)^{\log n}\label{eq:congestion probability short}
\end{align}
%
Note that we can assume that $K=\poly(n)$ since the largest edge weight is $\poly(n)$. For large enough $n$, (i.e., $(\log n)^{\log n}\geq 4Kn^6$), Eq.\eqref{eq:congestion probability short} will be bounded by $O(1/n^2)$ as desired.
\end{proof}
%
Thus, by allowing $\log n$ extra rounds between each step of the BFS-Style subroutine in Algorithm~\ref{algo:multi weight k apsp}, we can ensure that Algorithm~\ref{algo:multi weight k apsp} can send all messages it wants, with high probability. In this case, the BFS-Style subroutine finishes in $O(K\zero(G, \cW)\log n)$ rounds. Moreover, the algorithm can detect when it cannot send a message and can switch to the trivial $O(m)$-time algorithm where it aggregates all information to one node. We conclude with the following running time.

\begin{lemma}[Running Time]\label{observe:runtime of algo:multi weight k apsp}
Assuming that there is no congestion. Algorithm~\ref{algo:multi weight k apsp} with $\log n$ extra time between each step of the BFS-Style subroutine finishes sending messages at time $t_0+n+K\zero(G, \cW)\log n$ with high probability.
\end{lemma}
\begin{proof}
By the condition on Line~\ref{line:bfs style send message}, all nodes stop sending a message at time $\max_{s\in V(G)} \tau_s+K\zero(G, \cW)\log n$ (the extra $\log n$ factor is because we allow $\log n$ extra time). By Line~\ref{line:generate random delay start} and \ref{line:t_0}, $\tau_s\leq t_0+r_s\leq t_0+n$ for any $s$. The lemma follows.
\end{proof}



\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Previous version of the above lemma
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:no congestion}
The probability that there exists an edge $\overrightarrow{uv}$ and a set $\mset=\{(\vartheta_j, \tau_{\vartheta_j}, \ell_j)\}_{1\leq j\leq k}$ of $k>\log n$ messages such that all messages in $\mset$ are sent on $\overrightarrow{uv}$ at the same time is at most $1/n^2$.
\end{lemma}
\begin{proof}
First, observe that, in Algorithm~\ref{algo:sim bfs}, for any neighboring nodes $u$ and $v$, $u$ sends message of the form $(\vartheta, \tau_\vartheta, \ell)$ to $v$ {\em at most once}. In fact, this message is exactly $(\vartheta, \tau_\vartheta, \dist_{w_i^\vartheta}(\vartheta, u)+w_{i}^\vartheta(\overrightarrow{uv})$.
%
To see this, not that due to the condition in Line \ref{line:BFS style start}, node $u$ sends messages to its neighbors only when it receives $(\vartheta, \tau_\vartheta, \ell))$ for the first time, and it sends only one message to each neighbor (due to Line~\ref{line:forward message} and \ref{line:bfs style send message}).

Observe further that the time that $u$ sends to $v$ message $(\vartheta, \tau_\vartheta, \dist_{w_i^\vartheta}(\vartheta, u)+w_{i}^\vartheta(\overrightarrow{uv}))$ is determined by $\tau_\vartheta$. This is simply because Algorithm~\ref{algo:sim bfs} is deterministic.


Now we claim that the probability that there exists nodes $u$ and $v$, time $t$, and set $\mset=\{(\vartheta_j, \tau_{\vartheta_j}, \ell_j)\}_{1\leq j\leq k}$  of $k>\log n$ messages, such that $u$ wants to send all messages in $\mset$ at time $t$, is at most
{\small
\begin{align}
\sum_{k=1+\log n}^{n} (3n^3\log n) \binom{n}{k}\left(\frac{1}{n\log n^2}\right)^k\left(1-\frac{1}{n\log n^2}\right)^{n-k}\,.\label{eq:prob congestion happens}
\end{align}
}
To see this, consider any neighboring nodes $u$ and $v$, and let $t$ be any time during the computation. We will analyze the probability that $u$ wants to send more than $\log n$ messages to $v$ at the same time. To simplify the analysis, let us also assume that for all node $\vartheta$, there is a message $(\vartheta, \tau_\vartheta, \ell)$, for some $\tau_\vartheta$ and $\ell$, sent from $u$ to $v$ in some round. The probability that we analyze will be lower in the general case where there exists some node $\vartheta$ such that message $(\vartheta, \tau_\vartheta, \ell)$, for any $\tau_\vartheta$ and $\ell$, is never sent from $u$ to $v$.

Let $\mset$ be a set of $k$ messages. Recall that $\tau_{\vartheta}$, for any node $\vartheta$, has $n\log n^2$ possible values, due to the random number $r(S_{w_i}(\vartheta))$ added to the starting time of Algorithm~\ref{algo:sim bfs} in Line~\ref{line:delay start} of Algorithm~\ref{algo:light apsp}. Thus, for any node $\vartheta$, the probability that $u$ sends message $(\vartheta, \tau_\vartheta, \ell)$ to $v$ at time $t$ is at most $\frac{1}{n\log n^2}$. It follows that the probability that $u$ sends all messages in $\mset$ to $v$ at time $t$ is at most $(\frac{1}{n\log n^2})^k$. Moreover, the probability that $u$ sends no messages, among all $n$ possible messages for $n$ different values of $\vartheta$, that is not in $v$ is at most $(1-\frac{1}{n\log n^2})^{n-k}$. Thus, the probability that the messages sent from $u$ to $v$ at round $t$ is exactly those in $\mset$ is at most
\begin{align}
(\frac{1}{n\log n^2})^k(1-\frac{1}{n\log n^2})^{n-k}.\label{eq:prob exactly mset is sent}
\end{align}
Recall that there are $\binom{n}{k}$ possible sets $\mset$ since $u$ sends a message of the form $(\vartheta, \tau_\vartheta, \ell)$ at most once, for each node $\vartheta$. Also note that we can assume that $t_0\leq t\leq t_0+n\log n^2+2n\leq t_0+3n\log n$, where $t_0$ is the starting time of Algorithm~\ref{algo:light apsp}, as in Line~\ref{line:t_0} of Algorithm~\ref{algo:light apsp}. This is because Algorithm~\ref{algo:sim bfs} starts before round $t_0+n\log n^2$ and stops sending messages after $2n$ rounds. By summing Eq.\eqref{eq:prob exactly mset is sent} over all possible $n^2$ pairs of nodes, $3n\log n$ values of $t$, all possible values of $k$, and $\binom{n}{k}$ possible sets $\mset$, we obtain Eq.\eqref{eq:prob congestion happens}.

We end the proof by upper bounding Eq.\eqref{eq:prob congestion happens}. For note that for any $0<b<a$, $\binom{a}{b}\leq (ae/b)^b$. Thus, Eq.\eqref{eq:prob congestion happens} is at most
{\small
\begin{align*}
&\sum_{k=1+\log n}^{n} (3n^3\log n) \left(\frac{ne}{k}\right)^k\left(\frac{1}{n\log n^2}\right)^k\left(1-\frac{1}{n\log n^2}\right)^{n-k}\\ %\,.\label{eq:prob congestion happens 2}
&\leq \sum_{k=1+\log n}^{n} (3n^3\log n) \left(\frac{e}{k\log n^2}\right)^k\left(1-\frac{1}{n\log n^2}\right)^{n-k}\\
\end{align*}
}
For large enough $n$ (so that $(\log n)^{\log n}\geq 3n^4\log n$, the quantity above is bounded by $1/n$ as desired.
\end{proof}
\end{comment}

%\paragraph{Sharing information within supernodes (Line~\ref{line:end of light} of Algorithm~\ref{algo:light apsp})}


\begin{comment}
\paragraph{Summary of the Analysis} Let us summarize the analysis we show in this subsection. By Lemma~\ref{lem:no congestion} guarantee that all executions of Algorithm~\ref{algo:sim bfs} (starting at different nodes $\vartheta$) does not fail with high probability. Given that Algorithm~\ref{algo:sim bfs} does not fail, it will finish by time $\max_{\vartheta\in V(G)} \tau_\vartheta+(2n+1)\sqrt{n}$ by Lemma~\ref{lem:runtime of sim bfs}. This is less than $t_0+2n+(2n+1)\sqrt{n}$ since $\tau_\vartheta=t_0+n+r(S_{w_i}(\vartheta))<t_0+2n$. The following corollary follows.
%This means that
\begin{corollary}\label{cor:line delay start finish time}
Line~\ref{line:delay start} of Algorithm~\ref{algo:apsp} finishes before round $t_0+2n+(2n+1)\sqrt{n}$.
\end{corollary}
%
At the time Line~\ref{line:delay start} of Algorithm~\ref{algo:apsp} finishes, the distances between many $w_i$-light pairs are already discovered. In particular, Lemma~\ref{lem:correctness of light apsp} implies that for every $w_i$-light pair $(\vartheta, u)$, some node in $S_{w_i}(u)$ knows the value of $\dist_{w_i^\vartheta}(\vartheta, u)$, and if $u$ is $w_i$-light then $u$ knows the value of $\dist_{w_i^\vartheta}(\vartheta, u)$.
%
Note that we have not yet find  $\dist_{w_i^\vartheta}(\vartheta, u)$ between all pair of $w_i$-light pairs $(\vartheta, u)$. We will do so next.


\subsection{Finishing finding distances between light pairs (Line~\ref{line:end of light} of Algorithm~\ref{algo:light apsp})}\label{sec:light-final}
In Line~\ref{line:end of light} of Algorithm~\ref{algo:light apsp}, we make sure that for every $w_i$-light pair $(\vartheta, u)$, node $u$ knows the value of  $\dist_{w_i^\vartheta}(\vartheta, u)$. This is done by simply aggregating the messages $(\vartheta, \tau_\vartheta, \ell)$ from each node $u$ to the representative node of supernode $S_{w_i}(u)$. This can be done in $\tilde O(n)$ rounds since there are at most $n$ messages in each supernode (some of these messages may be stored by many nodes in the supernode): For each node $u$, the set of messages that nodes in $S_{w_i}(u)$ have is exactly  $\{(\vartheta, \tau_\vartheta, \dist_{w_i^\vartheta}(\vartheta, u) \mid \mbox{$(\vartheta, u)$ is $w_i$-light}\}$. TO ADD MORE DETAIL.

We conclude this section with the following theorem, which easily follows our analysis.

\begin{theorem}
Algorithm~\ref{algo:light apsp} find the distances between all $w_i$-light pairs with probability at least $\tilde \Omega(1-1/n)$. Moreover, it always finish in $\tilde O(n\sqrt{n})$ time.
\end{theorem}
\end{comment}


==> arXiv/omitted_proofs.tex <==
\section{Omitted Proofs}\label{sec:omitted proofs}

\subsection{Proof of Claim~\ref{claim:w_i time}}
{
\renewcommand{\thetheorem}{\ref{claim:w_i time}}
\begin{claim}[Restated]
Line~\ref{line:w_i} of Algorithm~\ref{algo:apsp} can be done in $O(n)$ time.
\end{claim}
\addtocounter{theorem}{-1}
}
\begin{proof}%[of Claim~\ref{claim:w_i time}]
Observe that each node $u$ can compute $\vec w_i^x({uv})$ and $\vec w_i^x({vu})$ if it knows the values of $\dist_{G, w_{i+1}}(x, v)$ for all nodes $x$ and neighbors $v$. Assuming that the algorithm successfully solves \apsp on $(G, w_{i+1})$ in Iteration $i+1$, the algorithm do the task in Line~\ref{line:w_i} easily in $\tilde O(n)$ time: Every node $v$ simultaneously send to all neighbors the values of $\dist_{G, w_{i+1}}(x, v)$, for all nodes $x$. Since there are $n$ messages of size $\tilde O(1)$ to be sent, this can be done in $O(n)$ time. Then, every node $u$ will have all necessary information to compute $\vec w_i^x({uv})$ and $\vec w_i^x({vu})$.
\end{proof}

\begin{comment}
\paragraph{Time:} We claim that a message of ID $i$ first reaches a node $j$ by time between in $[\dist(i,j), \dist(i,j)+i]$. This is clearly true for $i=1$ since no other message will block a message of ID $1$; thus, this message acts like a BFS algorithm. Now, assume that this is true for any $1\geq k<i$, we will show that this is true for $i$ as well. Suppose for the sake of contradiction there exists a node $j$ such that the message of ID $i$ first reaches $j$ at time $t>\dist(i, j)+i$.

Let $a$ be the ID of the last message that blocks message of ID $i$ before $i$ reaches node $j$. By the scheduling rule, $a<i$. Let $b$ and $t'$ be the node and time that this happens. Note that $t'\leq \dist(a, b)+a$. Also note that $t-t'-1=\dist(b, j)$ since message $i$ is not blocked after it leaves $b$ at time $t'+1$ and it will reach $j$ by a shortest $b$-$j$ path). Consider two cases.

{\em Case 1: $\dist(a, b)\leq \dist(i, b)$. In this case,
$$t=\dist(b, j)+t'+1\leq \dist(b, j)+\dist(a, b)+a+1\leq \dist(b, j)+\dist(i, b)+a+1\leq \dist(i, j)+a+1???$$

\begin{claim}
A message of ID $i$ first reaches a node $j$ by time between in $[\dist(i,j), \dist(i,j)+i]$.
\end{claim}
\end{comment}


\section{Proof of Lemma~\ref{lem:correctness of light apsp}}

{\renewcommand{\thetheorem}{\ref{lem:correctness of light apsp}}
\begin{lemma}[Restated]
Assume that is no congestion. For any nodes $s$ and $v$, the followings hold.
\begin{enumerate}[noitemsep]
\item $u$ does not receive message $(s, \ell)$ for any $\dist_{G, \vec w^s}(s, u)$.
\item $u$ receives message $(s, \dist_{G, \vec w^s}(s, u))$ before round $\tau_s+(\dist_{G, \vec w^s}(s, u)+1)\zero(G, \cW)$
\end{enumerate}
\end{lemma}
\addtocounter{theorem}{-1}
}

\begin{proof}
We prove this by induction. First, we show that all claims hold when $\ell=0$. To see this, observe that the message $(s, 0)$ will be sent through any path $P=\langle s=x_0, x_1, \ldots, x_k=u\rangle$ such that $\vec w^s(P)=0$, by Line~\ref{line:forward message} of Algorithm~\ref{algo:multi weight k apsp}. Thus, every node $u$ such that $\dist_{G, \vec w^s}(s, u)=0$ will receive this message. Moreover, such message will take $|P|\leq \zero(G, \cW)$ rounds to reach $u$. 

Now we consider any $L>0$. We show that if the lemma holds for any $\ell<L$, then it holds for $\ell=L$ as well. Throughout the proof, we let $u$ be any node such that $\dist_{G, \vec w^s}(s, u)=L$.

Now we prove the first claim. Assume that the first claim does not hold, i.e. some node $u$ such that $\dist_{G, \vec w^s}(s, u)=L$ receives a message $(s, \ell')$, for some $\ell'<\ell$. We call this event a {\em bad} event. Let $t$ be the earliest time that a bad event occurs, and let $u^*$ be the node that receives such message $(s, \ell')$ at time $t$. Let $v$ be the node that sends message $(s, \ell')$ to $u$ at time $t$. This means that $v$ has received message $(s, \ell'-\vec w^s(vu))$ at time $t'<t$. Note that $\dist_{G, \vec w^s}(s, v)\geq \dist_{G, \vec w^s}(s, u)-\vec w^s(vu)>\ell'-\vec w^s(vu)$. This means that a bad event also occurs at time $t'$, contradicting the assumption that $t$ is the earliest time that a bad event occurs. This proves the first claim for $\ell=L$.

Now we prove the second claim. Let $P=\langle s=x_0, x_1, \ldots, x_k=u\rangle$, for some $k$, be any shortest $s$-$u$ path in $(G, \vec w^s)$ (i.e., $\vec w^s(P)=L$).
%
Let $j$, where $0\leq j\leq k$, be the largest number such that $\dist_{G, \vec w^s}(x_j, u)>0$. Note that such $j$ exists since $\dist_{G, \vec w^s}(s, u)=L>0$. Moreover, by the definition of $x_j$, $\vec w^s(x_jx_{j+1})>0$, $\dist_{G, \vec w^s}(s, x_{j+1})=L$, and $\dist_{G, \vec w^s}(s, x_j)=L-\vec w^s(x_jx_{j+1})<L$. Let $\ell'=\dist_{G, \vec w^s}(s, x_j)$. 

%; otherwise, $\dist_{G, \vec w_i^\vartheta}(\vartheta, u)=0$ by Lemma~\ref{lem:scaling preserves zero}, contradicting the assumption that $\dist_{G, \vec w_i^\vartheta}(\vartheta, u)=L>0$ .
%
%Let $\ell'=\dist_{G, \vec w_i^\vartheta}(\vartheta, x_j)$. 

%Since $\dist_{G, \vec w_i^\vartheta}(\vartheta, x_{j+1})=L$ (since $x_{j+1}\in S_{w_i}(u)$) and $\vec w_i^\vartheta(x_jx_{j+1})>0$ (by Lemma~\ref{lem:scaling preserves zero}), $\ell'<L$. 

%Moreover, $x_j$ is $w_i$-light since $P$ is a $w_i$-light path. 


By the induction hypothesis, the first message that $x_j$ receives is $(s, \ell')$, and $x_j$ receives this message before round $\tau_s+(\ell'+1)\sqrt{n}$. Thus, it will send message $(s, L)$ to $x_{j+1}$ at time $\tau_s+L\zero(G, \cW)$ (by Line~\ref{line:bfs style send message} of Algorithm~\ref{algo:multi weight k apsp}). Assuming that the algorithm does not fail to send messages, $x_{j+1}$ will receive message $(s,  L)$ at time $\tau_s+L\zero(G, \cW)$. Then, the message $(s, L)$ will be sent from $x_{j+1}$ to $u$ in $\zero(G, \cW)$ rounds through a path $P'=\langle x_{j+1}, \ldots, x_k=u\rangle$ (since $\vec w^s(P')=0$). This proves the second claim.  
\end{proof}


%Thus, by the induction hypothesis, the first message that $x_j$ receives is $(\vartheta, \tau_\vartheta, \ell')$, and $x_j$ receives this message before round $\tau_\vartheta+(\ell'+1)\sqrt{n}$. Thus, it will send message $(\vartheta, \tau_\vartheta, L)$ to $x_{j+1}$ at time $\tau_\vartheta+L\sqrt{n}$ (by Line~\ref{line:bfs style send message} of Algorithm~\ref{algo:sim bfs}). Assuming that the algorithm does not fail, $x_{j+1}$ will receive message $(\vartheta, \tau_\vartheta, L)$ at time $\tau_\vartheta+L\sqrt{n}$. This proves the second claim since $x_{j+1}\in S_{\vec w_i^\vartheta}(u)$.

%Now we prove the third claim. By the second claim, some node $v$ in $S_{w_i}(u)$ receives  $(\vartheta, \tau_\vartheta, L)$ at time $L$. By the first claim, $v$ has not received any message of the form $(\vartheta, \tau_\vartheta, \ell')$ for any $\ell'<L$; so, by Line~\ref{line:forward message} of Algorithm~\ref{algo:sim bfs}, $v$ sends message $(\vartheta, \tau_\vartheta, L)$ to all neighbors in $S_{w_i}(v)=S_{w_i}(u)$. These neighbors again send the same message to their neighbors in $S_{w_i}(u)$ since they have not received any  message of the form $(\vartheta, \tau_\vartheta, \ell')$ for any $\ell'<L$, by the first claim. This process is repeated until message $(\vartheta, \tau_\vartheta, \ell')$ reach $u$. The time it takes for this message to reach $u$ is at most $|S_{w_i}(u)|-1$ rounds, which is at most $\sqrt{n}-1$ since $u$ is $w_i$-light. So, the message will reach $u$ before round $\tau_\vartheta+L\sqrt{n}+\sqrt{n}$ as in the third claim.


%\begin{proof}[of Lemma~\ref{lem:runtime of algo:multi weight k apsp}]
%\danupon{Have to change}
%By Line~\ref{line:bfs style send message} of Algorithm~\ref{algo:multi weight k apsp}, any message of the form $(s, \ell)$ must be such that $\ell\leq K$. This message is sent only at round $\tau_s+K\zero(G, \cW)$ in Line~\ref{line:bfs style send message}. This message is then sent for at most another $\zero(G, \cW)-1$ rounds along edges of weight zero in $w^s$, as in Line~\ref{line:forward message}. The lemma follows.
%\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ----------  The subsection below is already moved --------------
%
%\subsection{Proof of Lemma~\ref{lem:no congestion}}
%
%{\renewcommand{\thetheorem}{\ref{lem:no congestion}}
%\begin{lemma}[Restated]
%The probability that there exists an edge $uv$ and a set $\mset=\{(s_j, \ell_j)\}_{1\leq j\leq k}$ of $k>\log n$ messages such that all messages in $\mset$ are sent on $uv$ at the same time is $O(1/n^2)$.
%\end{lemma}
%\addtocounter{theorem}{-1}
%}
%\begin{proof}
%First, observe that, in Algorithm~\ref{algo:multi weight k apsp}, for any neighboring nodes $u$ and $v$, $u$ sends message of the form $(s, \ell)$ to $v$ {\em at most once} for each $s$. In fact, this message is exactly $(s, \dist_{G, \vec w^s}(s, u)+\vec w^s(uv))$.
%%
%To see this, note that due to the condition in Line \ref{line:BFS style start}, node $u$ sends messages to its neighbors only when it receives $(s, \ell)$ for the first time, and it sends only one message to each neighbor (due to Line~\ref{line:forward message} and \ref{line:bfs style send message}).
%
%Observe further that the time that $u$ sends to $v$ message $(s, \dist_{G, \vec w^s}(s, u)+\vec w^s(uv))$ is determined by $\tau_s$. This is simply because Algorithm~\ref{algo:multi weight k apsp} is deterministic.
%
%
%Now we claim that the probability that there exists nodes $u$ and $v$, time $t$, and set $\mset=\{(s_j, \ell_j)\}_{1\leq j\leq k}$  of $k>\log n$ messages, such that $u$ wants to send all messages in $\mset$ at time $t$, is at most
%{
%\begin{align}
%\sum_{k=1+\log n}^{n} 3Kn^3 \binom{n}{k}\left(\frac{1}{n}\right)^k\,.\label{eq:prob congestion happens}
%\end{align}
%}
%To see this, consider any neighboring nodes $u$ and $v$, and let $t$ be any time during the computation. Let $\mset$ be a set of $k$ messages. Recall that $\tau_{s}$, for any node $s$, has $n$ possible values, due to the random number $r_s\in [0, n-1]$ added to the starting time of the BFS-style subroutine. Thus, for any node $s$, the probability that $u$ sends message $(s, \ell)$, for some $\tau_s$ and $\ell$, to $v$ at time $t$ is at most $\frac{1}{n}$ (since there is only one value of $\tau_s$ that will make will make $u$ send $(s, \ell)$ exactly at time $t$). It follows that the probability that $u$ sends all messages in $\mset$ to $v$ at time $t$ is at most
%\begin{align}
%\left(\frac{1}{n}\right)^k.\label{eq:prob exactly mset is sent}
%\end{align}
%Note that there are $\binom{n}{k}$ possible sets $\mset$ where each set have $s_1\neq s_2\neq \ldots$. This is because $u$ sends a message of the form $(s, \ell)$ at most once to $v$, for each node $s$. Also note that we can assume that $t_0\leq t< t_0+n+(K+1)\zero(G, \cW)$, where $t_0$ as in Line~\ref{line:t_0} of Algorithm~\ref{algo:multi weight k apsp}. This is because the last round that Algorithm~\ref{algo:multi weight k apsp} can start is $t_0+r_s< t_0+n$, and it stops sending messages after time $\tau_s+(K+1)\zero(G, \cW)\leq t_0+n+(K+1)\zero(G, \cW)$ rounds. Thus, there are at most $n+(K+1)\zero(G, \cW)\leq 3Kn$ possible values of $t$.
%
%By summing Eq.\eqref{eq:prob exactly mset is sent} over all possible $n^2$ pairs of nodes, $3Kn$ possible values of $t$, all possible values of $\log n<k\leq n$, and $\binom{n}{k}$ possible sets $\mset$, we obtain Eq.\eqref{eq:prob congestion happens}.
%
%We end the proof by upper bounding Eq.\eqref{eq:prob congestion happens}. Note that for any $0<b<a$, $\binom{a}{b}\leq (ae/b)^b$. Thus, Eq.\eqref{eq:prob congestion happens} is at most
%%
%\begin{align}
%\sum_{k=1+\log n}^{n} 3Kn^3\left(\frac{ne}{k}\right)^k\left(\frac{1}{n}\right)^k \leq 3Kn^4 \left(\frac{e}{\log n}\right)^{\log n}\label{eq:congestion probability}
%\end{align}
%%
%Note that we can assume that $K=\poly(n)$ since the largest edge weight is $\poly(n)$. For large enough $n$, (i.e., $(\log n)^{\log n}\geq 4Kn^6$), Eq.\eqref{eq:congestion probability} will be bounded by $O(1/n^2)$ as desired.
%\end{proof}


==> arXiv/overview3.tex <==
\section{Proof Overview \& Organization}\label{sec:overview}
All our algorithms share the following same high-level idea: We start with a {\em pseudo-polynomial} time algorithm whose running time depends on edge weights. We then apply this algorithm on the network with {\em modified} edge weights in a suitable way that this algorithm is fast. How we modify edge weights depends on the problems. We illustrate this idea starting from the simple ideas for approximation algorithms to the more complicated ones for the exact algorithm.

\subsection{Approximation Algorithms}

...

Now, to approximate $D(G, w)$, we first compute $D'$ that $2$-approximates $D(G, w)$; this can be done easily by solving \sssp from an arbitrary source. We then use $D'$ to change $w$ slightly to $w'$ where $w'(uv)=\lceil \frac{2n w(uv)}{\epsilon D'}\rceil$. We then show the following.
\begin{proposition}\label{prop:approx diameter guarantee}{\sc (Properties of $D(G, w')$; Proof in Appendix~\ref{sec:approx diameter})}
$D(G, w')\leq (1+2/\epsilon)n$ and $D(G, w)$ $\leq$ $\frac{\epsilon D'}{2n}\times D(G, w')$ $\leq$ $(1+\epsilon)D(G, w).$
\end{proposition}
% and we can use $D(G, w')$ to approximate $D(G, w)$.
Thus, we can apply Proposition~\ref{prop:pseudopoly time} with $K=(1+2/\epsilon)n$ on $D(G, w')$ to compute $D(G, w')$. Then, we output $D'\times D(G, w')$ as an approximate solution of $D(G, w)$. 

The case of approximating $\rad(G, w)$ is done almost identically. We only have to change to way we compute $D'$ slightly. 

\medskip To solve \apsp approximately, we have to ``guess'' the distance between each pair of nodes in the form $2^i$. For each guessed distance $2^i$, we again change weight $w$ slightly to $w'_i$ where $w'_i(uv)=\lceil\frac{ 2nw(uv)}{\epsilon2^i}\rceil$. An important property that we will show is the following.
%
\begin{proposition}\label{prop:approx apsp guarantee}{\sc (Property of $(G, w'_i)$; Proof in Appendix~\ref{sec:approx apsp})}
For any nodes $u$ and $v$, if we let $\tilde d_{G, w}(u, v)$ = $\min_i  \frac{\epsilon D'_{i}}{2n}\times\dist^{(1+2/\epsilon)n}_{G, w'_i}(u, v)$, then $\dist_{G, w}(u, v)\leq \tilde d_{G,w}(u, v)\leq (1+\epsilon)\dist_{G, w}(u, v)$.
\end{proposition}
Thus, we can approximate \apsp on $(G, w)$ by applying Proposition~\ref{prop:pseudopoly time} on $(G, w_i)$ with $K=(1+2/\epsilon)n$, for all $i$.


%in such a way that for all nodes $u$ and $v$, $\dist_{G, w'}(u, v)\geq \dist_{G, w}(u, v)$; moreover, if $\dist_{G, w}(u, v)\leq 2^i$, then $\dist_{G, w'}(u, v)\leq \dist_{G, w}(u, v)$. We then apply Lemma~\ref{lem:pseudopoly time} with $K=2^i$

\subsection{Exact Algorithm}
Like the approximation algorithms, our exact algorithm relies on the idea of modifying edge weights and applying a pseudo-polynomial time algorithm to get an approximate solution. To arrive at the exact solution, we keep refining the modified edge weights until we finally get the correct solution. The refining step leads to many complications (especially, we will have to deal with edges of weight zero). For this reason, we need a more general version of Proposition~\ref{prop:pseudopoly time}, as well as several other ideas.


\paragraph{Weight Scaling} A naturally way to modify edge weights is by {\em weight scaling}. Recall that the general idea of this technique is to approximate \apsp on $(G, w_i)$, where $w_i(uv)=\lfloor w(uv)/2^i\rfloor$ for a large enough $i$ so that $w_i(uv)$ is small enough to run a pseudo-polynomial time algorithm for \apsp\footnote{We note that obstructions on the way make us end up using a slightly different way to do weight scaling, as we will discuss later in this section.}. We then keep reducing $i$ until $i=0$. While we cannot ensure that $w_i(uv)$ is small for a small $i$, we can use the solution on $(G, w_{i+1})$ to solve \apsp on $(G, w_i)$ quickly.

%write each edge weight $w(uv)$ as a binary string\footnote{We note that we will end up using something a bit different called {\em positive binary string}, as will be discussed later in this section.} $b_\beta(uv)$, $b_{\beta-1}(uv)$, $\ldots$, $b_0(uv)$, where $b_i(uv)\in \{0, 1\}$ for all $i$, and $w(uv)=\sum_{i=0}^\beta b_i(uv)2^i$. We then solve the problem in {\em iterations}, starting from Iteration $\beta$ {\em down to} Iteration $0$. In Iteration $i$, we solve \apsp on graph $(G, w_i)$, where $w_i(uv)$ is defined to be $b_\beta(uv)\ldots b_i(uv)$ in base two. The point is that the solution from Iteration $i+1$ will help speeding up our algorithm on Iteration $i$.

%To see why this technique is useful, first observe that $D(G, w_\beta)\leq n$ since $w_\beta(uv)\in \{0, 1\}$ for every edge $uv$. Thus, a pseudo-polynomial time algorithm (like that in Lemma~\ref{lem:pseudopoly time}) will be fast on $(G, w_\beta)$, except that there could be zero weights; this is one extra thing our new pseudo-polynomial time algorithm has to deal with.

More specifically, we use the solution of \apsp on $(G, w_{i+1})$ to change the weight $w_i$ into a {\em collection} of {\em asymmetric nonnegative} weight assignments $\cW_i=\{\vec w^s_i\}_{s\in V(G)}$. We emphasize that $\vec w_i$ is asymmetric and it could assign value zero to some edges. %This is the source of some complications we will face later. 

An important property of $(G, \cW_i)$ is that it has a small ``diameter'' in the following sense. Define the {\em multi-weight diameter} of $(G, \cW_i)$, denoted by $\ecc(G, \cW_i)$, to be $\ecc(G, \cW_i)=\max_{s, u\in V(G)} \dist_{G, \vec{w}^s_i}(s, u)$. We show that the multi-weight diameter of $(G, \cW_i)$ is small (for an intuition, compare this to Proposition~\ref{prop:approx diameter guarantee}).
%
\begin{proposition}\label{prop:multi-weight diameter}\label{PROP:MULTI-WEIGHT DIAMETER}{\sc (Multi-Weight Diameter Bound; Proof in Section~\ref{sec:multi weight diameter bound})}
$\ecc(G, \cW_i)\leq 2n.$
\end{proposition}
%
Moreover, we show that solving the following {\em Multi-Weight $K$-\apsp} problem on $(G, \cW_i)$ is enough to solve \apsp on $(G, w_i)$.
%
\begin{definition}\label{def:multi weight apsp} {\sc (Multi-Weight $K$-APSP)} Given a network $G$, a set of non-negative edge weights $\cW=\{\vec{w}^s\}_{s\in V(G)}$, and a number $K$, we want every node $u$ to know $\dist^K_{G, \vec w^s}(s, u)$ for all nodes $s$.
\end{definition}
%
Specifically, we can show that, for any $K\geq \ecc(G, \cW_i)$,\footnote{Again, obstructions on the way make us end up using something more complicated than what we show here. See Proposition~\ref{prop:d prime}.} 
\begin{align}\label{eq:ideal w_i recovery}
\dist_{G, w_i}(s, u)=2\dist_{G, w_{i+1}}(s, u)+\dist^K_{G, \vec w_i^s}(s, u)\,.
\end{align}
By Proposition~\ref{prop:multi-weight diameter}, $K=2n$ is enough. Moreover, we already know $\dist_{G, w_{i+1}}(s, u)$ since we assume that \apsp on $(G, w_{i+1})$ is already solved in the previous iteration.
%
Thus, our job is to solve multi-weight $K$-\apsp in time as close to $D(G, \cW_i)$ as possible. We do not achieve exactly this. The reason is that $\vec w$ could assign value zero to some edges. Let us first explain what we can do.

%We will end up solving this problem on another graph and have to do something more.


%In what follows, we  show an algorithm that depends on $D(G, \cW_i)$ and another parameter. We will then use this algorithm to ``partly'' solve the problem (as much as the other parameter allows).  Then, we slightly modify the weight scaling scheme to get an extra property of $(G, \cW_i)$ that allows us to use the new algorithm to remove the extra parameter.

%
%There is another thing that the new algorithm has to deal with: Observe that for any $i<\beta$, we could have $D(G, w_i)\gg n$. Thus, we need another way to solve \apsp on $(G, w_i)$. To do this, we will use the solution of \apsp on $(G, w_{i+1})$ to change the weight $w_i$ into a collection of {\em asymmetric} weight functions $\cW_i=\{\vec w^s_i\}_{s\in V(G)}$. An important property is that it has a small {\bf Generalized Diameter}, defined as $\ecc(G, \cW_i)=\max_{s, u\in V(G)} \dist_{G, \vec{w}^s_i}(s, u)$; in particular, in Lemma~XXX, we will show that
%\begin{align}\ecc(G, \cW_i)&=O(n)\label{eq:ecc bound}\end{align}
%


%we wish to solve the following problem on $(G, \cW_i)$.
%

%
%We will show that solving this problem on $(G, \cW_i)$ is enough for us to solve \apsp on $(G, w_i)$ (cf. Lemma~XXX).
%
% We won't state this since we'll actually solve the special case of multi-weight apsp
%\begin{lemma}
%Let $T_i$ be the time need to solve multi-weight \apsp on $(G, \cW_i)$. Then,
%\end{lemma}
%
%Solving this problem is an important subroutine in our algorithm.
%
%We now discuss how to do this with an algorithm whose running time depending on the multi-weight diameter $\ecc(G, \cW_i)$. In what follows, we will show an algorithm that depends on another parameter. Then, we slightly modify the weight scaling to get an extra property of $(G, \cW_i)$ that allows us to use this algorithm to remove the extra parameter.

\paragraph{Solving Multi-Weight $K$-APSP} Instead of an algorithm for multi-weight \apsp on $(G, \cW)$ whose running time solely depends on $\ecc(G, \cW)$, we show that there is an algorithm whose running time depends on $\ecc(G, \cW)$ and another parameter called the {\em longest zero path length}. This parameter is defined as $\zero(G, \cW)=\max_{P, s} |V(P)|$ where the maximization is over all simple paths $P$ and node $s$ in $G$ such that $\vec{w}^s(P)=0$; in other words, $\zero(G, \cW)$ is the number of nodes in the longest path of distance zero for some weight function in $\cW$. We show the following.
%
%
\begin{proposition}\label{prop:pseudopoly multi-weight}\label{PROP:PSEUDOPOLY MULTI-WEIGHT}{\sc (Pseudo-Polynomial Time Algorithm for Multi-Weight APSP; Proof in Section~\ref{sec:multi-weight k-apsp})}
The multi-weight $K$-\apsp problem on input $(G, \cW)$ can be solved by an algorithm that takes $\zero(G, \cW)$ as an input and, with high probability, finishes in $O(K\zero(G, \cW)\log n+n)$ time.
\end{proposition}
%
As an example, observe that we can use Proposition~\ref{prop:pseudopoly multi-weight} to prove Proposition~\ref{prop:pseudopoly time} with an extra $\log n$ factor by letting $\vec w^s=w$ for all $s$; in this case, $\ecc(G, \cW)=D(G, w)$ and $\zero(G, \cW)=1$.

The idea behind Proposition~\ref{prop:pseudopoly multi-weight} is similar to Proposition~\ref{prop:pseudopoly time}: we treat $(G, \vec w^s)$ as an unweighted graph and grow BFS trees from every node in $G$. For an intuition, first consider when $(G, \cW)$ has {\em no} zero edge weight. In this case, we can simply grow BFS trees to solve the problem. Each BFS algorithm will finish in $O(K)$ time, if it does not conflict with other algorithms (in sending messages). To avoid conflicts, we will use the {\em random delay} technique \cite{LeightonMR94}. (We cannot use the same deterministic rule as Proposition~\ref{prop:pseudopoly time} since there are many edge weights.) This causes the algorithm to be randomized and have an extra $\log n$ term in the running time. The total time will be $O(K\log n+n)$ in this case.

In order to deal with zero weights, we will grow the BFS tree from each node $s$ and pretend that edges $uv$ such that $\vec w^s(uv)=0$ are not in the network. Additionally, between each step of growing the BFS tree we will have an extra time of $O(\zero(G, \cW))$ rounds where nodes will communicate through edges of weight zero only. This extra time is used for nodes to send its distance along paths of distance zero (that is why we need $O(\zero(G, \cW))$ extra time). So, the total time changes from $O(K\log n+n)$ to $O(K\zero(G, \cW)\log n+n)$. 
%
We now discuss how to use Proposition~\ref{prop:pseudopoly multi-weight} to solve \apsp on $(G, w_i)$.

%Applying Lemma~\ref{lem:general pseudopoly}, we get the running time of $O(\ecc(G, \cW_i)\zero(G, \cW_i)\log n)$ for solving multi-weight \apsp on $(G, \cW_i)$. Next, we show how to replace $\zero(G, \cW_i)$ by $\sqrt{n}$.




\paragraph{Solving APSP on $(G, w_i)$} First, let us note that we will use a weight scaling scheme that is a bit different from the standard one we explain earlier: we will use what we call a {\em positive binary representation} to construct our weight scaling scheme (see Section~\ref{sec:scaling} for details). The advantage of this non-standard scheme is that we can convert $(G, w_i)$ to $(G, \cW_i)$ with the following additional property.
%
\begin{proposition}\label{prop:clustering}\label{PROP:CLUSTERING}{\sc (Node Clustering; Proof in Sec.~\ref{sec:clustering})}
Nodes in $G$ can be partitioned into {\em clusters} $C_1, C_2, \ldots, C_k$, for some $k$, such that 
%(1) the subgraph of $G$ induced by any cluster $C_j$ is connected, and (2) 
for any $\vec w\in \cW_i\cup \{w_i\}$, $\dist_{G, \vec w}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster.
%(2) $\dist_{G, \vec w_i^s}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster.
%\begin{itemize}[noitemsep]
%\item the subgraph of $G$ induced by any cluster $C_j$ is connected, and 
%\item for every node $s$, $\dist_{G, \vec w_i^s}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster.
%\end{itemize}
Moreover, such partition can be found in $O(n)$ time (in the end, every node $u$ knows which cluster every node $v$ is in; i.e., it knows the set $\{(v, \rep(C_j) \mid v\in C_j)\}$ where we define $\rep(C_j)$ to be $\rep(C_j)=\min_{v\in C_j} v$).
%; see details in Line~\ref{line:clustering} of Algorithm~\ref{algo:apsp}).% (see Sec.~\ref{sec:main algo} and Line~\ref{line:clustering} of Algorithm~\ref{algo:apsp} for details).%(as a result, for every node $u$ in each cluster $C_j$ knows iand its neighbors are in, as well as the sizes of these clusters).
\end{proposition}
%
%Line~\ref{line:clustering} of Algorithm~\ref{algo:apsp} for details of what the algorithm in the above lemma computes and
%
We exploit the above proposition to solve \apsp on $(G, w_i)$ in $O(n\sqrt{n}\log n)$ time as follows. Define $H$ to be a subgraph of $G$ where we delete all edges between two nodes in every cluster $C_i$ such that $|C_i|\geq \sqrt{n}$ (we call such $C_i$ a {\em big cluster}). Observe that the longest zero path length of $(H, \cW_i)$ is $\zero(H, \cW_i)\leq \sqrt{n}$ since any path of distance zero must be contained in one cluster. We then apply the algorithm in Proposition~\ref{prop:pseudopoly multi-weight} with $K=2n$ (so that $K\geq \ecc(G, \cW_i)$, by Proposition~\ref{prop:multi-weight diameter}) to solve multi-weight $(2n)$-\apsp on $(H, \cW_i)$ in $O(n\sqrt{n}\log n)$ time. We can use this result to get a solution to \apsp on $(G, w_i)$ for {\em some} pairs of nodes. In particular, we show that if the distance between two nodes in $(G, w_i)$ is preserved in $(H, w_i)$, then we can compute this distance correctly.
%
\begin{proposition}\label{prop:d prime}\label{PROP:D PRIME}{\sc (Property of $\dist'$; Proof in Section~\ref{sec:d prime})}
%Given the solutions to \apsp on $(G, w_{i+1})$ and $(2n)$-\apsp on $(H, \cW_i)$, without communication, every node $u$ can compute, for all nodes $v$, value $d'(u, v)$ such that $d'(u, v)\geq \dist_{G, w_i}(u, v)$, and if $\dist_{H, w_i}(u, v)=\dist_{G, w_i}(u, v)$, then $d'(u, v)=\dist_{G, w_i}(u, v)$.
%
Consider any $K\geq \ecc(G, \cW_i)$. For any nodes $s$ and $u$, let $d'(s, u)=2\dist_{G, w_{i+1}}(s, u)+\dist^{K}_{H, \vec w_i^s}(s, u)$. Then, $d'(u, v)\geq \dist_{G, w_i}(u, v)$. Moreover, if $\dist_{H, w_i}(u, v)=\dist_{G, w_i}(u, v)$, then $d'(u, v)=\dist_{G, w_i}(u, v)$.
\end{proposition}
%
To get a solution of \apsp on $(G, w_i)$, we characterize which pairs get the correct solution from the previous step. For an intuition, consider a pair $(u, v)$ such that there is a shortest $u$-$v$ path in $(G, w_i)$ that does not use any node in the big clusters. Intuitively, this path is also a shortest path in $(H, w_i)$ and thus the previous step will compute $d'(u, v)=\dist_{G, w_i}(u, v)$. Thus, we just have to ``fix'' those shortest paths involving nodes in big clusters. To do this, we show that it is enough to broadcast $d'(u, v)$ for all nodes $u$ in big clusters and all other nodes $v$, which can be shown to require $O(n\sqrt{n})$ time using the fact that there are at most $\sqrt{n}$ big clusters.

In particular, we show that each node $u$ can construct a weighted graph $(G'_u, w')$. Each node of $G'_u$ is in the form $c_j$ and represents each cluster $C_j$. Edge weight $w'(c_jc_{j'})$ corresponds to the distance $d'(C_jC_{j'})$ between clusters $C_j$ and $C_{j'}$ that node $u$ has learned so far. Then, we show that $u$ can compute its distance to every other nodes in $(G, w_i)$ using the following proposition.
%
\begin{proposition}\label{prop:G prime}\label{PROP:G PRIME}{\sc (Property of $(G_u', w')$; Proof in Section~\ref{sec:G prime})}
For any nodes $u$ and $v$, let $C_j$ and $C_{j'}$ be clusters that contain $u$ and $v$, respectively. Then, $\dist_{G, w_i}(u, v)=\dist_{G'_u, w'}(c_j, c_{j'}).$
\end{proposition}



\paragraph{Organization} In Section~\ref{sec:main algo}, we outline the main exact algorithm which formally defines some terms, as well as shows how to put all propositions introduced in this section together. The rest sections are devoted to proving the propositions.
%From Section \ref{sec:multi weight diameter bound} to \ref{sec:G prime}, we proof Proposition~\ref{prop:multi-weight diameter} to \ref{prop:G prime}, respectively.
%
Due to space limitation, the details of our approximation algorithms are shown in Appendix~\ref{sec:approx}. We also prove our lower bound (Observation~\ref{observe:lower bound}) in Appendix~\ref{sec:lower bound}. 

%%
%\begin{lemma}\label{lem:same zero}
%For any $s$, $u$ and $v$, $\dist_{G, w_i}(u, v)=0$ if and only if $\dist_{G, w^s_i}(u, v)=0$.
%\end{lemma}
%%
%We exploit the above property to solve \apsp on $(G, w_i)$ in $O(n\sqrt{n}\log n)$ time as follows. First, we partition nodes into {\em clusters}: nodes $u$ and $v$ are in the same cluster if and only if $\dist_{G, w_i}(u, v)=0$.
%%
%For any cluster having more than $\sqrt{n}$ nodes (``big clusters''), we delete all edges between two nodes in such cluster. Let $G'$ be the resulting graph. We then use Lemma~\ref{lem:same zero} to show that the longest zero path length $\zero(G', \cW_i)$ is $O(\sqrt{n})$ (essentially, this is because there is no edge of weight zero crossing between two clusters for any weight function in $\cW_i$). We then apply the algorithm in Lemma~\ref{lem:pseudopoly multi-weight} to solve multi-weight \apsp on $(G', \cW_i)$ in $O(\ecc(G, \cW)\sqrt{n}\log n)$ time, which is $O(n\sqrt{n}\log n)$ by \eqref{eq:ecc bound}. We use this result to get a solution to \apsp on $(G', w_i)$.
%%
%Finally, we show that, to solve \apsp on $(G, w_i)$ it is enough to broadcast $\dist_{G', w_i}(u, v)$ for all node $u$ in big clusters and all nodes $v$. Using the fact that there are at most $\sqrt{n}$ big clusters, we show that we only have to broadcast $O(n\sqrt{n})$ messages, which will take $O(n\sqrt{n})$ time in total.

%\paragraph{Running Time without $\zero(G, \cW_i)$ (Sec. XXX)} To eliminate $\zero(G, \cW_i)$ from the running time, we modify the weight scaling scheme slightly to make $(G, \cW_i)$ have the following {\em same-zero} property:
%%
%\begin{definition}[Same-Zero] We say that $(G, \cW=\{w^s\}_{s\in V(G)})$ is {\em same-zero} if for any nodes $u$, $v$, $s$ and $s'$, $\dist_{G, w_i^s}(u,v)=0$ $\implies$ $\dist_{G, w_i^{s'}}(u,v)=\dist_{G, w_i^{s'}}(v, u)=0$.
%\end{definition}
%%
%%\begin{align}
%%%\forall u, v, s, s':\ \ \vec{w}_i^s(uv)=0 \iff \vec{w}_i^{s'}(uv)=\vec{w}_i^{s'}(vu)=0\,.
%%\forall u, v, s, s':\ \ \dist_{G, w_i^s}(u,v)=0 \iff \dist_{G, w_i^{s'}}(u,v)=\dist_{G, w_i^{s'}}(v,u)=0\,.
%%\label{eq:property that gives cluster}
%%\end{align}
%%
%We guarantee the following.
%\begin{lemma}\label{lem:pseudopoly same-zero multiweight}{\sc (Pseudo-Polynomial Time Algorithm for Multi-Weight APSP on Same-Zero Inputs)}
%The multi-weight \apsp problem on input $(G, \cW)$ that is same-zero can be solved by an algorithm that, with high probability, finishes in $O(\ecc(G, \cW)\sqrt{n}\log n)$ time.
%\end{lemma}
%%
%The above lemma is proved by exploiting the same-zero property as follows. First, we partition nodes into {\em clusters}: nodes $u$ and $v$ are in the same cluster if and only if $\dist_{G, w_i^s}(u, v)=0$ for all $s$. Then, for any cluster having more than $\sqrt{n}$ nodes (``big cluster''), we delete all edges between two nodes in such cluster. Let $G'$ be the resulting graph. We then use the same-zero property to show that the longest zero path length $\zero(G', \cW_i)$ is $O(\sqrt{n})$ (essentially, this is because the same-zero property implies that there is no edge of weight zero crossing between two clusters). We then apply the algorithm in Lemma~\ref{lem:pseudopoly multi-weight} to solve multi-weight \apsp on $(G', \cW_i)$ in $O(\ecc(G, \cW)\sqrt{n}\log n)$ time. Finally, we show that we can solve multi-weight \apsp on $(G, \cW_i)$ by broadcasting distances between nodes in big clusters and all other nodes in ...

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%
%\section{Proof Overview \& Organization - OLD}
%
%A simple fact that plays a crucial role in previous algorithms on unweighted networks \cite{HolzerW12,PelegRT12} is that we can solve \apsp by efficiently parallelizing multiple BFS algorithms. Our algorithms also rely on this idea, but we will need several other ideas to deal with weights. Let us illustrate these ideas by first explaining our simple approximation algorithms before discussing what we need for the exact algorithm.
%
%%We illustrate our ideas starting from explaining our simple approximation algorithms before discussing what we need for the exact algorithm.
%
%\paragraph{Simple Approximation Algorithms (Sec. XXX)} The first idea of our approximation algorithms is that we can solve \apsp in {\em pseudo-polynomial time}:
%%
%\begin{lemma}\label{lem:weak pseudopoly time}
%\apsp on any weighted network $(G, w)$, with positive integral edge weights, can be solved in $O(n+D(G, w))$ time.
%\end{lemma}
%%
%This lemma simply exploits the fact that we can view $(G, w)$ as an unweighted network $G'$ by replacing an edge $uv$ of weight $w(uv)$ by a $u$-$v$ path of length $w(uv)$. We then grow BFS trees in $G'$ from every node in $V(G)$ to find distances between nodes in $V(G)$ and other nodes in $V(G')$.
%%
%Since we run many BFS algorithms in parallel, there could be {\em conflicts}; i.e., many BFS algorithms may want to send messages on the same edge at the same time. There are many ways to resolve this (e.g. Lemma~XXX). A nice way to do this efficiently and deterministically is to use the rule in the {\em $S$-Shortest Paths} algorithm of \cite{HolzerW12} to resolve the conflicts. This leads to an $O(D(G, w)+n)$ running time.
%
%Now, to get a linear-time $(1+\epsilon)$-approximation algorithm for computing $D(G, w)$, we simply change weight $w$ slightly to $w'$ so that $D(G, w')=O(n)$, and we can use $D(G, w')$ to approximate $D(G, w)$. We then apply Lemma~\ref{lem:weak pseudopoly time} to compute $D(G, w')$.
%
%To approximate \apsp, we need a slightly stronger version of Lemma~\ref{lem:weak pseudopoly time} where we want to find distances of nodes that are {\em nearby}:
%%
%\begin{lemma}\label{lem:strong pseudopoly time}
%For any weighted network $(G, w)$ with positive integral edge weights and integer $K$. There is an $O(n+K)$-time algorithm such that, at its termination, any nodes $u$ and $v$ know the value of $\dist(u, v)$ if $\dist(u, v)\leq K$; otherwise, they know that $\dist(u, v)> K$.
%\end{lemma}
%%
%The above lemma is obtained by modifying Lemma~\ref{lem:weak pseudopoly time} slightly (thus, it relies on the same idea of growing multiple BFS trees and use the rule of \cite{HolzerW12} to resolve conflicts).
%%
%We then approximate \apsp by ``guessing''the distance between each pair of nodes and apply Lemma~\ref{lem:strong pseudopoly time} on $(G, w')$ for some appropriate approximate weight $w'$ (using the guessed number). The guessing process introduces a $\log n$ factor in the running time; so we have a running time of $O(n\log n)$.
%
%
%\paragraph{Exact Algorithm (Sec XXX-XXX)}
%
%\paragraph{Parallel Breadth-First Search (BFS)} A simple fact that plays a crucial role in previous algorithms on unweighted networks \cite{HolzerW12,PelegRT12}, as well as our algorithm, is that we can solve \sssp using a BFS algorithm that treats an edge of weight $k$ as a path of length $k$. This algorithm works on {\em directed weighted} graphs. Its running time is bad, but it is easy to run many such algorithms in parallel. Since understanding this simple algorithm is important in understanding the rest of the paper, we describe this algorithm in Algorithm~\ref{algo:bfs} and briefly discuss its properties.
%%
%\begin{algorithm}
%\caption{{\sc WeightedBfs}$(\vec{G}, w, s, \Delta)$}\label{algo:bfs}
%{\bf Input:} Directed graph $\vec G$ with positive integral weight $w$ and source node $s$.
%
%{\bf Output:} Every node $v$ such that $\dist_{\vec G, w}(s, v)\leq \Delta$ knows $\dist_{\vec G, w}(s, v)$.
%
%%\medskip\textit{\textbf{Preprocessing}}
%%\medskip
%
%\begin{comment}
%\noindent\begin{algorithmic}[1]
%
%%\algstore{bfstwo}
%%\algrestore{bfstwo}
%
%\State Let $t$ be the time this algorithm starts.
%
%\State Initially, source node $s$ triggers the algorithm to start by sending a message $(s, t, 0)$ to itself.
%
%\algstore{bfsone}
%\end{algorithmic}
%
%
%\noindent\begin{itemize}[noitemsep]
%\item Let $t$ be the time this algorithm starts.
%
%\item Initially, source node $s$ triggers the algorithm to start by sending a message $(s, t, 0)$ to itself.
%\end{itemize}
%\end{comment}
%
%\medskip $\bullet$ Let $t$ be the time this algorithm starts. Initially, source node $s$ triggers the algorithm to start by sending a message $(s, t, 0)$ to itself.
%
%
%
%%\medskip\textit{\textbf{Main subroutine:}}
%
%$\bullet$ When a node $u$ receives a message $(s, \tau, \ell)$ for some $\ell$, it does the following.
%
%\begin{algorithmic}[1]
%
%%\algrestore{bfsone}
%
%\If{$u$ has {\em not} already received $(s, \tau, \ell')$ for some $\ell'$}\label{line:BFS start}
%
%\State $u$ now knows that $\dist_{\vec G, w}(s, u)=\ell$.\label{line:bfs compute distance}
%
%%\State $u$ sends through all directed edges $\overrightarrow{uv}$ a message $(s, t, \ell+w(\overrightarrow{uv}))$ at time $t+\ell+w(\overrightarrow{uv})$.\label{line:bfs send message}
%
%\State For any neighboring nodes $v\notin S_{G, w_i}(u)$ of $u$ such that $\ell+w(uv)\leq \Delta$, node $u$ sends to $v$ a message $(s, \tau, \ell+w(uv))$ at time $\tau+\ell+w(uv)$.\danupon{Address this change in the texts}\label{line:bfs send message}
%
%\EndIf\label{line:BFS end}
%
%\end{algorithmic}
%\end{algorithm}
%
%The algorithm simply makes sure that the first message that every node $v$ receives is $(s, t, \ell)$, where $\ell=\dist_{G, w}(s, v)$, and this message is received at time $t+\ell$. This fact, besides guaranteeing the correctness and time complexity, also guarantees that each node sends a message through each edge only {\em once}.
%%
%%\begin{claim}\label{lem:bfs style}
%%Algorithm~\ref{algo:bfs} solves \sssp from source $s$ in $O(D_{G, w}(s))$ time. Moreover, every node $u$ sends a message through each directed edge $\overrightarrow{uv}$ at most once.
%%\end{claim}
%%
%This gives us a hope that we can execute Algorithm~\ref{algo:bfs} from different sources in parallel since no edge will be ``overused''. In the case of unweighted undirected graphs, the cute deterministic scheduling of \cite{HolzerW12,PelegRT12} achieves exactly this.
%
%The problem of running Algorithm~\ref{algo:bfs} on weighted graphs $(G, w)$ is that it takes too much time to finish; i.e. it takes $O(D_{G, w}(s))=O(\max_v \dist_{G, w}(s,v))$ time. In what follows, we explain several ideas that we use to run algorithms similar to Algorithm~\ref{algo:bfs} faster, in parallel.
%
%
%%Our algorithm will use several ideas to enable us to run an algorithm similar to Algorithm~\ref{algo:bfs} faster and in parallel. One fact to note here: our algorithm will end up running parallel algorithms on {\em different directed weighted graphs}, and we will need the random delay technique of Leighton, Maggs, and Rao \cite{LeightonMR94} instead of the deterministic scheduling of \cite{HolzerW12,PelegRT12}.
%%
%%We now explain what we need to be able to run parallel BFS algorithms.
%
%
%
%\paragraph{Weight Scaling (details in Section \ref{sec:scaling})} A natural way to make Algorithm~\ref{algo:bfs} finish faster is to run it on $(G', w')$ such that $D_{G', w'}(s)$ is small. This leads us to the use of {\em weight scaling}. Recall that the general idea of this technique is to write each edge weight $w(uv)$ as a binary string $b_\beta(uv)$, $b_{\beta-1}(uv)$, $\ldots$, $b_0(uv)$, where $b_i(uv)\in \{0, 1\}$ for all $i$, and $w(uv)=\sum_{i=0}^\beta b_i(uv)2^i$. We then solve the problem in {\em iterations}, starting from Iteration $\beta$ {\em down to} Iteration $0$. In Iteration $i$ we solve the problem on graph $(G, w_i)$, where $w_i(uv)$ is defined to be $b_\beta(uv)\ldots b_i(uv)$ in base two. The point is that the solution from Iteration $i+1$ will help speeding up our algorithm on Iteration $i$.
%
%To see why this technique is useful, first observe that $D_{G, w_\beta}(s)\leq n$ since $w_\beta(uv)\in \{0, 1\}$ for every edge $uv$. Thus, we might be able to finish Algorithm~\ref{algo:bfs} quickly on $(G, w_\beta)$. For graphs $(G, w_i)$ in other iterations, we could have $D_{G, w_i}(s)> n$; however, we can use the solution on $(G, w_{i+1})$ to ``adjust'' the weight $w_i$ so that a similar property holds, without changing the solution. To be precise, we show that for any $i$ we can get a collection of $n$ directed weighted graphs $\{(\vec{G}, w_i^u)\}_{u \in V(G)}$ such that, for any node $u$, the $D_{\vec{G}, w^u_i}(u)=O(n)$. Moreover, any shortest $u$-$v$ path in $(\vec G, w^u_i)$ is also a shortest $u$-$v$ path in $(G, w_i)$.
%
%Note that we still cannot directly apply Algorithm~\ref{algo:bfs} at this point. The reason is that the graphs we obtain have zero edge weights (graph $(G, w_\beta)$ is one obvious example). One modification we have to make is to use what we call {\em positive binary representation} instead of the binary representation (the advantage of this will be clear when we prove Lemma~\ref{lem:properties of scaling}). Besides this, we have to introduce the notion of {\em supernodes} and modify Algorithm~\ref{algo:bfs} to deal with supernodes, as we discuss next.
%
%\paragraph{Supernodes (details in Section~\ref{sec:supernode})} We deal with zero weights using the following simple idea: We group nodes linked by edges of weight zero as a set called {\em supernode}. After identifying nodes in the same supernode (equivalently, contracting all edges of weight zero), we will not have zero weight left. Thus, we can run Algorithm~\ref{algo:bfs} on this graph.
%
%For example, let us consider any graph $(G, w)$ with weights zero and one. Let $(G', w')$ be the graph resulting from contracting all edges of weight zero. We call $(G, w')$ a {\em supergraph} and its nodes {\em supernodes}. Each supernode represents a set of nodes in $(G, w)$ linked by edges of weight zero. Observe that $(G', w')$ is an unweighted graph, on which Algorithm~\ref{algo:bfs} can be executed quickly.
%
%However, we cannot really execute Algorithm~\ref{algo:bfs} on $(G', w')$ directly, since it is {\em not a real network}. So, instead, we will execute an algorithm on $(G, w)$ that {\em simulates the Algorithm~\ref{algo:bfs} on supergraph $(G', w')$}.
%
%\paragraph{Simulating BFS by Light and Heavy Nodes (details in Section~\ref{sec:light}-\ref{sec:heavy})} Simulating Algorithm~\ref{algo:bfs} on supergraphs is still not a trivial task. The difficulty is that Algorithm~\ref{algo:bfs} heavily relies on the fact that all nodes are synchronized; i.e., every node sends the message $(s, t, \ell)$ at the same time $t+\ell$. While this is easy to do on a real network, it becomes harder on supergraphs since different supernodes in $(G', w')$ correspond to different number of nodes in $(G, w)$, which requires different time for ``internal communication'' (where nodes in the same supernode communicate to each other). One idea to fix this problem is to wait until the last supernode is ready to send the message $(s, t, \ell)$. This, however, requires some extra communication, which makes it hard to run many algorithms in parallel. Another obvious approach is to wait for $O(n)$ time between the execution of each round of Algorithm~\ref{algo:bfs}; i.e., instead of sending message $(s, t, \ell)$ at time $t+\ell$, we will send it at time $t+O(n\ell)$. The waiting time is used to guarantees that all supernodes finish their internal communication and are ready to send the message before the next round starts. This, however, increases the running time to $O(n^2)$.
%
%Our solution modifies the second approach by dividing supernodes into {\em light} and {\em heavy} supernodes: light supernodes are supernodes corresponding to at most $\sqrt{n}$ nodes, and heavy supernodes are the rest. We then simulate Algorithm~\ref{algo:bfs} {\em only until we find a heavy supernode that is not the source node}. In other words, a heavy supernode that is not $s$ will not execute Line~\ref{line:bfs send message} of Algorithm~\ref{algo:bfs}. This allows us to reduce the waiting time to $O(\sqrt{n})$. Thus, we will finish Algorithm~\ref{algo:bfs} in $O(n\sqrt{n})$ time. In fact, we can concurrently simulate many copies of Algorithm~\ref{algo:bfs} using different supernodes as a source in $O(n\sqrt{n})$ time!
%
%The algorithm above almost solves the problem except that it does not promise to find the distance between every pair of supernodes. In particular, it only finds the distance between {\em light pairs of supernodes} -- pairs of supernodes $u$ and $v$ such that some shortest $u$-$v$ paths in supergraph $(G', w')$ contains no internal heavy supernodes.
%
%We show that the above problem can be quickly fixed: We claim that the distance between other pairs can be found if every heavy supernode can broadcast to all other nodes what it obtains in the previous step (i.e., its distance to some other supernodes). This can be easily done in $O(n\sqrt{n})$ time because there are only $\sqrt{n}$ supernodes, each having at most $n$ pieces of information to broadcast.
%
%\paragraph{Parallelizing Algorithm~\ref{algo:bfs}}  We note that our algorithm cannot use the deterministic scheduling of \cite{HolzerW12,PelegRT12} since it runs simulations of Algorithm~\ref{algo:bfs} on many weighted directed graphs in parallel. Instead, we will use the random delay technique of Leighton, Maggs, and Rao \cite{LeightonMR94} and exploit the fact that Algorithm~\ref{algo:bfs} sends at most one message on each edge. This is the only part that relies on randomness.

%
%\medskip The main algorithm is described in Algorithm~\ref{algo:apsp}. We slowly explain this algorithm in detail in the next few sections.



==> arXiv/prelim.tex <==
\section{Preliminaries}\label{sec:prelim}

\subsection{Problems}

\subsection{Graph Theoretic Definitions}

%\subsection{Skeleton}




==> arXiv/sssp.tex <==
%\section{$\tilde O(n^{\frac{1}{2}+\frac{1}{2k}})$-Time $(k+\epsilon)$-Approximation Algorithm for SSSP}
\section{Algorithms on General Networks}
\label{sec:sssp}
\danupon{The time vs approx in the title is not the best we can say.}


%\subsection{Overview}
%
%%\paragraph
%
%
%%************************************
%
%\subsubsection*{Landmarks and Overlay Networks}
%The next step of our algorithm is randomly picking {\em landmarks}, a technique commonly used in data structure (e.g. XXX). Let $\ell$ be a parameter, which could depend on $n$. Every node in the network becomes a landmark with probability $n/\ell$ (thus, there will be $\ell$ landmarks in expectation). By a standard argument, it can be shown that if a node knows $(n/\ell)$-hop ....
%
%
%\begin{lemma}
%Let $h=n/\ell$. if a node $u$ knows $\dist_{G, w}^h(u, v)$
%
%\end{lemma}
%
%
%
%
%Then, we approximate $\dist_{G, w}^h(u, v)$ between any landmark $u$ and  
%
%solve the $k$-source $h$-hop 
%
% \ref{thm:k-source h-hop sp}
%
% use the algorithm for
%************************************
%
%\subsubsection*{Spanner of Overlay Network}
%
%
%
%
%\subsection{$k$-Source $h$-Hop \ksp}\label{sec:k-source h-hop shortest paths}
%We recall \Cref{thm:k-source h-hop sp}: \khsp*

In this section, we present algorithms for \sssp and \apsp on general distributed networks, as stated in \Cref{thm:main sssp} and \Cref{thm:linear apsp}. First, observe that \apsp is simply a special case of the $h$-hop $k$-source shortest paths problem defined in \Cref{sec:bounded-hop mssp} where we use $h=k=n$. Thus, by \Cref{thm:k-source h-hop sp}, there is an $(1+o(1))$-approximation algorithm that solves \apsp in $\tilde O(k+h+D)=\tilde O(n)$ time with high probability. This immediately proves \Cref{thm:linear apsp}. 
%
%in \Cref{sec:apsp general}, we show that the linear-time \apsp algorithm follows as a corollary from the light-weight bounded-hop \sssp algorithm developed in \Cref{sec:light-weight bounded-hop sssp}. 
% 
The rest of this section is then devoted to showing a $\tilde O(n^{1/2}\diam^{1/4}+\diam)$-time algorithm for \sssp as in \Cref{thm:main sssp}, which require several non-trivial steps. 


%\subsection{Linear-Time algorithm for \apsp}\label{sec:apsp general}




\subsection{Reduction to Single-Source Shortest Path on Overlay Networks}\label{sec:skeleton}\label{sec:overlay}

In this section, we show that solving the single source shortest path problem on a network $(G, w)$ can be reduced to the same problem on a certain type of an {\em overlay network}, usually known as a {\em landmark} or {\em skeleton} (e.g. \cite{Sommer12-survey,LenzenP13}). 
%
In general, an overlay network $G'$ is a {\em virtual} network of nodes and logical links that is built on top of an underlying {\em real} network $G$; i.e., $V(G')\subset V(G)$ and an edge in $G'$ (a ``virtual edge'') corresponds to a path in $G$ (see, e.g., \cite{EmekFKKP12}). Its implementation is usually abstracted as {\em a routing scheme} that maps virtual edges to underlying routes. However, for the purpose of this paper, we do not need a routing scheme but will need the notion of {\em hop-stretch} which captures the number of hops in $G$ between two neighboring virtual nodes in $V(G')$, as follows.
%
%In general, an overlay network is a virtual network of nodes and logical links that is built on top of an existing network with the purpose of implementing a network service that is not available in the existing network. 
%
%
%\begin{definition}[Overlay network of stretch $\lambda$]\label{def:overlay}
%Consider any network $G$. For any $\lambda$, a weighted network $(G', w')$ is said to be an {\em overlay network on $G$ of stretch $\lambda$} if $V(G')\subseteq V(G)$ and $\dist_G(u, v)\leq \lambda$ for all $u, v\in V(G')$. We say that network $G$ {\em knows} $(G', w')$ if for every virtual edge $uv\in E(G')$, both $u$ and $v$ (as a node in $G$) knows the value of $w'(uv)$.  
%\end{definition}
%
%
\begin{definition}[Overlay network of hop-stretch $\lambda$]\label{def:overlay}
Consider any network $G$. For any $\lambda$, a weighted network $(G', w')$ is said to be an {\em overlay network of hop-stretch $\lambda$ embedded in $G$} if 
\begin{enumerate}
\item $V(G')\subseteq V(G)$,
\item $\dist_G(u, v)\leq \lambda$ for every virtual edge $uv\in E(G')$, and
\item for every virtual edge $uv\in E(G')$, both $u$ and $v$ (as a node in $G$) knows the value of $w'(uv)$.
\end{enumerate}  
\end{definition}

We emphasize that $\lambda$ captures the number of hops ($\dist_G(u, v)$) between two neighboring nodes $u$ and $v$, not the weighted distance ($\dist_{G, w}(u, v)$). The main result of this section is an algorithm to construct an overlay network such that, if we can solve the single-source shortest path problem on such network, we can solve the single-source shortest path on the whole graph: 

%\begin{proposition}
%In $O(...)$ time, can embed an overlay network $H$ such that small size, if every node in $V(G)$ knows $(1+o(1))$ approximate distance of $\dist_H(s, v)$ for all $v\in V(H)$ then ...
%\end{proposition}

\begin{proposition}[Main result of \Cref{sec:skeleton}: Reduction to an overlay network]\label{thm:skeleton}\label{thm:overlay network}
For any weighted graph $(G, w)$, source node $s$, and integer $\alpha$, there is an $\tilde O(\alpha+n/\alpha+D)$-time distributed algorithm that embeds an overlay network $(G', w')$ in $G$ such that, with high probability, 
\begin{enumerate} %[label=(\arabic{*})]
\item $s\in V(G')$,
\item $|V(G')|=\tilde O(\alpha)$, and
\item if every node $u\in V(G)$ knows a $(1+o(1))$-approximate value of $\dist_{G', w'}(s, v)$ for every node $v\in V(G')$, then $u$ knows the  $(1+o(1))$-approximate value of $\dist_{G, w}(s, u)$. 
\end{enumerate}
\end{proposition}
\begin{proof}
Our algorithm is as follows. First, every node $u$ selects itself to be in $V(G')$ with probability $\alpha/n$. Additionally, we always keep source $s$ in $V(G')$; this guarantees the first condition. Observe that $E[|V(G')|] = 1+(\alpha/n)\cdot (n-1) \leq 2\alpha$; so, by Chernoff's bound (e.g. \cite[Theorem 4.4]{MitzenmacherU05}), 
%\begin{align*}
$Pr[|(G')|\geq 12\alpha\log n] \leq 1/n.$
%\end{align*}
This proves the second condition. 
% and shows that  the running time so far is $\tilde O(|S|) = O(\alpha).$ 
%
To guarantee the last condition, we have to define edges and their weights in $G'$. To do this, we invoke an algorithm for the bounded-hop multi-source shortest path problem in \Cref{thm:k-source h-hop sp} (page \pageref{thm:k-source h-hop sp}), with nodes in $V(G')$ as sources and $h=n\log n/\alpha$ hops. By \Cref{thm:k-source h-hop sp}, the algorithm takes $\tilde O(|V(G')|+h+D)=\tilde O(\alpha+n/\alpha+D)$ time, and every node $u\in V(G)$ will know $\dist'_{G, w}(u, v)$ such that 
\[
\dist_{G, w}^{h}(u, v)\leq \dist'_{G, w}(u, v)\leq (1+o(1))\dist_{G, w}^{h}(u, v)
\]
for all $v\in V(G')$. For any $u, v\in V(G')$ such that $\dist'_{G, w}(u, v)<\infty$, we add edge $uv$ with weight $w'(u, v)=\dist'_{G, w}(u, v)$ to $G'$. Note that both $u$ and $v$ knows the existence and weight of this edge. This completes the description of an overlay network $(G', w')$ embedded in $G$. 

We are now ready to show the third condition, i.e., if a node $u\in V(G)$ knows a $(1+o(1))$-approximate value of $\dist_{G', w'}(s, v)$ for all $v\in V(G')$, then it knows a $(1+o(1))$-approximate value of $\dist_{G, w}(s, u)$. Consider any node $u\in V(G)$, and let 
$$P=\langle u=v_0, v_1, \ldots, v_k=s\rangle,$$ 
for some $k$, be a shortest path between $s$ and $u$ in $(G, w)$. Observe that if $k\leq n\log n/\alpha$, then $u$ knows $\dist'_{G, w}(u, v)$ which is a $(1+o(1))$-approximate value of $\dist_{G, w}(s, u)$, and thus the third condition holds even when $u$ does not know a $(1+o(1))$-approximate value of $\dist_{G', w'}(s, v)$ for any $v\in V(G')$. It is thus left to consider the case where $k\geq n\log n/\alpha$. 
%
Let $i_1 < i_2 < \ldots < i_t$ be such that $v_{i_1}, \ldots, v_{i_t}$ are nodes in $P\cap V(G')$. Let $i_0=0$ (i.e., $v_{i_0}=u$). We note the following simple fact, which is very easy and well-known (e.g. \cite{UllmanY91}). We provide its proof here only for completeness. 
%
\begin{lemma}[Bound on the number of hops between two landmarks in a path]\label{thm:landmark}
For any $j$, $i_j-i_{j-1}\leq n \log n/\alpha$, with probability at least $1-2^{-\beta n}$, for some constant $\beta>0$ and sufficiently large $n$.
\end{lemma}
\begin{proof}
We note a well-known fact that a set of random selected nodes $|V(G')|$ of size $\alpha$ will ``hit'' a simple path of length at least $cn\log n/|V(G')$, for some constant $c$, with high probability. To the best of our knowledge, this fact was first shown in \cite{GreenKnuth81book} and has been used many times in dynamic graph algorithms (e.g. \cite{DemetrescuFI05} and references there in). The following fact appears as Theorem 36.5 in \cite{DemetrescuFI05} (attributed to \cite{UllmanY91}). 
%
%\danupon{Say something from here (from \cite{DemetrescuFI05}) ``In this section we recall an intuitive combinatorial property of long paths in a graph. Namely, if we pick a subset S of vertices at random from a graph G, then a sufficiently long path will intersect S with high probability. This can be very useful in finding a long path by using short searches. To the best of our knowledge, the long paths property was first given in [21], and later on it has been used may times in designing efficient algorithms for transitive closure and shortest paths (see e.g., [9, 28, 41, 42]). The following theorem is from [41].}
%
%
\begin{fact}[Ullman and Yannakakis \cite{UllmanY91}]\label{thm:UllmanY} 
Let $S \subseteq V(G)$ be a set of vertices chosen uniformly at random. Then the probability that a given simple path has a sequence of more than $(cn\log n)/|S|$ vertices, none of which are from $S$, for any $c > 0$, is, for sufficiently large $n$, bounded by $2^{-\beta n}$ for some positive $\beta$.
\end{fact}
%
Using $S=V(G')$, which has size $\tilde \Theta(\alpha)$, we have that every subpath of $P$ of length at least $n\log n/\alpha$ contains a node in $V(G')$, with high probability. The lemma follows by union bouding over the subpaths of $P$.\danupon{I'm a bit sketchy here.} This completes the proof of \Cref{thm:landmark}.
\end{proof}
%
It follows from the above lemma that $u$ knows $\dist'_{G, w}(u, v_{i_1})$ and, for any $j\geq 1$, $v_{i_j}v_{i_{j+1}}$ is an edge in the overlay network $G'$ of weight $w'(v_{i_j}v_{i_{j+1}})=\dist'_{G, w}(v_{i_j}, v_{i_{j+1}})$, with probability at least $1-2^{-\beta n}$. Thus, with high probability, 
%
\[\dist_{G', w'}(v_{i_1}, s)\leq \sum_{j=1}^{k-1} \dist'_{G, w}(v_{i_j}, v_{i_{j+1}}).\] 
%
Since $u$ already knows $\dist'_{G, w}(u, v_{i_1})$, it can now compute  
%
\[\dist'_{G, w}(u, v_{i_1})+\sum_{j=1}^{k-1} \dist'_{G, w}(v_{i_j}, v_{i_{j+1}})\] 
%
which is at least $\dist_{G, w}(u, s)$ and at most $(1+o(1))\dist_{G, w}(u, s)$. We note one detail that, in fact, $u$ does not known which node is $v_1$, so it has to use the value of
% 
\[\min_{v\in V(G')} \dist'_{G, w}(u, v) + \dist_{G', w'}(v, s)\] 
%
as an estimate.\danupon{Vague} By union bounding over all nodes $u$, \Cref{thm:overlay network} follows.\danupon{I'm quite sketchy here.}
\end{proof}

\subsection{Reducing the Shortest Path Diameter of Overlay Network $(G', w')$}\label{sec:reduce spd overlay}
In this section, we assume that we are given an overlay network $(G', w')$ embedded in the original network $(G, w)$, as show in \Cref{thm:overlay network}. Our goal is to solve the single-source shortest path problem on $(G', w')$. Recall that $(G', w')$ has $|V(G')|=\tilde O(\alpha)$ nodes, for some parameter $\alpha$, which will be fixed later. Note that the shortest path diameter ($\spdiam(G, w)$) of $(G', w')$  might be as large as $|V(G')|=\tilde O(\alpha)$.\danupon{Should recall ``shortest path diameter''} Since the running time of our algorithm for single-source shortest path will depend on the shortest path diameter, we wish to reduce the shortest path diameter. We will apply the technique from \Cref{sec:spd reduction} to do this task, as follows.

\begin{proposition}[\spdiam reduction of an overlay network]\label{thm:spd reduction overlay network}
For any parameter $\alpha$ and $\beta$, consider an overlay network $(G', w')$ of $\tilde O(\alpha)$ nodes, embedded in network $(G, w)$. There is a distributed algorithm that terminates in $\tilde O(\alpha\beta+\diam(G))$ time and gives an overlay network $(G'', w'')$ such that $V(G')=V(G'')$, $\spdiam(G'', w'') = \tilde O(\alpha/\beta)$, and for any nodes $u$ and $v$, $\dist_{G'', w''}(u, v)=\dist_{G', w'}(u, v)$. 
\end{proposition}
\begin{proof}
Consider the following algorithm. First, every node in the overlay network $(G', w')$ broadcasts to all other nodes the values of $\beta$ edges incident to it with smallest weights (breaking ties arbitrarily). This step takes $\tilde O(\alpha \beta)$ time since there are $\alpha\beta$ edges broadcasted. Using these broadcasted edges, every node $v$ can compute $\beta$ nodes nearest to it (since any shortest path algorithm -- Disjkstra's algorithm for example -- will only need to know $\beta$ smallest-weight edges to compute $\beta$ nearest nodes).  Thus, $v$ can add $\beta$ {\em shortcuts} to the network $(G', w')$ to construct network $(G'', w'')$. In fact, the added shortcuts could be broadcasted to all nodes in $\tilde O(\alpha\beta+\diam(G))$ time since each node will broadcast only $\beta$ shortcuts. This implies that we can build an overlay network $(G'', w'')$ in $\tilde O(\alpha\beta)$ time and, by \Cref{thm:spd reduction}, the shortest-path diameter of $(G'', w'')$ is $\spdiam(G'', w'') = \tilde O(\alpha/\beta).$\danupon{This proof is really rough.}
\end{proof}


\subsection{Computing \sssp on Overlay Network $(G'', w'')$}\label{sec:sssp overlay}

In the final step of our sublinear-time \sssp algorithm, we solve \sssp on overlay network $(G'', w'')$ embedded in $(G, w)$ obtained in the previous section. Recall that for parameters $\alpha$ and $\beta$ which will be fixed later, $|V(G'')|=\tilde \Theta(\alpha)$ and  $\spdiam(G'', w'')=\tilde O(\alpha/\beta)$.


\begin{lemma}[$(1+o(1))$-approximate \sssp on $(G'', w'')$]\label{thm:final step sssp}
We can $(1+o(1))$-approximate \sssp on $(G'', w'')$ in $\tilde O(\diam(G)\alpha/\beta + \alpha)$ time.
\end{lemma}
\begin{proof}
We will simulate the light-weight $h$-hop \sssp algorithm in \Cref{thm:light-weight sssp} on the overlay network $(G'', w'')$ by using $h=\spdiam(G'', w'') = \tilde O(\alpha/\beta)$. To simulate this algorithm, we will view $(G'', w'')$ as a {\em fully-connected} overlay network where every node can communicate with other nodes by {\em broadcasting}, i.e. sending a message to every node in the original network $G$, which takes $O(\diam(G))$ time. In particular, every node in $(G'', w'')$ will simulate each round of this algorithm and wait until the messages that are sent in such round by all nodes are received by all nodes before starting the next round (see \Cref{algo:simulate broadcast on overlay}). 

\begin{algorithm}
\caption{Similating a broadcasting algorithm on an overlay network $(G'', w'')$}\label{algo:simulate broadcast on overlay}
{\bf Input:} An overlay network $(G'', w'')$ embedded on network $G$ and an algorithm $\cA$ such that nodes communicate only by broadcasting a message to all its neighbors. 

{\bf Goal:} Simulate $\cA$ on $(G'', w'')$ when we view $G''$ as a fully-connected overlay network.

\begin{algorithmic}[1]
\For{each round $i$ of algorithm $\cA$} 

\State Count the number of nodes in $G''$ that want to broadcast a message in this round of $\cA$. Let $M_i$ be such number. Make every node in $G$ knows $M_i$. (This step takes $O(\diam(G))$ time.)

\State Every node in $G''$ that wants to send a message broadcasts such message to every node in $G$. Wait for $\diam(G)+M_i$ rounds to make sure that every node receives all $M_i$ messages before proceeding to round $i+1$.

\EndFor
\end{algorithmic}
\end{algorithm}

Simulating each round $i$ of this algorithm will take $\tilde O(\diam(G)+M_i)$, where $M_i$ is the total number of messages broadcasted by all nodes in round $i$. This is because broadcasting $M_i$ messages to all nodes in the network (not just all neighbors) takes  $\tilde O(\diam(G)+M_i)$ time. 
%
Note that, by \Cref{thm:light}, this algorithm finishes in $\tilde O(h)$ rounds; thus, the total time needed to simulate this algorithm is  $\tilde O(h\diam(G)+M)$ where $M$ is the total number of messages broadcasted by all nodes throughout the algorithm. Since this algorithm is light-weight, every node in $G''$ broadcasts only $O(\log n)$ messages, and thus we can bound $M$ by $\tilde O(|V(G'')|) = \tilde O(\alpha)$. So, the total running time is $\tilde O(h\diam(G)+\alpha) = \tilde O(\diam(G)\alpha/\beta + \alpha)$ as claimed. 
\end{proof}

\subsection{Putting Everything Together (Proof of \Cref{thm:main sssp})}\label{sec:sssp time analysis}

By \Cref{thm:final step sssp}, we can $(1+o(1))$-approximate \sssp on $(G'', w'')$ which, in turn,  $(1+o(1))$-approximates \sssp on $(G', w')$, by \Cref{thm:spd reduction overlay network}. Then, by \Cref{thm:overlay network}, we know that we can $(1+o(1))$-approximate \sssp on the original network $(G, w)$ as desired. 
%
We now analyze the running time. Constructing $(G', w')$ takes $\tilde O(\alpha+n/\alpha+\diam(G))$, as in \Cref{thm:overlay network}. Adding shortcuts to $(G', w')$ to construct $(G'', w'')$ takes $\tilde O(\alpha\beta+\diam(G))$, by \Cref{thm:spd reduction overlay network}. Finally, solving \sssp on $(G'', w'')$ takes $\tilde O(\diam(G)\alpha/\beta + \alpha)$ by \Cref{thm:final step sssp}. So, the total running time of our algorithm is 
\[
\tilde O(n/\alpha+\diam(G)+\alpha\beta+\diam(G)\alpha/\beta).
\]
By setting $\alpha=n^{1/2}/(\diam(G))^{1/4}$ and $\beta=(\diam(G))^{1/2}$, we get the running time of $\tilde O(n^{1/2}(\diam(G))^{1/4}+\diam(G))$ as desired. 
%
Note that it is possible that $\beta\geq \alpha$. In this case, we will simply set $\beta=\alpha$ to get the claimed running time; in fact, this happens only when $\diam(G)\geq n^{2/3}$, and the running time will be $\tilde O(\diam(G))$ in this case. 

%********************************************************
%********************************************************
%********************************************************

\endinput

%\begin{definition}[skeleton]\label{def:skeleton}
%For any weighted graph $(G, w)$, integer $h$, and set of nodes $S$, an {\em $(S, h)$-skeleton} is a weighted graph $(G', w')$ such that, $V(G')=V(G)$ and, for any nodes $u$ and $v$ such that $\dist^h_{G, w}(u, v)<\infty$, there is an edge $uv$ in $G'$ of weight $w'(uv)=\dist^h_{G, w}(u, v)$. 
%\end{definition}
%
%\begin{proposition}\label{thm:skeleton}
%For any weighted graph $(G, w)$, source node $s$, and integer $\alpha$, there is an $\tilde (n/\alpha)$-time distributed algorithm that construct a $(|S|, n/\alpha)$-skeleton, for some set $S$, such that with high probability,
%\begin{enumerate}[label=(\arabic{*})]
%\item $s\in S$, 
%\item $|S|= \tilde O(\alpha)$,
%\item 
%\end{enumerate}
%\end{proposition}

\begin{proposition}[Constructing a skeleton]\label{thm:skeleton}
For any weighted graph $(G, w)$, source node $s$, and integer $\alpha$, there is an $\tilde O(\alpha+n/\alpha+D)$-time distributed algorithm that gives a set $S\subseteq V(G)$ with the following properties at its termination, with high probability. 
\begin{enumerate}[label=(\arabic{*})]
\item $s\in S$.
\item Every node knows the IDs of all nodes in $S$. 
\item $|S|= \tilde O(\alpha)$.
\item Every node $u\in V(G)$ knows an approximate $(n/\alpha)$-hop distance (\Cref{def:bounded hop sssp}) to every node $v\in S$, i.e. $u$ knows $\dist'(u, v)$ such that 
\[\dist^{n/\alpha}_{G, w}(u, v)\leq \dist'(u, v) \leq (1+o(1))\dist^{n/\alpha}_{G, w}(u, v).\]
\end{enumerate}
\end{proposition}
%
\begin{proof}
Our algorithm is as follows. First, every node $u$ selects itself to be in $S$ with probability $\alpha/n$. Additionally, source $s$ which will always be in $S$. Then, every node in $S$ broadcasts its ID to all nodes in the network. These steps guarantee the first two conditions in \Cref{thm:skeleton} and take time $\tilde O(|S|)$ (for broadcasting $\tilde O(|S|)$ IDs). Now observe that $E[|S|] = 1+(\alpha/n)\cdot (n-1) \leq 2\alpha$; so, by Chernoff's bound (e.g. \cite[Theorem 4.4]{MitzenmacherU05}), 
%\begin{align*}
$Pr[|S|\geq 12\alpha\log n] \leq 1/n.$
%\end{align*}
This proves the third condition and shows that  the running time so far is $\tilde O(|S|) = O(\alpha).$ 
%
To guarantee the last condition, we invoke an algorithm for the bounded-hop multi-source shortest path problem in \Cref{thm:k-source h-hop sp} (page \pageref{thm:k-source h-hop sp}), with nodes in $S$ as sources and $h=n/\alpha$ hops. By \Cref{thm:k-source h-hop sp}, the algorithm takes $\tilde O(k+h+D)$ and every node $u$ will know $\dist'_{G, w}(u, v)$ such that 
\[
\dist_{G, w}^{h}(u, v)\leq \dist'_{G, w}(u, v)\leq (1+o(1))\dist_{G, w}^{h}(u, v)
\]
for all $v\in S$. This implies the last condition of \Cref{thm:skeleton} and completes the proof. 
\end{proof}

%
Our approximation algorithms use a pseudo-polynomial time algorithm for $K$-\apsp when edge weights are symmetric and positive as in the following proposition.
%
\begin{proposition}\label{prop:pseudopoly time}\label{PROP:PSEUDOPOLY TIME}{\sc(Pseudo-Polynomial Time Algorithm for $K$-APSP; Proof in Appendix~\ref{sec:proof of PROP:PSEUDOPOLY TIME})}
$K$-\apsp on network $G$ with {\em positive symmetric} integral weight $w$ can be solved in $O(n+K)$-time.
\end{proposition}
%
%To prove the above lemma, we view weighted network $(G, w)$ as an unweighted network $G'$ by replacing an edge $uv$ in $G$ by a $u$-$v$ path of $w(uv)$ nodes in $G'$. We then apply the the {\em $S$-Shortest Paths} algorithm of \cite{HolzerW12} on $G'$ to find the distances between all nodes in $S$, where we use $S=V(G)$, and all other nodes in $G'$.
%
This proposition simply exploits the fact that we can view the input weighted network $(G, w)$ as an unweighted network $G'$ by replacing every edge $uv$ of weight $w(uv)$ by a $u$-$v$ path of length $w(uv)$. We then grow breadth-first search (BFS) trees in $G'$ {\em in parallel} from every node in $V(G)$ to find distances between nodes in $V(G)$ and other nodes in $V(G')$.
%
Since we grow many BFS trees in parallel, there could be {\em conflicts}; i.e., many BFS tree algorithms may want to send messages on the same edge at the same time. There are many ways to resolve this.
%
For example, one can use the {\em random delay} technique \cite{LeightonMR94} to solve the problem in $O(K\log n+n)$ time with high probability (see Proposition~\ref{prop:pseudopoly multi-weight} below). A nicer way is to adapt the technique of the {\em $\cS$-Shortest Paths}\footnote{This problem is also called $k$-source shortest path \cite{Elkin05,KhanKMPT12}} algorithm from \cite{HolzerW12}, which gives us a deterministic $O(K+n)$ time algorithm.


Now, to approximate $D(G, w)$, we first compute $D'$ that $2$-approximates $D(G, w)$; this can be done easily by solving \sssp from an arbitrary source. We then use $D'$ to change $w$ slightly to $w'$ where $w'(uv)=\lceil \frac{2n w(uv)}{\epsilon D'}\rceil$. We then show the following.
\begin{proposition}\label{prop:approx diameter guarantee}{\sc (Properties of $D(G, w')$; Proof in Appendix~\ref{sec:approx diameter})}
$D(G, w')\leq (1+2/\epsilon)n$ and $D(G, w)$ $\leq$ $\frac{\epsilon D'}{2n}\times D(G, w')$ $\leq$ $(1+\epsilon)D(G, w).$
\end{proposition}
% and we can use $D(G, w')$ to approximate $D(G, w)$.
Thus, we can apply Proposition~\ref{prop:pseudopoly time} with $K=(1+2/\epsilon)n$ on $D(G, w')$ to compute $D(G, w')$. Then, we output $D'\times D(G, w')$ as an approximate solution of $D(G, w)$. 






==> arXiv/tools.tex <==
\section{Main Tools} \label{sec:tools}


\subsection{Light-Weight Bounded-Hop Single-Source and Multi-Source Shortest Paths}\label{sec:light-weight bounded-hop sssp}

A key tool for our algorithm is a simple idea for computing a bounded-hop single-source shortest path and its extensions. Informally, an $h$-hop path is a path containing at most $h$ edges. The $h$-hop distance between two nodes $u$ and $v$ is the minimum weight among all $u$-$v$ $h$-hop paths. The problem of $h$-hop \sssp is to find the $h$-hop distance between a given source node $s$ and all other nodes. Formally:
%
\begin{definition}[$h$-hop \sssp]\label{def:bounded hop sssp}
Consider any network $G$ with edge weight $w$ and integer $h$. For any nodes $u$ and $v$, let $\cP^h(u, v)$ be a set of $u$-$v$ paths containing at most $h$ edges. We call $\cP^h(u, v)$ a set of $h$-hop $u$-$v$ paths. 
%
Define the $h$-hop distance between $u$ and $v$ as %$\dist_{G, w}^{h}(u, v) = \min_{P\in \cP^h(u, v)} w(P)$ if $\cP^h(u, v)\neq \emptyset$ and $\dist_{G, w}^{h}(u, v) =\infty$ otherwise.
\begin{align*}
\dist_{G, w}^{h}(u, v) &= 
\begin{cases}
\min_{P\in \cP^h(u, v)} w(P) & \mbox{if $\cP^h(u, v)\neq \emptyset$}\\
\infty & \mbox{otherwise.}
\end{cases}
\end{align*}
%$ if $\cP^h(u, v)\neq \emptyset$ and $\dist_{G, w}^{h}(u, v) =\infty$ otherwise.
%
\danupon{To define: $w(P)$.} 
Let $h$-hop \sssp be the problem where, for a given weighted network $(G, w)$, source node $s$ (node $s$ knows that it is the source), and integer $h$ (known to every node), we want every node $u$ to know $\dist_{G, w}^{h}(s, u)$.\danupon{Does $u$ always know that $\dist_{G, w}^{h}(s, u)=\infty$?}
\end{definition}
%
This problem can be solved in $O(h+D)$ time using, e.g., the distributed version of Bellman-Ford's algorithm. However, previous algorithms are ``heavy-weight'' in the sense that they require so much communication (i.e., there could be as large as $\Omega(h)$ messages sent through an edge) and thus are not suitable for parallelization. In this paper, we show a simple algorithm that can $(1+o(1))$-approximate $h$-hop \sssp in $\tilde O(h+D)$ time. Our algorithm is {\em light-weight} in the sense that every node broadcasts a message (of size $O(\poly\log n)$) to their neighbors only $O(\log n)$ times:
%each node sends only one message (of size $O(\poly\log n)$) through each edge:
%
%\begin{proposition}[Light-weight $h$-hop \sssp algorithm; Proof in \Cref{sec:light-weight bounded-hop sssp}]\label{thm:light-weight sssp}\label{thm:light}
%There is an algorithm that solves $h$-hop \sssp on network $G$ with weight $w$\danupon{Don't forget that $w$ must be positive} in $O(h)$-time and, during the whole computation, every node $u$ sends a message of size $O(\poly\log n)$ to any of its neighbors $v$ at most once. 
%\end{proposition} 
%
\begin{restatable}[Light-weight $h$-hop \sssp algorithm; proof in \Cref{sec:proof of them:light}]{theorem}{lighthsp}\label{thm:light-weight sssp}\label{thm:light}
There is an algorithm that solves $h$-hop \sssp on network $G$ with weight $w$\danupon{Don't forget that $w$ must be positive} in $\tilde O(h+D)$-time and, during the whole computation, every node $u$ broadcasts $O(\log n)$ messages, each of size $O(\poly\log n)$, to its neighbors $v$. 
\end{restatable}
%
\Cref{thm:light}, in its own form, cannot be directly used. We will extend it to an algorithm for computing $h$-hop {\em multi-source shortest paths} (\mssp). (Later, in \Cref{sec:overlay} we will also extend this result to {\em overlay networks}.)
%
%We will extend it in two ways to get algorithms for computing $h$-hop {\em multi-source shortest paths} (\mssp)\danupon{Should define this problem either here or in prelim} and \sssp on {\em overlay networks}. These extensions will be explained in \Cref{sec:bounded-hop mssp} and XXX. 
%
The rest of this subsection is devoted to proving \Cref{thm:light-weight sssp}.\danupon{To do: Add some overview as commented below}

%The proof consists of two parts. In the first part, we show that edge weights can be rounded, with a small approximation factor, in such a way that 


%The algorithm for approximating \apsp is outlined in Algorithm~\ref{algo:approx apsp}. It is similar to the algorithm for approximating the diameter, except that we do not have $D'$, the two-approximation of the diameter. Instead, we will ``guess'' all possible values of the distance between every pair of nodes, using $D'_i=2^i$, as shown in the for-loop of Algorithm~\ref{algo:approx apsp}.

%\begin{lemma}\label{thm:approximate weight}
%For any $i$ and edge $xy$, let  $D'_i=2^i$ and $w'_i(xy)=\lceil \frac{2n w(xy)}{\epsilon D'_i}\rceil$. 
%Consider any node $u$ and $v$. For any $i$,
%\begin{align}
%\frac{\epsilon 2^i}{2n}\times \dist_{G, w'_i}(u, v)\geq \dist_{G, w}(u, v).\label{eq:apsp approx main one}
%\end{align}
%Moreover, for $i^*$  such that $2^{i^*-1}\leq \dist_{G, w}(u, v)\leq 2^{i^*}$, we have that
%\begin{align}
%\dist_{G, w'_{i^*}}(u, v)&\leq (1+2/\epsilon)n ~~\mbox{and}\label{eq:apsp approx main two}\\
%\frac{\epsilon D_{i^*}}{2n}\times \dist_{G, w'_{i^*}}(u, v) &\leq (1+\epsilon)\dist_{G, w}(u, v).\label{eq:apsp approx main three}
%\end{align}
%\end{lemma}

\subsubsection{Reducing Bounded-Hop Distance by Approximating Weights}


%\begin{lemma}
%Consider any $n$-node weighted graph $(G, w)$ and an integer $h$. Let $\epsilon=\log n$. For any $i$ and edge $xy$, let $D'_i=2^i$ and $w'_i(xy)=\lceil \frac{2h w(xy)}{\epsilon D'_i}\rceil$. 
%%
%For any nodes $u$ and $v$, if we let 
%$$\tilde d_{G, w}(u, v) = \min_i  \left(\frac{\epsilon D'_{i}}{2h}\times \dist^{(1+2/\epsilon)n}_{G, w'_i}(u, v)\right),$$ 
%then $\dist_{G, w}(u, v)\leq \tilde d_{G,w}(u, v)\leq (1+\epsilon)\dist_{G, w}(u, v)$.
%\end{lemma}

\danupon{To do: Explain. Below says that we can approximate bounded-hop distance $\dist^h_{G, w}$ by solving bounded-distance $\dist^{O(h)}_{G, w'_i}$ instead.}\danupon{To do: Recall what $d^h$ is.}


\begin{proposition}[Reducing Bounded-Hop Distance by Approximating Weights]\label{thm:approximate weight}
Consider any $n$-node weighted graph $(G, w)$ and an integer $h$. Let $\epsilon=1/\log n$. For any $i$ and edge $xy$, let $D'_i=2^i$ and $w'_i(xy)=\lceil \frac{2h w(xy)}{\epsilon D'_i}\rceil$. 
%
For any nodes $u$ and $v$, if we let 
%\[
%\tilde d^h_{G, w}(u, v) = \min_i  \left(\frac{\epsilon D'_{i}}{2h}\times \dist^{(1+2/\epsilon)h}_{G, w'_i}(u, v)\right),
%\]
%
\[
\widetilde \dist^h_{G, w}(u, v) = \min  \left\{\frac{\epsilon D'_{i}}{2h}\times \dist_{G, w'_i}(u, v) \mid i:\ \dist_{G, w'_i}(u, v)\leq (1+2/\epsilon)h\right\},
\]
%
%
%\[
%\tilde \dist^h_{G, w}(u, v) = \min_i  
%\begin{cases}
%\frac{\epsilon D'_{i}}{2h}\times \dist^{(1+2/\epsilon)h}_{G, w'_i}(u, v) & \mbox{if XXX}\\
%B & \mbox{otherwise}
%\end{cases}
%%\left(\frac{\epsilon D'_{i}}{2h}\times \dist^{(1+2/\epsilon)h}_{G, w'_i}(u, v)\right),$$ 
%\]
%
then $\dist^h_{G, w}(u, v)\leq \widetilde \dist^h_{G,w}(u, v)\leq (1+\epsilon)\dist^h_{G, w}(u, v)$.
\end{proposition}

Note that the min term in \Cref{thm:approximate weight} is over all $i$ such that $\dist_{G, w'_i}(u, v)\leq (1+2/\epsilon)h$. The proof of \Cref{thm:approximate weight} heavily relies on \Cref{thm:approximate weight detail} below. 


\begin{lemma}[Key Lemma for Reducing Bounded-Hop Distance by Approximating Weights]\label{thm:approximate weight detail}
Consider any nodes $u$ and $v$. For any $i$, let $w_i$ and $D'_i$ be as in  \Cref{thm:approximate weight}. Then, 
\begin{align}
\frac{\epsilon D'_i}{2h}\times \dist_{G, w'_i}(u, v)\geq \dist^h_{G, w}(u, v).\label{eq:apsp approx main one}
\end{align}
Moreover, for $i^*$  such that $D'_{i^*-1}\leq \dist^h_{G, w}(u, v)\leq D'_{i^*}$, we have that
\begin{align}
\dist_{G, w'_{i^*}}(u, v)&\leq (1+2/\epsilon)h ~~\mbox{and}\label{eq:apsp approx main two}\\
\frac{\epsilon D_{i^*}}{2h}\times \dist_{G, w'_{i^*}}(u, v) &\leq (1+\epsilon)\dist^h_{G, w}(u, v).\label{eq:apsp approx main three}
\end{align}
\end{lemma}
\begin{proof}
Let $P=\langle u=x_0, x_1, \ldots, x_\ell=v\rangle$ be any shortest $h$-hop path between $u$ and $v$ (thus $2^{i^*-1}\leq w(P)\leq 2^{i^*}$ and $\ell \leq h$). Then,
\begin{align}
\dist_{G, w'_{i^*}}(u, v)&=\sum_{j=0}^{\ell-1} \left\lceil \frac{2h w(x_jx_{j+1})}{\epsilon D'_{i^*}}\right\rceil\nonumber\\ %\label{eq:apsp approx one} \\
&\leq \frac{2h}{\epsilon D'_{i^*}}\sum_{j=0}^{\ell-1} w(x_jx_{j+1}) + \ell\nonumber\\ %\label{eq:apsp approx two}\\
&\leq \frac{2h}{\epsilon D'_{i^*}}\dist^h_{G, w}(u, v) + h \label{eq:apsp approx three}\\
&\leq (1+2/\epsilon)h \nonumber %\label{eq:apsp approx four}
\end{align}
where the last inequality is because $D'_{i^*}\geq \dist^h_{G, w}(u,v)$. This proves \Cref{eq:apsp approx main two}.
%
Using \Cref{eq:apsp approx three}, we also have that
\begin{align*}
\frac{\epsilon D'_{i^*}}{2h}\times \dist_{G, w'_{i^*}}(u, v)  & \leq \frac{\epsilon D'_{i^*}}{2h}\times \left(\frac{2h}{\epsilon D'_{i^*}}\dist^h_{G, w}(u, v) + h\right)\\
&\leq \dist^h_{G, w}(u, v)+\frac{\epsilon}{2}D'_{i^*}\\
&\leq (1+\epsilon)\dist^h_{G, w}(u, v)
\end{align*}
where the last inequality is because $D'_{i^*}=2D'_{i^*-1}\leq 2\dist^h_{G, w}(u, v)$. This proves \Cref{eq:apsp approx main three}. Finally, observe that for any $i$ and the path $P$ defined as before, we have
\begin{align*}
\dist_{G, w'_{i}}(u, v)&\geq \sum_{j=0}^{\ell-1} \frac{2h w(x_jx_{j+1})}{\epsilon D'_i}\nonumber\\
&= \frac{2h}{\epsilon D'_i}  \dist^h_{G, w}(u, v)\,.%\label{eq:diameter approx five}\,.
\end{align*}
It follows that
%
\begin{align*}
\frac{\epsilon D'_i}{2h}\times\dist_{G, w'_i}(u, v) & \geq \frac{\epsilon D'_i}{2h}\times \left(\frac{2h}{\epsilon D'_i}  \dist^h_{G, w}(u, v)\right)\\
&= \dist^h_{G, w}(u, v)\,.
\end{align*}
%
This proves \Cref{eq:apsp approx main one} and completes the proof of \Cref{thm:approximate weight detail}.
\end{proof}

Now we are ready to prove \Cref{thm:approximate weight}.

\begin{proof}[Proof of \Cref{thm:approximate weight}] Note that
\begin{align*}
\tilde d^h_{G, w}(u, v) &= \min  \left\{\frac{\epsilon D'_{i}}{2h}\times \dist_{G, w'_i}(u, v) \mid i:\ \dist_{G, w'_i}(u, v)\leq (1+2/\epsilon)h\right\}\\
&\leq  \frac{\epsilon D'_{i^*}}{2h}\times \dist_{G, w'_{i^*}}(u, v)\\
&\leq (1+\epsilon)\dist^h_{G, w}(u, v)
%&= \min  \left\{\frac{\epsilon D'_{i}}{2h}\times \dist_{G, w'_i}(u, v) \mid i\right\},
\end{align*}
%
%$$\tilde \dist^h_{G, w}(u, v)= \min_i \frac{\epsilon D'_{i}}{2n}\times\dist^{(1+2/\epsilon)n}_{G, w'_i}(u, v)= \min_i \frac{\epsilon D'_{i}}{2n}\times\dist_{G, w'_i}(u, v)$$
%
where $i^*$ is as in \Cref{thm:approximate weight detail}, the second inequality is due to the fact that $\dist_{G, w'_{i^*}}(u, v)\leq (1+2/\epsilon)h$ as in \Cref{eq:apsp approx main two}, and the third inequality follows from \Cref{eq:apsp approx main three}. This proves the second inequality in \Cref{thm:approximate weight}. The first inequality of \Cref{thm:approximate weight} simply follows from the fact that $\frac{\epsilon D'_i}{2h}\times \dist_{G, w'_i}(u, v)\geq \dist^h_{G, w}(u, v)$ for all $i$, by \Cref{eq:apsp approx main one}. 
%
%\begin{align*}
%\tilde d^h_{G, w}(u, v) &= \min  \left\{\frac{\epsilon D'_{i}}{2h}\times \dist_{G, w'_i}(u, v) \mid i:\ \dist_{G, w'_i}(u, v)\leq (1+2/\epsilon)h\right\}\\
%&\geq XXX
%\end{align*}
%Then, \Cref{eq:apsp approx main one,eq:apsp approx main three} imply that $\tilde \dist^h_{G, w}(u, v)\geq \dist^h_{G, w}(u, v)$ and $\tilde \dist^h_{G, w}(u, v)\leq (1+\epsilon)\dist^h_{G, w}(u, v)$, respectively.
\end{proof}



%\subsubsection{Pseudo-Polynomial Time Algorithm for Bounded-Distance \sssp}
%
%We first argue that there exists a $O(n+K)$-time algorithm for $K$-\apsp on network $G$ with positive symmetric integral weight $w$, as claimed in Proposition~\ref{PROP:PSEUDOPOLY TIME}. This algorithm is pseudo-polynomial since $K$ could be as large as $D(G, w)$.
%
%{\renewcommand{\thetheorem}{\ref{prop:pseudopoly time}}
%\begin{proposition}[Restated]
%$K$-\apsp on network $G$ with {\em positive symmetric} integral weight $w$ can be solved in $O(n+K)$-time.
%\end{proposition}
%\addtocounter{theorem}{-1}
%}
%
%Consider Algorithm~2 in \cite{HolzerW12} which is used for the problem called {\em $\cS$-shortest paths} (computing distances from sources in $\cS$ on an unweighted network $G$). This algorithm is outlined in Algorithm~\ref{algo:HolzerW12}. This algorithm executes the breadh-first search (BFS) algorithms from $q$ different sources in $\cS$ in parallel, where the BFS algorithm starting at node $u$ forwards $u$ (representing the unique ID of node $u$) in the BFS manner until every node receives $u$. We let BFS$_i$ denote the BFS algorithm starting at $s_i$, and $T_{s_i}$ denote the BFS tree constructed by BFS$_i$.




\subsubsection{Algorithm for Bounded-Hop \sssp (Proof of \Cref{thm:light})}\label{sec:proof of them:light}


We now show that we can solve $h$-hop \sssp in $\tilde O(h+D)$ time while each node broadcasts $O(\log n)$ messages of size $O(\log n)$, as claimed in \Cref{thm:light}. Our algorithm is outlined in \Cref{algo:bounded-hop sssp}. Given a parameter $h$ (known to all nodes) and weighted network $(G, w)$, it computes $w_i$, for all $i$, as defined in \Cref{thm:approximate weight}; i.e., every node $u$ internally computes $w_i(u, v)$ for all neighbors $v$. Note that this step needs no communication. Next, in Line~\ref{line:solve bounded distance sssp} of \Cref{algo:bounded-hop sssp}, for each value of $i$, the algorithm executes an algorithm for the bounded-distance \sssp problem with parameter $(G, w, s, K)$, where $(1+2/\epsilon)h$, as outlined in \Cref{algo:pseudo polynomial} (we will explain this algorithm next). At the end of the execution of \Cref{algo:pseudo polynomial}, every node $u$ knows $\dist_i'(s, u)$ such that $\dist_i'(s, u)=\dist_{G, w_i}(s, u)$ if $\dist_{G, w_i}(s, u)\leq K$ and $\dist_i'(s, u)=\infty$ otherwise. Finally, we set $\widetilde \dist^h_{G, w_i}(s, u) = \min_i \dist'_i(s, u)$. By \Cref{thm:approximate weight}, we have that $\dist^h_{G, w}(u, v)\leq \widetilde \dist^h_{G,w}(u, v)\leq (1+\epsilon)\dist^h_{G, w}(u, v) = (1+o(1))\dist^h_{G, w}(u, v)$ as desired.\danupon{Careful!!! If we use $\epsilon=1/\log n$, how many different values of $(1+\epsilon)^i$ are there? } 

We now explain \Cref{algo:pseudo polynomial} for solving the bounded-distance \sssp problem. It is a simple modification of a standard bread-first tree algorithm. It runs for $K$ rounds. In the initial round (Round $0$), the source node $s$ broadcasts a message $(s, 0)$ to all its neighbors to start the algorithm. This message is to inform all its neighbors that its distance from the source (itself) is $0$. In general, we will make sure that every node $v$ whose distance to $s$ is $\dist_{G, w}(s, u)=\ell$ will broadcast a message $(s, \ell)$ to its neighbor at Round $\ell$. Every time a node $u$ receives a message of the form $(s, \ell)$ from its neighbor $v$, it knows that $\dist_{G, w}(s, v)=\ell$; so, $u$ updates its distance to the minimum between the current distance and $\ell+w(uv)$. %The following claim is easy to check. 
%
%\begin{claim}
It is easy to check that every node $u$ such that $\dist_{G, w}(s, u)< K$ broadcasts its message to all neighbors {\em once} at Round $\ell=\dist_{G, w}(s, u)$. 
%\end{claim}
%
The correctness of \Cref{algo:pseudo polynomial} immediately follows. Moreover, since we execute \Cref{algo:pseudo polynomial} for $O(\log n)$ different values of $i$ (since the maximum weight is $\poly(n)$), it follows that every node broadcasts a message to their neighbors $O(\log n)$ times. \Cref{thm:light} follows. 



%This algorithm executes the breadh-first search (BFS) algorithms from $q$ different sources in $\cS$ in parallel, where the BFS algorithm starting at node $u$ forwards $u$ (representing the unique ID of node $u$) in the BFS manner until every node receives $u$. We let BFS$_i$ denote the BFS algorithm starting at $s_i$, and $T_{s_i}$ denote the BFS tree constructed by BFS$_i$.





\begin{algorithm}
\caption{Bounded-Hop \sssp $(G, w, s, h)$} \label{algo:bounded-hop sssp}
{\bf Input:} Weighted undirected graph $(G, w)$, source node $s$, and integer $h$. 

{\bf Output:} Every node $u$ knows the value of $\widetilde \dist^h_{G, w_i}(s, u)$ such that $\dist^h_{G, w}(s, u)\leq \widetilde \dist^h_{G, w_i}(s, u) \leq (1+o(1))\dist^h_{G, w_i}(s, u)$.

%\medskip 

%$\bullet$ Initially, at time $t$, source node $s$ triggers the algorithm to start by sending a message $(s, 0)$ to itself.

%\medskip\textit{\textbf{Main subroutine:}}

%$\bullet$ When a node $u$ receives a message $(s, \ell)$ for some $\ell$ from node $v$, it does the following.

\begin{algorithmic}[1]

%\algrestore{bfsone}


\State Let $\epsilon=1/\log n$. For any $i$ and edge $xy$, let $D'_i=2^i$ and $w'_i(xy)=\lceil \frac{2h w(xy)}{\epsilon D'_i}\rceil$. Let $K=(1+2/\epsilon)h$.


\State Let $t$ be the time this algorithm starts. We can assume that all nodes know $t$.

\ForAll{i}


%
%\Comment{This is Iteration $i$. We run a BFS-like algorithm on $(G, w_i)$}
%
%\State Let $t_i$ be the time this iteration starts. We can assume that all nodes know $t_i$.
%
%
%\State At time $t_i$, source node $s$ sends a message $(s, 0)$ to itself.
%
%%\medskip\textit{\textbf{Main subroutine:}}
%
%%\State When a node $u$ receives a message $(s, \ell)$ for some $\ell$ from node $v$, it does the following.
%
%%\StatexIndent[2]
%
%\If{a node $u$ receives a message $(s, \ell)$ for some $\ell$ from node $v$,}
%
%\If{$u$ has {\em not} already received $(s, \ell')$ for any $\ell'<\ell$}
%
%\State $u$ now knows that $\dist_{G}(s, u)=\ell+w(u, v)$.
%
%%\State $u$ sends through all directed edges $\overrightarrow{uv}$ a message $(s, t, \ell+w(\overrightarrow{uv}))$ at time $t+\ell+w(\overrightarrow{uv})$.\label{line:bfs send message}
%
%\State {\bf if} $\dist_{G}(s, u)<K$ {\bf then} $u$ broadcasts message $(s, \dist_{G}(s, u))$ to all its neighbors at time $t+\dist_{G}(s, u)$. 
%
%
%\EndIf
%\EndIf
%
%\State At time $t_i+K$ stop the execution of this iteration and proceed to the next value of $i$.

\State Solve bounded-distance \sssp with parameters $(G, w_i, s, K)$
% in $O(K)=O(h/\epsilon)$ time ()
using \Cref{algo:pseudo polynomial}. 
(This takes  $\tilde O(K)=\tilde O(h)$ time.)
%
Let $\dist'_i(s, u)$ be the distance returned to node $u$.\label{line:solve bounded distance sssp}

\EndFor

\State Each node $u$ computes $\widetilde \dist^h_{G, w_i}(s, u) = \min_i \dist'_i(s, u)$.


\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Bounded-Distance \sssp $(G, w, s, K)$} \label{algo:pseudo polynomial}
{\bf Input:} Weighted undirected graph $(G, w)$, source node $s$, and integer $K$. 

{\bf Output:} Every node $u$ knows $\dist'_{G, w}(s, u)$ where $\dist'_{G, w}=\dist_{G, w}(s, u)$ if $\dist_{G, w}(s, u)\leq K$ and $\dist'_{G, w}=\infty$ otherwise. 

%Every node $u$ knows the value of $\dist_{G, w}(s, u)$ if $\dist_{G, w}(s, u)\leq K$; otherwise, it knows that $\dist_{G, w}(s, u)>K$.

%\medskip $\bullet$ Let $t$ be the time this algorithm starts. We can assume that all nodes know $t$.
%
%$\bullet$ Initially, 
%
%$\bullet$ at time $t$, source node $s$ triggers the algorithm to start by sending a message $(s, 0)$ to itself.
%
%%\medskip\textit{\textbf{Main subroutine:}}
%
%$\bullet$ When a node $u$ receives a message $(s, \ell)$ for some $\ell$ from node $v$, it does the following.

\begin{algorithmic}[1]

%\algrestore{bfsone}

\State Let $t$ be the time this algorithm starts. We can assume that all nodes know $t$.

\State Initially, every node $u$ sets $\dist'_{G, w}(s, u)=\infty$. 

\State In the beginning of this algorithm (i.e., at time $t$) source node $s$ sends a message $(s, 0)$ to itself.

%\medskip\textit{\textbf{Main subroutine:}}

%\State When a node $u$ receives a message $(s, \ell)$ for some $\ell$ from node $v$, it does the following.

\If{a node $u$ receives a message $(s, \ell)$ for some $\ell$ from node $v$,}

%\If{$u$ has {\em not} already received $(s, \ell')$ for any $\ell'<\ell$}

\If{($\ell+w(u, v)\leq K$) and ($\ell+w(u, v)<\dist'_{G}(s, u)$)}

\State $u$ sets $\dist'_{G}(s, u)=\ell+w(u, v)$.

%\State $u$ sends through all directed edges $\overrightarrow{uv}$ a message $(s, t, \ell+w(\overrightarrow{uv}))$ at time $t+\ell+w(\overrightarrow{uv})$.\label{line:bfs send message}

\EndIf
\EndIf

\State For any $x\leq K$, at time $t+x$, every node $u$ such that $\dist'_{G}(s, u)=x$ broadcasts message $(s, x)$ to all its neighbors to announce that $\dist'_{G}(s, u)=x$.  

\end{algorithmic}
\end{algorithm}




%************************************************************************
%************************************************************************
%************************************************************************

%\paragraph
\subsubsection{Bounded-Hop Multi-Source Shortest Paths} \label{sec:bounded-hop mssp}
The fact that our algorithm for the bounded-hop single-source shortest path problem in \Cref{thm:light-weight sssp} is light-weight allows us to solve its {\em multi-source} version, where there are {\em many sources} in parallel. The problem of bounded-hop multi-source shortest path is as follows. 
%
\begin{definition}[$h$-hop $k$-source shortest paths]\label{def:bounded hop ksp}
Given a weighted network $(G, w)$, integer $h$ (known to every node), and sources $s_1, \ldots, s_k$ (each node $s_i$ knows that it is a source), the goal of the $h$-hop $k$-source shortest paths problem is to make every node $u$ knows $\dist_{G, w}^{h}(s_i, u)$ for all $1\leq i\leq k$.
\end{definition}
%
The main result of this section is an algorithm for solving this problem in $\tilde O(k+h+D)$ time, as follows. 
%
\begin{restatable}[$k$-source $h$-hop shortest path algorithm]{proposition}{khsp}\label{thm:k-source h-hop sp}
%
There is an algorithm that $(1+o(1))$-approximates the $h$-hop $k$-source  shortest paths problem on weighted network $(G, w)$ in $\tilde O(k+h+D)$ time; i.e., at its termination every node $u$ knows $\dist'_{G, w}(s_i, u)$ such that 
\[
\dist_{G, w}^{h}(s_i, u)\leq \dist'_{G, w}(s_i, u)\leq (1+o(1))\dist_{G, w}^{h}(s_i, u)
\]
for all sources $s_i$. 
%
\end{restatable}
%
The algorithm is conceptually easy: we simply run the algorithm for bounded-hop single-source shortest path in \Cref{thm:light-weight sssp} (i.e. \Cref{algo:bounded-hop sssp}) from $k$ sources {\em in parallel}. Obviously, this algorithm needs at least $\tilde \Omega(h+D)$ time since this is the guarantee we can get for the case of single source. Moreover, it is possible that one need has to broadcast $O(\log n)$ messages for each execution of \Cref{algo:bounded-hop sssp}, making a total of $O(k\log n)$ messages; this will require $\tilde O(k)$ time. So, the best running time we can hope for is $\tilde O(k+h+D)$. 
%
%Since each execution of \Cref{algo:bounded-hop sssp} finishes in $\tilde O(h+D)$ time and each node sends only $O(\log n)$ messages on each edge, running $k$ executions could finish in $\tilde O(h+k+D)$ time in an ideal case where . 
%
%However, this has to be carefully done since one execution could delay other executions. We show that this ideal running time can be achieved, simply by adapting the {\em random delay} technique for package scheduling \cite{LeightonMR94}. 
It is, however, not obvious to achieve this running time since one execution could {\em delay} other executions; i.e., it is possible that all executions of \Cref{algo:bounded-hop sssp} might want a node to send a message at the same time making some of them unable to proceed to the next round. We show that by simply adding a small {\em delay} to the starting time of each execution, it is {\em unlikely} that many executions will delay each other. 
%
%this ideal running time can be achieved, simply by adapting the {\em random delay} technique for package scheduling \cite{LeightonMR94}. 

%
% or the scheduling technique for {\em unweighted} $k$-source \ksp \cite{HolzerW12}\danupon{Really? Check!!!}. The algorithm based on the random delay technique has an advantage that it can be adapted to {\em directed networks}, the case that we
%
The algorithm is very simple: Instead of starting the execution of \Cref{algo:bounded-hop sssp} from different source nodes at the same time, each execution starts with a {\em random delay} randomly selected from integers from $0$ to $k\log n$. The algorithm is outlined in \Cref{algo:random delay}. 
%
\begin{algorithm}
\caption{Multi-Source Bounded-Hop Shortest Path $(G, w, \{s_1, \ldots, s_k\}, h)$} \label{algo:random delay}\label{algo:bounded-hop multi-source}
{\bf Input:} Weighted undirected graph $(G, w)$, $k$ source nodes $s_1, \ldots, s_k$, and integer $h$. 

{\bf Output:} Every node $u$ knows $\dist^h_{G, w}(s_i, u)$ for all $i$. 

%Every node $u$ knows the value of $\dist_{G, w}(s, u)$ if $\dist_{G, w}(s, u)\leq K$; otherwise, it knows that $\dist_{G, w}(s, u)>K$.

%\medskip $\bullet$ Let $t$ be the time this algorithm starts. We can assume that all nodes know $t$.
%
%$\bullet$ Initially, 
%
%$\bullet$ at time $t$, source node $s$ triggers the algorithm to start by sending a message $(s, 0)$ to itself.
%
%%\medskip\textit{\textbf{Main subroutine:}}
%
%$\bullet$ When a node $u$ receives a message $(s, \ell)$ for some $\ell$ from node $v$, it does the following.

\begin{algorithmic}[1]

%\algrestore{bfsone}

\State Let $r_1, \ldots, r_k$ be a number selected uniformly at random from $[0, k\log n]$. We can assume that all nodes know $r_i$, for all $r_i$. This can be done by, e.g., broadcasting all $r_i$ to all nodes in $O(k+D)$ time. 

\State Let $t$ be the time this algorithm starts. We can assume that all nodes know $t$.

\State At time $t+r_i$, execute the bounded-hop single-source shortest path algorithm (\Cref{algo:bounded-hop sssp}) on $(G, w, s_i, h)$.

\State If at any time, more than $\log n$ messages is sent through an edge, we say that the algorithm {\em fails}. (We show that the algorithm fails with probability $O(1/n^2)$ in \Cref{thm:no congestion}.)

\end{algorithmic}
\end{algorithm}
%
The crucial thing is to show that many executions of \Cref{algo:bounded-hop sssp} launched by \Cref{algo:random delay} {\em do not delay each other}. In particular, that we show that at most $\log n$ messages will be sent through each edge in every round, with high probability (if this does not happen, we say that the algorithm {\em fails}). We prove this in \Cref{thm:no congestion} below. Our proof is simply an adaptation of the random delay technique for package scheduling \cite{LeightonMR94}. \Cref{thm:no congestion} immediately implies \Cref{thm:k-source h-hop sp}, since each execution, which start at time $\tilde O(k)$ will finish in $\tilde O(h+D)$ rounds without being delayed.   
%
\begin{lemma}[Congestion guaranteed by the random delay technique]\label{thm:no congestion}
For any source $s_i$ and node $u$, let $\mset_{i, u}$ be the set of messages broadcasted by $u$ during the execution of \Cref{algo:bounded-hop sssp} with parameter $(G, w, s_i, h)$. Note that $|\mset_{i, u}|\leq c\log n$ for some constant $c$, by \Cref{thm:light-weight sssp}. 
%
%Let $\beta$ be such that each node sends at most $\beta$ messages during the whole execution of \Cref{algo:bounded-hop sssp} (by \Cref{thm:light-weight sssp}, $\beta=O(\log n)$).
%
%$M_{i, 1}, M_{i, 2}, \ldots, M_{i, \beta}$ be messages broadcasted by $u$ during the execution of \Cref{algo:bounded-hop sssp} with parameter $(G, w, s_i, h)$. 
%
Then, the probability that, in \Cref{algo:random delay}, there exists time $t$, node $u$, and a set $\mset\subseteq \bigcup_i \mset_{i, u}$ such that $|\mset|\geq \log n$, and all messages in $\mset$ are broadcasted by $u$ at time $t=O(k+h+D)$, is $O(1/n^2)$. 
%
%an edge $uv$ and a set $\mset=\{(s_j, \ell_j)\}_{1\leq j\leq k}$ of $k>\log n$ messages such that all messages in $\mset$ are sent on $uv$ at the same time is $O(1/n^2)$.
\end{lemma}
\begin{proof}
Fix any node $u$, time $t$, and set $\mset$ as above. Observe that, for any $i$, the time that a message $M\in \mset_{i, u}$, is broadcasted by $u$ is determined by the random delay $r_i$ -- there is only one value of $r_i$ that makes $u$ broadcasts $M$ at time $t$. In other words, for fixed $u$, $t$, and message $M\in \bigcup_i \mset_{i, u}$, 
\[
Pr[\mbox{$M$ is sent by $u$ at time $t$}]\leq \frac{1}{k\log n}. 
\] 
%
It follows that for fixed $u$, $t$, and set of messages $\mset$,
%
\[
Pr[\mbox{all messages in $\mset$ is sent by $u$ at time $t$}]\leq \left(\frac{1}{k\log n}\right)^{|\mset|}. 
\]
%
Note that we can assume that $|\mset\cap \mset_{i, u}|\leq 1$ since, for an execution of \Cref{algo:bounded-hop sssp} on a source $s_i$, every node $u$ broadcasts at most one message per round. This implies that $|\mset|\leq k$, and, for any $m\leq k$, the number of such set $\mset$ of size exactly $m$ is at most $\binom{k}{m}(c\log n)^m$ since each set $\mset$ can be constructed by picking $m$ different sets $\mset_{i, u}$, and picking one message out of $c\log n$ messages from each $\mset_{i, u}$. Thus, for fixed $u$ and $t$, the probability that there exists $\mset$ such that $|\mset|\geq \log n$ and all messages in $\mset$ is sent by $u$ at time $t$ is at most
\begin{align*}
%& Pr\left[\mbox{$\exists \mset$ s.t. $|\mset|> \log n$ and all messages in $\mset$ is sent by $u$ at time $t$}\right]\\
%&\ \  \leq 
\sum_{m=\log n}^{k} \binom{k}{m}(c\log n)^m\left(\frac{1}{k\log n}\right)^m. 
\end{align*}
%
Using the fact that for any $0<b<a$, $\binom{a}{b}\leq (ae/b)^b$, the previous quantity is at most
\begin{align*}
\sum_{m=\log n}^{k} \left(\frac{ke}{m}\right)^m (c\log n)^m\left(\frac{1}{k\log n}\right)^m
&\leq \sum_{m=\log n}^{k} \left(\frac{ec}{m}\right)^m\\
&\leq k\left(\frac{ec}{\log n}\right)^{\log n}.
\end{align*}
For large enough $n$, the above quantity is at most $1/n^4$. We conclude that for fixed $u$ and $t$, the probability that there exists $\mset$ such that $|\mset|\geq \log n$ and all messages in $\mset$ is sent by $u$ at time $t$ is at most  $1/n^4$. By summing this probability over all nodes $u$ and $t=O(k+h+D)=O(n)$, \Cref{thm:no congestion} follows.
\end{proof}

%
%\begin{proposition}[$k$-source $h$-hop \ksp algorithm; Proof in \Cref{sec:k-source h-hop sp}]\label{thm:k-source h-hop sp}
%%
%There is an algorithm that solves $h$-hop \sssp on network $G$ with weight $w$\danupon{Don't forget that $w$ must be positive} in $O(h)$-time and, during the whole computation, every node $u$ sends a message of size $O(\log n)$ to any of its neighbors $v$ at most once. 
%%
%\end{proposition} 
% 


\subsection{Shortest-Path Diameter Reduction Using Shortcuts}\label{sec:spd reduction}

%\danupon{Make sure to define \spdist and \spdiam in prelim}
%
In this section, we show a simple way to augment a graph with some edges (called ``shortcuts'') to reduce the shortest-path diameter. The notion of shortest path diameter is defined as follows.  
\begin{definition}[Shortest-path distance and diameter]\label{def:spdiam}
For any weighted graph $(G, w)$, the {\em shortest-path distance} between any two nodes $u$ and $v$, denoted by $\spdist_{G, w}(u, v)$, is the minimum integer $h$ such that $\dist_{G, w}^h(u, v)=\dist_{G, w}(u, v)$. That is, it is the minimum number of edges among the shortest $u$-$v$ paths. The {shortest-path diameter} of $(G, w)$, denoted by $\spdiam(G, w)$, is defined to be $\max_{u, v\in V(G)} \spdist_{G, w}(u, v)$. In other words, it is the minimum integer $h$ such that $\dist_{G, w}^h(u, v)=\dist_{G, w}(u, v)$ for all nodes $u$ and $v$. 
\end{definition}
%
%Recall from Definition~XXX that, for any weighted graph $(G, w)$, the shortest-path distance $\spdiam(G, w)$ is the minimum value of $h$ such that $\dist^h_{G, w}(u, v)=\dist^h_{G, w}(u, v)$ for all nodes $u$ and $v$. 
%
%for any weighted graph $(G, w)$, the shortest-path distance $\spdist_{G, w}(u, v)$  
%%
%%between two nodes $u$ and $v$ is the minimum number of edges among shortest $u$-$v$ paths, i.e., 
%%
%is the minimum integer $h$ such that $\dist^h_{G, w}(u, v)=\dist_{G, w}(u, v)$, and the shortest path diameter $\spdiam(G, w)$, is $\max_{u, v\in V(G)} \spdist_{G, w}(u, v)$. 
%% 
%Our main result is that for any $k$, by adding an edge from every node to {\em $k$ nearest nodes} (breaking tie arbitrarily), the shortest-path diameter of the resulting graph will be at most $n/k$, where $n$ is the number of nodes. We call the added edges {\em shortcuts} and the resulting graph a {\em $k$-shortcut graph}. 
%
%\begin{definition}[$(G, w)|_k$]\label{def:subgraph of k smallest edges}
%For any weighted graph $(G, w)$ and integer $k$, a {\em subgraph of $(G, w)$ of $k$ smallest edges}, denoted by $(G, w)|_k$ is a subgraph of $G$ consisting of $k$ edges of smallest weight incident to each node. Formally, for each node $u$ in $G$, we order the neighbors of $u$ as $v_1, v_2, \ldots$ so that $w(uv_i)\leq (uv_{i+1})$ for all $i$. Then, $(G, w)|_k$ is a subgraph of $(G, w)$ whose edges are $uv_1, \ldots, uv_k$, for all nodes $u$. 
%\end{definition}
%
%\begin{proposition}[Main result of \Cref{sec:diameter reduction}: Reducing the shortest-path diameter by shortcuts]\label{thm:shortcuts}
%For any weighted graph $(G, w)$ and an integer $k$, $\spdiam((G, w)|_k)\leq |V(G)|/k$. 
%%
%%Let $(G', w')$ denote $(G, w)|_k$, the subgraph of $(G, w)$ of $k$ smallest edges (\Cref{def:subgraph of k smallest edges}). Then, $\spdiam(G', w')$
%\end{proposition}
%
%\begin{definition}[$k$-shortcut graph]\label{def:shortcut graph}
%Consider any $n$-node weighted graph $(G, w)$ and an integer $k\neq n-1$. We define the {\em $k$-shortcut graph of $(G, w)$}, denoted by $(G, w)^k$, as a weighted graph $(G', w')$ constructed as follows. Initially, we let $(G', w')=(G, w)$. Then, for every node $u$, we order nodes in $G$ as $v_0, \ldots, v_{n-1}$ such that $\dist_{G, w}(u, v_i)\leq \dist_{G, w}(u, v_{i+1})$ for all $i$ (thus $v_0=u$), and add edges $uv_0, uv_1, \ldots, uv_k$ of weights $\dist_{G, w}(u, v_0), \dist_{G, w}(u, v_1), \ldots, \dist_{G, w}(u, v_k)$ to $(G', w')$.
%\end{definition}
%
\begin{definition}[$k$-shortcut graph]\label{def:shortcut graph}
Consider any $n$-node weighted graph $(G, w)$ and an integer $k\neq n-1$. For any node $u$, let $S^k_{G, w}(u)\subseteq V(G)$ be the set of exactly $k$ nodes nearest to $u$ (excluding $u$); i.e. $u\notin S^k_{G, w}(u)$, $|S^k_{G, w}(u)|=k$, and for all $v\in S^k_{G, w}(u)$ and $v'\notin S^k_{G, w}(u)$, $\dist_{G, w}(u,v)\leq \dist_{G, w}(u, v')$. 
%
The {\em $k$-shortcut graph of $(G, w)$}, denoted by $(G, w)^k$, is a weighted graph resulting from adding an edge $uv$ of weight $\dist_{G, w}(u, v)$ for every $u\in V(G)$ and $v\in S^k_{G, w}(u)$. When it is clear from the context, we will write $S^k(u)$ instead of $S^k_{G, w}(u)$.
\end{definition}
%
%We note that for some graph $(G, w)$, $S^k_{G, w}(u)$ might not be unique. To simplify our statement and proofs, we will assume that $(G, w)$ has the following property, which makes  $S^k_{G, w}(u)$ unique: 
%\begin{assumption}[Uniqueness of Distances]\label{assumption:unique distance}
%Every pair of nodes $u$ and $v$ has a unique value of $\dist_{G, w}(u, v).$ 
%\end{assumption}
%This assumption can be removed by breaking ties arbitrarily.  
%In this case, we call  $S^k_{G, w}(u)$ {\em the set of $k$ nodes nearest to $u$}.
%
\begin{proposition}[Main result of \Cref{sec:spd reduction}: Reducing the shortest-path diameter by shortcuts]\label{thm:shortcuts}\label{thm:spd reduction}
For any $n$-node weighted undirected graph $(G, w)$ and integer $k$, %$\spdiam((G, w)^k)\leq  4n/k$.\danupon{Don't forget to define $\spdiam((G, w))$ and say that we also use $\spdiam(G, w)$ instead of $\spdiam((G, w))$.}
if $(G', w')$ is the $k$-shortcut graph of $(G, w)$, then $\spdiam(G', w')<  4n/k$. 
\end{proposition}
\begin{proof}
Consider any nodes $u$ and $v$, and let 
\[
P=\langle u=x_0, x_1, \ldots, x_\ell=v\rangle
\]
be the shortest $u$-$v$ path in $(G', w')$ with smallest number of edges; i.e. there is no path $Q$ in $(G', w')$ such that $|E(Q)|<|E(P)|$\danupon{Define $E(P)$ and $w'(P)$} and $w'(Q)\leq w'(P)$. 
%
%there is no $u$-$v$ path having the same total edge weight and less number of edges. 
%
For any node $x$, let $S^k(x)$ be the set of $k$ nodes nearest to $x$ in $(G, w)$, as in \Cref{def:shortcut graph}. We claim that for any integer $0\leq i\leq (\ell/4)-1$, we have 
\[S^k(x_{4i})\cap S^k(x_{4(i+1)})=\emptyset.\]  
This claim immediately implies that $\ell< 4n/k$, thus \Cref{thm:shortcuts}; otherwise, $|\bigcup_{0\leq i\leq \ell/4}S_k(x_{4i})| \geq (k+1)(n/k) > n$, which is impossible. It is thus left to prove the claim that $S^k(x_{4i})\cap S^k(x_{4(i+1)})=\emptyset$. 
%
Now, consider any $1\leq i\leq \ell/4$. Observe that 
\begin{align}
\label{eq:spd reduction one}
x_{4i+2}\notin S^k(x_{4i}).
\end{align}
%
Otherwise, $(G', w')$ will contain edge $x_{4i}x_{4i+2}$ of weight $\dist_{G, w}(x_{4i},x_{4i+2})$. This implies that $P'=\langle x_0, \ldots, x_{4i-1}, x_{4i}, x_{4i+2}, x_{4i+3}, \ldots, x_\ell=v\rangle$ is a shortest $u$-$v$ path in $(G', w')$ containing $\ell-1$ edges, contradicting the fact that $P$ has the smallest number of edges among shortest $u$-$v$ paths in $(G', w')$.  By the same argument, we have 
\begin{align}
\label{eq:spd reduction two}
x_{4i+2}\notin S^k(x_{4(i+1)}).
\end{align}
%
By the definition of $S^k$, \Cref{eq:spd reduction one,eq:spd reduction two} imply that 
% for all $v\in S^k(x_{4i})$, 
\begin{align}
\label{eq:spd reduction three}\forall y\in S^k(x_{4i}) && \dist_{G, w}(x_{4i}, y) &\leq \dist_{G, w}(x_{4i}, x_{4i+2}), ~~~\mbox{and}\\
\label{eq:spd reduction four}\forall y\in S^k(x_{4(i+1)}) && \dist_{G, w}(x_{4(i+1)}, y) &\leq \dist_{G, w}(x_{4(i+1)}, x_{4i+2})
\end{align} 
respectively. Now, assume for a contradiction that there is a node $y\in S^k(x_{4i}) \cap  S^k(x_{4(i+1)})$. Consider a path 
\[
P''=\langle x_0, \ldots, x_{4i-1}, x_{4i}, y, x_{4(i+1)}, x_{4(i+1)+1}, \ldots, x_\ell=v\rangle.
\] 
Observe that $P''$ contains $\ell-3$ edges. Moreover, \Cref{eq:spd reduction three,eq:spd reduction four} imply that 
\begin{align*}
w'(x_{4i}y) &=\dist_{G, w}(x_{4i}, y)  \leq \dist_{G, w}(x_{4i}, x_{4i+2}) ~~~\mbox{and}~~~\\ 
w'(x_{4(i+1)}y) &= \dist_{G, w}(x_{4(i+1)}, y) \leq \dist_{G, w}(x_{4(i+1)}, x_{4i+2})
\end{align*}
which further imply that $w'(P'')\leq w'(P)$. This means that $P''$ is a shortest $u$-$v$ paths in $(G', w')$ and contradicts the fact that $P$ has the smallest number of edges among shortest $u$-$v$ paths in $(G', w')$. Thus,  $S^k(x_{4i}) \cap  S^k(x_{4(i+1)})=\emptyset$ as desired. 
\end{proof}

We note a simple fact that will be used throughout this paper: we can compute $S^k_{G, w}(u)$ and $\dist_{G, w}(u, v)$ for all $v\in S^k_{G, w}(u)$ if we know $k$ smallest edges incident to {\em every} nodes. The precise statement is as follows.

%fact that we can construct a $k$-shortcut graph, thus reducing the shortest path diameter, if we augment $(G, w)$ with the distance obtained  $k$ smallest 

\begin{definition}[$E^k(u)$ and $(G^k, w)$]\label{def:E^k(u) set of k smallest weight }
For any node $u$, let $E^k(u)$ be the set of $k$ edges incident to $u$ with minimum weight (breaking tie arbitrarily); i.e., for every edge $uv\in E^k(u)$ and $uv'\notin E^k(u)$, we have $w(uv)\leq w(uv')$. Let $(G^k, w)$ be the subgraph of $(G, w)$ whose edge set is $\bigcup_{v\in V(G)} E^k(v)$.
\end{definition}

We note that for some graph $(G, w)$, the sets $E^k(u)$ and $S^k_{G, w}(u)$ might not be uniquely defined. To simplify our statement and proofs, we will assume that $(G, w)$ has the following property, which makes both $S^k_{G, w}(u)$ and $S^k_{G^k, w}(u)$ unique: every edge $uv\in E(G)$ has a unique value of $w(uv)$, and every pair of nodes $u$ and $v$ has a unique value of $\dist_{G, w}(u, v)$ and $\dist_{G^k, w}(u, v).$ Removing these assumptions can be easily done by breaking ties arbitrarily. 

\begin{observation}[Computing shortcut edges using $(G^k, w)$]\label{thm:shortcuts from smallest edges}
For any node $u$, 
\begin{itemize}
\item $S^k_{G, w}(u)=S^k_{G^k, w}(u)$, and
\item $\dist_{G, w}(u, v)= \dist_{G^k, w}(u, v)$, for any $v\in S^k_{G, w}(u)$.
\end{itemize}
In other words, using only edges in  $\bigcup_{v\in V(G)} E^k(v)$ and their weights, we can compute all $k$-shortcut edges.
\end{observation}
\begin{proof} The intuition behind \Cref{thm:shortcuts from smallest edges} is that Dijkstra's algorithm can be used to compute  $S^k_{G, w}(u)$ and $\{\dist_{G, w}(u, v)\}_{v\in S^k_{G, w}(u)}$ by executing it for $k$ iterations, and this process will never need any edge besides those in $(G^k, w)$. Below we provide a formal proof that does not require the knowledge of Dijkstra's algorithm. 

Let $T_u$ be a shortest path tree rooted at $u$ in $(G, w)$. Assume for a contradiction that there is a node $v\in  S^k_{G, w}(u)\setminus  S^k_{G^k, w}(u)$. Let $z$ be the parent of $v$ in $T_u$. The fact that $v\notin S^k_{G^k, w}(u)$ implies that $zv\notin E^k(z)$\danupon{More detail?}; thus, there exists $v'$ in $E^k(z)\setminus S^k_{G^k, w}(u)$ (since $|E^k(z)|= |S^k_{G^k, w}(u)|=k$ and $S^k_{G^k, w}(u)\setminus E^k(z)\neq \emptyset$). 
%
Note that since $v\notin E^k(z)$, we have $w(zv')<w(zv)$ (recall that we assume that edge weights are distinct). This, however, implies that 
\[
\dist_{G, w}(u, v')\leq \dist_{G, w}(u, z)+w(zv') < \dist_{G, w}(u, v).
\]
This contradicts the fact that $v\in S^k_{G, w}(u)$ and  $v\notin S^k_{G, w}(u)$.
\end{proof}

%\begin{proof}
%The main idea is to show that Dijkstra's algorithm can be used to compute  $S^k_{G, w}(u)$ and $\{\dist_{G, w}(u, v)\}_{v\in S^k_{G, w}(u)}$, and it will never need any edges besides those in $(G^k, w)$. Recall that Dijkstra's algorithm iteratively adds a node to the shortest path tree rooted at $u$, denoted by $T_u$. It is proved that in each iteration this algorithm adds to $T_u$ a node $v\notin T_u$ such that $v=\arg\min_{v'\notin T_u} \dist_{G, w}(u, v)$. Thus, by running this algorithm for $k$ iterations we will get  $S^k_{G, w}(u)$ (which is exactly $T_u$ after the $k^{th}$ iteration) and $\{\dist_{G, w}(u, v)\}_{v\in S^k_{G, w}(u)}$. 
%
%\danupon{I'm still not very happy with this proof.}Let $i$ be the first iteration where Dijkstra's algorithm adds to $T_u$ a node that is {\em not} in $S^k_{G^k, w}(u)$; i.e., $i$ is the minimum positive integer $i'\leq k$ such that, at iteration $i'$, Dijkstra's algorithm adds a node $v\notin S^k_{G^k, w}(u)$ to $T_u$. (We can assume that such $i$ exists; otherwise,  $S^k_{G, w}(u)= S^k_{G^k, w}(u)$ and we are done proving \Cref{thm:shortcuts from smallest edges}.) Let $z$ be the parent of $v$ in $T_u$. The fact that $v\notin S^k_{G^k, w}(u)$ implies that $zv\notin E^k(z)$\danupon{More detail?}; thus, $w(zv')<w(zv)$ for all $v'\in v'\in E^k(z)$. Since $|T_u\setminus \{v\}|=i-1<k$, there is a node $v'\in E^k(z)\setminus T_u$. ...
%
%\end{proof}


%\begin{lemma}[Computing shortcut edges using small-weight edges]\label{thm:shortcuts from smallest edges}
%%Consider any $n$-node weighted undirected graph $(G, w)$ and integer $k$.
%%
%Using only edges in  $\bigcup_{v\in V(G)} E^k(v)$ and their weights, we can compute, for every node $u$, the set $S^k(u)$ and distance $\dist_{G, w}(u, v)$ for all $v\in S^k(u)$. 
%\end{lemma}
%\danupon{To do: Use $S^k_u$ instead of $S^k(u)$.}
%\begin{proof}
%Let $(G^k, w)$ be the subgraph of $(G, w)$ whose edge set is $\bigcup_{v\in V(G)} E^k(v)$. We assume 
%%Let $S^k(u)$ be the set of $k$ nodes nearest to $u$ in $(G^k, w)$; i.e., for any $v\in S^k(u)$ and $v'\notin S^k(u)$, $\dist_{G^k, w}(u, v)\leq \dist_{G^k, w}(u, v')$. 
%%
%We will show that
%\begin{itemize}
%\item $S^k_{G,w}(u)$ is also the set of $k$ nodes nearest to $u$ in $(G, w)$; i.e., for any $v\in S^k(u)$ and $v'\notin S^k(u)$, we have $\dist_{G, w}(u, v)\leq \dist_{G, w}(u, v')$
%\item For any $v\in S_u$, $\dist_{G, w}(u, v)= \dist_{G^k, w}(u, v)$.
%\end{itemize}
%The above claims immediately imply \Cref{thm:shortcuts from smallest edges}. Now we prove the above claims. 
%%
%To simplify the argument, we will assume that every edge has a unique edge weight and every node $v$ has a unique value of $\dist_{G,w}(u, v)$. Consider when we run Dijkstra's algorithm to solve \sssp on $(G, w)$ using $u$ as a source. Consider the first $k$ iteration where we add $k$ nodes (besides $u$) to the shortest path tree. Clearly, these nodes are the $k$ nodes
%
%Assume for a contradiction that the first claim does not hold; i.e. 
%
%there are nodes $v\in S^k(u)$ and $v'\notin S^k(u)$ such that $\dist_{G, w}(u, v)> \dist_{G, w}(u, v')$. Let $T$ be a shortest tree rooted at $u$ in $(G, w)$, and $T'$ be the subtree of $T$ induced by nodes in $S^k(u)$. Note that $T'$ must be connected by the definition of $S^k(u)$\danupon{More detail here?}.   
%\end{proof}

%\subsection{Simulating a Broadcast Network on an Overlay Network and Consequences}\label{sec:broadcast to overlay}\label{sec:overlay}
%
%
%An overlay network is a virtual network of nodes and logical links that is built on top of an existing network with the purpose of implementing a network service that is not available in the existing network.
%
%Corollaries: sparisification and light-weight sssp on overlay network\danupon{This comes first since we will use light-weight sssp.}
%
%
%%----------- Notes ---------------
%
%
%%From http://cs.brown.edu/~jj/papers/thesis-phd02.pdf:  We will use three metrics to evaluate how eciently an overlay network is operating. Stress indicates the number of times that a semantically identical packet traverses a given link. In IP Multicast, stress never exceeds one. On the other hand, overlay networks could not hope to achieve such eciencies because packets being forwarded by an edge node will traverse (at least) the node's local link twice. Stretch indicates the ratio of latency in an overlay network compared to some baseline, generally IP unicast or multicast. Misres measures the number of times that duplicate packets are mistakenly sent to the same destination. These metrics are used to evaluate overlay performance with the primitives proposed in this thesis in Chapter 7.




==> clustering.tex <==
\section{Node Clustering (Proposition~\ref{prop:clustering})}\label{sec:clustering}

In this Section, we prove Proposition~\ref{prop:clustering}: Nodes in $G$ can be partitioned into {\em clusters} $C_1, C_2, \ldots, C_k$, for some $k$, such that for any $\vec w\in \cW_i\cup \{w_i\}$, $\dist_{G, \vec w}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster. Moreover, such partition can be found in $O(n)$ time. 

%Nodes in $G$ can be partitioned into {\em clusters} $C_1, C_2, \ldots, C_k$, for some $k$, such that,for any $\vec w\in \cW_i\cup \{w_i\}$, $\dist_{G, \vec w}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster. Moreover, such partition and their sizes can be found in $O(n)$ time. In the end, every node $u$ knows which cluster every node $v$ is in; i.e., it knows the set $\{(v, \rep(C_j) \mid v\in C_j\}$ where we define $\rep(C_j)$ to be $\rep(C_j)=\min_{v\in C_j} v$.

%In this section, we prove Lemma~\ref{lem:clustering}.
%
To prove this, consider the node partition $\cC=\{C_1, \ldots, C_{k}\}$ where, for any node $u$ and $v$, $u$ and $v$ are in the same partition if and only if $\dist_{G, w_i}(u,v)=0$.
%
Note the following important property of $(G, \cW_i)$.
%
\begin{claim}\label{claim:scaling preserves zero}
For any node $s$, $u$ and $v$, $\vec w_i^s(uv)\geq 0$. Moreover, $\vec w_i^s(uv)=0$ if and only if $w_i(uv)=0$.
\end{claim}
%
\begin{proof}
Recall that $b_i(uv)$ is the $i^{th}$ bit of $w(uv)$ (cf. Definition~\ref{def:w_i}), and note that $w_{i}(uv)=2w_{i+1}(uv)+b_i(uv).$ It follows from the definition of $\vec w_i^s$ (Line~\ref{line:w_i} of Algorithm~\ref{algo:apsp}) that
\begin{align*}
\vec w_i^s(uv) &= 2\dist_{G, w_{i+1}}(s, u)-2\dist_{G,w_{i+1}}(s, v)+w_i(uv)\\
&=2\dist_{G,w_{i+1}}(s, u)-2\dist_{G,w_{i+1}}(s, v)+2w_{i+1}(uv)+b_i(uv)\\
&\geq b_i(uv)\,.
\end{align*}
Note that last inequality follows from the triangle inequality property of the distance function; i.e. for any $w'$, $\dist_{G,w'}(s, u)+w'(uv)\geq \dist_{G,w'}(s, v)$. It follows immediately that $\vec w_i^s(uv)\geq 0$.

Moreover, if $w_i(uv)>0$, then  $b_i(uv)>0$ (since $b_i(uv)$ is a bit in the {\em positive} binary representation of $w_i(uv)$); thus, $w_i(uv)>0$ implies that $\vec w_i^s(uv)>0$. 

Finally, if $w_i(uv)=0$, then clearly $w_{i+1}(uv)=0$, and thus $\dist_{G,w_{i+1}}(s, u)=\dist_{G,w_{i+1}}(s, v)$. It follows that, $\vec w_i^s(uv)= 2\dist_{G, w_{i+1}}(s, u)-2\dist_{G,w_{i+1}}(s, v)+w_i(uv)=w_i(uv)=0$.
\end{proof}
%
The above claim implies that, for any nodes $s$, $u$ and $v$, $\dist_{G, \vec w_i^s}(u, v)=0$ if and only if $\dist_{G, w_i}(u, v)=0$. It follows from the definition of $\cC$ that $\dist_{G, \vec w_i^s}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster. This shows that $\cC$ satisfies the property claimed in Proposition~\ref{prop:clustering}.

Computing $\cC$ in $O(n)$ time is very easy. First, every node broadcasts the minimum ID it has seen so far {\em through edges of weight zero only}. After repeating this for $n-1$ rounds, it is easy to see that the minimum ID that node $u$ has seen so far is exactly $\rep(C_j)$, where $j$ is such that $u\in C_j$.
%
Next, every node $u$ broadcasts to all other nodes a message $(u, \rep(C_j))$ where $C_j$ is the cluster that contains $u$. Since there are exactly $n$ messages broadcasted, we only need $O(n+D(G))=O(n)$ time for broadcasting them.
%
%(In fact, repeating this for $\max_j |C_j|$
%
%Every node $u$ then broadcasts the pair $(u, \rep(S_{w_i}(u)))$ so that other nodes knows $\rep(S_{w_i}(u))$ (this can be done by, e.g., aggregating and broadcasting on a BFS tree).
%
%Secondly, for each cluster $C_j$, $\rep(C_j)$ computes a BFS tree rooted at $u$ using only edges of weight zero. It can then use this BFS tree to compute $|C_j|$ and broadcast this value to all nodes in $S_{w_i}(u)$. The BFS trees from these nodes can be computed in parallel, taking $\max_j |C_j|=O(n)$ rounds in total.


==> diameter_bound.tex <==
\section{Multi-Weight Diameter (Proposition~\ref{prop:multi-weight diameter})}\label{sec:multi weight diameter bound}
In this section, we prove Proposition~\ref{prop:multi-weight diameter}: $\ecc(G, \cW_i)\leq 2n.$ In particular, fix any nodes $s$ and $u$, we show that $\dist_{G, \vec w_i^s}(s, u)\leq 2n.$

To prove this, recall that $b_i(xy)$ is the $i^{th}$ bit of $w(xy)$ (cf. Definition~\ref{def:w_i}), and observe that
\begin{align}
w_{i}(xy)&=2w_{i+1}(xy)+b_i(xy). \label{eq:w_i equal w_i+1 plus b_i}
\end{align}
%Also recall from Line~\ref{line:w_i} of Algorithm~\ref{algo:apsp} that 
%$$\vec w_i^s(uv)=2\dist_{w_{i+1}}(s, u)-2\dist_{w_{i+1}}(s, v)+w_i({uv}).$$ 
%
Let $P=\langle s=x_0, x_1, \ldots, x_\ell=u\rangle$ be any shortest $s$-$u$ path in weighted network $(G, w_{i+1})$. The length of this path in $(G, \vec w_i^s)$ is

\noindent{\fontsize{8}{0}\selectfont
%\small
\noindent\hspace{-.05in}\parbox{1.06\linewidth}{
\begin{align}
\vec w_i^s(P)  &= \sum_{j=0}^{\ell-1} \vec w_i^s(x_jx_{j+1})\nonumber\\
&=\left(2\dist_{G, w_{i+1}}(s, x_0)-2\dist_{G, w_{i+1}}(s, x_{1})+w_i(x_0x_{1})\right)\nonumber\\
&\ +\left(2\dist_{G, w_{i+1}}(s, x_1)-2\dist_{G, w_{i+1}}(s, x_{2})+w_i(x_1x_{2})\right)\nonumber\\
&\ +\ldots \nonumber\\
&\ +\left(2\dist_{G, w_{i+1}}(s, x_{\ell-1})-2\dist_{G, w_{i+1}}(s, x_{\ell})+w_i(x_{\ell-1}x_{\ell})\right)\label{eq:multi diam one}\\
%&=\sum_{j=0}^{\ell-1}\left(2\dist_{G, w_{i+1}}(s, x_j)-2\dist_{G, w_{i+1}}(s, x_{j+1})+w_i(x_jx_{j+1})\right)\label{eq:multi diam one}\\
&= \sum_{j=0}^{\ell-1} w_i(x_jx_{j+1})-2\dist_{G,w_{i+1}}(s, x_k)+2\dist_{G,w_{i+1}}(s, x_0)\label{eq:multi diam two}\\
&= \sum_{j=0}^{\ell-1} w_i(x_jx_{j+1})-2\sum_{j=0}^{\ell-1} w_{i+1}(x_jx_{j+1})\label{eq:multi diam three}\\
&= \sum_{j=0}^{\ell-1} b_i(x_jx_{j+1}))\label{eq:multi diam four}
\end{align}
}
}
where Eq.\eqref{eq:multi diam one} is by the definition of $\vec w_i^s$ (cf. Line~\ref{line:w_i} of Algorithm~\ref{algo:apsp}), Eq.\eqref{eq:multi diam two} is by telescoping sum,  Eq.\eqref{eq:multi diam three} uses the fact that $s=x_0$ and $P$ is a shortest $s$-$u$ path in $(G, w_{i+1})$, and Eq.\eqref{eq:multi diam four} follows from Eq.\eqref{eq:w_i equal w_i+1 plus b_i}.

It follows that $\dist_{G, \vec w_i^s}(s, u)\leq \vec w_i^s(P)=\sum_{j=0}^{\ell-1} b_i(x_jx_{j+1})$ which is at most $2\ell$ since $b_i(xy)\leq 2$ for any edge $xy$. Thus,  $\dist_{G, \vec w_i^s}(s, u)\leq 2\ell\leq 2n$ as claimed. 


==> dprime.tex <==
\section{Property of {\lowercase{\large$\mathbf{d'}$}} (Proposition~\ref{prop:d prime})}\label{sec:d prime}

In this section, we prove Proposition~\ref{prop:d prime}: for any $K\geq \ecc(G, \cW_i)$, we show that $d'(s, u)=2\dist_{G, w_{i+1}}(s, u)+\dist^{K}_{H, \vec w_i^s}(s, u)$ has the property that (1) $d'(u, v)\geq \dist_{G, w_i}(u, v)$, and (2) if $\dist_{H, w_i}(u, v)=\dist_{G, w_i}(u, v)$, then $d'(u, v)=\dist_{G, w_i}(u, v)$.

First, we note the following important claim.

%\begin{claim}\label{claim:dist w_i from dist w_i^u}
%For any nodes $s$ and $u$,
%$$\dist_{H, w_i}(s, u)=2\dist_{H, w_{i+1}}(s, u)+\dist_{H, \vec w_i^s}(s, u).$$
%\end{claim}
%\begin{proof}
%Let $P=\langle s=x_0, x_1, \ldots, x_\ell=u\rangle$ be any $s$-$u$ path in $G$. By definition, the length of this path in $(H, \vec w_i^s)$ is
%%
%{\small
%\begin{align*}
%\vec{w}_i^s(P)  &= \sum_{j=0}^{\ell-1}2\dist_{H, w_{i+1}}(s, x_j)-2\dist_{H, w_{i+1}}(s, x_{j+1})+w_i(x_jx_{j+1})\\
%&= 2\dist_{H, w_{i+1}}(s, x_0)-2\dist_{H, w_{i+1}}(s, x_k)+\sum_{j=0}^{k-1} w_i(x_jx_{j+1}).
%\end{align*}
%}
%%
%Using $\dist_{H, w_{i+1}}(s, x_0)=0$ (since $s=x_0$), $x_k=u$, and $\sum_{j=0}^{k-1} w_i(x_jx_{j+1})=w_i(P)$, we can rewrite this to $w_i(P)=2\dist_{H, w_{i+1}}(s, u)+\vec w_i^s(P).$ Thus,
%\begin{align*}
%\dist_{H, w_i}(s, u)&=\min_{\mbox{$P$: $s$-$u$ path}} w_i(P)\\
%&=2\dist_{H, w_{i+1}}(s, u) + \min_{\mbox{$P$: $s$-$u$ path}} w_i^s(P)\\
%&=2\dist_{H, w_{i+1}}(s, u)+\dist_{H, \vec w_i^s}(s, u)
%\end{align*}
%as claimed. \danupon{Define $w_i(P)$!!}
%\end{proof}
\begin{claim}\label{claim:dist w_i from dist w_i^u}
For any $K\geq \ecc(G, \cW_i)$ and nodes $s$ and $u$,
$$\dist_{G, w_i}(s, u)=2\dist_{G, w_{i+1}}(s, u)+\dist^{K}_{G, \vec w_i^s}(s, u).$$
\end{claim}
\begin{proof}
Note that, since $K\geq \ecc(G, \cW_i)$, $K\geq \dist_{G, \vec w_i^s}(s, u)$ for all nodes $s$ and $u$. Thus, by the definition of $\dist^K_{G, \vec w_i^s}$ (cf. Definition~\ref{def:bounded dist apsp}), $\dist^K_{G, \vec w_i^s}(s, u)=\dist_{G, \vec w_i^s}(s, u)$. So, we will drop the superscript and use $\dist_{G, \vec w_i^s}$ instead of $\dist^K_{G, \vec w_i^s}$.


Let $P=\langle s=x_0, x_1, \ldots, x_\ell=u\rangle$ be any $s$-$u$ path in $G$. By definition, the length of this path in $(G, \vec w_i^s)$ is
%
{\small
\begin{align*}
\vec{w}_i^s(P)  &= \sum_{j=0}^{\ell-1} \left(2\dist_{G, w_{i+1}}(s, x_j)-2\dist_{G, w_{i+1}}(s, x_{j+1})+w_i(x_jx_{j+1})\right)\\
&= 2\dist_{G, w_{i+1}}(s, x_0)-2\dist_{G, w_{i+1}}(s, x_k)+\sum_{j=0}^{k-1} w_i(x_jx_{j+1}).
\end{align*}
}
%
Using $\dist_{G, w_{i+1}}(s, x_0)=0$ (since $s=x_0$), $x_k=u$, and $\sum_{j=0}^{k-1} w_i(x_jx_{j+1})=w_i(P)$, we can rewrite this to 
$$w_i(P)=2\dist_{G, w_{i+1}}(s, u)+\vec w_i^s(P).$$ 
Thus (recall that $\cP_G(s, u)$ is the set of all simple paths from $s$ to $u$ in $G$),
\begin{align*}
\dist_{G, w_i}(s, u)&=\min_{P\in \cP_G(s, u)} w_i(P)\\
&=2\dist_{G, w_{i+1}}(s, u) + \min_{P\in \cP_G(s, u)} \vec w_i^s(P)\\
&=2\dist_{G, w_{i+1}}(s, u)+\dist_{G, \vec w_i^s}(s, u)
\end{align*}
as claimed.
\end{proof}
%
Now, note that $\dist^{K}_{H, \vec w_i^s}(s, u)\geq \dist^{K}_{G, \vec w_i^s}(s, u)$ since $H$ is a subgraph of $G$. Thus,
\begin{align}
d'(s, u) &= 2\dist_{G, w_{i+1}}(s, u)+\dist^{K}_{H, \vec w_i^s}(s, u)\\
&\geq 2\dist_{G, w_{i+1}}(s, u)+\dist^{K}_{G, \vec w_i^s}(s, u)\label{eq:d prime one}\\
&=\dist_{G, w_i}(s, u),
\end{align}
where the last equality is by Claim~\ref{claim:dist w_i from dist w_i^u}. This proves the first claim of Proposition~\ref{prop:d prime}.
%
For the second claim, we note that if  $\dist_{H, \vec w_i^s}(s, u)= \dist_{G, \vec w_i^s}(s, u)$ then  $\dist^{K}_{H, \vec w_i^s}(s, u)=\dist^{K}_{G, \vec w_i^s}(s, u)$ since $K\geq \ecc(G, \cW_i)\geq \dist_{G, \vec w_i^s}(s, u)$. Thus, ``$\geq$'' in Eq.~\eqref{eq:d prime one} can be replaced by ``$=$''.
%\end{proof}


==> main_algo5.tex <==
\section{Exact Algorithm (Main)}\label{sec:main algo}\label{sec:scaling}

\begin{algorithm*}[t]
\caption{{\sc Main}($G, w$) (detail in Section~\ref{sec:main algo})}\label{algo:apsp}
{\bf Input:} Undirected weighted network $(G, w)$ (note that $w$ is symmetric).

{\bf Output:} For every node $u$ and $v$, both $u$ and $v$ know $\dist_{G, w}(u, v)$.

\begin{algorithmic}[1]


\State Compute $w_i$ and $\beta$ as in Definition~\ref{def:w_i}. {\small \it // As a result, every node $u$ knows $\beta$ and $w_i(uv)$ for every edge $uv$ in $G$. This takes $O(n)$ time.}
%{\small \it // As a quick reminder, we write $w$ as $\beta$-bit positive binary number (cf. Def.~\ref{def:positive binary representation}), and $w_i$ consists of the $\beta^{th}$ to $i^{th}$ bits.}\label{line:beta}

\For{$i=\beta, \beta-1, \ldots, 0$} %\Comment{This is Iteration $i$.}

\State {\small\it // This is Iteration $i$. We will solve \apsp on $(G, w_i)$.} %Let $t_i$ be the round at the beginning of this iteration.


\vspace{.1em}
\State \label{line:w_i} Every node $u$ in $G$ computes $\vec w_i^s(uv)$ defined as $\vec w_i^s(uv)=2\dist_{w_{i+1}}(s, u)-2\dist_{w_{i+1}}(s, v)+w_i({uv})$, for every edge $uv\in E(G)$ and every node $s$ in the network. Let $\cW_i=\{\vec w_i^s\}_{s\in V(G)}$.  {\small \it // Can be done in $O(n)$ time (cf. Claim~\ref{claim:w_i time}).}


\vspace{.1em}
\State Partition nodes into clusters $C_1, \ldots, C_k$, for some $k$, with properties as in Proposition~\ref{prop:clustering}. As a result, every node $u$ knows which cluster every node $v$ is in; i.e., it knows the set $\{(v, \rep(C_j) \mid v\in C_j)\}$ where we define $\rep(C_j)$ to be $\rep(C_j)=\min_{v\in C_j} v$. {\small\it // $O(n)$ time by Proposition~\ref{prop:clustering}.} \label{line:clustering}

%; i.e., for every node $s$, $\dist_{G, \vec w_i^s}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster. {\small\it // As a result, every node $u$ in cluster $C_j$ knows $\rep(C_j)=\min_{v\in C_j} v$ and $|C_j|$. This step takes $O(n)$ time by Lemma~\ref{lem:clustering}.} \label{line:clustering}

%
%\hspace{.5em}
%{\small \it As a result, every node $u$ in cluster $C_j^i$ knows $\rep(C_j^i)$ the smallest ID node in $C_j^i$}


%\hspace{.5em} {\small // The above can be done in $O(n)$ time.}

\vspace{.2em}
\State For all $j$, let $E_j=\{uv\in E(G)\mid u, v\in C_j\}$.  Compute $H$ defined as the subgraph of $G$ with edge set $E(H)=E(G)\setminus (\bigcup_{j: |C_j|>\sqrt{n}} E_j)$.  {\small\it // As a result, every node in network $G$ knows which edges in $E(G)$ incident to it are in the subgraph $H$. This step needs no communication.}\label{line:compute H}
%In other words, we obtain $H$ by deleting all edges between two nodes in $C_i$ for all $C_i$ such that $|C_i|>\sqrt{n}$.



\vspace{.2em}
\State Solve multi-weight $(2n)$-\apsp (cf. Definition~\ref{def:multi weight apsp}) on $(H, \cW_i)$ using Proposition~\ref{prop:pseudopoly multi-weight} with $\zero(H, \cW_i)=\sqrt{n}$. {\small\it // Finishes in $O(n\sqrt{n}\log n)$ time with high probability. As a result, every node $u$ knows $\dist^{2n}_{H, \vec w_i^s}(s, u)$ for all $s$.} \label{line:multi-weight apsp}


\State Every node $u$ computes the candidate distance function $d'(s, u)=2\dist_{G, w_{i+1}}(s, u)+\dist^{K}_{H, \vec w_i^s}(s, u)$ for all nodes $s$, as in Proposition~\ref{prop:d prime}. {\small\it // Need no communication.}\label{line:d prime}
%See Lemma~\ref{lem:d prime} for the meaning of $d'$.}

%\State Every node $u$ computes, for all nodes $s$, $\dist^{2n}_{H, w_i}(s, u)$ using the following formula: $\dist^{2n}_{H, w_i}(s, u)=2\dist^{2n}_{G, w_{i+1}}(s, u)+\dist^{2n}_{H, \vec w_i^s}(s, u)$. {\small\it // No communication. Lemma~\ref{lem:dist w_i from dist w_i^u} guarantees correctness.}\label{line:solve apsp on H w_i}



\vspace{.2em}
\State For all $j\neq j'$, every node $u$ in cluster $C_j$ computes $d'(C_j, C_{j'})$ defined as $d'(C_j, C_{j'})=\min_{u\in C_j, v\in C_{j'}}d'(u, v)$. {\small\it // Can be done in $O(n)$ time (cf. Claim~\ref{claim: running time of line:collect distance within cluster}).}\label{line:collect distance within cluster}



\vspace{.2em}
\State For every cluster $C_j$ such that $|C_j|>\sqrt{n}$, $\rep(C_j)$ broadcasts $d'(C_j, C_{j'})$, for all $j'\neq j$, to all nodes in the network. {\small\it // Can be done in $O(n\sqrt{n})$ time since there are at most $O(n\sqrt{n})$ messages broadcasted (cf. Claim~\ref{claim: running time of line:broadcast big cluster}).}\label{line:broadcast big cluster}

%\hspace{.5em} {\small // The above can be done in $O(n\sqrt{n})$ time since there are at most $O(n\sqrt{n})$ messages broadcasted (cf. Lemma~XXX).}



\vspace{.2em}
\State For every cluster $C_j$ and node $u\in C_j$, node $u$ internally constructs graph $G'_u$ consisting of node set $V(G'_u)=\{c_1, \ldots, c_k\}$ and edge sets $E(G'_u)=E_1'\cup E'_2$ where $E_1'=\{c_jc_{j'} \mid j'\neq j\}$ and $E_2'=\{c_{j'}c_{j''} \mid j'\neq j''\ \wedge\ |C_{j'}|>\sqrt{n}\ \wedge\ |C_{j''}|>\sqrt{n}\}$. Define edge weight $w'$ as $w(c_{j'}c_{j''})=d'(C_{j'}, C_{j''})$ for any edge $c_{j'}c_{j''}$. {\small \it // Need no communication since all required information is already computed in Line~\ref{line:collect distance within cluster} and \ref{line:broadcast big cluster} (cf. Claim~\ref{claim:running time of line:G prime}).}\label{line:G prime}


\vspace{.2em}
\State Node $u$ computes, for every node $v\neq u$, $\dist_{G, w_i}(u, v)$ using Proposition~\ref{prop:G prime}: $\dist_{G, w_i}(u, v)=\dist_{G'_u, w'}(c_j, c_{j'})$ where $j$ and $j'$ are such that $u\in C_j$ and $v\in C_{j'}$. {\small // Need no communication.} \label{line:final computation}


\EndFor

\end{algorithmic}
\end{algorithm*}



%\begin{algorithm*}
%\caption{Computing $\dist_{w_i^x}(x, u)$. (Detail in Section~\ref{sec:supernode}-\ref{sec:heavy}.)}\label{algo:compute dist_i^u}
%{\bf Input:} Every node $u$ knows $w_i^x(\overrightarrow{uv})$ and $G, w_i^x(\overrightarrow{vu})$ for all neighbors $v$ and any node $x$.
%
%{\bf Output:} Every node $u$ knows $\dist_{w_i^x}(x, u)$ for all nodes $x$.
%
%\begin{algorithmic}[1]
%
%
%
%
%
%\State Now every node $u$ knows $\dist_{w_i^x}(x, u)$ for all nodes $x$, regardless of whether $(x, u)$ is $(G, w_i)$-light or $(G, w_i)$-heavy.
%\end{algorithmic}
%\end{algorithm*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this section, we explain the main algorithm for solving \apsp exactly, as outlined in Algorithm~\ref{algo:apsp}. Our algorithm uses the weight scaling technique, which is based on the {\em positive binary representation} of weights. This is similar to the standard binary representation except that every bit is either one or two:
%
\begin{definition}\label{def:positive binary representation}
For any positive integer $x$, we say that a sequence of integers $b_0, b_1, \ldots, b_k\in \{1, 2\}$ is a {\em positive binary representation} of $x$ if $x=\sum_{i=0}^k b_i2^i$.
\end{definition}
%
We note again that we cannot use the standard binary representation since Proposition~\ref{prop:clustering} will not hold in this case. Also note that, for any positive integer $x$, a positive binary representation always exists and can be easily computed by the following algorithm: Let $x_0=x$, and define $x_1, x_2, \ldots$ and $b_0, b_1, \ldots$ as follows. For any $i\geq 0$ such that $x_i>0$, if $x_i$ is odd, then we let $b_i=1$ and $x_{i+1}=(x_i-1)/2$; otherwise, let $b_i=2$ and $x_{i+1}=(x_i-2)/2$. Also note that it can be proved that any $x$ has a unique positive binary representation, but we will not need this fact here.\danupon{To do: Write this as claim.}

%Let $\beta=\lceil\log W\rceil$. Our algorithm solves \apsp on graphs $(G, w_0)$, $(G, w_1)$, $\ldots$, $(G, w_\beta)$, where  $w_i$ consists of bits of $w$ from the $i^{th}$ bit to the last bit. Formally:

Algorithm~\ref{algo:apsp} runs in {\em iterations}. In Iteration $i$, we solve \apsp on graph $G$ with weight function $w_i$, where $w_i$ is defined as the number consisting of bits of $w$ from the $i^{th}$ bit to the $k^{th}$ bit, as follows.
%
\begin{definition}[$w_i$ and $\beta$]\label{def:w_i} For any edge $uv$, let $k_{uv}$ and $b_0(uv)$, $\ldots$, $b_{k_{uv}}(uv)$ be the binary representation of $w(uv)$. Also let $b_i(uv)=0$ for all $i>k_{uv}$.
%
Let
$$\beta=\max_{uv\in E(G)} k_{uv} ~~\mbox{ and }~~ w_i(uv)=\sum_{j=i}^{\infty} b_j(uv)2^j$$
for any $i\geq 0$.
\end{definition}
%
%%
%In order to solve \apsp at Iteration $i$ quickly, we use the solution from Iteration $i+1$ (i.e. $\dist_{w_{i+1}}(uv)$ for all edges $uv$) to compute several {\em directed} weighted graphs and solve \sssp on these graphs instead. In particular, we define a weight function $w_i^x$ on directed edges as follows.
%%
%\begin{definition}\label{def:w_i^u}
%For any node $x$ and directed edge $\overrightarrow{uv}$ in $\overrightarrow{}$, define $w_i^x$ as $w_i^x(\overrightarrow{uv})=2\dist_{w_{i+1}}(x, u)-2\dist_{w_{i+1}}(x, v)+w_i(uv)$.
%\end{definition}
%
Note that $\beta=O(\log n)$ since the largest weight is $O(\poly(n))$, and we can make every node know $\beta$ in $O(D(G))=O(n)$ rounds.
%
Our algorithm starts from Iteration $\beta$ down to Iteration $0$ (see the for-loop in Algorithm~\ref{algo:apsp}). In each Iteration $i$, the algorithm does the following.

First, it transforms weight function $w_i$ to a collection $\cW_i=\{\vec w_i^s\}_{s\in V(G)}$ of $n$ weight functions, as in {\bf Line~\ref{line:w_i}} of Algorithm~\ref{algo:apsp}. At the end of this step, every node $u$ knows $\vec w_i^s(uv)$ for all neighbors $v$ and nodes $s$. We note that this step can be completed in $O(n)$ time, simply by exchanging $n$ messages between neighbors, as in the following claim.
%
\begin{claim}[Proof in Appendix~\ref{sec:omitted proofs}]\label{claim:w_i time}\label{CLAIM:W_I TIME}
Line~\ref{line:w_i} of Algorithm~\ref{algo:apsp} can be done in $O(n)$ time.
\end{claim}
%
Next, in {\bf Line~\ref{line:clustering}}, the algorithm partitions nodes into {\em clusters} using Proposition~\ref{prop:clustering} introduced in Section~\ref{sec:overview}. At the end of this step, every node $u$ knows the following information about all other nodes $v$.

For any cluster $C_j$, we define the {\em representative node of $C_j$}, denoted by $\rep(C_j)$, as the minimum node ID in $C_j$, i.e. $\rep(C_j)=\min_{v\in C_j} v$. At the end of Line~\ref{line:clustering}, we want every node $u$ to know, for all $v$, $\rep(C_j)$ where $C_j$ is the cluster that contains $v$. As claimed in Proposition~\ref{prop:clustering}, this step takes $O(n)$ time.

In {\bf Line~\ref{line:compute H}}, we compute the subgraph $H$ obtained from $G$ by deleting all edges in clusters of size more than $\sqrt{n}$ (we call these clusters {\em big clusters}); i.e., we delete all edges in $\{uv\in E(G) \mid \exists j:\ u, v\in C_j\ \&\ |C_j|>\sqrt{n}\}$. To compute $H$, every node $u$ simply check whether it is in a big cluster. If it is in a big cluster, then it marks all edges $uv$, for all neighbors $v$ that are in the same cluster, as ``deleted''. Note that this step can be done without any communication since every node knows the clusters other nodes are in from  Line~\ref{line:clustering}; so it can use  use this information to check which clusters it and its neighbors are in, as well as the sizes.

Now that we have the subgraph $H$, we will, in {\bf Line~\ref{line:multi-weight apsp}}, solve the multi-weight $K$-\apsp problem (cf. Definition~\ref{def:multi weight apsp}) on $(H, \cW_i)$, using $K=2n$. This is guaranteed to be doable in $O(n\sqrt{n}\log n)$ time, by Proposition~\ref{prop:pseudopoly multi-weight} and the following claim. (Recall that $\zero(G, \cW)$ is the longest zero path length of $(G, \cW)$ defined before we state Proposition~\ref{prop:pseudopoly multi-weight}.)
\begin{claim}
$\zero(H, \cW_i)\leq \sqrt{n}.$
\end{claim}
\begin{proof}
For any node $s$ and $\ell>0$, let $P=\langle x_0, x_1, \ldots, x_\ell\rangle$ be any simple path of distance zero in $\vec w_i^s$; i.e., $\vec w_i^s(x_ix_{i+1})=0$ for all $0\leq i\leq \ell-1$. By Proposition~\ref{prop:clustering},
$w_i(x_ix_{i+1})=0$ for all $0\leq i\leq \ell-1$. It follows that all nodes in $P$ must be in the same cluster. Since we delete all edges within big clusters (in Line~\ref{line:compute H}) and $P$ has at least one edge, nodes in $P$ must be in $C_j$ such that $|C_j|\leq \sqrt{n}$. In other words, $\ell\leq \sqrt{n}$. This implies that any simple path of distance zero (for any edge weight $\vec w_i^s$) has length at most $\sqrt{n}$, i.e., $\zero(H, \cW_i)\leq \sqrt{n}.$
\end{proof}
%
In {\bf Line~\ref{line:d prime}}, the algorithm {\em tries} to use the solution of multi-weight $(2n)$-\apsp on $(H, \cW_i)$ to solve $(2n)$-\apsp on $(G, w_i)$. This results in the {\em candidate distance function} $d'$. While it is not true that $d'(u, v)=\dist_{G, w_i}(u, v)$ for all nodes $u$ and $v$ (we would have got this if we can use Eq.\eqref{eq:ideal w_i recovery}), this is the case for the pairs of nodes whose distances are preserved by $(H, w_i)$, as shown by Proposition~\ref{prop:d prime}.
%
Note that this step needs no communication since $u$ already knows $\dist_{G, w_{i+1}}(s, v)$, for all nodes $s$, from Iteration $i+1$, and $\dist_{H, \vec w_i^s}(s, u)$ is computed in Line~\ref{line:multi-weight apsp}.
%
%The correctness of this step is guaranteed by the following lemma.
%


Next, in {\bf Line~\ref{line:collect distance within cluster}}, every node $u$ computes $d'(C_j, C_{j'})=\min_{u\in C_j, v\in C_{j'}}d'(u, v)$ for all nodes $v$, where $C_j$ and $C_{j'}$ are clusters containing $u$ and $v$, respectively. We note that the running time of this step is $O(n)$:
%
\begin{claim}\label{claim: running time of line:collect distance within cluster}
Line~\ref{line:collect distance within cluster} of Algorithm~\ref{algo:apsp} finishes in $O(n)$ time.
\end{claim}
\begin{proof}
The algorithm simply performs an ``internal communication'' within each cluster. In particular, for each cluster $C_j$, the representative node $\rep(C_j)$ collects $d'(C_j, C_{j'})$, for all $j'$. This is done by constructing a BFS tree $T$ spanning the (connected) subgraph of $G$ induced by $C_j$. Then, every node $u\in C_j$ sends to its parent
$d'(T_u, C_{j'})$ $=\min_{u'\in T_u, v\in C_{j'}}$ $d'(u', v)$
where $T_u$ is the subtree of $T$ rooted at $u$. This can be easily done in $O(\delta_T+k)$ time, where $\delta_T$ is the depth of $T$ and $k$ is the number of clusters: every node $u$ at level $\ell$ in $T$ (the root node has level $0$) sends $d'(T_u, C_{j'})$ to its parent, for any $j'$, exactly once at time $\delta_T-\ell+j'$.

After collecting the distance information, $\rep(C_j)$ can broadcast this information to all nodes in $C_j$ in $O(\delta_T+k)$ time. The total time is thus $O(\delta_T+k)=O(n)$.% This leads to the following running time claim.
\end{proof}
%
In the next step, {\bf Line~\ref{line:broadcast big cluster}}, we make sure that every node knows the value of $d'(C_j, C_{j'})$ between any big cluster $C_j$ (i.e. $|C_j|>\sqrt{n}$) and any other cluster $C_{j'}$. This is easily done by having the representative node of each big cluster $C_j$, i.e. $\rep(C_j)$, broadcasting $d'(C_j, C_{j'})$, for every $j'$, which is computed in the previous step. Since there are less than $\sqrt{n}$ big clusters and the representative node of each cluster broadcasts $k\leq n$ message (where $k$ is the number of clusters), this step can be easily done in $(n\sqrt{n})$ time (e.g., by collecting all information at one node before broadcasting).
%
\begin{claim}\label{claim: running time of line:broadcast big cluster}
Line~\ref{line:broadcast big cluster} of Algorithm~\ref{algo:apsp} finishes in $O(n\sqrt{n})$ time.
\end{claim}
%
In the last two steps, each node $u$ uses the values of $d'$ it gets from Lines~\ref{line:collect distance within cluster} and \ref{line:broadcast big cluster} to determine $\dist_{G, w_i}(u, v)$, for all nodes $v$, without communicating with other nodes. First, in {\bf Line~\ref{line:G prime}}, it constructs a weighted graph $(G'_u, w')$ which consists of nodes $c_1, \ldots, c_k$ where each node $c_j$ represents cluster $C_j$. Edges in $G'_u$ are between the pairs of clusters that $u$ knows their candidate distances $d'$. In particular, we have two types of edges: Edges of the first type (i.e. $E_1'$ in Line~\ref{line:G prime}) are in the form $c_jc_{j'}$ for any $j'$, where $C_j$ is the cluster containing $u$. Weights of these edges are candidate distances $d'(C_j, C_{j'})$ computed in Line~\ref{line:collect distance within cluster}. Edges of the second type (i.e. $E_2'$ in Line~\ref{line:G prime}) are in the form $d'(C_{j'}, C_{j''})$ for any $j'$ and $j''$ such that $|C_{j'}|>\sqrt{n}$. Weights of these edges are candidate distances $d'(C_{j'}, C_{j''})$, which are broadcasted to every node in Line~\ref{line:broadcast big cluster}. This completes the description of $G'_u$.
%
Since $u$ has all information needed to construct $G'_u$ before we start Line~\ref{line:G prime}, we have the following claim.
\begin{claim}\label{claim:running time of line:G prime}
Line~\ref{line:G prime} needs no communication.
\end{claim}
%
Finally, in {\bf Line~\ref{line:final computation}}, node $u$ uses $G'_u$ to compute distance $\dist_{G, w_i}(u, v)$  to all nodes $v$. This is done simply by using Proposition~\ref{prop:G prime}. This completes one iteration of Algorithm~\ref{algo:apsp} where we compute $\dist_{G, w_i}$.

We conclude this section with the running time of our main algorithm. Since every step takes $O(n\sqrt{n}\log n)$ time and we have $\beta=O(\log n)$ iterations, we have that Algorithm~\ref{algo:apsp} finishes in $O(n\sqrt{n}\log^2 n)$ with high probability. Theorem~\ref{theorem:exact} follows.
%
%, the following lemma easily follows.
%%
%\begin{lemma}[Time Complexity]\label{lem:time}
%Algorithm~\ref{algo:apsp} finishes in $O(n\sqrt{n}\log^2 n)$ with high probability.
%\end{lemma}
%%





==> multi_weight_k_apsp.tex <==
\section{Multi-Weight {\large $\mathbf{K}$}-APSP (Proposition \ref{prop:pseudopoly multi-weight})}\label{sec:multi-weight k-apsp}

In this section, we prove Proposition~\ref{prop:pseudopoly multi-weight}: multi-weight $K$-\apsp on $(G, \cW)$ can be solved by an algorithm that takes $\zero(G, \cW)$ as an input and, with high probability, finishes in $O(K\zero(G, \cW)\log n+n)$ time.

The main idea of our algorithm is based on growing several BFS trees in parallel and using the random delay technique \cite{LeightonMR94} to avoid conflicts. The algorithm is outlined in Algorithm~\ref{algo:multi weight k apsp}. We will show that Algorithm~\ref{algo:multi weight k apsp} causes a congestion of at most $\log n$ with high probability; i.e., at any point in time, there will be at most $\log n$ messages sent through any edge. Moreover, we will show that Algorithm~\ref{algo:multi weight k apsp} finishes in $O(K\zero(G, \cW)+n)$ time if there is no congestion. By allowing an extra $\log n$ time between each step of Algorithm~\ref{algo:multi weight k apsp}, there will be no congestion with high probability. Additionally, if the algorithm fails to send any message due to congestion (which we can detect), we can run the trivial algorithm where we collect all information to one node. This makes the algorithm never fail and have a running time of $O((K\zero(G, \cW)+n)\log n)$ with high probability.
%
We also note that the random delay technique can also be used to remove the assumption that $\zero(G, \cW)$ is known to every node, with an extra $O(n)$ running time. However, this is not necessary for us so we do not include it here to avoid making the algorithm more complicated.




\begin{algorithm}[t]
\caption{{\sc Multi-Weight $K$-Apsp}({\small $G$, $\cW$, $K$, $\zero(G, \cW)$})}
\label{algo:multi weight k apsp}
{\bf Input:} Every node $u$ knows (1) $\vec w^s(uv)$ for all neighbors $v$ and nodes $s$, (2) $K$, and (3) $\zero(G, \cW)$.

{\bf Output:} Every node $u$ knows $\dist_{G, \vec w^s}^K(s, u)$ for all nodes $s$.

\begin{algorithmic}[1]
%\State Make every node knows $\zero(G, \cW)$. {\small\it // Can be done in $O(n)$ time. See description in text}\label{line:BFS compute zero}

\State Every node $s$ selects an integer $r_s$ uniformly at random from $[0, n-1]$ and broadcast $r_s$ to all other nodes.
{\small\it // Takes $O(n)$ time since $n$ messages are broadcasted.}\label{line:generate random delay start}


\State Let $\tau_s=t_0+r_s$ where $t_0$ is the time that the previous step finishes.\label{line:t_0}


\State Every node $s$ sends a message $(s, 0)$ to itself at time $\tau_s$ to initiate the BFS-style subroutine below.\label{line:start BFS}

\algstore{multiapsp}
\end{algorithmic}

\smallskip\textit{\textbf{BFS-Style Subroutine:}} When a node $u$ receives a message $(s, \ell)$ for some $s$ and $\ell$, it does the following.

\smallskip
\begin{algorithmic}[1]

\algrestore{multiapsp}

\If{$u$ has {\em not} already received $(s, \ell')$ for some $\ell'$}\label{line:BFS style start}

\State $u$ now knows that $\dist_{G, \vec w^s}(s, u)=\ell$. {\small \it // See Lemma~\ref{lem:correctness of light apsp} for correctness.)}\label{line:BFS style compute distance}


%\If{($\ell=0$) or ($u\in C_j\ s.t.\ |C_j|\leq \zero(G, \cW)$)}\label{line:check light}


\State $u$ sends $(s, \ell)$ through any edge $uv$ such that $\vec w^s(uv)=0$.\label{line:forward message}

\State For any neighboring nodes $v$ such that $\vec w^s(uv)>0$ and $\ell+\vec w^s(uv)\leq K$, node $u$ sends to $v$  a message $(s, \ell+\vec w^s(uv))$ at time $\tau_s+(\ell+\vec w^s(uv))\zero(G, \cW)$.\label{line:bfs style send message}

%\State If $u$ cannot send any message at the desired time (due to congestion), then the algorithm {\em fails} and solves the problem using a trivial algorithm (aggregate all information to one node) instead. \label{line:fail}

%\EndIf

\EndIf\label{line:BFS style end} %\linebreak
%
\end{algorithmic}
\end{algorithm}

%In {\bf Line~\ref{line:BFS compute zero}}, the algorithm makes sure that all nodes know $\zero(G, \cW)$. This can be easily done as follows. Initially, every node $u$, for every node $s$, sends message $(s, u)$ to all neighbors $v$ such that $\vec w^s(vu)=0$. When node $u$ receives a new message $(s, u')$, it forward this message to




Algorithm~\ref{algo:multi weight k apsp} starts, in {\bf Line~\ref{line:generate random delay start}}, by generating a random delay for each node $s$, denoted by $r_s$. Then it makes sure that every node knows $r_s$ by broadcasting these numbers. Since there are $n$ numbers broadcasted in this step, this step takes $O(n)$ time (e.g. by collecting all numbers at one node before broadcasting them out).

The algorithm waits until Line~\ref{line:generate random delay start} finishes. Then, in {\bf Line~\ref{line:t_0}-\ref{line:start BFS}}, every node $s$ starts growing a BFS tree rooted at $s$ by sending to itself a message $(s, 0)$.  This step will tricker the {\em BFS-style subroutine} to start. Instead of doing this immediately, however, node $s$ waits until time $\tau_s=t_0+r_s$,  where $t_0$ is the time the algorithm step finishes. This is the key step that will give us the claimed running time.


\paragraph{BFS-Style Subroutine} We now explain the BFS-style subroutine (Line~\ref{line:BFS style start} -- \ref{line:BFS style end} of Algorithm~\ref{algo:multi weight k apsp}). For an intuition, note that this subroutine can be viewed as a generalization the BFS tree algorithm in the sense that if we let $\vec w^s(uv)=1$ for all nodes $s$ and edge $uv$ (in this case, $\zero(G, \cW)=1$, then this algorithm will behave exactly like the BFS tree algorithm. However, for the more general case, we will insert a {\em waiting time} of $\zero(G, \cW)$ between each step.


In particular, when a node $u$ receives a message $(s, \ell)$, it does the followings.
%
First, in {\bf Line~\ref{line:BFS style start}}, it checks whether this is the first time it receives any message of the form $(s, \ell')$.
%
If this is the first time, then it knows that $\dist_{G, \vec w^s}(s, u)=\ell$, as in {\bf Line~\ref{line:BFS style compute distance}} (we show that this is correct in Lemma~\ref{lem:correctness of light apsp} below).


%Next, in {\bf Line~\ref{line:check light}}, node $u$ will proceed only if one of the following conditions hold: (1) $\ell=0$ or (2) $u$ is $w_i$-light, i.e. $|S_{w_i}(u)|\leq \sqrt{n}$. The purpose of the first condition is to allow $u$ to proceed, regardless of whether it is $w_i$-light or $w_i$-heavy when it receives a message to itself, which is sent to activate Algorithm~\ref{algo:sim bfs} (as in Line~\ref{line:delay start} of Algorithm~\ref{algo:light apsp}).
%
%The second condition is used because we want to find distances only between $w_i$-light pairs of nodes. We will show that it suffices to let a node to proceed only when it is light.


Next, in {\bf Line~\ref{line:forward message}}, node $u$ forwards the same message $(s, \ell)$ it receives to all neighbors along edges of weight zero in $\vec w^s$. This is to make sure that all nodes $v$ such that $\dist_{G, \vec w^s}(u,v)=0$ knows the current distance $\dist_{G, \vec w^s}(s, u)$. If such $v$ has not received any $(s, \ell')$ earlier, then it also sets $\dist_{G, \vec w^s}(s, v)=\ell$, by Line~\ref{line:BFS style compute distance} (Lemma~\ref{lem:correctness of light apsp} guarantees the correctness).

Finally, in {\bf Line~\ref{line:bfs style send message}}, node $u$ waits until time $\tau_s+(\ell+\vec w^s(uv))\zero(G, \cW)$ before sending the message $(s, \ell+\vec w^s(uv))$ to node $v$. The reason $u$ has to wait until this time is that it wants to make sure that no message of the form $(s, \ell')$, for any $\ell'<\ell+\vec w^s(uv)$, will be sent to $v$ {\em after} it sends $(s, \ell+\vec w^s(uv))$ to $v$. This is to guarantee that $v$ will correctly set $\dist_{G, \vec w^s}(s, v)$ to $(s, \ell+\vec w^s(uv))$ if it has not received any message $(s, \ell')$, for any $\ell'<\ell+\vec w^s(uv))$, {\em earlier}. In addition to waiting, $u$ also sends the message to $v$ only when $\ell+\vec w^s(uv)\leq K$. This is because we are only interested the distance up to $K$.


%This is similar to Line~\ref{line:bfs send message} of Algorithm~\ref{algo:bfs} where $u$ waits until time  $\tau_\vartheta+\ell+w_i^\vartheta(uv)$ before sending the message, except that there is an extra $\sqrt{n}$ term. This term is used to ensure that all nodes in $S_{ w_i}(u)$ already receive the message $(\vartheta, \tau_\vartheta, \ell)$ (by the process in Line~\ref{line:forward message}). In fact, this term will ensure that all nodes {\em in all light supernodes of distance $\ell$ from $\vartheta$} will receive such message (we will prove this shortly, in Lemma~\ref{lem:correctness of light apsp}). Thus, the message $(\vartheta, \tau_\vartheta, \ell+i)$, for any $i$, will be synchronously sent out at the same time $\tau_\vartheta+(\ell+i)\sqrt{n}$.
%
%Additionally, node $u$ will send a message to node $v$ {\em only if} $\ell+w_i^\vartheta(\vartheta, v)\leq 2n$. This is to make sure that Algorithm~\ref{algo:sim bfs} stops sending a message at time $\tau_\vartheta+n\sqrt{n}$. Sending a message after this time is unnecessary and could interrupt the communication of other algorithms (recall that we run Algorithm~\ref{algo:sim bfs} from many nodes $\vartheta$ simultaneously).

%As stated in Line~\ref{line:fail}, we say that Algorithm~\ref{algo:sim bfs} {\em fails} if some node $u$ cannot send a message at the desired time. This can happens in two cases: (1) In Line~\ref{line:forward message}, $u$ cannot send a message immediately. (2) In Line~\ref{line:bfs style send message}, $u$ cannot send a message $(\vartheta, \tau_\vartheta, \ell+w_i^\vartheta(uv))$ at time $\tau_\vartheta+(\ell+w_i^\vartheta(uv))\sqrt{n}$. The only possibility that any of these cases happens is when many copies of Algorithm~\ref{algo:sim bfs} (started at different nodes) want to send a message through the same node at the same time. We will shortly show that this is unlikely (due to the random delay). Before we doing so, let us first analyze Algorithm~\ref{algo:sim bfs} by assuming that it does not fail.

%The following lemma (proof in Appendix) guarantees the correctness of Algorithm~\ref{algo:multi weight k apsp}, assuming that there is no congestion.

%\paragraph{Analysis when there is no congestion}

\medskip Assuming that there is no congestion (i.e., all messages are sent successfully), the correctness of Algorithm~\ref{algo:multi weight k apsp} can be guaranteed as in the following lemma.
%
\begin{lemma}[Proof in Appendix~\ref{sec:omitted proofs}]\label{lem:correctness of light apsp}\label{LEM:CORRECTNESS OF LIGHT APSP}
Assume that there is no congestion. For any nodes $s$ and $v$, the followings hold.
\begin{enumerate}[noitemsep]
\item $u$ does not receive message $(s, \ell)$ for any $\dist_{G, \vec w^s}(s, u)$.
\item $u$ receives message $(s, \dist_{G, \vec w^s}(s, u))$ before round $\tau_s+(\dist_{G, \vec w^s}(s, u)+1)\zero(G, \cW)$
\end{enumerate}
\end{lemma}
%
%\begin{observation}\label{observe:runtime of algo:multi weight k apsp}
%Assume that there is no congestion. Algorithm~\ref{algo:multi weight k apsp} finishes sending messages at time $t_0+n+K\zero(G, \cW)$.
%\end{observation}
%\begin{proof}
%By the condition on Line~\ref{line:bfs style send message}, all nodes stop sending a message at time $\max_{s\in V(G)} \tau_s+K\zero(G, \cW)$. By Line~\ref{line:generate random delay start} and \ref{line:t_0}, $\tau_s\leq t_0+r_s\leq t_0+n$ for any $s$.
%\end{proof}
%

%\begin{corollary}\label{lem:runtime of light apsp}
%Algorithm~\ref{algo:light apsp} finishes Line~\ref{line:BFS style start} in $\tilde O(n\sqrt{n})$ time.
%\end{corollary}

\paragraph{Congestion Analysis}  We show that it is unlikely that Algorithm~\ref{algo:multi weight k apsp} sends many messages on one edge at the same time. In particular, we show that, with high probability, there will be at most $\log n$ messages of the form $(s, \ell)$ sent through each edge in each round.  Our analysis follows an idea in \cite{LeightonMR94}, using the special property of Algorithm~\ref{algo:multi weight k apsp} that each node $u$ sends message $(s, \ell)$ at most {\em once}.
%
\begin{lemma}[Congestion]\label{lem:no congestion}
The probability that there exists an edge $uv$ and a set $\mset=\{(s_j, \ell_j)\}_{1\leq j\leq k}$ of $k>\log n$ messages such that all messages in $\mset$ are sent on $uv$ at the same time is $O(1/n^2)$.
\end{lemma}
\begin{proof}[Sketch](Full Proof in Appendix~\ref{sec:omitted proofs}) First, observe that, in Algorithm~\ref{algo:multi weight k apsp}, for any neighboring nodes $u$ and $v$, $u$ sends message of the form $(s, \ell)$ to $v$ {\em at most once} for each $s$. In fact, this message is exactly $(s, \dist_{w^s}(s, u)+w^s(uv))$. %
Observe further that the time that $u$ sends to $v$ message $(s, \dist_{w^s}(s, u)+w^s(uv))$ is determined by $\tau_s$. Using these facts, it can be shown that the probability that there exists nodes $u$ and $v$, time $t$, and set $\mset=\{(s_j, \ell_j)\}_{1\leq j\leq k}$  of $k>\log n$ messages, such that $u$ wants to send all messages in $\mset$ at time $t$, is at most
{
\begin{align}
\sum_{k=1+\log n}^{n} 3Kn^3 \binom{n}{k}\left(\frac{1}{n}\right)^k\,.\label{eq:prob congestion happens short}
\end{align}
}
%
%We end the proof by upper bounding Eq.\eqref{eq:prob congestion happens}.
%
Note that for any $0<b<a$, $\binom{a}{b}\leq (ae/b)^b$. Thus, Eq.\eqref{eq:prob congestion happens short} is at most
%
\begin{align}
\sum_{k=1+\log n}^{n} 3Kn^3\left(\frac{ne}{k}\right)^k\left(\frac{1}{n}\right)^k \leq 3Kn^4 \left(\frac{e}{\log n}\right)^{\log n}\label{eq:congestion probability short}
\end{align}
%
Note that we can assume that $K=\poly(n)$ since the largest edge weight is $\poly(n)$. For large enough $n$, (i.e., $(\log n)^{\log n}\geq 4Kn^6$), Eq.\eqref{eq:congestion probability short} will be bounded by $O(1/n^2)$ as desired.
\end{proof}
%
Thus, by allowing $\log n$ extra rounds between each step of the BFS-Style subroutine in Algorithm~\ref{algo:multi weight k apsp}, we can ensure that Algorithm~\ref{algo:multi weight k apsp} can send all messages it wants, with high probability. In this case, the BFS-Style subroutine finishes in $O(K\zero(G, \cW)\log n)$ rounds. Moreover, the algorithm can detect when it cannot send a message and can switch to the trivial $O(m)$-time algorithm where it aggregates all information to one node. We conclude with the following running time.

\begin{lemma}[Running Time]\label{observe:runtime of algo:multi weight k apsp}
Assuming that there is no congestion. Algorithm~\ref{algo:multi weight k apsp} with $\log n$ extra time between each step of the BFS-Style subroutine finishes sending messages at time $t_0+n+K\zero(G, \cW)\log n$ with high probability.
\end{lemma}
\begin{proof}
By the condition on Line~\ref{line:bfs style send message}, all nodes stop sending a message at time $\max_{s\in V(G)} \tau_s+K\zero(G, \cW)\log n$ (the extra $\log n$ factor is because we allow $\log n$ extra time). By Line~\ref{line:generate random delay start} and \ref{line:t_0}, $\tau_s\leq t_0+r_s\leq t_0+n$ for any $s$. The lemma follows.
\end{proof}



\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Previous version of the above lemma
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:no congestion}
The probability that there exists an edge $\overrightarrow{uv}$ and a set $\mset=\{(\vartheta_j, \tau_{\vartheta_j}, \ell_j)\}_{1\leq j\leq k}$ of $k>\log n$ messages such that all messages in $\mset$ are sent on $\overrightarrow{uv}$ at the same time is at most $1/n^2$.
\end{lemma}
\begin{proof}
First, observe that, in Algorithm~\ref{algo:sim bfs}, for any neighboring nodes $u$ and $v$, $u$ sends message of the form $(\vartheta, \tau_\vartheta, \ell)$ to $v$ {\em at most once}. In fact, this message is exactly $(\vartheta, \tau_\vartheta, \dist_{w_i^\vartheta}(\vartheta, u)+w_{i}^\vartheta(\overrightarrow{uv})$.
%
To see this, not that due to the condition in Line \ref{line:BFS style start}, node $u$ sends messages to its neighbors only when it receives $(\vartheta, \tau_\vartheta, \ell))$ for the first time, and it sends only one message to each neighbor (due to Line~\ref{line:forward message} and \ref{line:bfs style send message}).

Observe further that the time that $u$ sends to $v$ message $(\vartheta, \tau_\vartheta, \dist_{w_i^\vartheta}(\vartheta, u)+w_{i}^\vartheta(\overrightarrow{uv}))$ is determined by $\tau_\vartheta$. This is simply because Algorithm~\ref{algo:sim bfs} is deterministic.


Now we claim that the probability that there exists nodes $u$ and $v$, time $t$, and set $\mset=\{(\vartheta_j, \tau_{\vartheta_j}, \ell_j)\}_{1\leq j\leq k}$  of $k>\log n$ messages, such that $u$ wants to send all messages in $\mset$ at time $t$, is at most
{\small
\begin{align}
\sum_{k=1+\log n}^{n} (3n^3\log n) \binom{n}{k}\left(\frac{1}{n\log n^2}\right)^k\left(1-\frac{1}{n\log n^2}\right)^{n-k}\,.\label{eq:prob congestion happens}
\end{align}
}
To see this, consider any neighboring nodes $u$ and $v$, and let $t$ be any time during the computation. We will analyze the probability that $u$ wants to send more than $\log n$ messages to $v$ at the same time. To simplify the analysis, let us also assume that for all node $\vartheta$, there is a message $(\vartheta, \tau_\vartheta, \ell)$, for some $\tau_\vartheta$ and $\ell$, sent from $u$ to $v$ in some round. The probability that we analyze will be lower in the general case where there exists some node $\vartheta$ such that message $(\vartheta, \tau_\vartheta, \ell)$, for any $\tau_\vartheta$ and $\ell$, is never sent from $u$ to $v$.

Let $\mset$ be a set of $k$ messages. Recall that $\tau_{\vartheta}$, for any node $\vartheta$, has $n\log n^2$ possible values, due to the random number $r(S_{w_i}(\vartheta))$ added to the starting time of Algorithm~\ref{algo:sim bfs} in Line~\ref{line:delay start} of Algorithm~\ref{algo:light apsp}. Thus, for any node $\vartheta$, the probability that $u$ sends message $(\vartheta, \tau_\vartheta, \ell)$ to $v$ at time $t$ is at most $\frac{1}{n\log n^2}$. It follows that the probability that $u$ sends all messages in $\mset$ to $v$ at time $t$ is at most $(\frac{1}{n\log n^2})^k$. Moreover, the probability that $u$ sends no messages, among all $n$ possible messages for $n$ different values of $\vartheta$, that is not in $v$ is at most $(1-\frac{1}{n\log n^2})^{n-k}$. Thus, the probability that the messages sent from $u$ to $v$ at round $t$ is exactly those in $\mset$ is at most
\begin{align}
(\frac{1}{n\log n^2})^k(1-\frac{1}{n\log n^2})^{n-k}.\label{eq:prob exactly mset is sent}
\end{align}
Recall that there are $\binom{n}{k}$ possible sets $\mset$ since $u$ sends a message of the form $(\vartheta, \tau_\vartheta, \ell)$ at most once, for each node $\vartheta$. Also note that we can assume that $t_0\leq t\leq t_0+n\log n^2+2n\leq t_0+3n\log n$, where $t_0$ is the starting time of Algorithm~\ref{algo:light apsp}, as in Line~\ref{line:t_0} of Algorithm~\ref{algo:light apsp}. This is because Algorithm~\ref{algo:sim bfs} starts before round $t_0+n\log n^2$ and stops sending messages after $2n$ rounds. By summing Eq.\eqref{eq:prob exactly mset is sent} over all possible $n^2$ pairs of nodes, $3n\log n$ values of $t$, all possible values of $k$, and $\binom{n}{k}$ possible sets $\mset$, we obtain Eq.\eqref{eq:prob congestion happens}.

We end the proof by upper bounding Eq.\eqref{eq:prob congestion happens}. For note that for any $0<b<a$, $\binom{a}{b}\leq (ae/b)^b$. Thus, Eq.\eqref{eq:prob congestion happens} is at most
{\small
\begin{align*}
&\sum_{k=1+\log n}^{n} (3n^3\log n) \left(\frac{ne}{k}\right)^k\left(\frac{1}{n\log n^2}\right)^k\left(1-\frac{1}{n\log n^2}\right)^{n-k}\\ %\,.\label{eq:prob congestion happens 2}
&\leq \sum_{k=1+\log n}^{n} (3n^3\log n) \left(\frac{e}{k\log n^2}\right)^k\left(1-\frac{1}{n\log n^2}\right)^{n-k}\\
\end{align*}
}
For large enough $n$ (so that $(\log n)^{\log n}\geq 3n^4\log n$, the quantity above is bounded by $1/n$ as desired.
\end{proof}
\end{comment}

%\paragraph{Sharing information within supernodes (Line~\ref{line:end of light} of Algorithm~\ref{algo:light apsp})}


\begin{comment}
\paragraph{Summary of the Analysis} Let us summarize the analysis we show in this subsection. By Lemma~\ref{lem:no congestion} guarantee that all executions of Algorithm~\ref{algo:sim bfs} (starting at different nodes $\vartheta$) does not fail with high probability. Given that Algorithm~\ref{algo:sim bfs} does not fail, it will finish by time $\max_{\vartheta\in V(G)} \tau_\vartheta+(2n+1)\sqrt{n}$ by Lemma~\ref{lem:runtime of sim bfs}. This is less than $t_0+2n+(2n+1)\sqrt{n}$ since $\tau_\vartheta=t_0+n+r(S_{w_i}(\vartheta))<t_0+2n$. The following corollary follows.
%This means that
\begin{corollary}\label{cor:line delay start finish time}
Line~\ref{line:delay start} of Algorithm~\ref{algo:apsp} finishes before round $t_0+2n+(2n+1)\sqrt{n}$.
\end{corollary}
%
At the time Line~\ref{line:delay start} of Algorithm~\ref{algo:apsp} finishes, the distances between many $w_i$-light pairs are already discovered. In particular, Lemma~\ref{lem:correctness of light apsp} implies that for every $w_i$-light pair $(\vartheta, u)$, some node in $S_{w_i}(u)$ knows the value of $\dist_{w_i^\vartheta}(\vartheta, u)$, and if $u$ is $w_i$-light then $u$ knows the value of $\dist_{w_i^\vartheta}(\vartheta, u)$.
%
Note that we have not yet find  $\dist_{w_i^\vartheta}(\vartheta, u)$ between all pair of $w_i$-light pairs $(\vartheta, u)$. We will do so next.


\subsection{Finishing finding distances between light pairs (Line~\ref{line:end of light} of Algorithm~\ref{algo:light apsp})}\label{sec:light-final}
In Line~\ref{line:end of light} of Algorithm~\ref{algo:light apsp}, we make sure that for every $w_i$-light pair $(\vartheta, u)$, node $u$ knows the value of  $\dist_{w_i^\vartheta}(\vartheta, u)$. This is done by simply aggregating the messages $(\vartheta, \tau_\vartheta, \ell)$ from each node $u$ to the representative node of supernode $S_{w_i}(u)$. This can be done in $\tilde O(n)$ rounds since there are at most $n$ messages in each supernode (some of these messages may be stored by many nodes in the supernode): For each node $u$, the set of messages that nodes in $S_{w_i}(u)$ have is exactly  $\{(\vartheta, \tau_\vartheta, \dist_{w_i^\vartheta}(\vartheta, u) \mid \mbox{$(\vartheta, u)$ is $w_i$-light}\}$. TO ADD MORE DETAIL.

We conclude this section with the following theorem, which easily follows our analysis.

\begin{theorem}
Algorithm~\ref{algo:light apsp} find the distances between all $w_i$-light pairs with probability at least $\tilde \Omega(1-1/n)$. Moreover, it always finish in $\tilde O(n\sqrt{n})$ time.
\end{theorem}
\end{comment}


==> omitted_proofs.tex <==
\section{Omitted Proofs}\label{sec:omitted proofs}

\subsection{Proof of Claim~\ref{claim:w_i time}}
{
\renewcommand{\thetheorem}{\ref{claim:w_i time}}
\begin{claim}[Restated]
Line~\ref{line:w_i} of Algorithm~\ref{algo:apsp} can be done in $O(n)$ time.
\end{claim}
\addtocounter{theorem}{-1}
}
\begin{proof}%[of Claim~\ref{claim:w_i time}]
Observe that each node $u$ can compute $\vec w_i^x({uv})$ and $\vec w_i^x({vu})$ if it knows the values of $\dist_{G, w_{i+1}}(x, v)$ for all nodes $x$ and neighbors $v$. Assuming that the algorithm successfully solves \apsp on $(G, w_{i+1})$ in Iteration $i+1$, the algorithm do the task in Line~\ref{line:w_i} easily in $\tilde O(n)$ time: Every node $v$ simultaneously send to all neighbors the values of $\dist_{G, w_{i+1}}(x, v)$, for all nodes $x$. Since there are $n$ messages of size $\tilde O(1)$ to be sent, this can be done in $O(n)$ time. Then, every node $u$ will have all necessary information to compute $\vec w_i^x({uv})$ and $\vec w_i^x({vu})$.
\end{proof}

\begin{comment}
\paragraph{Time:} We claim that a message of ID $i$ first reaches a node $j$ by time between in $[\dist(i,j), \dist(i,j)+i]$. This is clearly true for $i=1$ since no other message will block a message of ID $1$; thus, this message acts like a BFS algorithm. Now, assume that this is true for any $1\geq k<i$, we will show that this is true for $i$ as well. Suppose for the sake of contradiction there exists a node $j$ such that the message of ID $i$ first reaches $j$ at time $t>\dist(i, j)+i$.

Let $a$ be the ID of the last message that blocks message of ID $i$ before $i$ reaches node $j$. By the scheduling rule, $a<i$. Let $b$ and $t'$ be the node and time that this happens. Note that $t'\leq \dist(a, b)+a$. Also note that $t-t'-1=\dist(b, j)$ since message $i$ is not blocked after it leaves $b$ at time $t'+1$ and it will reach $j$ by a shortest $b$-$j$ path). Consider two cases.

{\em Case 1: $\dist(a, b)\leq \dist(i, b)$. In this case,
$$t=\dist(b, j)+t'+1\leq \dist(b, j)+\dist(a, b)+a+1\leq \dist(b, j)+\dist(i, b)+a+1\leq \dist(i, j)+a+1???$$

\begin{claim}
A message of ID $i$ first reaches a node $j$ by time between in $[\dist(i,j), \dist(i,j)+i]$.
\end{claim}
\end{comment}


\section{Proof of Lemma~\ref{lem:correctness of light apsp}}

{\renewcommand{\thetheorem}{\ref{lem:correctness of light apsp}}
\begin{lemma}[Restated]
Assume that is no congestion. For any nodes $s$ and $v$, the followings hold.
\begin{enumerate}[noitemsep]
\item $u$ does not receive message $(s, \ell)$ for any $\dist_{G, \vec w^s}(s, u)$.
\item $u$ receives message $(s, \dist_{G, \vec w^s}(s, u))$ before round $\tau_s+(\dist_{G, \vec w^s}(s, u)+1)\zero(G, \cW)$
\end{enumerate}
\end{lemma}
\addtocounter{theorem}{-1}
}

\begin{proof}
We prove this by induction. First, we show that all claims hold when $\ell=0$. To see this, observe that the message $(s, 0)$ will be sent through any path $P=\langle s=x_0, x_1, \ldots, x_k=u\rangle$ such that $\vec w^s(P)=0$, by Line~\ref{line:forward message} of Algorithm~\ref{algo:multi weight k apsp}. Thus, every node $u$ such that $\dist_{G, \vec w^s}(s, u)=0$ will receive this message. Moreover, such message will take $|P|\leq \zero(G, \cW)$ rounds to reach $u$. 

Now we consider any $L>0$. We show that if the lemma holds for any $\ell<L$, then it holds for $\ell=L$ as well. Throughout the proof, we let $u$ be any node such that $\dist_{G, \vec w^s}(s, u)=L$.

Now we prove the first claim. Assume that the first claim does not hold, i.e. some node $u$ such that $\dist_{G, \vec w^s}(s, u)=L$ receives a message $(s, \ell')$, for some $\ell'<\ell$. We call this event a {\em bad} event. Let $t$ be the earliest time that a bad event occurs, and let $u^*$ be the node that receives such message $(s, \ell')$ at time $t$. Let $v$ be the node that sends message $(s, \ell')$ to $u$ at time $t$. This means that $v$ has received message $(s, \ell'-\vec w^s(vu))$ at time $t'<t$. Note that $\dist_{G, \vec w^s}(s, v)\geq \dist_{G, \vec w^s}(s, u)-\vec w^s(vu)>\ell'-\vec w^s(vu)$. This means that a bad event also occurs at time $t'$, contradicting the assumption that $t$ is the earliest time that a bad event occurs. This proves the first claim for $\ell=L$.

Now we prove the second claim. Let $P=\langle s=x_0, x_1, \ldots, x_k=u\rangle$, for some $k$, be any shortest $s$-$u$ path in $(G, \vec w^s)$ (i.e., $\vec w^s(P)=L$).
%
Let $j$, where $0\leq j\leq k$, be the largest number such that $\dist_{G, \vec w^s}(x_j, u)>0$. Note that such $j$ exists since $\dist_{G, \vec w^s}(s, u)=L>0$. Moreover, by the definition of $x_j$, $\vec w^s(x_jx_{j+1})>0$, $\dist_{G, \vec w^s}(s, x_{j+1})=L$, and $\dist_{G, \vec w^s}(s, x_j)=L-\vec w^s(x_jx_{j+1})<L$. Let $\ell'=\dist_{G, \vec w^s}(s, x_j)$. 

%; otherwise, $\dist_{G, \vec w_i^\vartheta}(\vartheta, u)=0$ by Lemma~\ref{lem:scaling preserves zero}, contradicting the assumption that $\dist_{G, \vec w_i^\vartheta}(\vartheta, u)=L>0$ .
%
%Let $\ell'=\dist_{G, \vec w_i^\vartheta}(\vartheta, x_j)$. 

%Since $\dist_{G, \vec w_i^\vartheta}(\vartheta, x_{j+1})=L$ (since $x_{j+1}\in S_{w_i}(u)$) and $\vec w_i^\vartheta(x_jx_{j+1})>0$ (by Lemma~\ref{lem:scaling preserves zero}), $\ell'<L$. 

%Moreover, $x_j$ is $w_i$-light since $P$ is a $w_i$-light path. 


By the induction hypothesis, the first message that $x_j$ receives is $(s, \ell')$, and $x_j$ receives this message before round $\tau_s+(\ell'+1)\sqrt{n}$. Thus, it will send message $(s, L)$ to $x_{j+1}$ at time $\tau_s+L\zero(G, \cW)$ (by Line~\ref{line:bfs style send message} of Algorithm~\ref{algo:multi weight k apsp}). Assuming that the algorithm does not fail to send messages, $x_{j+1}$ will receive message $(s,  L)$ at time $\tau_s+L\zero(G, \cW)$. Then, the message $(s, L)$ will be sent from $x_{j+1}$ to $u$ in $\zero(G, \cW)$ rounds through a path $P'=\langle x_{j+1}, \ldots, x_k=u\rangle$ (since $\vec w^s(P')=0$). This proves the second claim.  
\end{proof}


%Thus, by the induction hypothesis, the first message that $x_j$ receives is $(\vartheta, \tau_\vartheta, \ell')$, and $x_j$ receives this message before round $\tau_\vartheta+(\ell'+1)\sqrt{n}$. Thus, it will send message $(\vartheta, \tau_\vartheta, L)$ to $x_{j+1}$ at time $\tau_\vartheta+L\sqrt{n}$ (by Line~\ref{line:bfs style send message} of Algorithm~\ref{algo:sim bfs}). Assuming that the algorithm does not fail, $x_{j+1}$ will receive message $(\vartheta, \tau_\vartheta, L)$ at time $\tau_\vartheta+L\sqrt{n}$. This proves the second claim since $x_{j+1}\in S_{\vec w_i^\vartheta}(u)$.

%Now we prove the third claim. By the second claim, some node $v$ in $S_{w_i}(u)$ receives  $(\vartheta, \tau_\vartheta, L)$ at time $L$. By the first claim, $v$ has not received any message of the form $(\vartheta, \tau_\vartheta, \ell')$ for any $\ell'<L$; so, by Line~\ref{line:forward message} of Algorithm~\ref{algo:sim bfs}, $v$ sends message $(\vartheta, \tau_\vartheta, L)$ to all neighbors in $S_{w_i}(v)=S_{w_i}(u)$. These neighbors again send the same message to their neighbors in $S_{w_i}(u)$ since they have not received any  message of the form $(\vartheta, \tau_\vartheta, \ell')$ for any $\ell'<L$, by the first claim. This process is repeated until message $(\vartheta, \tau_\vartheta, \ell')$ reach $u$. The time it takes for this message to reach $u$ is at most $|S_{w_i}(u)|-1$ rounds, which is at most $\sqrt{n}-1$ since $u$ is $w_i$-light. So, the message will reach $u$ before round $\tau_\vartheta+L\sqrt{n}+\sqrt{n}$ as in the third claim.


%\begin{proof}[of Lemma~\ref{lem:runtime of algo:multi weight k apsp}]
%\danupon{Have to change}
%By Line~\ref{line:bfs style send message} of Algorithm~\ref{algo:multi weight k apsp}, any message of the form $(s, \ell)$ must be such that $\ell\leq K$. This message is sent only at round $\tau_s+K\zero(G, \cW)$ in Line~\ref{line:bfs style send message}. This message is then sent for at most another $\zero(G, \cW)-1$ rounds along edges of weight zero in $w^s$, as in Line~\ref{line:forward message}. The lemma follows.
%\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ----------  The subsection below is already moved --------------
%
%\subsection{Proof of Lemma~\ref{lem:no congestion}}
%
%{\renewcommand{\thetheorem}{\ref{lem:no congestion}}
%\begin{lemma}[Restated]
%The probability that there exists an edge $uv$ and a set $\mset=\{(s_j, \ell_j)\}_{1\leq j\leq k}$ of $k>\log n$ messages such that all messages in $\mset$ are sent on $uv$ at the same time is $O(1/n^2)$.
%\end{lemma}
%\addtocounter{theorem}{-1}
%}
%\begin{proof}
%First, observe that, in Algorithm~\ref{algo:multi weight k apsp}, for any neighboring nodes $u$ and $v$, $u$ sends message of the form $(s, \ell)$ to $v$ {\em at most once} for each $s$. In fact, this message is exactly $(s, \dist_{G, \vec w^s}(s, u)+\vec w^s(uv))$.
%%
%To see this, note that due to the condition in Line \ref{line:BFS style start}, node $u$ sends messages to its neighbors only when it receives $(s, \ell)$ for the first time, and it sends only one message to each neighbor (due to Line~\ref{line:forward message} and \ref{line:bfs style send message}).
%
%Observe further that the time that $u$ sends to $v$ message $(s, \dist_{G, \vec w^s}(s, u)+\vec w^s(uv))$ is determined by $\tau_s$. This is simply because Algorithm~\ref{algo:multi weight k apsp} is deterministic.
%
%
%Now we claim that the probability that there exists nodes $u$ and $v$, time $t$, and set $\mset=\{(s_j, \ell_j)\}_{1\leq j\leq k}$  of $k>\log n$ messages, such that $u$ wants to send all messages in $\mset$ at time $t$, is at most
%{
%\begin{align}
%\sum_{k=1+\log n}^{n} 3Kn^3 \binom{n}{k}\left(\frac{1}{n}\right)^k\,.\label{eq:prob congestion happens}
%\end{align}
%}
%To see this, consider any neighboring nodes $u$ and $v$, and let $t$ be any time during the computation. Let $\mset$ be a set of $k$ messages. Recall that $\tau_{s}$, for any node $s$, has $n$ possible values, due to the random number $r_s\in [0, n-1]$ added to the starting time of the BFS-style subroutine. Thus, for any node $s$, the probability that $u$ sends message $(s, \ell)$, for some $\tau_s$ and $\ell$, to $v$ at time $t$ is at most $\frac{1}{n}$ (since there is only one value of $\tau_s$ that will make will make $u$ send $(s, \ell)$ exactly at time $t$). It follows that the probability that $u$ sends all messages in $\mset$ to $v$ at time $t$ is at most
%\begin{align}
%\left(\frac{1}{n}\right)^k.\label{eq:prob exactly mset is sent}
%\end{align}
%Note that there are $\binom{n}{k}$ possible sets $\mset$ where each set have $s_1\neq s_2\neq \ldots$. This is because $u$ sends a message of the form $(s, \ell)$ at most once to $v$, for each node $s$. Also note that we can assume that $t_0\leq t< t_0+n+(K+1)\zero(G, \cW)$, where $t_0$ as in Line~\ref{line:t_0} of Algorithm~\ref{algo:multi weight k apsp}. This is because the last round that Algorithm~\ref{algo:multi weight k apsp} can start is $t_0+r_s< t_0+n$, and it stops sending messages after time $\tau_s+(K+1)\zero(G, \cW)\leq t_0+n+(K+1)\zero(G, \cW)$ rounds. Thus, there are at most $n+(K+1)\zero(G, \cW)\leq 3Kn$ possible values of $t$.
%
%By summing Eq.\eqref{eq:prob exactly mset is sent} over all possible $n^2$ pairs of nodes, $3Kn$ possible values of $t$, all possible values of $\log n<k\leq n$, and $\binom{n}{k}$ possible sets $\mset$, we obtain Eq.\eqref{eq:prob congestion happens}.
%
%We end the proof by upper bounding Eq.\eqref{eq:prob congestion happens}. Note that for any $0<b<a$, $\binom{a}{b}\leq (ae/b)^b$. Thus, Eq.\eqref{eq:prob congestion happens} is at most
%%
%\begin{align}
%\sum_{k=1+\log n}^{n} 3Kn^3\left(\frac{ne}{k}\right)^k\left(\frac{1}{n}\right)^k \leq 3Kn^4 \left(\frac{e}{\log n}\right)^{\log n}\label{eq:congestion probability}
%\end{align}
%%
%Note that we can assume that $K=\poly(n)$ since the largest edge weight is $\poly(n)$. For large enough $n$, (i.e., $(\log n)^{\log n}\geq 4Kn^6$), Eq.\eqref{eq:congestion probability} will be bounded by $O(1/n^2)$ as desired.
%\end{proof}


==> overview3.tex <==
\section{Proof Overview \& Organization}\label{sec:overview}
All our algorithms share the following same high-level idea: We start with a {\em pseudo-polynomial} time algorithm whose running time depends on edge weights. We then apply this algorithm on the network with {\em modified} edge weights in a suitable way that this algorithm is fast. How we modify edge weights depends on the problems. We illustrate this idea starting from the simple ideas for approximation algorithms to the more complicated ones for the exact algorithm.

\subsection{Approximation Algorithms}

...

Now, to approximate $D(G, w)$, we first compute $D'$ that $2$-approximates $D(G, w)$; this can be done easily by solving \sssp from an arbitrary source. We then use $D'$ to change $w$ slightly to $w'$ where $w'(uv)=\lceil \frac{2n w(uv)}{\epsilon D'}\rceil$. We then show the following.
\begin{proposition}\label{prop:approx diameter guarantee}{\sc (Properties of $D(G, w')$; Proof in Appendix~\ref{sec:approx diameter})}
$D(G, w')\leq (1+2/\epsilon)n$ and $D(G, w)$ $\leq$ $\frac{\epsilon D'}{2n}\times D(G, w')$ $\leq$ $(1+\epsilon)D(G, w).$
\end{proposition}
% and we can use $D(G, w')$ to approximate $D(G, w)$.
Thus, we can apply Proposition~\ref{prop:pseudopoly time} with $K=(1+2/\epsilon)n$ on $D(G, w')$ to compute $D(G, w')$. Then, we output $D'\times D(G, w')$ as an approximate solution of $D(G, w)$. 

The case of approximating $\rad(G, w)$ is done almost identically. We only have to change to way we compute $D'$ slightly. 

\medskip To solve \apsp approximately, we have to ``guess'' the distance between each pair of nodes in the form $2^i$. For each guessed distance $2^i$, we again change weight $w$ slightly to $w'_i$ where $w'_i(uv)=\lceil\frac{ 2nw(uv)}{\epsilon2^i}\rceil$. An important property that we will show is the following.
%
\begin{proposition}\label{prop:approx apsp guarantee}{\sc (Property of $(G, w'_i)$; Proof in Appendix~\ref{sec:approx apsp})}
For any nodes $u$ and $v$, if we let $\tilde d_{G, w}(u, v)$ = $\min_i  \frac{\epsilon D'_{i}}{2n}\times\dist^{(1+2/\epsilon)n}_{G, w'_i}(u, v)$, then $\dist_{G, w}(u, v)\leq \tilde d_{G,w}(u, v)\leq (1+\epsilon)\dist_{G, w}(u, v)$.
\end{proposition}
Thus, we can approximate \apsp on $(G, w)$ by applying Proposition~\ref{prop:pseudopoly time} on $(G, w_i)$ with $K=(1+2/\epsilon)n$, for all $i$.


%in such a way that for all nodes $u$ and $v$, $\dist_{G, w'}(u, v)\geq \dist_{G, w}(u, v)$; moreover, if $\dist_{G, w}(u, v)\leq 2^i$, then $\dist_{G, w'}(u, v)\leq \dist_{G, w}(u, v)$. We then apply Lemma~\ref{lem:pseudopoly time} with $K=2^i$

\subsection{Exact Algorithm}
Like the approximation algorithms, our exact algorithm relies on the idea of modifying edge weights and applying a pseudo-polynomial time algorithm to get an approximate solution. To arrive at the exact solution, we keep refining the modified edge weights until we finally get the correct solution. The refining step leads to many complications (especially, we will have to deal with edges of weight zero). For this reason, we need a more general version of Proposition~\ref{prop:pseudopoly time}, as well as several other ideas.


\paragraph{Weight Scaling} A naturally way to modify edge weights is by {\em weight scaling}. Recall that the general idea of this technique is to approximate \apsp on $(G, w_i)$, where $w_i(uv)=\lfloor w(uv)/2^i\rfloor$ for a large enough $i$ so that $w_i(uv)$ is small enough to run a pseudo-polynomial time algorithm for \apsp\footnote{We note that obstructions on the way make us end up using a slightly different way to do weight scaling, as we will discuss later in this section.}. We then keep reducing $i$ until $i=0$. While we cannot ensure that $w_i(uv)$ is small for a small $i$, we can use the solution on $(G, w_{i+1})$ to solve \apsp on $(G, w_i)$ quickly.

%write each edge weight $w(uv)$ as a binary string\footnote{We note that we will end up using something a bit different called {\em positive binary string}, as will be discussed later in this section.} $b_\beta(uv)$, $b_{\beta-1}(uv)$, $\ldots$, $b_0(uv)$, where $b_i(uv)\in \{0, 1\}$ for all $i$, and $w(uv)=\sum_{i=0}^\beta b_i(uv)2^i$. We then solve the problem in {\em iterations}, starting from Iteration $\beta$ {\em down to} Iteration $0$. In Iteration $i$, we solve \apsp on graph $(G, w_i)$, where $w_i(uv)$ is defined to be $b_\beta(uv)\ldots b_i(uv)$ in base two. The point is that the solution from Iteration $i+1$ will help speeding up our algorithm on Iteration $i$.

%To see why this technique is useful, first observe that $D(G, w_\beta)\leq n$ since $w_\beta(uv)\in \{0, 1\}$ for every edge $uv$. Thus, a pseudo-polynomial time algorithm (like that in Lemma~\ref{lem:pseudopoly time}) will be fast on $(G, w_\beta)$, except that there could be zero weights; this is one extra thing our new pseudo-polynomial time algorithm has to deal with.

More specifically, we use the solution of \apsp on $(G, w_{i+1})$ to change the weight $w_i$ into a {\em collection} of {\em asymmetric nonnegative} weight assignments $\cW_i=\{\vec w^s_i\}_{s\in V(G)}$. We emphasize that $\vec w_i$ is asymmetric and it could assign value zero to some edges. %This is the source of some complications we will face later. 

An important property of $(G, \cW_i)$ is that it has a small ``diameter'' in the following sense. Define the {\em multi-weight diameter} of $(G, \cW_i)$, denoted by $\ecc(G, \cW_i)$, to be $\ecc(G, \cW_i)=\max_{s, u\in V(G)} \dist_{G, \vec{w}^s_i}(s, u)$. We show that the multi-weight diameter of $(G, \cW_i)$ is small (for an intuition, compare this to Proposition~\ref{prop:approx diameter guarantee}).
%
\begin{proposition}\label{prop:multi-weight diameter}\label{PROP:MULTI-WEIGHT DIAMETER}{\sc (Multi-Weight Diameter Bound; Proof in Section~\ref{sec:multi weight diameter bound})}
$\ecc(G, \cW_i)\leq 2n.$
\end{proposition}
%
Moreover, we show that solving the following {\em Multi-Weight $K$-\apsp} problem on $(G, \cW_i)$ is enough to solve \apsp on $(G, w_i)$.
%
\begin{definition}\label{def:multi weight apsp} {\sc (Multi-Weight $K$-APSP)} Given a network $G$, a set of non-negative edge weights $\cW=\{\vec{w}^s\}_{s\in V(G)}$, and a number $K$, we want every node $u$ to know $\dist^K_{G, \vec w^s}(s, u)$ for all nodes $s$.
\end{definition}
%
Specifically, we can show that, for any $K\geq \ecc(G, \cW_i)$,\footnote{Again, obstructions on the way make us end up using something more complicated than what we show here. See Proposition~\ref{prop:d prime}.} 
\begin{align}\label{eq:ideal w_i recovery}
\dist_{G, w_i}(s, u)=2\dist_{G, w_{i+1}}(s, u)+\dist^K_{G, \vec w_i^s}(s, u)\,.
\end{align}
By Proposition~\ref{prop:multi-weight diameter}, $K=2n$ is enough. Moreover, we already know $\dist_{G, w_{i+1}}(s, u)$ since we assume that \apsp on $(G, w_{i+1})$ is already solved in the previous iteration.
%
Thus, our job is to solve multi-weight $K$-\apsp in time as close to $D(G, \cW_i)$ as possible. We do not achieve exactly this. The reason is that $\vec w$ could assign value zero to some edges. Let us first explain what we can do.

%We will end up solving this problem on another graph and have to do something more.


%In what follows, we  show an algorithm that depends on $D(G, \cW_i)$ and another parameter. We will then use this algorithm to ``partly'' solve the problem (as much as the other parameter allows).  Then, we slightly modify the weight scaling scheme to get an extra property of $(G, \cW_i)$ that allows us to use the new algorithm to remove the extra parameter.

%
%There is another thing that the new algorithm has to deal with: Observe that for any $i<\beta$, we could have $D(G, w_i)\gg n$. Thus, we need another way to solve \apsp on $(G, w_i)$. To do this, we will use the solution of \apsp on $(G, w_{i+1})$ to change the weight $w_i$ into a collection of {\em asymmetric} weight functions $\cW_i=\{\vec w^s_i\}_{s\in V(G)}$. An important property is that it has a small {\bf Generalized Diameter}, defined as $\ecc(G, \cW_i)=\max_{s, u\in V(G)} \dist_{G, \vec{w}^s_i}(s, u)$; in particular, in Lemma~XXX, we will show that
%\begin{align}\ecc(G, \cW_i)&=O(n)\label{eq:ecc bound}\end{align}
%


%we wish to solve the following problem on $(G, \cW_i)$.
%

%
%We will show that solving this problem on $(G, \cW_i)$ is enough for us to solve \apsp on $(G, w_i)$ (cf. Lemma~XXX).
%
% We won't state this since we'll actually solve the special case of multi-weight apsp
%\begin{lemma}
%Let $T_i$ be the time need to solve multi-weight \apsp on $(G, \cW_i)$. Then,
%\end{lemma}
%
%Solving this problem is an important subroutine in our algorithm.
%
%We now discuss how to do this with an algorithm whose running time depending on the multi-weight diameter $\ecc(G, \cW_i)$. In what follows, we will show an algorithm that depends on another parameter. Then, we slightly modify the weight scaling to get an extra property of $(G, \cW_i)$ that allows us to use this algorithm to remove the extra parameter.

\paragraph{Solving Multi-Weight $K$-APSP} Instead of an algorithm for multi-weight \apsp on $(G, \cW)$ whose running time solely depends on $\ecc(G, \cW)$, we show that there is an algorithm whose running time depends on $\ecc(G, \cW)$ and another parameter called the {\em longest zero path length}. This parameter is defined as $\zero(G, \cW)=\max_{P, s} |V(P)|$ where the maximization is over all simple paths $P$ and node $s$ in $G$ such that $\vec{w}^s(P)=0$; in other words, $\zero(G, \cW)$ is the number of nodes in the longest path of distance zero for some weight function in $\cW$. We show the following.
%
%
\begin{proposition}\label{prop:pseudopoly multi-weight}\label{PROP:PSEUDOPOLY MULTI-WEIGHT}{\sc (Pseudo-Polynomial Time Algorithm for Multi-Weight APSP; Proof in Section~\ref{sec:multi-weight k-apsp})}
The multi-weight $K$-\apsp problem on input $(G, \cW)$ can be solved by an algorithm that takes $\zero(G, \cW)$ as an input and, with high probability, finishes in $O(K\zero(G, \cW)\log n+n)$ time.
\end{proposition}
%
As an example, observe that we can use Proposition~\ref{prop:pseudopoly multi-weight} to prove Proposition~\ref{prop:pseudopoly time} with an extra $\log n$ factor by letting $\vec w^s=w$ for all $s$; in this case, $\ecc(G, \cW)=D(G, w)$ and $\zero(G, \cW)=1$.

The idea behind Proposition~\ref{prop:pseudopoly multi-weight} is similar to Proposition~\ref{prop:pseudopoly time}: we treat $(G, \vec w^s)$ as an unweighted graph and grow BFS trees from every node in $G$. For an intuition, first consider when $(G, \cW)$ has {\em no} zero edge weight. In this case, we can simply grow BFS trees to solve the problem. Each BFS algorithm will finish in $O(K)$ time, if it does not conflict with other algorithms (in sending messages). To avoid conflicts, we will use the {\em random delay} technique \cite{LeightonMR94}. (We cannot use the same deterministic rule as Proposition~\ref{prop:pseudopoly time} since there are many edge weights.) This causes the algorithm to be randomized and have an extra $\log n$ term in the running time. The total time will be $O(K\log n+n)$ in this case.

In order to deal with zero weights, we will grow the BFS tree from each node $s$ and pretend that edges $uv$ such that $\vec w^s(uv)=0$ are not in the network. Additionally, between each step of growing the BFS tree we will have an extra time of $O(\zero(G, \cW))$ rounds where nodes will communicate through edges of weight zero only. This extra time is used for nodes to send its distance along paths of distance zero (that is why we need $O(\zero(G, \cW))$ extra time). So, the total time changes from $O(K\log n+n)$ to $O(K\zero(G, \cW)\log n+n)$. 
%
We now discuss how to use Proposition~\ref{prop:pseudopoly multi-weight} to solve \apsp on $(G, w_i)$.

%Applying Lemma~\ref{lem:general pseudopoly}, we get the running time of $O(\ecc(G, \cW_i)\zero(G, \cW_i)\log n)$ for solving multi-weight \apsp on $(G, \cW_i)$. Next, we show how to replace $\zero(G, \cW_i)$ by $\sqrt{n}$.




\paragraph{Solving APSP on $(G, w_i)$} First, let us note that we will use a weight scaling scheme that is a bit different from the standard one we explain earlier: we will use what we call a {\em positive binary representation} to construct our weight scaling scheme (see Section~\ref{sec:scaling} for details). The advantage of this non-standard scheme is that we can convert $(G, w_i)$ to $(G, \cW_i)$ with the following additional property.
%
\begin{proposition}\label{prop:clustering}\label{PROP:CLUSTERING}{\sc (Node Clustering; Proof in Sec.~\ref{sec:clustering})}
Nodes in $G$ can be partitioned into {\em clusters} $C_1, C_2, \ldots, C_k$, for some $k$, such that 
%(1) the subgraph of $G$ induced by any cluster $C_j$ is connected, and (2) 
for any $\vec w\in \cW_i\cup \{w_i\}$, $\dist_{G, \vec w}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster.
%(2) $\dist_{G, \vec w_i^s}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster.
%\begin{itemize}[noitemsep]
%\item the subgraph of $G$ induced by any cluster $C_j$ is connected, and 
%\item for every node $s$, $\dist_{G, \vec w_i^s}(u, v)=0$ if and only if $u$ and $v$ are in the same cluster.
%\end{itemize}
Moreover, such partition can be found in $O(n)$ time (in the end, every node $u$ knows which cluster every node $v$ is in; i.e., it knows the set $\{(v, \rep(C_j) \mid v\in C_j)\}$ where we define $\rep(C_j)$ to be $\rep(C_j)=\min_{v\in C_j} v$).
%; see details in Line~\ref{line:clustering} of Algorithm~\ref{algo:apsp}).% (see Sec.~\ref{sec:main algo} and Line~\ref{line:clustering} of Algorithm~\ref{algo:apsp} for details).%(as a result, for every node $u$ in each cluster $C_j$ knows iand its neighbors are in, as well as the sizes of these clusters).
\end{proposition}
%
%Line~\ref{line:clustering} of Algorithm~\ref{algo:apsp} for details of what the algorithm in the above lemma computes and
%
We exploit the above proposition to solve \apsp on $(G, w_i)$ in $O(n\sqrt{n}\log n)$ time as follows. Define $H$ to be a subgraph of $G$ where we delete all edges between two nodes in every cluster $C_i$ such that $|C_i|\geq \sqrt{n}$ (we call such $C_i$ a {\em big cluster}). Observe that the longest zero path length of $(H, \cW_i)$ is $\zero(H, \cW_i)\leq \sqrt{n}$ since any path of distance zero must be contained in one cluster. We then apply the algorithm in Proposition~\ref{prop:pseudopoly multi-weight} with $K=2n$ (so that $K\geq \ecc(G, \cW_i)$, by Proposition~\ref{prop:multi-weight diameter}) to solve multi-weight $(2n)$-\apsp on $(H, \cW_i)$ in $O(n\sqrt{n}\log n)$ time. We can use this result to get a solution to \apsp on $(G, w_i)$ for {\em some} pairs of nodes. In particular, we show that if the distance between two nodes in $(G, w_i)$ is preserved in $(H, w_i)$, then we can compute this distance correctly.
%
\begin{proposition}\label{prop:d prime}\label{PROP:D PRIME}{\sc (Property of $\dist'$; Proof in Section~\ref{sec:d prime})}
%Given the solutions to \apsp on $(G, w_{i+1})$ and $(2n)$-\apsp on $(H, \cW_i)$, without communication, every node $u$ can compute, for all nodes $v$, value $d'(u, v)$ such that $d'(u, v)\geq \dist_{G, w_i}(u, v)$, and if $\dist_{H, w_i}(u, v)=\dist_{G, w_i}(u, v)$, then $d'(u, v)=\dist_{G, w_i}(u, v)$.
%
Consider any $K\geq \ecc(G, \cW_i)$. For any nodes $s$ and $u$, let $d'(s, u)=2\dist_{G, w_{i+1}}(s, u)+\dist^{K}_{H, \vec w_i^s}(s, u)$. Then, $d'(u, v)\geq \dist_{G, w_i}(u, v)$. Moreover, if $\dist_{H, w_i}(u, v)=\dist_{G, w_i}(u, v)$, then $d'(u, v)=\dist_{G, w_i}(u, v)$.
\end{proposition}
%
To get a solution of \apsp on $(G, w_i)$, we characterize which pairs get the correct solution from the previous step. For an intuition, consider a pair $(u, v)$ such that there is a shortest $u$-$v$ path in $(G, w_i)$ that does not use any node in the big clusters. Intuitively, this path is also a shortest path in $(H, w_i)$ and thus the previous step will compute $d'(u, v)=\dist_{G, w_i}(u, v)$. Thus, we just have to ``fix'' those shortest paths involving nodes in big clusters. To do this, we show that it is enough to broadcast $d'(u, v)$ for all nodes $u$ in big clusters and all other nodes $v$, which can be shown to require $O(n\sqrt{n})$ time using the fact that there are at most $\sqrt{n}$ big clusters.

In particular, we show that each node $u$ can construct a weighted graph $(G'_u, w')$. Each node of $G'_u$ is in the form $c_j$ and represents each cluster $C_j$. Edge weight $w'(c_jc_{j'})$ corresponds to the distance $d'(C_jC_{j'})$ between clusters $C_j$ and $C_{j'}$ that node $u$ has learned so far. Then, we show that $u$ can compute its distance to every other nodes in $(G, w_i)$ using the following proposition.
%
\begin{proposition}\label{prop:G prime}\label{PROP:G PRIME}{\sc (Property of $(G_u', w')$; Proof in Section~\ref{sec:G prime})}
For any nodes $u$ and $v$, let $C_j$ and $C_{j'}$ be clusters that contain $u$ and $v$, respectively. Then, $\dist_{G, w_i}(u, v)=\dist_{G'_u, w'}(c_j, c_{j'}).$
\end{proposition}



\paragraph{Organization} In Section~\ref{sec:main algo}, we outline the main exact algorithm which formally defines some terms, as well as shows how to put all propositions introduced in this section together. The rest sections are devoted to proving the propositions.
%From Section \ref{sec:multi weight diameter bound} to \ref{sec:G prime}, we proof Proposition~\ref{prop:multi-weight diameter} to \ref{prop:G prime}, respectively.
%
Due to space limitation, the details of our approximation algorithms are shown in Appendix~\ref{sec:approx}. We also prove our lower bound (Observation~\ref{observe:lower bound}) in Appendix~\ref{sec:lower bound}. 

%%
%\begin{lemma}\label{lem:same zero}
%For any $s$, $u$ and $v$, $\dist_{G, w_i}(u, v)=0$ if and only if $\dist_{G, w^s_i}(u, v)=0$.
%\end{lemma}
%%
%We exploit the above property to solve \apsp on $(G, w_i)$ in $O(n\sqrt{n}\log n)$ time as follows. First, we partition nodes into {\em clusters}: nodes $u$ and $v$ are in the same cluster if and only if $\dist_{G, w_i}(u, v)=0$.
%%
%For any cluster having more than $\sqrt{n}$ nodes (``big clusters''), we delete all edges between two nodes in such cluster. Let $G'$ be the resulting graph. We then use Lemma~\ref{lem:same zero} to show that the longest zero path length $\zero(G', \cW_i)$ is $O(\sqrt{n})$ (essentially, this is because there is no edge of weight zero crossing between two clusters for any weight function in $\cW_i$). We then apply the algorithm in Lemma~\ref{lem:pseudopoly multi-weight} to solve multi-weight \apsp on $(G', \cW_i)$ in $O(\ecc(G, \cW)\sqrt{n}\log n)$ time, which is $O(n\sqrt{n}\log n)$ by \eqref{eq:ecc bound}. We use this result to get a solution to \apsp on $(G', w_i)$.
%%
%Finally, we show that, to solve \apsp on $(G, w_i)$ it is enough to broadcast $\dist_{G', w_i}(u, v)$ for all node $u$ in big clusters and all nodes $v$. Using the fact that there are at most $\sqrt{n}$ big clusters, we show that we only have to broadcast $O(n\sqrt{n})$ messages, which will take $O(n\sqrt{n})$ time in total.

%\paragraph{Running Time without $\zero(G, \cW_i)$ (Sec. XXX)} To eliminate $\zero(G, \cW_i)$ from the running time, we modify the weight scaling scheme slightly to make $(G, \cW_i)$ have the following {\em same-zero} property:
%%
%\begin{definition}[Same-Zero] We say that $(G, \cW=\{w^s\}_{s\in V(G)})$ is {\em same-zero} if for any nodes $u$, $v$, $s$ and $s'$, $\dist_{G, w_i^s}(u,v)=0$ $\implies$ $\dist_{G, w_i^{s'}}(u,v)=\dist_{G, w_i^{s'}}(v, u)=0$.
%\end{definition}
%%
%%\begin{align}
%%%\forall u, v, s, s':\ \ \vec{w}_i^s(uv)=0 \iff \vec{w}_i^{s'}(uv)=\vec{w}_i^{s'}(vu)=0\,.
%%\forall u, v, s, s':\ \ \dist_{G, w_i^s}(u,v)=0 \iff \dist_{G, w_i^{s'}}(u,v)=\dist_{G, w_i^{s'}}(v,u)=0\,.
%%\label{eq:property that gives cluster}
%%\end{align}
%%
%We guarantee the following.
%\begin{lemma}\label{lem:pseudopoly same-zero multiweight}{\sc (Pseudo-Polynomial Time Algorithm for Multi-Weight APSP on Same-Zero Inputs)}
%The multi-weight \apsp problem on input $(G, \cW)$ that is same-zero can be solved by an algorithm that, with high probability, finishes in $O(\ecc(G, \cW)\sqrt{n}\log n)$ time.
%\end{lemma}
%%
%The above lemma is proved by exploiting the same-zero property as follows. First, we partition nodes into {\em clusters}: nodes $u$ and $v$ are in the same cluster if and only if $\dist_{G, w_i^s}(u, v)=0$ for all $s$. Then, for any cluster having more than $\sqrt{n}$ nodes (``big cluster''), we delete all edges between two nodes in such cluster. Let $G'$ be the resulting graph. We then use the same-zero property to show that the longest zero path length $\zero(G', \cW_i)$ is $O(\sqrt{n})$ (essentially, this is because the same-zero property implies that there is no edge of weight zero crossing between two clusters). We then apply the algorithm in Lemma~\ref{lem:pseudopoly multi-weight} to solve multi-weight \apsp on $(G', \cW_i)$ in $O(\ecc(G, \cW)\sqrt{n}\log n)$ time. Finally, we show that we can solve multi-weight \apsp on $(G, \cW_i)$ by broadcasting distances between nodes in big clusters and all other nodes in ...

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%
%\section{Proof Overview \& Organization - OLD}
%
%A simple fact that plays a crucial role in previous algorithms on unweighted networks \cite{HolzerW12,PelegRT12} is that we can solve \apsp by efficiently parallelizing multiple BFS algorithms. Our algorithms also rely on this idea, but we will need several other ideas to deal with weights. Let us illustrate these ideas by first explaining our simple approximation algorithms before discussing what we need for the exact algorithm.
%
%%We illustrate our ideas starting from explaining our simple approximation algorithms before discussing what we need for the exact algorithm.
%
%\paragraph{Simple Approximation Algorithms (Sec. XXX)} The first idea of our approximation algorithms is that we can solve \apsp in {\em pseudo-polynomial time}:
%%
%\begin{lemma}\label{lem:weak pseudopoly time}
%\apsp on any weighted network $(G, w)$, with positive integral edge weights, can be solved in $O(n+D(G, w))$ time.
%\end{lemma}
%%
%This lemma simply exploits the fact that we can view $(G, w)$ as an unweighted network $G'$ by replacing an edge $uv$ of weight $w(uv)$ by a $u$-$v$ path of length $w(uv)$. We then grow BFS trees in $G'$ from every node in $V(G)$ to find distances between nodes in $V(G)$ and other nodes in $V(G')$.
%%
%Since we run many BFS algorithms in parallel, there could be {\em conflicts}; i.e., many BFS algorithms may want to send messages on the same edge at the same time. There are many ways to resolve this (e.g. Lemma~XXX). A nice way to do this efficiently and deterministically is to use the rule in the {\em $S$-Shortest Paths} algorithm of \cite{HolzerW12} to resolve the conflicts. This leads to an $O(D(G, w)+n)$ running time.
%
%Now, to get a linear-time $(1+\epsilon)$-approximation algorithm for computing $D(G, w)$, we simply change weight $w$ slightly to $w'$ so that $D(G, w')=O(n)$, and we can use $D(G, w')$ to approximate $D(G, w)$. We then apply Lemma~\ref{lem:weak pseudopoly time} to compute $D(G, w')$.
%
%To approximate \apsp, we need a slightly stronger version of Lemma~\ref{lem:weak pseudopoly time} where we want to find distances of nodes that are {\em nearby}:
%%
%\begin{lemma}\label{lem:strong pseudopoly time}
%For any weighted network $(G, w)$ with positive integral edge weights and integer $K$. There is an $O(n+K)$-time algorithm such that, at its termination, any nodes $u$ and $v$ know the value of $\dist(u, v)$ if $\dist(u, v)\leq K$; otherwise, they know that $\dist(u, v)> K$.
%\end{lemma}
%%
%The above lemma is obtained by modifying Lemma~\ref{lem:weak pseudopoly time} slightly (thus, it relies on the same idea of growing multiple BFS trees and use the rule of \cite{HolzerW12} to resolve conflicts).
%%
%We then approximate \apsp by ``guessing''the distance between each pair of nodes and apply Lemma~\ref{lem:strong pseudopoly time} on $(G, w')$ for some appropriate approximate weight $w'$ (using the guessed number). The guessing process introduces a $\log n$ factor in the running time; so we have a running time of $O(n\log n)$.
%
%
%\paragraph{Exact Algorithm (Sec XXX-XXX)}
%
%\paragraph{Parallel Breadth-First Search (BFS)} A simple fact that plays a crucial role in previous algorithms on unweighted networks \cite{HolzerW12,PelegRT12}, as well as our algorithm, is that we can solve \sssp using a BFS algorithm that treats an edge of weight $k$ as a path of length $k$. This algorithm works on {\em directed weighted} graphs. Its running time is bad, but it is easy to run many such algorithms in parallel. Since understanding this simple algorithm is important in understanding the rest of the paper, we describe this algorithm in Algorithm~\ref{algo:bfs} and briefly discuss its properties.
%%
%\begin{algorithm}
%\caption{{\sc WeightedBfs}$(\vec{G}, w, s, \Delta)$}\label{algo:bfs}
%{\bf Input:} Directed graph $\vec G$ with positive integral weight $w$ and source node $s$.
%
%{\bf Output:} Every node $v$ such that $\dist_{\vec G, w}(s, v)\leq \Delta$ knows $\dist_{\vec G, w}(s, v)$.
%
%%\medskip\textit{\textbf{Preprocessing}}
%%\medskip
%
%\begin{comment}
%\noindent\begin{algorithmic}[1]
%
%%\algstore{bfstwo}
%%\algrestore{bfstwo}
%
%\State Let $t$ be the time this algorithm starts.
%
%\State Initially, source node $s$ triggers the algorithm to start by sending a message $(s, t, 0)$ to itself.
%
%\algstore{bfsone}
%\end{algorithmic}
%
%
%\noindent\begin{itemize}[noitemsep]
%\item Let $t$ be the time this algorithm starts.
%
%\item Initially, source node $s$ triggers the algorithm to start by sending a message $(s, t, 0)$ to itself.
%\end{itemize}
%\end{comment}
%
%\medskip $\bullet$ Let $t$ be the time this algorithm starts. Initially, source node $s$ triggers the algorithm to start by sending a message $(s, t, 0)$ to itself.
%
%
%
%%\medskip\textit{\textbf{Main subroutine:}}
%
%$\bullet$ When a node $u$ receives a message $(s, \tau, \ell)$ for some $\ell$, it does the following.
%
%\begin{algorithmic}[1]
%
%%\algrestore{bfsone}
%
%\If{$u$ has {\em not} already received $(s, \tau, \ell')$ for some $\ell'$}\label{line:BFS start}
%
%\State $u$ now knows that $\dist_{\vec G, w}(s, u)=\ell$.\label{line:bfs compute distance}
%
%%\State $u$ sends through all directed edges $\overrightarrow{uv}$ a message $(s, t, \ell+w(\overrightarrow{uv}))$ at time $t+\ell+w(\overrightarrow{uv})$.\label{line:bfs send message}
%
%\State For any neighboring nodes $v\notin S_{G, w_i}(u)$ of $u$ such that $\ell+w(uv)\leq \Delta$, node $u$ sends to $v$ a message $(s, \tau, \ell+w(uv))$ at time $\tau+\ell+w(uv)$.\danupon{Address this change in the texts}\label{line:bfs send message}
%
%\EndIf\label{line:BFS end}
%
%\end{algorithmic}
%\end{algorithm}
%
%The algorithm simply makes sure that the first message that every node $v$ receives is $(s, t, \ell)$, where $\ell=\dist_{G, w}(s, v)$, and this message is received at time $t+\ell$. This fact, besides guaranteeing the correctness and time complexity, also guarantees that each node sends a message through each edge only {\em once}.
%%
%%\begin{claim}\label{lem:bfs style}
%%Algorithm~\ref{algo:bfs} solves \sssp from source $s$ in $O(D_{G, w}(s))$ time. Moreover, every node $u$ sends a message through each directed edge $\overrightarrow{uv}$ at most once.
%%\end{claim}
%%
%This gives us a hope that we can execute Algorithm~\ref{algo:bfs} from different sources in parallel since no edge will be ``overused''. In the case of unweighted undirected graphs, the cute deterministic scheduling of \cite{HolzerW12,PelegRT12} achieves exactly this.
%
%The problem of running Algorithm~\ref{algo:bfs} on weighted graphs $(G, w)$ is that it takes too much time to finish; i.e. it takes $O(D_{G, w}(s))=O(\max_v \dist_{G, w}(s,v))$ time. In what follows, we explain several ideas that we use to run algorithms similar to Algorithm~\ref{algo:bfs} faster, in parallel.
%
%
%%Our algorithm will use several ideas to enable us to run an algorithm similar to Algorithm~\ref{algo:bfs} faster and in parallel. One fact to note here: our algorithm will end up running parallel algorithms on {\em different directed weighted graphs}, and we will need the random delay technique of Leighton, Maggs, and Rao \cite{LeightonMR94} instead of the deterministic scheduling of \cite{HolzerW12,PelegRT12}.
%%
%%We now explain what we need to be able to run parallel BFS algorithms.
%
%
%
%\paragraph{Weight Scaling (details in Section \ref{sec:scaling})} A natural way to make Algorithm~\ref{algo:bfs} finish faster is to run it on $(G', w')$ such that $D_{G', w'}(s)$ is small. This leads us to the use of {\em weight scaling}. Recall that the general idea of this technique is to write each edge weight $w(uv)$ as a binary string $b_\beta(uv)$, $b_{\beta-1}(uv)$, $\ldots$, $b_0(uv)$, where $b_i(uv)\in \{0, 1\}$ for all $i$, and $w(uv)=\sum_{i=0}^\beta b_i(uv)2^i$. We then solve the problem in {\em iterations}, starting from Iteration $\beta$ {\em down to} Iteration $0$. In Iteration $i$ we solve the problem on graph $(G, w_i)$, where $w_i(uv)$ is defined to be $b_\beta(uv)\ldots b_i(uv)$ in base two. The point is that the solution from Iteration $i+1$ will help speeding up our algorithm on Iteration $i$.
%
%To see why this technique is useful, first observe that $D_{G, w_\beta}(s)\leq n$ since $w_\beta(uv)\in \{0, 1\}$ for every edge $uv$. Thus, we might be able to finish Algorithm~\ref{algo:bfs} quickly on $(G, w_\beta)$. For graphs $(G, w_i)$ in other iterations, we could have $D_{G, w_i}(s)> n$; however, we can use the solution on $(G, w_{i+1})$ to ``adjust'' the weight $w_i$ so that a similar property holds, without changing the solution. To be precise, we show that for any $i$ we can get a collection of $n$ directed weighted graphs $\{(\vec{G}, w_i^u)\}_{u \in V(G)}$ such that, for any node $u$, the $D_{\vec{G}, w^u_i}(u)=O(n)$. Moreover, any shortest $u$-$v$ path in $(\vec G, w^u_i)$ is also a shortest $u$-$v$ path in $(G, w_i)$.
%
%Note that we still cannot directly apply Algorithm~\ref{algo:bfs} at this point. The reason is that the graphs we obtain have zero edge weights (graph $(G, w_\beta)$ is one obvious example). One modification we have to make is to use what we call {\em positive binary representation} instead of the binary representation (the advantage of this will be clear when we prove Lemma~\ref{lem:properties of scaling}). Besides this, we have to introduce the notion of {\em supernodes} and modify Algorithm~\ref{algo:bfs} to deal with supernodes, as we discuss next.
%
%\paragraph{Supernodes (details in Section~\ref{sec:supernode})} We deal with zero weights using the following simple idea: We group nodes linked by edges of weight zero as a set called {\em supernode}. After identifying nodes in the same supernode (equivalently, contracting all edges of weight zero), we will not have zero weight left. Thus, we can run Algorithm~\ref{algo:bfs} on this graph.
%
%For example, let us consider any graph $(G, w)$ with weights zero and one. Let $(G', w')$ be the graph resulting from contracting all edges of weight zero. We call $(G, w')$ a {\em supergraph} and its nodes {\em supernodes}. Each supernode represents a set of nodes in $(G, w)$ linked by edges of weight zero. Observe that $(G', w')$ is an unweighted graph, on which Algorithm~\ref{algo:bfs} can be executed quickly.
%
%However, we cannot really execute Algorithm~\ref{algo:bfs} on $(G', w')$ directly, since it is {\em not a real network}. So, instead, we will execute an algorithm on $(G, w)$ that {\em simulates the Algorithm~\ref{algo:bfs} on supergraph $(G', w')$}.
%
%\paragraph{Simulating BFS by Light and Heavy Nodes (details in Section~\ref{sec:light}-\ref{sec:heavy})} Simulating Algorithm~\ref{algo:bfs} on supergraphs is still not a trivial task. The difficulty is that Algorithm~\ref{algo:bfs} heavily relies on the fact that all nodes are synchronized; i.e., every node sends the message $(s, t, \ell)$ at the same time $t+\ell$. While this is easy to do on a real network, it becomes harder on supergraphs since different supernodes in $(G', w')$ correspond to different number of nodes in $(G, w)$, which requires different time for ``internal communication'' (where nodes in the same supernode communicate to each other). One idea to fix this problem is to wait until the last supernode is ready to send the message $(s, t, \ell)$. This, however, requires some extra communication, which makes it hard to run many algorithms in parallel. Another obvious approach is to wait for $O(n)$ time between the execution of each round of Algorithm~\ref{algo:bfs}; i.e., instead of sending message $(s, t, \ell)$ at time $t+\ell$, we will send it at time $t+O(n\ell)$. The waiting time is used to guarantees that all supernodes finish their internal communication and are ready to send the message before the next round starts. This, however, increases the running time to $O(n^2)$.
%
%Our solution modifies the second approach by dividing supernodes into {\em light} and {\em heavy} supernodes: light supernodes are supernodes corresponding to at most $\sqrt{n}$ nodes, and heavy supernodes are the rest. We then simulate Algorithm~\ref{algo:bfs} {\em only until we find a heavy supernode that is not the source node}. In other words, a heavy supernode that is not $s$ will not execute Line~\ref{line:bfs send message} of Algorithm~\ref{algo:bfs}. This allows us to reduce the waiting time to $O(\sqrt{n})$. Thus, we will finish Algorithm~\ref{algo:bfs} in $O(n\sqrt{n})$ time. In fact, we can concurrently simulate many copies of Algorithm~\ref{algo:bfs} using different supernodes as a source in $O(n\sqrt{n})$ time!
%
%The algorithm above almost solves the problem except that it does not promise to find the distance between every pair of supernodes. In particular, it only finds the distance between {\em light pairs of supernodes} -- pairs of supernodes $u$ and $v$ such that some shortest $u$-$v$ paths in supergraph $(G', w')$ contains no internal heavy supernodes.
%
%We show that the above problem can be quickly fixed: We claim that the distance between other pairs can be found if every heavy supernode can broadcast to all other nodes what it obtains in the previous step (i.e., its distance to some other supernodes). This can be easily done in $O(n\sqrt{n})$ time because there are only $\sqrt{n}$ supernodes, each having at most $n$ pieces of information to broadcast.
%
%\paragraph{Parallelizing Algorithm~\ref{algo:bfs}}  We note that our algorithm cannot use the deterministic scheduling of \cite{HolzerW12,PelegRT12} since it runs simulations of Algorithm~\ref{algo:bfs} on many weighted directed graphs in parallel. Instead, we will use the random delay technique of Leighton, Maggs, and Rao \cite{LeightonMR94} and exploit the fact that Algorithm~\ref{algo:bfs} sends at most one message on each edge. This is the only part that relies on randomness.

%
%\medskip The main algorithm is described in Algorithm~\ref{algo:apsp}. We slowly explain this algorithm in detail in the next few sections.



==> prelim.tex <==
\section{Preliminaries}\label{sec:prelim}

\subsection{Problems}

\subsection{Graph Theoretic Definitions}

%\subsection{Skeleton}



